Don't Leak Your Keys: Understanding, Measuring, and Exploiting the AppSecret Leaks in Mini-Programs

Mobile mini-programs in WeChat have gained significant popularity since their debut in 2017, reaching a scale similar to that of Android apps in the Play Store. Like Google, Tencent, the provider of WeChat, offers APIs to support the development of mini-programs and also maintains a mini-program market within the WeChat app. However, mini-program APIs often manage sensitive user data within the social network platform, both on the WeChat client app and in the cloud. As a result, cryptographic protocols have been implemented to secure data access. In this paper, we demonstrate that WeChat should have required the use of the "appsecret" master key, which is used to authenticate a mini-program, to be used only in the mini-program back-end. If this key is leaked in the front-end of the mini-programs, it can lead to catastrophic attacks on both mini-program developers and users. Using a mini-program crawler and a master key leakage inspector, we measured 3,450,586 crawled mini-programs and found that 40,880 of them had leaked their master keys, allowing attackers to carry out various attacks such as account hijacking, promotion abuse, and service theft. Similar issues were confirmed through testing and measuring of Baidu mini-programs too. We have reported these vulnerabilities and the list of vulnerable mini-programs to Tencent and Baidu, which awarded us with bug bounties, and also Tencent recently released a new API to defend against these attacks based on our findings.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.


==> algorithm/backward.tex <==
\begin{algorithm}[t]
\caption{Configuration Path Extraction}
\label{alg:backward}
\scriptsize
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Fn}{Function}{}{}
\Input{$G$: Control flow graph, $D$: A set of dependent variables, $A$: Function invocation address, $B$: Current block, $s$: current path}
\Output{$S$: A global set of configuration paths}
\Fn{ConfigPathExtract($G$, $D$, $A$, $B$, $s$)} {
    % $s \leftarrow $ $\{\}$ \label{line:a2_init} \\
    \For{each instruction $i$ of $B$ in reverse order starting from $A$}{ \label{line:a2_for_start}
        \If{$i$ modifies the value of any target variables in $D$}{ \label{line:a2_if_start}
            $D \leftarrow $ $D$ $\cup$ All other variables in $i$ \\ 
            $D \leftarrow $ $D$ $-$ The target variables \\ 
            $s \leftarrow $ $s$ $\cup$ $i$ \\
        } \label{line:a2_if_end}
    } \label{line:a2_for_end}
    
    
    % \If{$D$ is empty or no previous block}{ \label{line:a2_if_start1}
    \If{A fixed point is reached}{ \label{line:a2_if_start1}
        $S \leftarrow$ $S$ $\cup$ $s$ \\
        \Return
    } \label{line:a2_if_end1}
    
    \tcp{To previous blocks}

    \For{each previous block $b$ of $B$ in $G$} { \label{line:a2_for_start1}
        $d \leftarrow $ A new copy of $D$ \\
        $s' \leftarrow $ A new copy of $s$ \\
        $a \leftarrow $ Last address of $b$ \\
        ConfigPathExtract($G$, $d$, $a$, $b$, $s'$) \\
    } \label{line:a2_for_end1}
    
    % $P \leftarrow $ Disassembling F with a default base \label{line:a1_disassemble} \\
    % $S \leftarrow $ Starting address of $P$ \\
    % $B \leftarrow \{\}$  \tcp{Set of absolute addresses} \label{line: a1_init}
    % $C \leftarrow \{\}$  \tcp{Set of base address candidates} \label{line: a1_init2}
    
    % \tcp{Step 1: Base address estimation}
    % \While{$S \neq $ Ending address of $P$}{ \label{line:a1_while_start}
        
    %     $I \leftarrow $ Instruction at $S$ \\
    %     \If {$I$ is a load instruction} {
    %         $B \leftarrow B$ $\cup$ Absolute address referenced in $I$ \\
    %     }
    %     $S \leftarrow $ Next address \\
    % } \label{line:a1_while_end}
    
    % $B \leftarrow$ Sort $B$ in ascending order \label{line:a1_sort} \\
    
    % \For{each index $i$ $\in$ $B$} { \label{line:a1_for_start}
    %     \If {$B[i+1] - B[i] > Threshold$} { \label{line:a1_threshold}
    %         $C \leftarrow C$ $\cup$ $B[i]$ \\ 
    %     }
    % } \label{line:a1_for_end}
    
    % \tcp{Step 2: Brute-force base searching}
    % \For{each candidate $c$ in $C$} { \label{line:a1_for_start2}
    %     \If{Disassembling with $c$ yields the best score}{
    %         $O \leftarrow c$ \\
    %     }
    % } \label{line:a1_for_end2}
    
    % \Return $O$ \label{line:a1_return}
}
% \vspace{-0.3in}
\end{algorithm}
% \vspace{-0.2in}
% \setlength{\textfloatsep}{2pt}


==> algorithm/base.tex <==
\begin{algorithm}[t]
\caption{The BAS algorithm}
\label{alg:bae}
\footnotesize
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Fn}{Function}{}{}
\Input{$F$: a bare-metal firmware}
\Output{$O$: the optimal base address}
\Fn{BAS(F)} {
    $P \leftarrow $ Disassembling F with a default base \label{line:a1_disassemble} \\
    $S \leftarrow $ Starting address of $P$ \\
    $B \leftarrow \{\}$  \tcp{Set of absolute addresses} \label{line: a1_init}
    $C \leftarrow \{\}$  \tcp{Set of base address candidates} \label{line: a1_init2}
    
    \tcp{Step 1: Base address estimation}
    \While{$S \neq $ Ending address of $P$}{ \label{line:a1_while_start}
        
        $I \leftarrow $ Instruction at $S$ \\
        \If {$I$ is a load instruction} {
            $B \leftarrow B$ $\cup$ Absolute address referenced in $I$ \\
        }
        $S \leftarrow $ Next address \\
    } \label{line:a1_while_end}
    
    $B \leftarrow$ Sort $B$ in ascending order \label{line:a1_sort} \\
    
    \For{each index $i$ $\in$ $B$} { \label{line:a1_for_start}
        \If {$B[i+1] - B[i] > Threshold$} { \label{line:a1_threshold}
            $C \leftarrow C$ $\cup$ $(B[i] - sizeof(F))$ \\ 
        }
    } \label{line:a1_for_end}
    
    \tcp{Step 2: Brute-force base searching}
    \For{each candidate $c$ in $C$} { \label{line:a1_for_start2}
        $c \leftarrow $ $c$ rounds up to the nearest possible address \\
        \For {each slightly incremental interval $i$} {
            \If{Disassembling with $c+i$ yields the best score}{
                $O \leftarrow c$ \\
            }
        }
    } \label{line:a1_for_end2}
    
    \Return $O$ \label{line:a1_return}
}
\end{algorithm}

==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> paper/00_abs.tex <==
%
%


==> paper/01_introduction.tex <==
%\AY{I would suggest that we change the title from 'API design' to security mechanisms. Both the cause and the defense countermeasures of these security problems are all related to a broader security mechanisms}
%
%Recently, there is a tremendous growth of mini-programs,
\ignore{
\AY{CURRENT STATUS:}
\begin{itemize}
    \item SEC III: Done
    \item SEC IV
    \begin{itemize}
        \item SUB A: Done
        \item SUB B: Done
        \item SUB C: \AY{Waiting for data}
    \end{itemize}
    \item SEC V
    \begin{itemize}
        \item SUB A: Done
        \item SUB B: Done, figure needs polish
        \item SUB C: \AY{Waiting for data}
    \end{itemize}
    \item SEC VI: Done
\end{itemize}
Aiming for the draft in 12/1
\AY{TODOLIST: END}


\begin{itemize}
    \item Step 1 (now): flow between section and subsections
    \item Step 2 Tomorrow: flow between paragraphs and sentences, plus data & table & missing case; Yue: Step 1
    \item 12.1 eve/12.2 morning: Yue: Step 2; Me: Introduction/Abstract
    \item 12.2 
\end{itemize}
}


  
Mini-program, a size restricted ``small'' program running inside a mobile super-app~\cite{diaz2021super}, is becoming increasingly popular on social network platforms such as \wechat~\cite{WhatareW95:online}, the third most popular messenger app with 1.2 billion monthly active users~\cite{Mostpop46:online}. These mini-programs have significantly enriched the functionalities of the super-apps. 
For example, \wechat has become almost an operating system, providing more than $900$ APIs~\cite{wechatapi} to allow the execution of more than 4 million mini-programs~\cite{wechat3M} in this platform, satisfying all kinds of user's daily demands such as online shopping in virtual stores or scan-to-buy in physical stores.  
There are many popular mini-programs running inside the \wechat platform, such as \texttt{PinDuoDuo} (a group-buy platform).  
Recently, Elon Musk, a business magnate, who is considering converting Twitter to a \wechat-alike super app, mentioned that: ``{\it If you're in China, you kind of live on WeChat, it does everything. It's sort of like Twitter, plus PayPal, plus a whole bunch of other things. And all rolled into one great interface}''~\cite{musksuperapps}. 

%Recently,  Tesla CEO Elon Musk said that the social media platforms such as Twitter could become super apps similar to \wechat, \textit{``If you're in China, you kind of live on \wechat, it does everything. It's sort of like Twitter, plus PayPal, plus a whole bunch of other things. And all rolled into one great interface''~\cite{musksuperapps}.} \looseness=-1 

% @misc{musksuperapps,
% author = {Andrew Asmakov},
% title = {Elon Musk Wants Twitter to Be WeChat-Style 'Super App' With Payments },

% In the past four years, 


% the number of mini-programs in \wechat has exploded, grown from thousands to millions (it has been reported that there are more than 3 million mini-programs~\cite{wechat3M}), reaching almost the same level as the number of Android apps in Google Play. Today, \wechat has become almost like an operating system, providing over $500$ application programming interfaces (APIs)~\cite{wechatapi} to allow developers to easily develop mini-programs in order to satisfy all kinds of user's daily demands such as online shopping at virtual stores or scan-to-buy at physical stores. %, and travel and transportation (e.g., ride-hailing). 
% There are many well-known mini-programs running inside the \wechat platform such as \texttt{Tencent Video}, \texttt{QQ Music}, and \texttt{Pinduoduo} (a well-known Chinese group-buying app). 

 %Recently, Tesla CEO Elon Musk said that social media platform could become super apps similar to the Chinese WeChat, ``If you're in China, you kind of live on WeChat, it does everything. It's sort of like Twitter, plus PayPal, plus a whole bunch of other things. And all rolled into one great interface''~\cite{musksuperapps}. 


%which engages its 300 million users simply through its mini-program. \looseness=-1 %Even supermarket giant Walmart has a `{\tt Scan to Buy}' mini-program, offering services to more than 10 million users.



% \ignore{
% Increasingly, mini-program paradigm, in which a mini-program is executed inside a host-app, is emerging as one of the important computing paradigms in mobile computing in the past few years. This paradigm allows light-weight host-app alike applications programmed by third party developers, to run inside a host app. The host app, which can be an independent native app such as \texttt{Facebook}, \texttt{Tiktok}, or \wechat (the 5th widely used app in the world~\cite{wechat5th})
% which act as a operating system to provide a running environment and resources management for the mini-programs. 
% %
% %(\eg, \wechat,  the 5th widely used app in the world~\cite{wechat5th})
% % 
% %()
% %\AY{\@ZY, could you provide the original webpage here too? lol}) 
% %In this computing paradigm, a host app 
% % app-like software models from third party developers, called mini-programs, to run atop the it. 
% Although a number of tech-giants such as Facebook, Google, and Apple have all begun integrating their own mini-program frameworks in recent years, none of their mini-programs is comparable from both the diversity and technology maturity the to \wechat, which currently has more than one million mini-programs, and 400 million daily active users after four year's development.% Therefore, our paper mainly focused on \wechat. 
% }


% \ignore{
% \wechat mini-program attracts not only a large amount of users, but also service providers, as they can benefit from the huge amount of daily user data to improve their service and make huge profits.
% % and users are attracted by the convenient usage and light-weight application package
% For example, Walmart attracted more than 10 million new users in one year from its wildly successful mini-program ``Scan to Buy'';  \texttt{Pinduoduo}, a well-known Chinese group-buying platform, has also acquired more than 300 million new users in three-years through its mini-program. To stay competitive and attract more vendors is not easy, and therefore, \wechat keep releasing new components and APIs for the vendors to customize their mini-programs\ZQ{can you provide a longitudinal statistics showing how Tecent has been releasing and improving its APIs?}\AY{I will get to the update history to summarize the added APIs each year/month}, allowing the mini-program users to achieve native-app-like experiences. Now, benefited from those powerful mini-program APIs, the mini-programs not only can access data remotely from the back-ends (\eg, online shops), but also have the capabilities to use peripherals such as Bluetooth devices (e.g., Bluetooth locker).
% }

% As mini-programs of \wechat are gradually tied to the daily life of the users, a large amount of service providers have been attracted to integrate their functionalities into \wechat mini-program platform. For example, Walmart harvested more than 10 million new users in one year  from its wildly successful mini-program ``Scan to Buy'';  Pinduoduo, a famous Chinese group-buying platform, has also acquired more than 300 million new users in three-years  through its mini-program. To stay competitive and attract more vendors,  \wechat also provides abundant components and APIs for the vendors to customize their mini-programs, allowing the mini-program users to achieve native-app-like experiences. For example, benefit from those powerful mini-program APIs, the mini-programs can not only access data remotely from the back-ends (e.g., online shops), but also have the capabilities to use peripherals such as Bluetooth devices (e.g., Bluetooth locker).


%the mini-program APIs cover a wide range of functionalities from resource and data access to interface and redirection. With these APIs, the mini-programs cannot only act as web-apps by communicating with their back-end servers with data (e.g., online shops), but also act as native apps to communicate with peripheral devices such as Bluetooth devices (e.g., Bluetooth locker), and even between mini-programs.   


%As the mobile devices gradually gains popularity, the large user base and massive user data processed by daily communication and socializing vendors are gradually turning into emerging mobile infrastructures. \wechat, for instance, has an massive user base of over one billion \ZY{Citation}. As \wechat is gradually tied to the daily life of the users, a large amount of service providers have been attracted to integrate their functionalities into these vendors.


%Motivated by this vastly emerging need of providing more convenient and secure functionality for users, \wechat introduced a novel computing paradigm, the `app-in-app' paradigm, that allows mini-programs developed by third-party service providers to run atop the vendor apps and provided services. Up to now, there have been a total of more than \AY{todo} mini-programs that are running on wechat. 
% \ZY{Allen, since we did our investigation and experiments on WeChat,  we should introduce WeChat as early as possible (After introducing the concept of mini-program paradigm, we should quickly go to introuduce WeChat). Please re-write the first paragraph. You can refer to our SIGMETRICS paper.  }

% Such an ambitious computing paradigm extends the functionalities of the host app by implementing a unified cross-platform sandbox within the host app with JavaScript and V8 engine, where a wide variety of APIs have been provided. With these APIs, the mini-programs can have the access to the local resources of the smartphone (e.g., contact information),  peripheral devices (e.g., Bluetooth devices), and cloud back-ends, which significantly elevated user experiences. On top of these APIs that provide various functionalities, \wechat also enforces a customized permission management mechanisms, called ``scope'', to secure sensitive data: sensitive data such as user location are secured by only allowing mini-programs to access them when corresponding scopes are granted. \ZY{Why we need the last sentence? it 1)breaks the flow, and 2) we do not need to emphasize the concept of permission management mechanisms}

%In an app-in-app paradigm, \wechat provides abundant components and APIs for their mini-programs to achieve native-app-like  development experiences. These APIs cover a wide range of functionalities from resource and data access to  interface and redirection. With these APIs, the mini-programs cannot only act as web-apps by communicating with their back-end servers with data (e.g., online shops), but also act as native apps to communicate with peripheral devices such as Bluetooth devices (e.g., Bluetooth locker), and even between mini-programs.    

%Undoubtedly, such a sophisticated mini-program platform that involves not only back-ends but also local peripherals requires a carefully-designed security mechanism to ensure its security. 

% \AY{This following two paragraphs are changed.} 

%The success of \wechat lies in the 
%Different from many social network platforms (\eg, Facebook~\cite{facebookAPIs}) have provided APIs for 3rd-party developers to query and use the collected social network information, the super apps such as \wechat go far beyond and make  it even more open through its mini-program paradigm. 
%Again, taking \wechat as an example, 
%One important factor that contributes to \wechat's success is that a lot user information that collected by \wechat is now also available to the third-party mini-program developers.  

Mini-programs   have access to a range of user-specific data through rich super-app managed APIs. The data is maintained by both the local host-app and the remote cloud. For example, a \wechat mini-program can use APIs like \texttt{getPhoneNumber}  to access a user's phone number, \texttt{getUserProfile} to access a user's gender and address, and \texttt{getWeRunData} to track a user's daily steps. Additionally, WeChat provides various cloud services, such as Optical Character Recognition (OCR), to enhance the functionality of mini-programs without the need for additional engineering. OCR can convert images, such as national ID cards and driver's licenses, into text. To ensure the proper security of resource access by mini-programs and prevent potential data leaks or abuse, \wechat has implemented a cryptography-based access control mechanism. This involves the distribution of a master key (\appsecret for short) to the developers of each mini-program. The mini-programs can then use the \appsecret to fetch the necessary encryption keys or access tokens to access resources managed by the super-app. This is important in order to avoid incidents like the Cambridge Analytica scandal.


% Unlike native mobile apps, which have limited access to local resources through OS-managed APIs, mini-programs have access to a range of user-specific data through rich super-app managed APIs. The data is maintained by both the local host-app and the remote cloud. For example, a \wechat mini-program can use the \texttt{getPhoneNumber} API to access a user's phone number, the  \texttt{getUserProfile} API to access a user's gender and address, and the \texttt{getWeRunData} API to track a user's daily steps. Additionally, \wechat provides various cloud services, including Optical Character Recognition (OCR), to enhance the functionality of mini-programs without the need for additional engineering. OCR, for example, can convert images such as national ID cards and driver's licenses into text. As super-apps collect and provide access to a large amount of sensitive data and various cloud services, it is important for these platforms to properly secure resource access by mini-programs to prevent potential data leaks or abuse. Our analysis shows that platforms like \wechat have implemented a cryptography-based access control mechanism to secure resource access and transmission. This mechanism involves the distribution of a master key (\appsecret for short) to the developers of each mini-program. The mini-programs can then use the appsecret to fetch the necessary encryption keys or access tokens to access resources managed by the super-app. This is important to prevent incidents like the Cambridge Analytica scandal from occurring again.\looseness=-1

% %Unlike native mobile apps which have a limited set of OS-managed APIs to access just local resources (\eg, Bluetooth),  
% mini-programs have rich super-app managed APIs to access various user-specific data in the platform (maintained by both the local host-app and the remote cloud).
% For example, by invoking \texttt{getPhoneNumber}, a \wechat mini-program can obtain the user's telephone number;  
%  by invoking \texttt{getUserProfile}, it can obtain the user's gender and the address of residence; by invoking \texttt{getWeRunData}, it can track the user's daily walked steps.  
%  Moreover,  
%  to enrich the functionalities of the mini-programs without additional engineering barriers, \wechat also provides many cloud services (some need to be paid), e.g., Optical Character Recognition (OCR), which can convert images (e.g., camera-captured national ID card, or driver license) to texts. \looseness=-1

%\looseness=-1 
%This feature is similar to the legacy app plugins, where one small app can fetch data from other apps  using the APIs provided by these apps (\eg, \texttt{FaceBook} APIs~\cite{facebookAPIs}).% But, since the mini-programs running inside \wechat, \wechat takes the fuller control of the sensitive data.

% Now that the super-apps have collected a huge amount of  sensitive data and provided various cloud services,   
% the platform must properly guard the resource accesses by mini-programs in order to prevent any potential data leaks or abuse (e.g., collecting the sensitive information in a large scale or consuming the services for free); 
% otherwise, incidents like Cambridge Analytica Scandal with Facebook~\cite{Cambridg93:online} could happen again.  
% Our analysis reveals that super apps such as \wechat have introduced a cryptography-based  access control mechanism to guard the resource access and its transmission, with which the super apps first distribute a master key (\appsecret for short) to the developers of each mini-program, and then they use the corresponding \appsecret to fetch the encryption keys or access tokens to consume the resources managed by the super apps.  
%\looseness=-1  

It is well-known that the weak point of modern cryptography is key management; any misuse or leaking of keys can completely undermine the protection. To identify weaknesses in the cryptography-based access control of mini-programs, it is important to understand how the keys are distributed and managed. In contrast to traditional API keys, which are used at the client side of an app to consume third-party services (e.g., Google Map services)~\cite{googlemapkey}, the front-end of a mini-program in a super-app  cannot be trusted (since the front-end of a mini-program can be easily reverse-engineered). Instead, the decryption and consumption of sensitive resources  must be performed on the back-end or server side of the mini-programs.  

% It is well-known that the weakest point of modern cryptography lies in key management: any misuse or leaking of the keys can completely void the protection.  
% Therefore, to identify the weaknesses of the cryptography-based access control in mini-programs, we must first understand how the keys are distributed and managed.   
% Unlike traditional API keys that need to be used at the client side of the app to consume third-party services (e.g., Google Map services)~\cite{googlemapkey}, we notice that in super apps such as \wechat, the front-end cannot be trusted (since the front-end of a mini-program can be easily reverse-engineered), and instead it requires that the decryption and the consumption of sensitive resource from \wechat servers be performed in the back-ends (\ie, the server sides) of the mini-programs.   

%such mechanism can only protect the user specific-resources from being leaked, and

%\wechat users trusted \wechat, and authorized \wechat to collect so many sensitive information. If \wechat distributes the collected sensitive information directly to other third-party mini-program vendors without protection, the sensitive information can be leaked, and the reputation of \wechat can be seriously damaged. Over the past decades, we have seen many data leakage examples due to the mis-management of the provided APIs (\eg, Cambridge collecting user data from Facebook \cite{FacebookvsCambridge}).  
%To achieve so, the permission mechanism is not enough, 

% For instance, \wechat user's nick name, gender, phone number, addresses, etc., are all protected with encryption, and they need to be decrypted with the corresponding APIs when used. %A mini-program also cannot aggressively query the user information from the \wechat servers as \wechat requires a login token for the query, and this token is refreshed very often for the rate limiting. 
% Moreover, since the front-end of the mini-program can be easily compromised (\eg, an attacker can intercept the traffic between a mini-program and its server on a rooted phone), \wechat does not trust the front-end, and requires that the decryption of sensitive data from \wechat servers must be performed in the back-end of the mini-programs. \looseness=-1


%
%herefore, \wechat token top priority for security, and  introduced a suit of protocols to secure the sensitive data transmission. In the protocol, three types of keys including an \appsecret, a token and \sessionkey is generated from \wechat server and distributed to mini-program developers, and four communication entities including the front-end of \wechat, back-end of \wechat, front-end of the mini-program and the back-end of the mini-program are supposed to collaboratively communicate with each other to use the two types of keys to protect the sensitive data. 
%As the front-end of the mini-program can be easily comprised by attacker (\eg, the attacker can intercept the traffic between the mini-program and its server), \wechat does not trust the front-end, and requires the data decryption must be occur on the back-end of the mini-program. 

% Unfortunately,  
% not all developers understand the implication of the untrustworthiness of the mini-program front-end, and therefore they can mistakenly distribute (\eg, hard-code) the \appsecret to the front-end of the mini-program, as confirmed with our manual analysis with  
% a number of popular mini-programs that store their \texttt{MK}s in the mini-program code. 
% To understand concretely the severity and implications of \appsecret leakage, we have proposed two types of novel attacks: attacks against sensitive data and attacks against cloud services. Those attacks have significant security implications, and can cause devastating consequences such as user account hijacking (where an attacker can log into arbitrary user's account for fun and profit), promotion abuse (where the attacker can maliciously collect coupons and rewards through data manipulation), and service theft (where the attacker can consume the cloud services for free). \looseness=-1

Unfortunately, not all developers fully understand the implications of the untrustworthiness of the mini-program front-end, and may mistakenly distribute the \appsecret to the front-end of the mini-program, as we confirmed through manual analysis of a number of popular mini-programs that store their master keys (MKs) in the mini-program code. To understand the severity and implications of \appsecret leakage, we have proposed two types of novel attacks: attacks against sensitive data and attacks against cloud services. These attacks  can lead to devastating consequences such as user account hijacking, promotion abuse, and service theft. For example, an attacker could log into an arbitrary user's account for personal gain, manipulate data to collect coupons and rewards maliciously, or consume cloud services for free.\looseness=-1


By scanning a dataset of \totalanalyzedapps crawled mini-programs, we have identified \sessionstrings unique 32-byte hexstrings from the unpacked miniapp code, and with \numofsecrethour hours' \appsecret online validation, we have detected \leakedapps miniapps that have leaked their \appsecret{s}. We have identified that certain mini-apps have accessed sensitive data such as phone numbers, werun data, user information, and mini-app share information, and have accessed at least one cloud service. These mini-apps are all vulnerable to various attacks such as account hijacking, promotion abuse, and service theft. Our evaluation also revealed that vulnerable mini-apps include many popular mini-apps from high-profile vendors such as \textit{Nestle}, \textit{HP}, and \textit{Tencent}.

%, and are subject to those attacks.



We have disclosed \appsecret leakage vulnerabilities and the list of the vulnerable mini-programs to {\it Tencent}, and were awarded with bug bounties. We also learned that {\it Tencent} is actively working with the developers to fix this vulnerability and some of the mini-programs have already removed the \texttt{MK} from the mini-program code.  Furthermore,  {\it Tencent} recently also released a new
API to defend against our attacks based on our recommended defense~\cite{checkEncryptedData}. \looseness=-1
 
% Leaking \texttt{MK} from mini-program front-end code can lead to a variety of devastating attacks %against both mini-program users and servers 
% such as user account hijacking, promotion abuse, and service theft. % consuming paid services for free. 
% For instance, %\AY{ since the mini-programs can access the phone numbers of users,} \sout{
% a common practice to index users is through their phone numbers in \wechat ecosystem. Unfortunately, in an attacker controlled environment, with the leaked {\tt MK} of the vulnerable mini-program, an attacker can easily query the \sessionkey from \wechat servers to decrypt any encrypted data delivered from \wechat servers. If the mini-program back-end uses the phone number to index the users (very likely true in most mini-programs), an attacker can easily change his or her phone number to any victims’ for account hijacking since the attacker has the decryption \sessionkey, thereby achieving arbitrary user login through such a data manipulation attack. Moreover, all the data maintained by the victim’s account (e.g., user’s citizen ID issued by the government, and his or her shipping address) can also be leaked to the attacker. 
% Furthermore,
% %In other attacks, 
% there could be financial losses for the victims. For instance, 
% we even demonstrate that an attacker can use a controlled account to gain cashback and coupons from the victim vendors by manipulating these sensitive data such as groupchat information with the leaked {\tt MK}. Finally, with the obtained \texttt{MK}, the attacker can consume the paid services, which have purchased by the victims, for free.\looseness=-1

%Specifically, many vendors will reward the users who share their products information to their friends (by post the information to the groupchat) with coupons or cashback in the purpose of promoting their products. To ensure the users to share the products information to different set of their friends, the vendors will collect and track the groupchat information. However, given that the groupchat information can be manipulated by the attacker when {\tt MK} gets leaked, the attacker can keep collecting those cashback and coupons without restrictions.     


%For instance, an attacker can preform arbitrary data manipulation against the sensitive data even when the data is encrypted. Meanwhile, a lot of mini-programs use the user's phone numbers to authenticate their users, and the phone numbers are protected by the \sessionkey. In this case, if the attacker obtains the \sessionkey, the attacker can then change his own phone number to any victims’ phone number, and pretend to be the victim,  achieving arbitrary user login by such a manipulation. If so, all the data maintained by the victim’s account (e.g., user’s citizen ID in government mini-programs and home address in food mini-programs) will be compromised by the attacker.

%which an attacker can easily perform a variety of attacks against their mini-program servers, such as account hijacking, information leakage, and data manipulation. 

%the implementation of data decryption and key management (\ie, the \appsecret management and the \sessionkey management) are totally left for the third-party developers. However,  the free choice of implementing the protocol may give too much freedom for the developers to maintain these essential mechanisms as the third-party developers and \wechat developers are two groups of people, and the developers may misunderstand the design easily. Specifically, in addition to the complexity of the protocol which requires the third-party developers to handle the relationship between the four parties,  some implicit assumptions under the novel mini-program paradigm may also confuse the developers (\eg, the front-end of the mini-program is un-trusted). As such, it is very likely for third-party developers to implement the protocol in improper ways. \looseness=-1 
 
%This paper investigate the costs of such a freedom. Intuitively, given the new assumption (the front-end of the mini-program should not be trusted) may confuse the developers, one of the improper implementation is that the developer mistakenly distribute the \appsecret or the \sessionkey to the front-end of the mini-program. As discussed, the front-end can be easily comprised by the attackers, and therefore, in the controlled environment, 

%an attacker can preform arbitrary data manipulation against the sensitive data even when the data is encrypted. Meanwhile, a lot of mini-programs use the user's phone numbers to authenticate their users, and the phone numbers are protected by the \sessionkey. In this case, if the attacker obtains the \sessionkey, the attacker can then change his own phone number to any victims’ phone number, and pretend to be the victim,  achieving arbitrary user login by such a manipulation. If so, all the data maintained by the victim’s account (e.g., user’s citizen ID in government mini-programs and home address in food mini-programs) will be compromised by the attacker.
 
%We now use an example to demonstrate the sensitive data transformation, and we assume the user has logged into his \wechat account and entered the \texttt{Walmart} mini-program. \texttt{Walmart} is the mini-program that attempts to fetch the user sensitive data from \wechat server.  First, \wechat assigns the master key, \appsecret, to \texttt{Walmart}, and requires the key to be maintained on the back-end of \texttt{Walmart}.  Second, when \texttt{Walmart} asks a token from the front-end of \wechat, and the token is associated with the current logged user. Third, \texttt{Walmart} front-end sends the token to \texttt{Walmart} back-end, and \texttt{Walmart} back-end sends \appsecret, the token, and mini-program ID (\ie, the unique identifier of each mini-program) to the \wechat server to get the \sessionkey that associated with the user. Fourth, when \texttt{Walmart} attempts to fetch sensitive information,  \wechat first encrypts the sensitive data with the \sessionkey and distributes the cipher of sensitive data to the front-end of \texttt{Walmart}. Finally, \texttt{Walmart} front-end sends the cipher to the its back-end, and back-ends de


  



% the resources maintained by the back-end of \wechat are also available to the mini-programs. As discussed, \wechat has more than 498 Million monthly active users, and a lot of valuable information has been collected from these users. Now,  


% including the \wechat's front-end and back-end, since a number of  



% While providing versatile functionalities, ensuring the security of such a complex system is always a challenging task. 







% To secure the mini-program framework and sensitive user data, \wechat has designed cryptographic key management mechanism, which involved 
 

% both built-in and add-on security mechanism: (1) The built-in security mechanisms are mandatory to all mini-programs. For example, \wechat provides a permission management framework to manage mini-program specific sensitive data and devices, e.g., the user account info. Similar to Android system, mini-programs can only access these resources when granted with the corresponding permissions.  (2) Considering the various needs of developers, \wechat also designed %some mechanisms that can be 
% a number of add-on security mechanisms that provide freedom to developers and only require them to be partially involved, and implement security functionalities based on \wechat's requirements. Although those security measures are not mandatory, if they are not correctly implemented, the consequences can be devastating. Therefore, \wechat explicitly or implicitly offered instructions for the developers to refer. For example,  for each app, \wechat assigns the developers a cryptographic key (called app secret), to allow the mini-programs to fetch sensitive user information from \wechat server (e.g., gender of users, phone number). Such a key, which explicitly required by \wechat, should be securely maintained by the back-end of the mini-program and not to be leaked to the front-end. 

%to be heavily involved and implement on their own. For example, when communicating with peripheral devices, developers can configure the security level of the device communication according to the devices' capabilities by setting whether the read/write encryption is enabled. This combination of built-in and add-on security mechanisms is expected to secure the mini-program framework well while keeping the mini-program versatile and convenient.

% Unfortunately, although the add-on security mechanisms are intended to enhance the framework security, we are surprised to discover that \wechat framework provides too much freedom of the add-on mechanisms, and this freedom, especially when misused or misconfigured, may significantly undermine the security and privacy of the entire framework. For example, we notice that there are cases where the global data decryption key, the aforementioned app-secret, is hard-coded in the front-end source code, which is written in Javascript and can be easily leaked when inspecting the mini-program APKs. This enables an attacker to arbitrarily modify the sensitive encrypted data, and may potentially fake their identify to attack the mini-program or make profit with multiple faked accounts at a low cost. Since this security issue is mainly caused by overwhelming freedom of the framework security mechanisms, We call this type of attack as \textit{C}ost \textit{OF} \textit{F}r\textit{EE}dom (\textsf{Coffee}) attack. 
% % \wechat did not perform any detection, auditing, or programmatic warning of potential session-key leakage in mini-program front-ends, except for a sentence in their official documentations, making developers unaware if a session-key is leaked by sloppy programmers in their development team.

% %We argue that there is an balance between build-in and add-on security measures, and in the context of mini-programs, \wechat fails to achieve it. Being an OS-alike entity, \wechat should enforce the security measures that   For example, OSes such as Android

% The \textsf{Coffee} attacks not only occur in these ``Add-on'' security functionalities that secure communication between the mini-program front-end and its back-end, but also occur in some other security related components. In the Bluetooth communication, instead of enforcing ``build-in'' secure configuration, \wechat allows the developers to customize the (or even disable) the secure configurations,  which allows the attacker to achieve unauthorized data access or MITM attacks.  We also found that in the cross-app communication, \wechat have removed a build-in whitelist mechanism that allowed the mini-programs to communicate with only ``trusted'' mini-programs, to give the flexibility to the developers.    With such a build-in white-list removed, the communication channel between two apps should be secured by the ``Add-on'' access control,  which implemented by the developers. 
% However, no instructions are given by \wechat by the time of our writing,  and as a result, the developers may ignore implementing the access control, leaving their cross-mini-program channels unprotected. 


% As such, in this paper, we investigate how a misused or misconfigured add-on security mechanism may undermine the built-in security of mini-program frameworks, making it vulnerable to \textsf{Coffee} attack. To further investigate this problem in this paper, we first summarize the security mechanisms of \wechat mini-programs, and compare the built-in and add-on mechanisms. Then, we present 
% Therefore, we first categorize and compare the add-on and built-in security mechanisms, and then raised five research questions of the add-on security mechanism usages. In this paper, we present 
%\textsf{MiniLyzer}, 


%a static analysis tool that scans security mechanism usage in mini-program packages with Control Flow analysis and Data Flow analysis, based on JavaScript Abstract Syntax Tree (AST), and automatically detect potential mechanism misuse, misconfiguration, and credential leakage.

%\ZY{Need to compare with the MK leak and other key leak}


% To understand the severity and prevalence of \appsecret leakage attacks,  we develop an efficient {\it mini-program crawler} that is able to search mini-programs based on keywords and download the mini-programs automatically using a special mini-program we developed, 
% %is built on top of the mini-program development framework (essentially a mini-program just for mini-program downloading), 
% and an {\it appsecret leakage vulnerability detector}.
% With a crawled mini-program, our detector scans the \appsecret, a 32-byte hexadecimal strings, and leverages an API provided by \wechat to confirm its genuineness. 
% \AY{To evaluate the prevalence of this problem, we scanned a total of 2 million mini-programs available on the \wechat mini-program market, and we found that there are a total of \leakedapps mini-programs have exposed their \appsecret, some of which are from high profile vendors, have leaked their {\appsecret}s, allowing attackers to manipulate enumerable data to break other user's account, or manipulate non-predictable data for fun and profit. Prior to the large-scale analysis, we manually identified a total of \largecompanycases mini-programs that are believed to be developed by top vendors, (\eg, \textit{Nestle}, \textit{HP}, and \textit{Tencent}), and we immediately reported this problem to \tencent to mitigate and inform the developers of their problem. \ZY{We do not have these any longer, right?} To measure their response to the disclosure, we re-downloaded the \largecompanycases mini-programs two months after our initial disclosure. We were surprised to find that, although some developers have fixed the exposure by removing the credential from their mini-programs, there are still developers who act passively to the disclosure: some developers merely refreshed their \appsecret, and some other developers left the leaked \appsecret{s} in their code without even refreshing them.} \sout{Our evaluation with the analyzed \totalanalyzedapps popular mini-programs, \leakedapps of them including some high profile vendors (\eg, \textit{Nestle}, \textit{HP}, and \textit{Tencent}) have leaked their {\appsecret}s, allowing attackers to manipulate enumerable data to break other user's account, or manipulate non-predictable data for fun and profit.} 
% To mitigate and/or prevent such vulnerability, we advocate that the platform vendor should
% %As such, we advocate a set of more prudent mini-program security mechanisms, including 
% vet mini-programs more systematically, design better data transmission protocols, use PKI to authenticate mini-program back-ends, and enforce signing and integrity checking. Finally, we have also disclosed \appsecret leakage vulnerabilities with the corresponding vulnerable apps to {\it Tencent}, and awarded with the bug bounty. We also learn that Tencent is actively working with the developers to fix this vulnerability and some of the mini-programs have already fixed it. \looseness=-1

%, and the corresponding fix is still in progress.


\ignore{
In this paper, we seek to understand the severity and prevalence of \appsecret leakage attacks, and meanwhile develop tools to detect the vulnerable mini-programs in the \wechat eco-system. To this end, we 
%
To measure the impact and severity of our attack, we implemented a tool and tested it with more than 1.2 million mini-programs.  our study revealed a concerning situation. We found that 3\% of the mini-programs leaked \appsecret, over 2\% of these mini-programs contained potential \sessionkey leakage. \ZY{Allen, please add some interesting results here to impress our readers}
}

%This credential leakage may enable attacker to intercept and modify arbitrary encrypted data to attack mini-programs for profit or steal sensitive user information. On top of that, we also found that none of the mini-program performs entry checking, making malicious mini-program may perform re-directions with fake extra data to attack these vulnerable mini-programs. This result indicates that there is still vulnerabilities undiscovered, although the mini-program framework had enforced various security mechanism, and therefore the balance between built-in and add-on mechanisms still needs to be re-evaluated. \AY{the data here is not real data yet.}\ZY{I think we need to discuss that we should make all security measures as build-in measure.}

% 
% enforced multiple build-in security mechanisms,  which do not require the third-party developers to be heavily involved (i.e., the developers can achieve these security protections by using simple API calls or configurations). For example, similar to Android system, mini-program framework has a permission management system that assigns permission to APIs associated with sensitive information such as user location and information.  To protect the network traffic,  \wechat also enforces an access control system based on network whitelist, under which only {\tt HTTPS} requests are allowed to be sent from mini-programs, and only trusted back-ends can be accessed. 

% Other than those build-in security mechanisms, \wechat also provided a number of ``Add-on'' security mechanisms, which require the developers to be partly involved, and implement security functionalities based on their own requirements. Although those security measures are not mandatory, if they are not correctly implemented, the consequences can be devastating. Therefore, \wechat explicitly or implicitly offered a well-documented instructions for the developers to refer. For example,  for each app, \wechat assigns the developers a cryptographic key (called app secret), to allow the mini-programs to fetch sensitive user information from \wechat server (e.g., user's gender, phone number). Such a key, which explicitly required by \wechat, should be securely maintained by the back-end of the mini-program and not to be leaked to the front-end.  


\ignore{
That is, instead of enforcing those mission critical security measures directly, \wechat gives the power of implementing security functionalities to developers, and those security functionalities  may server as safe-guard of sensitive data maintained by \wechat. This may causes grave consequences, as a sloppy third-party developers may implement the security measures in various faulty ways. For example, we observed that many mini-programs mistakenly hard-coded the aforementioned app-secrets in their source codes and as a result, the attackers can arbitrarily read, modify, and relay the sensitive information to perform an Man-In-The-Middle (MITM) attack. %In another of our example, \wechat provide security levels for Bluetooth pairing, 
We denoted this type of attack as \textsf{Coffee} (\textbf{C}ost \textbf{OF} \textbf{F}r\textbf{EE}dom) attack. 

The \textsf{Coffee} attacks not only occur in these ``Add-on'' security functionalities that secure communication between the mini-program front-end and its back-end, but also occur in some other security related components. In the Bluetooth communication, instead of enforcing ``build-in'' secure configuration, \wechat allows the developers to customize the (or even disable) the secure configurations,  which allows the attacker to achieve unauthorized data access or MITM attacks.  We also found that in the cross-app communication, \wechat have removed a build-in whitelist mechanism that allowed the mini-programs to communicate with only ``trusted'' mini-programs, to give the flexibility to the developers.    With such a build-in white-list removed, the communication channel between two apps should be secured by the ``Add-on'' access control,  which implemented by the developers. 
However, no instructions are given by \wechat by the time of our writing,  and as a result, the developers may ignore implementing the access control, leaving their cross-mini-program channels unprotected. 

To understand the impact of \textsf{Coffee} attack, we design an measurement tool, \tool, and analyzed \totalnumber mini-programs. We found that .....

The most important lesson learnt from our research is that it should never to assume that all developers are benign and hence offer the developers the freedom of security mechanism implementation, as the developers may not have the patience to read the documentations and understand the mechanism and significance of properly implementing secure measures well due to the frequent document updating and various other reasons. To ensure the security of such a complex paradigm that involves not only various platforms and devices but also heterogeneous back-ends, the designer of the platform are supposed to be aware that the mini-program developers should never be trusted. Therefore, instead of letting the mini-program developers to implement security features on top of APIs provided, the framework should have encapsulated all the vital security mechanisms well, and make them transparent to the developers.
}

%. On the other hand, the mini-program community is still actively introducing new features and frequently updating APIs and documentations, which makes it impossible for every developer to keep the most up-to-date understanding of the entire mini-program framework. t


%The most important lesson learnt from our research is that it should not offer the developers the freedom of security mechanism implementations even if we can assume that developers are benign, especially when designing the security mechanism over some novel paradigm. The developers may not have the patience to read the documentations and understand the mechanism and significance of properly implementing secure measures well due to the unaware of the threat model and various other reasons.  To ensure the security of such a complex paradigm that involves not only numerous users but also heterogeneous front-ends and the corresponding back-ends, instead of letting the mini-program developers to implement security features on top of APIs provided, the designer of the platform should have encapsulated all the vital security mechanisms well, and make them transparent to the developers.




%We argue that a security measure ``must'' be positioned as built-in,  as long as it ``can'' be positioned as built-in. The add-on security measures may be useful only when the security measures cannot be a part of the framework. For example, in the traditional programming frameworks provided by OSes, user authentication cannot be included as one of the built-in security mechanisms, since the user information is maintained at the server of the native apps rather than the OS. In this case, the add-on security measure is the only option. However, in the context of the mini-programs, \wechat maintains the user database, and it has the capabilities of including user authentication as a built-in security measure. Therefore, \wechat has integrated the user authentication as one of their built-in security measures. Such a practice secures the user authentication.  
%While \wechat has integrated many built-in security measures, it still leaves quite a few security measures as ``add-on''



\paragraph{Contributions} We make the following contributions: %The contributions are outlined as follows:
\begin{packeditemize}
    \item {\bf Systematic Understanding (\S\ref{sec:understanding}).} We are the first to systematically inspect the sensitive resource access protocols of mini-programs, leading to the discovery of the \appsecret leakage vulnerabilities in mini-programs.
    
    
    \item {\bf Practical Attacks (\S\ref{subsec:attackworkflow}).} We propose two types of novel attacks with leaked \appsecret: attacks against sensitive resources and attacks against cloud services.  
    %
     %
    %\item {\bf Practical Tool.} We develop a practical pipe-lined analysis framework that is able to automatically crawl mini-programs using keywords and detect the mini-programs that are subject to the \appsecret leakage attacks. Our crawler is developed using mini-program APIs and is more efficient and practical than existing crawlers. %The source code will be made public available.
    %
   % \item {\bf Real-world Implications.} 
    %Our evaluation with the automatically crawled \totalanalyzedapps mini-programs, the largest set of mini-programs,  shows that \leakedapps mini-programs that contain \appsecret leakage vulnerability. 
  %  We perform case studies on some vulnerable mini-programs from high-profile vendors such as Nestle, Bank of China and even Tencent themselves. 
  We demonstrate that these attacks can have devastating impacts in the super app ecosystem, such as hijacking user's account,  manipulating user's sensitive data, or consuming cloud services for free. %\textcolor{red}{We found that there are \leakedapps that are vulnerable to those attacks. }
    
    %attack case studies further show that with the leaked \appsecret, the attacker can log into arbitrary user's account, and manipulate various sensitive data for fun and profit (e.g., earning cashback and coupons).   
    
  \item {\bf Empirical Measurement (\S\ref{sec:measurement}).} Our evaluation with the automatically crawled \totalanalyzedapps mini-programs, the largest set of mini-programs,  shows that currently around \leakedapps of mini-programs that contain \appsecret leakage vulnerability.
   
   \item {\bf Possible Countermeasures (\S\ref{sec:discussion}).}  In addition to the responsible disclosure of this vulnerability as well as the list of \leakedapps mini-programs that leaked {\tt MK}s to \Tencent, we also shed light on the possible mitigations and preventions, particularly on how \Tencent could have fixed this issue.
    %\item We made responsible disclosure to \Tencent and our findings have been acknowledge by \Tencent developer team. \AY{Besides, we will release our analysis tool for the community to call for the awareness of potential vulnerabilities in this emerging paradigm.}

\end{packeditemize}

%\paragraph{Roadmap} 







%Such a practice 





%usually the weakest link of a system,     

 


% \ZY{Need to explain why the \sessionkey or app secret is needed} 
%The benefit of using such a cryptographic key instead of using an on-the-shelf interface is that  That is, instead of enforcing those security measures directly, \wechat provided more flexible interfaces for developers to customize, allowing the developers to have a balance between security and other considerations (e.g., usability).

\ignore{



It is surprising that such a mini-program platform involved with huge user base and massive sensitive data would allow developers to maintain the most vital keys on their own. To ensure the security of such a complex paradigm that involves not only various platforms and devices but also heterogeneous back-ends, the designer of the platform are supposed to be aware that the mini-program developers should never be trusted. Therefore, instead of letting the mini-program developers to implement security features on top of APIs provided, the framework should have encapsulated all the vital security mechanisms well, and make them transparent to the developers. Unfortunately, we found that for some of their most important security measures like maintaining \sessionkey, wechat merely provides a set of APIs and descriptions of how to properly maintain sensitive data in their documentations, rather than a mechanism to check whether the security mechanisms are properly implemented.


%based on their documented instructions. 


%to make sure that the network request of API invocation comes from a valid user. 

%Third, each mini-program has to go through a reviewing process before being published to the wechat mini-program market to identify potentially malicious or illegal mini-programs (e.g., fraudulous mini-programs). Fourth, wechat provides a special user risk detection API for developers to check whether a user is involved with fraudulous actions such as batch registration.



% may bring extra burde wechat mini-program marketens and sec being published to thurity concerns for developers: on one hand, the large amount of mini-program APIs that are constantly being revised, added, and removed makes the developers hard to obtain a correct, thorough, and up-to-date understanding; on the other hand, this complexity of mini-program functionalities opens various communication channels that can likely impair the security of mini-programs if they are mis-configured or misused by developers unfamiliar with mini-programs.

% the more APIs the mini-program host has, the longer the learning curve of getting familiar with those APIs will be. For the host apps, having a sophisticated API that may confuse the developers (e.g., require the developer handling the platforms' inconsistency), and when the API is related to security,  the app that uses the API may be subject to various vulnerabilities due to the sloppy implementations of unskilled developers. 

%Although these complex security mechanisms are supposed to protect mini-program against malicious mini-programs and users well, we are surprised to find that the mini-program security mechanism did not protect As an example of the serious security impact that a sloppy developer may bring to this complex subsystem, we observed that some mini-programs mistakenly leaks the session-key from their back-end server to the mini-program front-end. This session-key is the key to decrypt sensitive data sent from front-end to make sure the data is protected and not modified, which is supposed to be securely maintained by the back-end server and not to be leaked to the front-end. However, the developer mistakenly ignores the instructions of not leaking the \sessionkey and immediately sends the \sessionkey from the back-end server when the user logs in. As a result, the attackers can arbitrarily read, modify, and relay the sensitive information to perform an MITM attack.




It is never practical or secure to assume that all developers are benign and  hence offer the developers the freedom of security mechanism implementation. On one hand, the developers may not have the patience to read the documentations and understand the mechanism and significance of properly implementing secure measures well. On the other hand, the mini-program community is still actively introducing new features and frequently updating APIs and documentations, which makes it impossible for every developer to keep the most up-to-date understanding of the entire mini-program framework. Therefore, without a set of properly designed APIs that encapsulates necessary security mechanisms, vulnerability is inevitable when developers make mistakes when implementing these mechanisms on their own.


% Nevertheless, the developers are not the ones to be blamed. By looking into the official documentations, {\red{we found that although wechat had realized the challenge of enhancing the security of mini-program platforms and introduced mechanisms including scope management and cloud functions, their security countermeasures unfortunately merely covers minimal security requirements such as permission-like management and basic encryptions.}}\ZY{The description itself doesn't have too much connections with the previously provided example. In that example, you talk about \sessionkey and back-end etc. In the descriptions here, which based on my understanding, should be an explanations for the example,  however, you talk about some other stuffs including the scope management and cloud functions. I don't think the logic here flows.    }
% unfortunately do not cover all scenes due to the complexity of the paradigm. 
As to additional security measures, \wechat framework merely provided instructions and APIs for developers themselves to implement part of the security measures at their own risks, instead of providing a uniformed encapsulation in the SDKs or directly making these mechanisms transparent to developers.

This brings a common dilemma faced by app-in-app paradigms that combine native apps and webapps together in a sandbox-like subsystem: the dilemma between enhancing security and supporting versatile functionality. When the mini-program framework involves complex and heterogeneous platforms, devices, and self-configured back-ends, the framework can no longer enforce all security measures by itself with built-in mechanisms, because it can no longer control every involved entities.  \ZY{You story totally changed here. Our argument is being a cross-platform framework, \wechat should take care of everything. Now, you are saying that the framework can no longer enforce all the security measures by itself. So, what is our insight? The point is that \wechat can do something that makes the system more secure but they didn't do, not \wechat cannot do the security measures, so they have to leave it for the developers. In the second case, \wechat should not be blamed. } As a result, the framework may choose to prioritize their functionality requirements, offering freedom to mini-program developers at the expense of failure in splitting built-in and add-on security mechanisms properly to minimize the security impact of misuse and misconfiguration of sloppy developers.

In this paper, we investigate the communication security problems lying underneath the prosperity of mini-program freedom with static analysis of mini-program packages. Our study reveals a concerning situation. We discovered that foo and bar. \AY{I think this is going to be the first draft}
% that are rooted in the improperly designed security mechanisms and misunderstandings between developers and the framework.
% For example,  instead of providing an on-the-shelf transparent API for accessing WeChat data (e.g., Wechat user information), WeChat requires the developer to interact with the WeChat server multiple times, where encryption, authentication, and decryption are all involved.  Moreover, WeChat also requires the developers to protect the cryptographic keys used in the procedure. Obviously, all these requirements are too overwhelming for regular developers, therefore incurring various security holes for the developed mini-programs. In one of our examples, the attackers can arbitrarily record or even modify the encrypted network packets due to the leakage of the cryptographic keys, deploy MITM attacks against mini-programs. 

%\ZY{Allen, I have written three paragraphs based on my understanding. Please check and feel free to reach me out. }


%Such an ambitious computing paradigm extends the security and usability of host app by implementing a unified cross-platform webapp sandbox within the host app with JavaScript and V8 engine, where the access to peripheral devices, sensitive information, and cloud back-ends are monitored and managed by the host apps: developers can perform various actions ranging from accessing peripheral devices to communicating to back-ends through a set of mini-program-specific APIs with permission control or credential management mechanisms. With these APIs and mechanisms, the vendor host apps are able to provide the developers with versatility and security.

%However, although these mini-programs are believed to be properly managed and secured by the host apps, we are surprised to find that security problems still occur: for instance, we discovered that there are mini-programs that leaked their session-key which is a universally unique decryption key throughout the lifecycle of mini-programs. As a result, the communication security of the mini-program is significantly weakened, since attackers may arbitrarily record and edit the encrypted network packets to attack the mini-program. \ZY{We go too fast to the discoveries here. }

}

==> paper/02_background.tex <==
\section{Background}
\begin{figure}
    \includegraphics[width=\linewidth]{image/arch.pdf}
    \caption{The Three Mini-app Layers}
    \label{fig:arch}
\end{figure}

\subsection{The Mini-app Architecture}
As shown in \cref{fig:arch}, the architecture of \wechat mini-app framework consists of three layers: the host OS \ZY{OS? I think OS is not a part of the mini-app.}, the mini-app front-ends, and the mini-app back-ends.
\begin{itemize}[leftmargin=*]
    % \item \paragraph{Host OS layer} The host app runs atop the host OS. It provides and manages various OS system resources to the mini-apps.
    \item \paragraph{Mini-app front-end layer} The front-end mini-apps are distributed in the form of .wxapkg files that consists of JavaScript (JS) code, \wechat Marking Language files (WXML, wechat version of HTML), and \wechat Style Sheets (WXSS, wechat version of CSS). This front-end runs in a JavaScript environment provided by the host app. In this sandbox-like environment, the mini-app framework enforces various security mechanisms such as mini-app isolation and permission managements, as well as various functionalities via mini-app APIs for the mini-apps.
    \item \paragraph{Mini-app back-end layer} In most of the cases, there is a back-end server that processes network request and manages data generated by various users. This back-end can be a third-party server that runs \wechat server SDK, or a \wechat cloud base that provides cloud function feature.
\end{itemize}

\begin{table*}[]
    \centering
    \small
    \begin{tabular}{c|l|l|l}
    \toprule 
    Type&Mechanism&Built-in&Add-on\\ \midrule
    front-end&Permission management&authorization&---\\ 
    front-end&Device management&---&configuration\\
    front-end&In-mini-program plugins&isolation&---\\
    front-end&In-mini-program storage&isolation&---\\
    front-end&Background mini-app&lifecycle handling&---\\
    front-end&Mini-app redirection&whitelist&checking\\
    front-end&Private sharing&---&checking\\
    % front-end&Background management&y&\\
    back-end&Domain whitelist&whitelist \& blacklist$^{*}$&---\\
    back-end&Cloud API token (appsecret)&generation \& validation&maintainence\\
    back-end&Data encryption/decryption&encryption&decryption\\
    back-end&Cloud function&maintainance \& decryption&---\\
    % &&&---\\
    \bottomrule
    \end{tabular}
    \caption{mini-program Security Mechanisms}
    \label{tab:mechanisms}
\end{table*}

\subsection{Mini-app Security Mechanisms}
The complexity of mini-app framework makes it challenging to design security mechanisms to protect user data and cloud communication from being intercepted and exploited. To achieve this goal, \wechat combined the built-in and add-on security mechanisms to balance the security and usability. In this section, we introduce the built-in and add-on mechanisms separately and compare their advantages and their disadvantages.
% The reason why wechat has adopted such a complex security mechanism lies in the complex functionality involved in the mini-app paradigm. To gain an edge from native applications in terms of usability, funcitonality, and security, wechat is not merely a normal native application any more, but instead an OS-like ecosystem that involves both native OS resources and heterogeneous back-ends. On top of that, the requirement of using their own third-party servers from business vendors that would like to integrate their services into mini-apps requires wechat to support third-party back-ends and enforce data encryption, which elevated the challenge of securing the mini-app data while maintaining the versatile functionality. In this section, we discuss the threat model that wechat mini-app adopts as described in their official documentations when designing these mechanisms, and then provide a detailed comparison of wechat security mechanisms.
\ZY{How about remove host OS section, and put the content at the mini-app front-end?}
% \subsection{Host OS}
% In the mini-app paradigm, the host app plays a critical role in OS resource management. The security mechanisms in this layer to manage and secure the resource accesses can be summarized into three main categories: built-in permission management, which requires developers' configuration; built-in storage isolation, which is fully transparent to developers, and device management, which provides optional add-on security for developers.

\begin{figure}[h!]
    \includegraphics[width=\linewidth]{image/permission.pdf}
    \caption{Three ways to use mini-app authorization scopes}
    \label{fig:permission}
\end{figure}

\begin{figure*}[ht]
    \includegraphics[width=.8\linewidth]{image/front-end.pdf}
    \caption{The Front-end Mini-apps}
    \label{fig:front-end}
\end{figure*}

\subsubsection{Mini-app Front-end}
As shown in \cref{fig:front-end}, the complex mini-app framework does not only manages system resources, but also handles the mini-app front-end lifecycles. The mini-apps can be shared among different users, where users can click on the link to enter mini-apps. Aside from directly clicking to enter, mini-apps can also be launched via cross-mini-program navigation. To manage these mini-apps, the framework not only handles the background mini-app behavior, but also enforces isolation to protect mini-app data.


\paragraph{System resource management}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Permission management} To protect sensitive resources, the mini-app framework introduces the concept of `authorization scope', the mini-app version of system permission, to manage different types of OS resources. Built atop the host OS, compared with the host OS permission system, the mini-app permission mechanism focuses more on sensitive user information at a finer granularity: aside from camera, location, and recording, there are also scopes associated with user data such as account info, user album and \wechat sport data. As shown in \cref{fig:permission}, the mini-app can actively trigger the users to authorize the scopes by invoking \texttt{wx.authorize()} API (line 02 of main.js) or configuring the required permission in the \texttt{app.json} file (line 02 of app.json). Otherwise, the user will be notified to allow or reject the scope usage when the associated APIs is invoked (e.g., when \texttt{startRecord()} is invoked in line 05). If the user have already grant a scope, the user's preference will be saved, and this granted permission will not be revoked until the user uninstalls the mini-app or manually opens the menu to cancel the scope authorization.
    \item \paragraph{Device management} When accessing various peripheral devices, developers can configure the device to enable certain security features to enhance security or disable them, according to the capability of the devices. For instance, the developers can set the parameter \texttt{writeEncryptionRequired} to \texttt{true} or \texttt{false} to enable or disable encryption when reading or writing data.
\end{itemize}

\paragraph{In-miniapp management}
\begin{itemize}[leftmargin=*]
\item \paragraph{In-miniapp plugin management} Many mini-app developers have integrated plugins, a special type of mini-app, in their own mini-apps to to extend the functionality. To prevent plugins from eavesdropping sensitive information from the mini-apps, the in-app page redirection is restricted: only redirection from mini-app to plugin is allowed: plugins cannot actively redirect to a specific mini-app page via \texttt{wx.redirectTo()}. However, both mini-apps and plugins can redirect to their own pages.

\item \paragraph{In-miniapp storage management} To defend against horizontal privilege escalation, mini-apps running in \wechat are isolated at user level, meaning that different users and different mini-apps cannot access the isolated storage space between each other. In Android, each mini-app has a local storage in the \texttt{com.tencent.mm/} folder, which is not accessible by normal phone users unless the device is rooted. Each user in each mini-app can only access their own storage space.
\item \paragraph{Background mini-app management} The mini-app lifecycle is maintained by the mini-app framework. When the user exits a mini-app, the mini-app will stay in background, so that it loads quicker if the user re-enters the mini-app. If the background mini-app exceeds the limit or there is not enough system resources, the framework will kill the mini-app to release the system resource. 
% in background: if there are over 5 mini-apps in the background, the earliest mini-app will be killed. 
On top of that, the background mini-app functionalities are restricted. For example, the timer of sensors become inaccurate in the background, and background behaviors such as voice recording will be ineffective. However, there is one exception: if the mini-app is granted with the specific background location updating scope, it can keep on updating user's location in the background without being restricted.
\end{itemize}
\paragraph{Cross-miniapp management}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Cross-miniapp redirection} A user can navigate to multiple mini-apps via \texttt{wx.navigateToMiniprogram()}. This API allows mini-apps to redirect to other mini-apps with extra data to perform complex actions. \wechat had a built-in whitelist mechanism that required every developer to declare up to 10 navigation mini-app targets in the configuration file. However, this requirement is discontinued after version \AY{todo}, and hence it is for developers to check the mini-app navigation source since there is no longer built-in mechanism. The developers can check which mini-app the user is navigating from by obtaining the \texttt{appId} parameter in the \texttt{referrerInfo} when the mini-app launches.
    \item \paragraph{Private sharing} Generally, a mini-app can be shared by multiple users, but developers can also control the distribution of the mini-app with private sharing feature. When a user uses this feature to share a mini-app to a certain friend or a group, this mechanism only allows first-hand receiver (the specific friend, or the users in the group) to enter the mini-app, whereas second-handed users (users receiving the re-shared invitation) cannot. When some mini-app vendors offer special discount for a high-level user when he/she introduces new members to use their mini-apps or services, this feature will be useful to prevent malicious users from acquiring multiple account to repeatedly get the discounts to make profit. Developers can check whether the shared link is valid via \texttt{wx.authPrivateMessage}
\end{itemize}
\subsubsection{Mini-app Back-end}
\begin{figure}
    \includegraphics[width=\linewidth]{image/back-end.pdf}
    \caption{The Back-end Communication Key Mechanism}
    \label{fig:back-end}
\end{figure}
The mini-app mechanism relies heavily on network communications with \wechat servers and cloud back-ends to process user data and provide various functions. As such, it is vital to secure the communication of user's sensitive data properly from being intercepted by malicious users or exploited by attackers. \wechat has enforced multiple security mechanisms to deal with this problem, which can be summarized into the following four categories.

\paragraph{Third-party back-ends}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Domain whitelist} \wechat enforced a domain whitelist mechanism to make sure that a mini-app can only communicate with pre-configured domains. Developers can control which domain a mini-app can communicate any time. Meanwhile, mini-app front-ends cannot communicate with the \wechat network API domain: these APIs are supposed to only be accessible by third-party back-ends. This is enforced to prevent the insecure front-end from accessing sensitive data directly from wechat server, since malicious users may be able to intercept the network packets.
    \item \paragraph{Network API token} Since \wechat has a set of network APIs for back-end servers that can be invoked via network requests, if a network API is invoked by malicious user, it may reveal sensitive information that exposes mini-apps in danger. To verify whether the invoker of a network API is valid, \wechat assigns a specific credential called `appsecret' to each mini-app. When invoking these network APIs, developers have to provide both the mini-app id and the corresponding appsecret.
    % viral data such as api invocation token and session key used by mini-app users.
    \item \paragraph{Data encryption and decryption} As shown in \cref{fig:back-end}, every time when a user logs in, a login token will be generated by the \wechat host app. Then, this login token is sent to the back-end server who eventually acquires and maintains the essential session key, the global encryption key of user data, of the current user. This is done by invoking the network API \texttt{jscode2session} with the mini-app id and appsecret. Then the cloud back-end can use the appsecret to invoke wechat network APIs to acquire various user information (e.g., user account info) or perform various actions (e.g., generate an invoice), and use the session key to decrypt all the encrypted sensitive data ,including user account info, weRun data, and invoices. 
\end{itemize}
\paragraph{Wechat built-in back-ends}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Cloud functions} To make the development safer and easier, \wechat provides a cloud function feature for developers to access user sensitive data. This cloud function mechanism encapsulates the session-key exchange and data decryption to prevent developers from mis-configuring the maintenance of appsecrets and session-keys. For example, when invoking \texttt{wx.getWeRunData()}, developers does not need to decrypt the encrypted data by themselves. Instead, the developers can used a \texttt{cloudID} returned by the JS API that is mapped to the specific sensitive data and directly obtain the decrypted data from the wechat server with \texttt{wx.cloud.CloudID()}.
\end{itemize}





\subsection{Built-in VS Add-on}
\paragraph{The Limitation of Built-in Mechanism}

% In the wechat mini-app framework, the built-in mechanisms can be summarized into the following two mechanisms:
% \begin{itemize}
%     \item \paragraph{Non-interactive mechanism} These mechanisms are non-configurable and transparent to the developers: the developers cannot intefere or customize the mechanisms. The storage and plugin isolation and domain
%     \item \paragraph{Interactive mechanism}
% \end{itemize}
% The built-in security mechanisms of wechat mini-app includes isolation, lifecycle handling, whitelists, blacklists, permission authorization, and data encryption.
% \paragraph{Usability or security, that is a question} 
To ensure the safety of mini-apps running in \wechat, mandatory built-in mechanisms ensures that all the mini-apps running in the framework have enforced the necessary security protections. For example, each developers must request and authorize permissions when using specific system resources. Therefore, the OS resource will never be accessed if the permission is not granted. Secure as these built-in mechanisms are, however, they still suffer from disadvantages in two ways:
\begin{itemize}[leftmargin=*]
    \item \paragraph{Impairing usability} The built-in security mechanisms may require mandatory configuration from the developers, thus making the development process more complex. For example, in an earlier stage of mini-app framework, all developers are required to configure a navigation mini-app id list. As such, navigation to mini-apps that are not in this white list will not be allowed. This mechanism is initially designed to prevent unexpected navigation if malicious attackers hijacks the mini-app by hooking mini-app interfaces. However, when developers need to redirect to additional mini-apps, they have to re-configure the mini-app ids in their configuration files, re-compile the mini-app, and make users to update the mini-apps. This had raised complaints about the usability of mini-app frameworks among developers in the forum. As a result, \wechat removed the requirement of mini-app navigation configuration starting from 2018.
    \item \paragraph{Limiting functionality} Built-in security mechanisms may limit the functionalities of mini-apps. For example, although \wechat provided a `cloud function' feature to let users easily communicate with cloud back-ends without knowing the login authentication and data decryption mechanisms, they still allow developers to use third-party back-ends. Since there is a great amount of companies that wish to make use of their own back-end servers to link user account info and data with other platforms (e.g., PC app, Android app, etc.), it is not practical for \wechat to force all mini-app developers to use cloud function features, otherwise the mini-app loses its edge against native apps for the service providers due to the limited functionalities.
\end{itemize}
\paragraph{The Cost of Add-on Freedom}
There is no doubt that the add-on security mechanisms enforced atop built-in mechanisms are supposed be enhancing the framework security. 
However, we are surprised to find that it is not always true, 
especially when they are misused by developers, which is inevitable: instead of merely making add-on configuration ineffective, the misuse of add-on security may leak critical information that undermines the entire security mechanism of mini-app framework. \AY{Originally, the rest of this part is now in }

==> paper/02_background_back.tex <==



\section{Mini-app Security Mechanisms}
\begin{figure}
    \includegraphics[width=\linewidth]{image/arch.pdf}
    \caption{The Three Mini-app Layers}
    \label{fig:arch}
\end{figure}
As shown in \cref{fig:arch}, the architecture of \wechat mini-app framework consists of three layers: the host OS, which provides various system resources to the mini-apps; the front-end, which runs in a JavaScript environment provided by \wechat host app; an optional mini-app back-end, which provides cloud-based functionalities for developers to maintain user data, process cloud requests, and communicate with the \wechat server. The JavaScript environment provides various mini-app APIs for the front-ends to request OS resources (e.g., user data and peripheral devices), and send network requests to their back-ends. For the back-ends, mini-app functionalities can be provided via the \wechat cloud function service or their own back-end servers, to communicate with the mini-app front-end and \wechat host server via network requests.

% \paragraph{Host OS} The mini-apps are webapp-like applications running in the JavaScript environment of host app \wechat. This environment provides and manages various system resources to the mini-apps, ranging from peripheral devices to user media and user data.

% \paragraph{Mini-app front-end} The mini-apps are distributed to the user devices in the form of `wxapkg' file, a compressed binary file that consists of JavaScript codes, Wechat Mark Language (WXML) files and Wechat style sheet (WXSS) files. The JavaScript codes in the package forms the essential part of mini-app front-end where most of the functionalities of mini-apps are performed via various mini-app APIs. 

% \paragraph{Cloud back-end} In most of the cases, the mini-app relies on a cloud back-end to handle user data generated by various users from their devices. This cloud back-end can either be a third-party server that runs mini-app back-end SDK or the \wechat cloud functions. The communication with \wechat server and front-end users are performed via network requests when the developers use third-party back-ends, and mini-apps API \texttt{wx.cloud.callFunction()} when using \wechat cloud function.

% and provides functionalities by sending network requests to various urls in wechat API domain \texttt{api.weixin.qq.com}, or by developing wechat cloud functions and using mini-apps API \texttt{wx.cloud.callFunction} to access them.

For all these three layers, as shown in \cref{tab:mechanisms},  wechat has designed various security mechanisms, both built-in and add-on:
% , to achieve a balance between usability and security.
the built-in mechanisms are mandatory, which means that the developers cannot customize the mechanism (e.g., storage isolation) or must configure the mechanism to run their mini-apps in the framework (e.g., permission authorization); the add-on mechanisms are optional, which can be configured by developers if they need to enforce additional protection for their mini-apps (e.g., private sharing).

\begin{table*}[]
\belowrulesep=0pt
\aboverulesep=0pt
    \centering
    \begin{tabular}{c|l|l|l}
    \toprule 
    Type&Mechanism&Built-in&Add-on\\ \midrule
    OS&permission management&permission authorization&---\\ 
    OS&device management&---&device secuirty configuration\\
    front-end&in-mini-program plugins&mini-app plugin isolation&---\\
    front-end&in-mini-program storage&mini-app storage isolation&---\\
    front-end&background mini-app&mini-app lifecycle handling&---\\
    front-end&mini-app redirection&mini-app redirection whitelist&redirection source checking\\
    front-end&mini-app private sharing&---&private sharing checking\\
    % front-end&Background management&y&\\
    back-end&back-end communication&domain whitelist \& blacklist$^{*}$&---\\
    back-end&network API token (appsecret)&token generation \& validation&API token maintenance\\
    back-end&data encryption (session key)&data encryption&data decryption \& session key management\\
    back-end&cloud function&user validation \& data decryption &---\\
    % &&&---\\
    \bottomrule
    \end{tabular}
    \caption{Miniapp Security Mechanisms}
    \label{tab:mechanisms}
\end{table*}

\subsection{OS Resources}
\begin{figure}
    \includegraphics[width=\linewidth]{image/permission.pdf}
    \caption{Three ways to use mini-app permission scopes}
    \label{fig:permission}
\end{figure}
In the mini-app paradigm, the host app plays a critical role in OS resource management. The security mechanisms in this layer to manage and secure the resource accesses can be summarized into three main categories: built-in permission management, which requires developers' configuration; built-in storage isolation, which is fully transparent to developers, and device management, which provides optional add-on security for developers.

\paragraph{Permission management} To protect sensitive resources, the mini-app framework introduces the concept of `authorization scope', the mini-app version of system permission, to manage different types of OS resources. Built atop the host OS, compared with the host OS permission system, the mini-app permission mechanism focuses more on sensitive user information at a finer granularity: aside from camera, location, and recording, there are also scopes associated with user data such as account info, user album and \wechat sport data. As shown in \cref{fig:permission}, the mini-app can actively trigger the users to authorize the scopes by invoking \texttt{wx.authorize()} API (line 02 of main.js) or configuring the required permission in the \texttt{app.json} file (line 02 of app.json). Otherwise, the user will be notified to allow or reject the scope usage when the associated APIs is invoked (e.g., when \texttt{startRecord()} is invoked in line 05). If the user have already grant a scope, the user's preference will be saved, and this granted permission will not be revoked until the user uninstalls the mini-app or manually opens the menu to cancle the scope authorization.

% This scope usage can be granted in two ways, either statically or dynamically: developers can configure the scope in their config file, and thus the users will have to confirm the scope usage when they first enters the mini-app; or the developers can use \texttt{wx.authorize()} API to dynamically request the scopes, and then the user will have to confirm the scope usage in a prompted dialog.

\paragraph{Device management} When accessing various peripheral devices, developers can configure the device to enable certain security features to enhance security or disable them, according to the capability of the devices. For instance, the developers can set the parameter \texttt{writeEncryptionRequired} to \texttt{true} or \texttt{false} to enable or disable encryption when reading or writing data.

% \item Resource management. To defend against permission escalation, wechat built a resource management system themselves atop the host OS. This system secures the access to system resources through permission granting and prompted dialogs. On one hand, it defined a set of `authorization scopes' (similar to permissions in Android system) that covers sensitive devices and information such as cameras, recorders, user weRun data (wechat sports data), and user location. Mini-apps should either declare their required scopes in their config file, then the users will have to grant all of them when first entering the mini-app; or use wx.authorize(scope) API to grant scopes dynamically, then user has to confirm the scope usage in a prompted dialog). On the other hand, however, there is a set of critical system resources that has to be confirmed by users every time the mini-app requests it, e.g., user's account info and user contacts. 

\subsection{Front-ends}
\begin{figure*}
    \includegraphics[width=\linewidth]{image/front-end.pdf}
    \caption{The Front-end Mini-apps}
    \label{fig:front-end}
\end{figure*}
As shown in \cref{fig:front-end}, the complex mini-app lifecycles are handled by the mini-app framework. The mini-apps can be shared among different users, where users can click on the link to enter mini-apps. Aside from directly clicking to enter, mini-apps can also be launched via cross-miniapp navigation. To manage these mini-apps, the framework not only handles the background mini-app behavior, but also enforces isolation to protect mini-app data.

% mini-apps running in the host apps can be launched by direct clicking the mini-apps, or automatically redirected from an already launched mini-app. These mini-apps can be shared among different users as links. The lifecycle of these mini-apps are maintained by the framework.
% The framework decides when to destroy mini-app based on the background mini-app limit and the available system resources. 
% Besides, there is a cross-miniapp communication mechanism similar to Android Intent 
% , and is similar to that of Android native app in that there are multiple ways to launch and destroy a mini-app. When launching a mini-app, a user can either click open a mini-app or redirect to another mini-app via a prompted dialog. To destroy a mini-app, a user can either manually kill the instance or move it to background and let the framework decide how to maintain and destroy the mini-app. Mini-apps can perform complex functionalities by collaborating with other mini-apps: mini-apps can integrate plugins, a special type of mini-app that provides modular functionalities for mini-apps Similar to the Android Intent, \wechat has a cross-miniapp communication mechanism 
% in which developers can attach extra data when redirecting to another mini-app. In general, the front-end mechanism can be summarized into four categories: mini-app entry checking, in-miniapp isolation, cross-miniapp navigation, and background mini-app management.


\paragraph{In-miniapp mechanisms}
\begin{itemize}[leftmargin=*]
\item \paragraph{In-miniapp plugin management} Many mini-app developers have integrated plugins, a special type of mini-app, in their own mini-apps to to extend the functionality. To prevent plugins from eavesdropping sensitive information from the mini-apps, the in-app page redirection is restricted: only redirection from mini-app to plugin is allowed: plugins cannot actively redirect to a specific mini-app page via \texttt{wx.redirectTo()}. However, both mini-apps and plugins can redirect to their own pages.

\item \paragraph{In-miniapp storage management} To defend against horizontal privilege escalation, mini-apps running in \wechat are isolated at user level, meaning that different users and different mini-apps cannot access the isolated storage space between each other. In Android, each mini-app has a local storage in the \texttt{com.tencent.mm/} folder, which is not accessible by normal phone users unless the device is rooted. Each user in each mini-app can only access their own storage space.
\item \paragraph{Background mini-app management} The mini-app lifecycle is maintained by the mini-app framework. When the user exits a mini-app, the mini-app will stay in background, so that it loads quicker if the user re-enters the mini-app. If the background mini-app exceeds the limit or there is not enough system resources, the framework will kill the mini-app to release the system resource. 
% in background: if there are over 5 mini-apps in the background, the earliest mini-app will be killed. 
On top of that, the background mini-app functionalities are restricted. For example, the timer of sensors become inaccurate in the background, and background behaviors such as voice recording will be ineffective. However, there is one exception: if the mini-app is granted with the specific background location updating scope, it can keep on updating user's location in the background without being restricted.
\end{itemize}
\paragraph{Cross-miniapp mechanisms}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Cross-miniapp redirection} A user can navigate to multiple mini-apps via \texttt{wx.navigateTomini-program()}. This API allows mini-apps to redirect to other mini-apps with extra data to perform complex actions. \wechat had a built-in whitelist mechanism that required every developer to declare up to 10 navigation mini-app targets in the configuration file. However, this requirement is discontinued after version \AY{todo}, and hence it is for developers to check the mini-app navigation source since there is no longer built-in mechanism. The developers can check which mini-app the user is navigating from by obtaining the \texttt{appId} parameter in the \texttt{referrerInfo} when the mini-app launches.
    \item \paragraph{Private sharing} Generally, a mini-app can be shared by multiple users, but developers can also control the distribution of the mini-app with private sharing feature. When a user uses this feature to share a mini-app to a certain friend or a group, this mechanism only allows first-hand receiver (the specific friend, or the users in the group) to enter the mini-app, whereas second-handed users (users receiving the re-shared invitation) cannot. When some mini-app vendors offer special discount for a high-level user when he/she introduces new members to use their mini-apps or services, this feature will be useful to prevent malicious users from acquiring multiple account to repeatedly get the discounts to make profit. Developers can check whether the shared link is valid via \texttt{wx.authPrivateMessage}
\end{itemize}





    
% \item Redirection checking. In mini-app redirection, extra information can be attached just like Android Intent. If a mini-app is launched via mini-app redirection (other than clicking-open), the developers can read the extra data, appid, and url params by getting the \texttt{referrerInfo} via \texttt{wx.getLaunchOptions} or \texttt{wx.getLoadOptions}. Developers can check the extradata with these information to prevent null redirection intents.
    % \item Secret sharing verification. In a recent update, wechat introduced a new feature called secret sharing. 
\subsection{Back-ends}
\begin{figure}
    \includegraphics[width=\linewidth]{image/back-end.pdf}
    \caption{The Back-end Communication Key Mechanism}
    \label{fig:back-end}
\end{figure}
The mini-app mechanism relies heavily on network communications with \wechat servers and cloud back-ends to process user data and provide various functions. As such, it is vital to secure the communication of user's sensitive data properly from being intercepted by malicious users or exploited by attackers. \wechat has enforced multiple security mechanisms to deal with this problem, which can be summarized into the following four categories.

\paragraph{Third-party back-ends}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Domain whitelist} \wechat enforced a domain whitelist mechanism to make sure that a mini-app can only communicate with pre-configured domains. Developers can control which domain a mini-app can communicate any time. Meanwhile, mini-app front-ends cannot communicate with the \wechat network API domain: these APIs are supposed to only be accessible by third-party back-ends. This is enforced to prevent the insecure front-end from accessing sensitive data directly from wechat server, since malicious users may be able to intercept the network packets.
    \item \paragraph{Network API token} Since \wechat has a set of network APIs for back-end servers that can be invoked via network requests, if a network API is invoked by malicious user, it may reveal sensitive information that exposes mini-apps in danger. To verify whether the invoker of a network API is valid, \wechat assigns a specific credential called `appsecret' to each mini-app. When invoking these network APIs, developers have to provide both the mini-app id and the corresponding appsecret.
    % viral data such as api invocation token and session key used by mini-app users.
    \item \paragraph{Data encryption and decryption} As shown in \cref{fig:back-end}, every time when a user logs in, a login token will be generated by the \wechat host app. Then, this login token is sent to the back-end server who eventually acquires and maintains the essential session key, the global encryption key of user data, of the current user. This is done by invoking the network API \texttt{jscode2session} with the mini-app id and appsecret. Then the cloud back-end can use the appsecret to invoke wechat network APIs to acquire various user information (e.g., user account info) or perform various actions (e.g., generate an invoice), and use the session key to decrypt all the encrypted sensitive data ,including user account info, weRun data, and invoices. 
\end{itemize}
\paragraph{Wechat built-in back-ends}
\begin{itemize}[leftmargin=*]
    \item \paragraph{Cloud functions} To make the development safer and easier, \wechat provides a cloud function feature for developers to access user sensitive data. This cloud function mechanism encapsulates the session-key exchange and data decryption to prevent developers from mis-configuring the maintenance of appsecrets and session-keys. For example, when invoking \texttt{wx.getWeRunData()}, developers does not need to decrypt the encrypted data by themselves. Instead, the developers can used a \texttt{cloudID} returned by the JS API that is mapped to the specific sensitive data and directly obtain the decrypted data from the wechat server with \texttt{wx.cloud.CloudID()}.
\end{itemize}

% \begin{itemize}
    % \item Credential maintainence. Although wechat provides a cloud function mechanism that makes the session-key management and data decryption fully transparent to developers to make the developement easier and more secure, there are still a large number of mini-app that uses third-party server for more versatile functionalities. Therefore, when the developers are configuring their third-party servers, they have to maintain these credentials properly and prevent sensitive information, especially appsecrets and session-keys from being leaked to the front-end.
% \end{itemize}


%To run mini-apps across platforms in the host apps, the host app integrates a JavaScript runtime with a set of mini-app specific JavaScript APIs. The mini-apps are developed in JavaScript language with multiple WXML (WeiXin Markup Language) and WXSS (WeiXin Style Sheet) files that are built upon HTML and CSS with mini-app specific features.

% The mini-apps are webapp packages with js, wxml, and wxss that run in mini-app framework. The framework handles both mini-apps, peripheral devices, and network communication.
\ignore{
\subsection{Mini-app Communication}

To achieve the native experiences for mini-apps, the mini-apps have to access to different types of data that available in our smart devices (e.g., Android phones or iOS phones), and this is achieved through different communication mechanisms.
Since all the mini-apps run atop the host app (i.e., \wechat), the host app is now responsible for establishing the communication channels between each app and other communication entities such as the underlying OS, a remote server and another mini-app. 
 
%As shown in \autoref{tab:resouces}, for achieving better understanding, we compare the  mini-app security measures with that of native apps.  
 
  
 
\paragraph{Communication with OS} One of the most impressive features of mini-apps is that the mini-apps have the capabilities of communicating with the underlying OS, through which the mini-apps can provide native-app-like experiences for its users, especially with better support for peripheral access (e.g., Bluetooth device access). This is also one major difference between the mini-apps and the traditional Web-apps (which host into browsers instead of running on the top of native apps)~\cite{whitepaper20}. To communicate with the OS and use its resources (e.g., location services, microphone), \wechat extends the permission check mechanism from the mainstream OSes, through which \wechat can deliver the resources selectively based on the developers configuration and the user's selection. That is, before the use of the system resources, the developer shall configure the corresponding permissions while programming, and each permission must be granted by the user to obtain the resources. %The permission check mechanism is similar to that in native apps. 


\paragraph{Communication with Back-ends} Similar to the native apps, mini-apps can also have back-ends. As discussed, the accesses to network data of an mini-app are also monitored (i.e., network whitelisting policy) or fully controlled (i.e., Cloud base) by the host app. Particularly, in order to attract more vendors to host their mini-apps onto the platform and provide better services,  \wechat offers the interfaces for the back-ends of mini-apps to fetch sensitive data collected by \wechat. The data includes user basic information such as the gender, regions that the user lives and the phone number. By using these data, vendors may have better profile of their user, and achieve personalized recommendation or advertisements.  

\paragraph{Communication with Other Apps} Two mini-apps can also communicate with each other to exchange the data of interest. This is extremely common in the world of mini-app (based on our experiment, {\red{XXX}} mini-apps have enabled such an channel).  This is because the each mini-app can have a maximal size of 12 MB, which can implement relatively limited functionalities. Having the capabilities of communicating with other mini-apps will enrich the functionalities of each mini-app without consuming the valuable storage resources. For example, we observed some mini-apps, which do not have the capabilities of playing video, may deliver the video url to another media player mini-app for video playing.     
 
The communication channel is established through a pair of API, namely \textsf{navigateToMiniProgram} and \textsf{navigateBackMiniProgram}. To be more specific one mini-app $mini_{A}$ can launch and deliver messages to another mini-app $mini_{B}$ by calling \textsf{navigateToMiniProgram(Object msg)} (\texttt{msg} is the message that $mini_{A}$ attempts to deliver). The message contains a unique identifier of $mini_{B}$, and $mini_{B}$ can also react to the API call by calling \textsf{navigateBackMiniProgram(Object msg)} to respond back to $mini_{A}$.% \autoref{listing:cross} demonstrate the cross-app communication process. 


  
\ignore{ 

\begin{minipage}{1\textwidth}
\noindent\begin{minipage}{0.95\textwidth}
\begin{lstlisting} [caption={}, basicstyle=\footnotesize\ttfamily ]
 wx.navigateToMiniProgram({
  appId: "wx2d495bf4b2xxxxxx",
  extraData: {
    a: 39,
    b: 40
  },
  success: function (e) {
    // data transmission succeeded
  },
  fail: function (e) {
    // data transmission failed
  },
});
\end{lstlisting} 
\end{minipage} 
 
 
\noindent\begin{minipage}{0.95\textwidth}
\begin{lstlisting} [caption={},label={list:navigate},basicstyle=\footnotesize\ttfamily  ]
//code fragment to receive data
var options = wx.getLaunchOptionsSync();
 
var a;
a=options.referrerInfo.extraData.a;
var b
b=options.referrerInfo.extraData.b;

wx.navigateBackMiniProgram({
  extraData: {
    feed_back: "data received",
  },
});
\end{lstlisting} 
\end{minipage}
 \end{minipage}\makeatletter\def\@captype{lstlisting}\makeatother\caption{Cross-app communication channel}\label{listing:cross} 
 }
 
\subsection{Security Mechanisms of Mini-apps}
 
As there are three major communication entities that a mini-app can communicate with, the security measures are mainly provided for securing the three corresponding procedures. Particularly, these security measures can be categorized into two groups, i.e., build-in security measures that enforced by \wechat and add-on security measures that customized by the developers. In the following, we enumerate the major security measures: 

\paragraph{Securing Communication with OS} The available build-in security measures for securing the channel between the mini-app and the underlying OS is the permission checking mechanism. As discussed earlier, the system resources can only be consumed after the user's consent. Among all the available permissions,  some permissions such as Bluetooth need to be granted every time the user uses the related system resources, while others such as location based services, the user only need to grant the permission once. \wechat enforces the use of permission checking for the major system resources, meaning that without configuring and requesting the permission, developers cannot access those system resources. 

Other than the build-in security measures, some resources are also protected by add-on security measures. Bluetooth security level is one of these add-on security measures, where the developers can customize the security levels to protect the data provided by the mini-app.  In particular, a mini app can provide data services for other smartphones or some  peripherals to consume, and the mini-app can require a minimal security level, which specifies how services can be accessed. When the security status does not suffice the required security level (e.g., requiring the link encryption but only plaintext communication are achieved), the data access request will be rejected by \wechat. Different from the build-in protection policies, the security levels are configured by the developers through API \texttt{addServices} and the passed parameters. For example, \texttt{readEncryptionRequired} indicates that services can only be accessed when the link is encrypted.   

\paragraph{Securing Communication with Back-ends}
Appsecret mechanism. 

Session-key mechanism. In the security model of wechat mini-app, the front-end is always untrusted. To protect the communication with back-ends, wechat enforced a session-key mechanism, in which the session key is only known to mini-app backends and wechat servers, whereas the untrusted mini-app frontend is fully unaware of the session-key. To achieve this, the entire communication process starts when the mini-app user triggers \texttt{wx.login()}. When the user successfully logs in, wechat server returns a login token, which is then sent to the back-end server to eventually get the user identifier (the `openid') and the session-key used to decrypt the encrypted sensitive data sent by wechat native app such as WeRun data. To access session-keys from the back-end, the server invokes a network API with its appid, appsecret (a secret key generated by wechat for each mini-app to verify the invoker of each network API), and the user login token. During this process, the untrusted front-end is only aware of the user token, and the sensitive appsecret and session-key is maintained by the back-end server and shall never be leaked to the front-end.

Cloud function. (Why still allows third-party server) To make the cloud development safer and easier, wechat provided a cloud function feature for developers to access user sensitive data. This cloud function mechanism encapsulates the session-key exchange and decryption to prevent developers from mis-configuring the maintainence of appsecrets and session-keys. For example, when invoking wx.getWeRunData(), developers does not need to decrypt the encrypted data by themselves. Instead, the developers can used a cloudID that is mapped

% To protect sensitive user information sent to back-ends such as user info from being intercepted during back-end communication, wechat encrypts these sensitive data with session keys. Wechat framework provides a cloud function feature that automatically handles these keys and the decryptions of sensitive data to make the development safer and easier. However, since 
% Although wechat allows developers to use their third-party servers to handle user data,
% To help developers to securely communicate with backends and process user data, wechat introduced the cloud function feature where the encryptions and decryptions are 


\paragraph{Securing Communication with Other Mini-apps} 


%the data access should be rejected by the device. The security levels are determined by the pairing method, as shown in \autoref{tab:seclevel}. This is because in some of the pairing methods, an out of band channel or a user is involved, and such a engagement improves the security of the pairing process. For example, in the \textsf{Passkey Entry}, a user is required to approve the pairing request by inputting the displayed \textsf{PIN}, and such a interaction assists the pairing devices to complete the authenticate process. Therefore, pairing method such as \textsf{Passkey Entry} or \textsf{Numeric Comparison} can defend against Man-in-the-Middle (MitM) attacks or unauthorized data access.  Alternatively,  \textsf{Just Works} does not require either the approval from a user or a trust out of band channel to be involved, and it is subject to various Bluetooth attacks. 



 

  


%of mini-apps can be broken into 5 categories, the  

%now in charge of data access, and therefore, security measures are required to protect sensitive data. Security measures of a mini-app can be broken into five categories regarding the different sensitive information the host app intends to protect, i.e., system resources, host app data, data from specific mini-apps, 
%data exchanged between two mini-apps and data from the back-end. 


%\item \textit{Host app data.} Other than the system resources, the host app may allow the mini-apps to access the data collected by the host app. Those data may have privacy concerns and the host app, therefore, enforces the self-defined permission checks against the privacy leakage. For example, \wechat defines permission named \texttt{scope.userInfo} to protect the user information collected by \wechat (e.g.,residence, gender) to be accessed by an unauthorized mini-app. Since  native apps do not have a host app, a similar mechanism is not provided. 

 \looseness=-1 

  


\subsection{The miniap workflow}
Similar to the native apps that run atop host OSes, the mini-apps run atop host apps, where host apps provide necessary permission and peripheral device managements. In this paradigm, access to user information, peripheral devices(e.g., Bluetooth and WiFi), and phone sensors (e.g., gyroscope) are managed by host apps via specific APIs and permissions defined by host apps, provided that the permissions to access these information and devices are already granted to the host apps. As such, the host app partly acts as an `Operating System' for the specific mini-apps.
% Similarly in mini-app paradigm, the permission, peripheral device, and information managements are performed by host apps, and these host apps serve as host apps to the OS themselves as well. 
(). Therefore, the mini-apps rely heavily on network communications to provide convinient service to the users. In general, the mini-app workflow involves three aspects: permission acquisition, resource access

% The mini-app paradigm is similar to the webapp paradigm, where the host app resembles the role of web browsers such as Google chrome, and the mini-apps resemble the role of webapps runnning atop the chrome browser. In this special paradigm, the mini-apps obtain access to peripheral devices and user information through the host apps, and relies heavily on network connection to interact with mini-app backends and wechat API servers. In general, the mini-app workflow involves three processes: permission requests, resource accesses, and server communications.

\paragraph{Requesting permissions}

\paragraph{Accessing resources}

\subsection{The Mini-app Architecture}
\subsection{The Mini-app Security Mechanisms}
\subsection{Developing Wechat Mini-apps}
Similar to webapps that are written in Javascript, HTML, and CSS, wechat mini-apps are also written in Javascripts with wechat-specific APIS, and WXML (wechat-version HTML) and WXSS (wechat-version CSS).

(How is mini-app compiled, and how developers can obfuscate the source code to protect the mini-apps; associated with the code obfuscation and protection)

(The variety of developer backgrounds, third-party plugins and the mini-app template services; associated with the potential third-party security issues)
\AY{=====SPLITTER=====}

The Mini-App is a novel paradigm, a hybrid solution which leverages on the Web technologies (e.g., JavaScript) and the capabilities (e.g., the capabilities to access diverse devices such as Bluetooth peripherals) of the native apps. The native apps, which are the apps installed onto the OS directly (e.g., \wechat, \tik), are the hosts of these mini-apps, offering the mini-apps running environments. Benefit from that, the mini-apps are featured installation-free and resource-saving, since the mini-apps reuse the components and resources provided by the native apps. At the same time, mini-apps are able to offer native app like experiences to its users, and can achieve the equivalent functionalities (e.g., entertainment, financial, e-commerce, banking, health) as the native apps. Benefit from those, the mini-apps are gaining popularity in the past a few years, and have been supported by many apps such as \wechat, \tik and \textsf{Snapchat}. \autoref{tab:popularity} summarizes most popular mini-apps platforms we have studied. Miniapps from \textsf{Snapchat} are not included since they are not open to public at the time of writing. 

%More recently, Apple states that the mini-apps feature, which called ``App Clips'', will be a part of the latest iOS 14 \cite{iphoneminiapp20}. 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\resizebox{1\columnwidth}{!}
{
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Platform}} & \multicolumn{3}{c}{\textbf{Host App}}                                                                                              & \multicolumn{3}{c}{\textbf{MiniApps}}                                                       \\ \cmidrule(l){2-7} 
                                   & \textbf{Functionality}                                                   & \textbf{MAU}         & \multicolumn{1}{l}{\textbf{DAU}} & \multicolumn{1}{l}{\textbf{Released Date}} & \textbf{Number} & \textbf{MAU}         \\ \cmidrule(r){1-7}
WeChat \cite{wechatmau20,wechatdau19,wechatmini20}                             & \begin{tabular}[c]{@{}c@{}}Instant Message;\\  Social Media\end{tabular} & 1.2 B+                & 450M+                             & 2017                                       & 3.2M+                   & 440 M+                \\
Alipay \cite{alimau20,alidau20}                            & \begin{tabular}[c]{@{}c@{}}M+obile Wallet;\\ Finance\end{tabular}         & 881 M+                & 320 M+                            & 2018                                       & 1M+                     & 230M+                 \\
Baidu \cite{baidumdau20}                             & \begin{tabular}[c]{@{}c@{}}News;\\ Short Videos\end{tabular}             & 665M+                 & 200M+                             & 2019                                       & 0.15M+                  & 270M+                 \\
Tiktok \cite{tiktokmdau20}                            & \begin{tabular}[c]{@{}c@{}}Short Videos;\\ Social Media\end{tabular}     & 800M+                 & 400M+                             & 2019                                       & N/A                     & 500M+                 \\
 \midrule 
\end{tabular}}
\caption{Popularity of miniapps and their host apps. MAU means the number of Monthly Active Users, and DAU means the number of Daily Active Users.  }
\label{tab:popularity}
\end{table}
 

\subsection{Mini-app Architecture}
\label{subsec:architecture} 

Being a novel type of app,  a mini-app relies on its (I) front-end running atop a host app for user interaction,  and (II) its back-end, which is optional, for sophisticated services providing.  We illustrate the typical mini-app architecture in  \autoref{fig:overview}.
 
\textbf{(I) Front-end.} As shown in \autoref{fig:overview}, mini-apps relay on the host apps for bridging the underlying system API interfaces, which enable the mini-apps to have capabilities of accessing the peripheral devices (e.g., Bluetooth and NFC) and system resources (e.g.,  Cameras, GPS). Particularly, a mini-app runs atop its host app as a separated process, and the host app integrates a mini-app layer, where all mini-apps are sand-boxed and can only request the resource or device access under the supervision of the host app. For that purpose, the host app provides multiple in-app APIs for the mini-apps to invoke, and those APIs define the kinds of requests that can be made by these mini-apps, allowing the mini-apps developers to customize the functionalities independently of the implementation. 
Each in-app API calling request is also monitored by the host app, and a in-app permission check mechanism is provided to determine if a mini-app has the privileges of accessing the resources or devices. For example, when the mini-app app calls in-app API (e.g., \textsf{createBLEConnection(.)} to connect Bluetooth devices), the host app's in-app permission check mechanism will check if the mini-app (i.e., the caller) is enabled the corresponding permissions.  
If so, the request will be delivered to the corresponding lib function, which is implemented based on the system APIs of a specific OS. Afterwards, the lib function invoke the corresponding system APIs (e.g. \textsf{connectGatt(.)}), and the System level permission check mechanism of OS ultimately determine whether the call can be made. \looseness=-1


%To have capabilities of accessing the peripheral devices (e.g., Bluetooth and NFC) and system resources (e.g.,  Cameras, GPS),  mini-apps relay on the host apps for device management and resource scheduling.  





% 
%to complete the execution. T 

%an \textsf{Encapsulation lib}, and then \textsf{Encapsulation lib} 


%It can be observed from the architecture of the front-end that ($i$) All the resource access requests are monitored and delegated by the host app, and the in-app permission check mechanism will determine if a mini-app has the privileges of accessing the resources.

%($ii$) the host app is implemented differently through APIs provided by various OSes, while the mini-apps are programmed using the same API, which provided by the host app. Therefore, the APIs of mini-apps is the subset of all APIs from different OSes. 

 

 



\begin{figure}  
\centering
\includegraphics[width=1\columnwidth]{image/overview.pdf}\\
%\vspace{-2mm}
\caption{Typical mini-app architecture} 
%\vspace{-3mm}
\label{fig:overview}
\end{figure}

\textbf{(II) Back-end.}
%Other than the local system resources, the network resources of mini-apps are also be restricted and monitored by the host app. 
Being a native app, the host app was only supposed to communicate with its own back-end before the mini-app's emerging. However, after being hosted by the miniapps, the native app 
has to communicate with multiple back-ends corresponding to each mini-app, since the mini-apps are implemented independently by different vendors and each vendor may have its own back-end for providing specific services. 
This may bring security risks against the host app as well as OS. For example, if there was no protections in place, the malicious mini-app may connect a server to mount a backdoor or load malicious payload, giving intruders the abilities to 
remotely access the system resources or issue system commands. 

The host apps, obviously, are aware of the risks and therefore, all of the host apps (e.g., \wechat, \alipay, and \baidu) we investigated offer isolation mechanisms to 
allow the mini-apps to use the network within the bounds of the host app. That is, an mini-app must communicate its back-end under the host's monitor; Other wise, the network requests will be blocked by the host app. As illustrated in \autoref{fig:overview}, there are two options available including the cloud base mode and gateway mode for mini-apps to use the network resources securely: 

\begin{itemize}
\item \textbf{Cloud base mode.} The host apps recommend the mini-app  developers to use a boxed back-ends (named Cloud Base) within the server of the host app.  The cloud base encapsulates the basic features (e.g.,database access and file storage) of a regular back-end. The cloud base also allows the developers to customize specific services by running the web server applications. For security concerns, the files, databases and functions can be configured with different permissions for users with specific roles to access (e,g., a particular file can only be accessed by the creator of the file). 

\item \textbf{Gateway mode.} However, the ``mini back-end'' solutions may be insufficient to tackle all the scenarios. 
Therefore,  the host apps also supports a gateway mode, where the host app's back-end will work as the gateway and discard the insecure network requests. In such a mode, the mini-apps developer will be required to submit the domain name of the back-end for the host app back-end to vet. Only the quantified back-ends are allowed to access (e.g., non HTTPS requests are not allowed). The communication between a mini-app and the its remote back-end  can be protected by a cryptographic key, and the key is usually generated and maintained by the host apps \cite{wechatkey20}.  





%the mini-apps to configure a trust domain(s) before accessing the network, and the trust domain(s) should suffice a set of regulations. For instance, the domain should use HTTPS not HTTP. Under this mode, the host app back-end works as the gateway of the mini-app, and will discard the requests that are not listed in the configuration. 



%For example, some mini-apps are extended from native apps, and these native apps may have the requirements to access their original back-ends for better services (e.g., the original back-end may have more computational resources when compared with those ``mini back-ends''). To balance the security and usability,
\end{itemize}


 \subsection{Provision of ``OS-level'' Services}
\label{subsec:securitymeausres}
Being a OS-like entity for the mini apps, the host app is now responsible for provision of multiple services including device (hardware) management, resources management, inter-processes communication management and User Interface (UI) management. 


now in charge of data access, and therefore, security measures are required to protect sensitive data. 
Security measures of a mini-app can be broken into five categories regarding the different sensitive information the host app intends to protect, i.e., system resources, host app data, data from specific mini-apps, 
data exchanged between two mini-apps and data from the back-end. 

%As shown in \autoref{tab:resouces}, for achieving better understanding, we compare the  mini-app security measures with that of native apps.  

 
\textbf{Hardware Management.}


\textbf{Resource Management and Data Isolation.}
\begin{itemize}
\item \textit{System Resources.}  The host app usually extends the permission check mechanism from the mainstream OSes. System resources such as location services or microphone usage, which treated as sensitive resources by major OSes (e.g., Android or iOS), are also restricted to use by the host app for the mini-apps to access. That is, before the use of the system resources, the developer shall configure the corresponding permissions while programming, and each permission must be granted by the user to obtain the resources. The permission check mechanism is similar to that in native apps. 

\item \textit{Host app data.} Other than the system resources, the host app may allow the mini-apps to access the data collected by the host app. Those data may have privacy concerns and the host app, therefore, enforces the self-defined permission checks against the privacy leakage. For example, \wechat defines permission named \texttt{scope.userInfo} to protect the user information collected by \wechat (e.g.,residence, gender) to be accessed by an unauthorized mini-app. Since  native apps do not have a host app, a similar mechanism is not provided. 
\item  \textit{Mini-App data.} The mini-apps may have the requirements to save specific data onto the disk and the data can be used for various purposes such as profiling a user, maintaining the mini-app's states. To that end, the host app allocates 
each mini-app an isolated space for extra data storage. Each isolated storage is a folder created by the host app, and the folder for a specific mini-app is labeled with a unique ID, which uniquely identifies a mini-app.
%One mini-app can not access the storage other than the allocated folder.
As comparisons, similar mechanisms are also enforced by the major OSes for native apps. For example, Android creates each app a isolated folder and labels each folder with the app's package name. \looseness=-1 

\item \textit{Network data.} As discussed earlier, the accesses to network data of an mini-app are also partly controlled (i.e., trust domain policy) or fully supervised (i.e., cloud base) by the host app. Particularly, in the context of the cloud base, the mini-app front-end is only supposed to communicate with its mini-app back-end, and all the requests or responses are monitored by the host app. This is a unique feature of mini-app.
\end{itemize}

\textbf{Inter-processes Communication Management.}

\textbf{UI Management.}
  



 
 
 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}





\subsection{Comparison with Native Apps}
\label{subsec:goodfeatures}

Being a novel paradigm, mini-apps have the multiple advanced new features when compared with the legacy native apps according to MiniApp Standardization White Paper from \textsf{World Wide Web Consortium} (W3C) \cite{whitepaper20}. Inspired by the official document and our investigation, we summarize three advanced features as follows. Basically, mini-apps are superior to the native apps from the capabilities of cross-platform, storage saving, and back-end resources isolation. 
%It can be observed that the 
  
 

\begin{itemize}


\item \textbf{Cross-platform}. A mini-app can be distributed to multiple platforms (i.e., Android, iOS, Linux, Windows), since the environment required for miniapps to run are built by the same host app.  Unlike in the native apps, developers may need to learn different languages to support the compatibility across platforms, and maintain duplicate projects for different platforms.

\item \textbf{Storage saving}. To offer instant and installation free experience for users, mini-apps usually less than 10 MB, and it is supposed to only contain the core engine of a full version native app (if any). For that purpose, the host app provide simplified APIs when compared with the native APIs, which only serve the core logic of the functionalities.  
 
 

\item \textbf{Back-end resources isolation}. As discussed in \S\ref{subsec:securitymeausres}, other than the mandatory permissions check extending from the traditional OSes (e.g., Android's permission mechanism), the network resources from back-end can also be controlled and monitored by the host app. %Due to the specific architecture of mini-apps, the mechanism is not observed from any native apps.    
 
\end{itemize}

%  
}

==> paper/02_background_new.tex <==
\section{Mini-app Security Mechanisms}
\label{sec:back}



\begin{table*}[]
\setlength\tabcolsep{2pt}
\footnotesize
\aboverulesep=0pt
\belowrulesep=0pt
\begin{tabular}{@{}clccr|rrll@{}}
\toprule

\multicolumn{5}{c}{\textbf{Security Mechanism}}                                                                                                                                                                                                                                                    & \multicolumn{3}{|c}{\textbf{Attacks}}                                                                                \\ \midrule
 
\textbf{At}  
 

& \textbf{Mechanism}                       & \textbf{Built-in}       & \textbf{Add-on}         & \textbf{Representative API(s)}                                                                                                                                         & \multicolumn{1}{c}{\textbf{Name}} & \multicolumn{1}{c}{\textbf{Misuse}}  \\ \cmidrule(r){1-9}
 \multirow{9}{*}{\rot{Front-end}} & \textbf{Underlying Resources Protection} &                         &                         &                                                                                                                                                                        &                                   &                                                                             \\
                           & ~~Permission management                    & \tickYes &                         & N/A                                                                                                                                                                    &                                   &                                                                              \\
                           & ~~Device Communication Encryption          &                         & \tickYes & \texttt{BLEPeripheralServer.addService}                                                                                                               & Unauthorized Access               & Fail to enable encryption                               \\ \cdashline{2-9}
                           & \textbf{Mini-app Isolation}              &                         &                         &                                                                                                                                                                        &                                   &                                                                          \\
                           & ~~Mini-app Storage Isolation               & \tickYes &                         & \texttt{wx.getStorage},  \texttt{wx.setStorage} &                                   &                                                                         \\
                           & ~~Mini-app Plugin Isolation                & \tickYes &                         & \texttt{requirePlugin},\texttt{wx.redirectTo}                                                                                        &                                   &                                                                          \\\cdashline{2-9}
                           & \textbf{Mini-app Redirection}            &                         &                         &                                                                                                                                                                        &                                   &                                                                         \\
                           & ~~Cross-Mini-app Communication Protection  &                         & \tickYes & \texttt{wx.navigateToMiniProgra}                                                                 & Fake Message Injection            & Fail to authenticate mini-app                                  \\
                           & ~~Cross-User Sharing Protection            &                         & \tickYes &   \texttt{wx.updateShareMenu},\texttt{wx.authPrivateMessage}                              & ~~Private Sharing Abusing           & Fail to authenticate user                                     \\ \cmidrule(r){1-9}
\multirow{5}{*}{\rot{Back-end}}  & \textbf{Third-party Back-end Protection} &                         &                         &                                                                                                                                                                        &                                   &                                     &                                           \\
                           & ~~Domain Acceptlist                        & \tickYes &                         & \texttt{wx.request}                                                                                                                                   &                                   &                                                                            \\
                           & ~~Communication Encryption                 &                         & \tickYes & \texttt{wx.login}, \texttt{code2Session}                                                                                             &   Data Manipulation       & Key leakage                                             \\
                           & ~~Back-end Authentication & \tickYes &                         & \texttt{wx.login}, \texttt{code2Session}                                                                                             &                                   &                                                                             \\
                           & \textbf{Cloud-based Back-end Protection} & \tickYes & \multicolumn{1}{c}{}    & \texttt{cloudID}                                                                                                                                      &                                   &                                                                           \\ \bottomrule %cmidrule(l){1-9} 
\end{tabular}
 
\caption{Summary of Mini-app Security Mechanisms.  }
    \label{tab:mechanisms}
\end{table*}

%\begin{figure}
%    \includegraphics[width=\linewidth]{image/arch.pdf}
 %   \caption{The Three Mini-app Layers\ZY{Two backends there. Don't forget to change them.}\AY{Sorted.}}
  %  \label{fig:arch}
%\end{figure}

%\subsection{Mini-app Architecture}
%\label{sub:arch}
%As shown in \autoref{fig:arch}, in the mini-app paradigm of \wechat, mini-apps run atop a running environment provided by the host app. The host app manages system resources and extends the mini-app functionalities with various mini-app APIs. Each mini-app consists of two main components: (i) a front-end running in the \wechat host app that uses various mini-app APIs provided by the host app to access system resources; (ii) a back-end (optional) communicating with the front-end that hosts and processes user data. The back-end can either be a third-party server that runs \wechat mini-app server SDK, or be \wechat cloud base that provides cloud function feature for developers to safely and easily develop their back-ends.
% mini-app front-ends run atop \wechat host app, which provides a running environment and various mini-app APIs for mini-apps to extend their functionalities and access system resources. For each mini-app in \wechat, aside from the front-end packages that run in the host app, 

% While running onto \wechat,  the mini-apps use the (i) a front-end to fetch the system resources from \wechat and interact with user, and (ii) a back-end to fetch remote resources, as shown in \autoref{fig:arch}.\looseness=-1
  %to provide native-app-alike services for the users,

%the architecture of \wechat mini-app framework consists of two layers, the mini-app front-ends, and the mini-app back-ends.

%\begin{itemize}[leftmargin=*]
    %\item \paragraph{Host OS layer} The host app runs atop the host OS. It provides and manages various OS system resources to the mini-apps.
 %   \item \paragraph{Mini-app front-end} Similar to the native apps (\eg, Android apps), mini-app front-ends are compiled, compressed, and distributed as \texttt{.wxapkg} file. This application package file mainly consists of four types of files: (1) a JSON file named \texttt{app.json} containing the basic information and configurations of the mini-app; (2) multiple JavaScript (JS) files that use native or mini-app specific APIs to provide their functionalities, ranging from resource access to network communications; (3) multiple WXML (Wechat Marking Language, \wechat-extended version of HTML) files specifying the user interface pages; and (4) multiple WXSS (Wechat Style Sheet, \wechat-extended version of CSS) files to represent the styles of WXML pages. 
    % The mini-app front-ends are hosted by a sandbox-like JavaScript environment of \wechat. In this environment, mini-apps run with their separated storage space, and provide various functionalities via mini-app APIs, provided by the environment. 
    
%    \item \paragraph{Mini-app back-end} \wechat mini-apps can also can an optional back-end to support cloud computing features. These back-ends can either be \wechat cloud servers that provide mini-app cloud function features, or be third-party back-end server that run \wechat server SDK. These back-ends are mainly used for acquiring, hosting, and processing sensitive user data sent from \wechat and the front-end.
    % process network requests and manages data generated by various users. Now, there are two approaches for the mini-apps to use their back-end services: (1) a mini-app can use cloud base back-end hosted in the back-end of \wechat, where the front-ends can directly interact with the back-ends using the \wechat APIs. (2) a mini-app can access a back-end that are not hosted in the \wechat back-end. In this case, \wechat will work as a gateway to monitor and vet all the incoming and outgoing traffics. \looseness=-1    
    %This back-end can be a third-party server that runs \wechat server SDK, or a \wechat cloud base that provides cloud function feature.
%\end{itemize}


%\ZQ{Please do not copy any text from SIGMETRICS paper (self plagiarism). We must rewrite everything. Section 2.1 and also Figure 1 appear to be too similar to that paper.}




 

%\subsection{Mini-app Security Mechanisms}

%In the mini-app paradigm of \wechat, mini-apps run atop a running environment provided by the \wechat. \wechat manages system resources and extends the mini-app functionalities with mini-app APIs.  

Similar to many native apps,  a mini-app is often composed of (1) a front-end that fetches resources and interacts with users and (2) an optional back-end that maintains user-specific data and provides various online services. To secure both the front-end and the back-end, the designers of \wechat introduced both the built-in security measures and add-on security measures. The built-in security measures are mandatory when configured by the developers, but the add-on security measures require the developers to implement extra functionalities (\eg, authenticating the users) even when configured.
To systematically study these security measures, we manually went through \wechat official development document and APIs to inspect their usage.  Particularly, we group the security measures into two categories, as shown in left part of  \autoref{tab:mechanisms}, including (1) the security measures deployed at the front-end (\S\ref{subsubsec:secmeasures-front}) and (2) the security measures deployed at the back-end (\S\ref{subsec:secmeasures-back}).  \looseness=-1


%Therefore, it is undoubtedly a challenging task to design security mechanisms to protect both local system resources and cloud communication for such a complex system.



%communicating with the front-end that hosts and processes user data.


%As discussed in \cref{sub:arch}, a mini-app can have both a front-end and a back-end to support both native-like features and cloud computing capabilities.
% , which are supposed to be secured by \wechat.

% from being intercepted and exploited. 
%As such, \wechat has enforced multiple security measures, either mandatory or optional, both at front-end and back-end, to secure their mini-apps.
% In this section, we organize the security measures into two categories: \ie, (1) the security measures deployed at the front-end (See \S\ref{subsubsec:secmeasures-front}) and (2) the security measures deployed at the back-end (See \S\ref{subsubsec:secmeasures-back}). 



%{\red{\wechat combined the built-in security measures, which is mandatory when configured, and add-on security mechanisms, which require the developer to implement extra modules even when configured. In this section, we introduce the built-in and add-on mechanisms in greater details from the perspective of architecture, }} \ZY{It is too early to introduce the conception of add-on and build-in. I will fix this latter.}

%and compare their advantages and their disadvantages.

% The reason why wechat has adopted such a complex security mechanism lies in the complex functionality involved in the mini-app paradigm. To gain an edge from native applications in terms of usability, funcitonality, and security, wechat is not merely a normal native application any more, but instead an OS-like ecosystem that involves both native OS resources and heterogeneous back-ends. On top of that, the requirement of using their own third-party servers from business vendors that would like to integrate their services into mini-apps requires wechat to support third-party back-ends and enforce data encryption, which elevated the challenge of securing the mini-app data while maintaining the versatile functionality. In this section, we discuss the threat model that wechat mini-app adopts as described in their official documentations when designing these mechanisms, and then provide a detailed comparison of wechat security mechanisms.
%\ZY{How about remove host OS section, and put the content at the mini-app front-end?}



%\subsection{Host OS}
% In the mini-app paradigm, the host app plays a critical role in OS resource management. The security mechanisms in this layer to manage and secure the resource accesses can be summarized into three main categories: built-in permission management, which requires developers' configuration; built-in storage isolation, which is fully transparent to developers, and device management, which provides optional add-on security for developers.

%\begin{figure}[h!]
%    \includegraphics[width=\linewidth]{image/permission.pdf}
%    \caption{Three ways to use mini-app authorization scopes}
%    \label{fig:permission}
%\end{figure}
\begin{figure*} 
\centering
\begin{minipage}[t]{0.67\textwidth}
\includegraphics[width=\textwidth]{image/workflow-all-in-all.pdf}
\caption{Security measures at mini-app}  
 \label{fig:allsecure}
\end{minipage}
\vspace{1mm}
\begin{minipage}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{image/allkeys.pdf}
\captionsetup{justification=centering}
\caption{Data flow during authentication and encryption}  
 \label{fig:key}
\end{minipage}
\end{figure*}

% \begin{figure*}[ht]
%     \includegraphics[width=.6\linewidth]{image/overview-final.pdf}
%     % \hspace{0.01\linewidth}
%         \includegraphics[width=.39\linewidth]{image/dataflow.pdf}
        
% \end{figure*}

\subsection{\textbf{Security Measures at Mini-app Front-end}}
\label{subsubsec:secmeasures-front}
%The host app plays a vital role in managing mini-apps running inside it. To protect those mini-apps, the mini-app framework enforces multiple security mechanisms to manage the resource access, mini-app isolation, as well as the cross-miniapp communications and their distributions.
%The security measures deployed at the front-end offers:  
As shown in \autoref{fig:allsecure},
\wechat provides the following security measures at mini-app front-end including: 
(1) underlying resources protection (including the data resources such as location service data, and the device resources such as peripherals that connected to the mobile); (2)  mini-app isolation and (3) redirection protection (as a mini-app may redirect to another mini-app or another user). We present in greater details of these security measures in the following.


%two mini-apps can communicate with each other to exchange data and (5) cross-user sharing, as one user may share a mini-app of interest to other users. 
%do not only manages system resources, handles the mini-app front-end life-cycles. The mini-apps can be shared among different users, where users can click on the link to enter mini-apps. Aside from directly clicking to enter, mini-apps can also be launched via cross-mini-app navigation. To manage these mini-apps, the framework not only handles the background mini-app behavior, but also enforces isolation to protect mini-app data.

\paragraph{(1) Underlying Resources Protection} 
In general, there are two types of resources that \wechat framework manages: (1) on-device resources including the data collected by the on-device sensors (\eg, GPS) and resources collected by \wechat (\eg, user's gender and residences), and (2) the off-device resources including the peripherals connected to the mobile. 
For the on-device resources, \wechat enforces a built-in permission authorization. For off-device peripherals, \wechat provides add-on configurable service protection for developers. 

\begin{itemize}[leftmargin=*]
\item \paragraph{Authorization Scope (\ding{182})} Similar to Android OS, \wechat enforces the authorization scope, the mini-app version of the permission checking, to prevent a mini-app from abusing resources. One specific scope is used to protect a scope of APIs related to a certain system resource. For example,  
\texttt{scope.userLocation}, protect the user location, which inovles the authorization of \texttt{wx.getLocation}, \texttt{wx.chooseLocation}, and \texttt{wx.choosePoi}. 
Compared with Android, aside from system resources such as user \texttt{Album} and location, \wechat adopts a broader authorization scope (\eg, such as \wechat sport data, and invoice information generated by \texttt{WeChatPay}). Specifically, to use APIs that require certain user permission, the mini-app framework will prompt the user to approve or decline the scope requirement when corresponding API is actually being invoked. If the user have  granted a scope, the user's preference will be saved: the granted permissions will not be revoked until the user uninstalls the mini-app or manually opens the menu to cancel the scope authorization.
%\AY{I will delete the .json part. Our analysis focuses on JS}

\item \paragraph{Configurable Service Protection ({\blue{\ding{183}}})} 
\wechat mini-apps can access the the peripherals connected to the mobile device through Bluetooth. Meanwhile, \wechat APIs also allow the mini-app to make the smartphone work as a peripheral that provides data services (by using the API \texttt{addService}) for other devices. When configuring the services, developers can require the communication encryption by setting the parameter \texttt{readEncryptionRequired} and \texttt{writeEncryptionRequired} as \texttt{ture}. When configured, the incoming data reading and writing requests will be approved only when the Bluetooth traffic is encrypted. However, whether or not the traffic is encrypted depends on the presence of the link key, which is negotiated through the Bluetooth pairing~\cite{5.1} between two devices.        



%Aside from one-to-one Bluetooth communication, developers can assign one mobile device as the `central' that processes data provided by other peripherals when there are multiple mobile devices working mutually via Bluetooth. Under this circumstance, mini-apps can be assigned as peripherals to broadcast data for the central devices by configuring Bluetooth peripheral services with \texttt{addService()}. When configuring this service, developers can enabled or disable the read/write encryption according to the Bluetooth capabilities by setting \texttt{read/writeEncryptionRequired} parameter.
% , since two smartphone may communicate with each other via Bluetooth,
% where one mobile works as the central (\ie, the device consume the data) and the other mobile work as the peripheral (\ie, the device provide the data),  \wechat APIs also allow the mini-app to make the smartphone working as a peripheral. When working as a peripheral,  
% developers can configure the mobile to enable certain security levels to protect their data. For instance, the mobile can set the parameter \texttt{writeEncryptionRequired} to \texttt{true} to grantee the Bluetooth communication is encrypted.  
  
%\ZY{I am not sure to include the word `management' in the names of all security measures is a good way to introduce the security measures. It looked not very intuitive.  }\AY{Sorted, and patched flows , so there might be drastical changes in the presentation.}
%set the parameter \texttt{writeEncryptionRequired} to \texttt{true} or \texttt{false} to enable or disable encryption when reading or writing data.
\end{itemize}
\paragraph{(2) Mini-app Isolation} Since the mini-app framework hosts multiple mini-apps, it is vital to enforce isolation mechanisms to prevent cross-app attacks such as horizontal privilege escalation~\cite{suciu2020horizontal}. Therefore, \wechat framework enforces two built-in isolation mechanisms for mini-apps.
% As a mini-app, it may maintain multiple resources, which should also be protected properly. For example, a mini-app can maintain the their user's credentials or some other sensitive information collected from the user. \wechat protect the mini-app specific data by using the following security measures: \looseness=-1


\begin{itemize}[leftmargin=*]
\item \paragraph{Mini-app Storage Isolation (\ding{184})} Mini-apps running in \wechat framework are isolated. Each mini-app has a local storage in the \texttt{com.tencent.mm/} folder, which is not accessible by other mini-apps. Aside from user images and videos that can be accessed with corresponding permission granted, each mini-app can only access files in its local storage, and cannot access files in user folder that are outside \wechat native app storage (e.g., user files stored in \texttt{/sdcard/Download}).

% indicating that they run in separate directories, and the local user data is not accessible to each other.mini-apps running in \wechat are isolated at user level,\ZY{What do you mean by user level? I do not think it is correct here.  } meaning that different users and different mini-apps cannot access the isolated storage space between each other. In Android, e \looseness=-1  
\item \paragraph{Mini-app Plugin Isolation (\ding{185})} Many mini-app developers have integrated plugins, a special type of mini-app, in their own mini-apps to extend the functionalities. To prevent plugins from manipulating the UI rendering of the host mini-apps (\eg, a malicious plugin may navigate to the ``Payment success'' page of a mini-app without the payment process), only the host mini-app can open the specific graphic window of the plugins, and pass the parameter to the plugins; Plugins cannot actively opens a specific graphic window of the mini-app.   



% \item \paragraph{Mini-app Background Running Management} The mini-app life-cycle is maintained by the mini-app framework. When the user exits a mini-app, the mini-app will stay in background, so that it loads quicker if the user re-enters the mini-app. If the background mini-app exceeds the limit or there is not enough system resources, the framework will terminate the mini-app to release the system resource.  On top of that, the background mini-app functionalities are restricted. For example, the timer of sensors become inaccurate in the background, and background behaviors such as voice recording will be ineffective. However, there is one exception: if the mini-app is granted with the specific background location updating scope, it can keep on updating user's location in the background without being restricted.
\end{itemize}
 
\paragraph{(3) Redirection Protection } While using a mini-app, the user can redirect to another mini-app or share the mini-app to another user depending on the different scenarios. To protect the data being transferred in the redirection process, \wechat provides two types of add-on security measures, \ie, cross-mini-app communication protection and cross-user sharing protection:   

%Since the mini-app framework hosts multiple mini-apps, it is vital to enforce isolation mechanisms to prevent cross-app attacks such as horizontal privilege escalation~\cite{suciu2020horizontal}. Therefore, \wechat framework enforces two built-in isolation mechanisms for mini-apps.

\begin{itemize}[leftmargin=*]
 
    \item \paragraph{Cross-Miniapp Authentication ({\blue{\ding{186}}})} The cross-miniapp navigation mechanism is similar to that of Android Intent, which allows two mini-apps to communicate with each other. A mini-app can invoke \texttt{wx.navigateToMiniprogram()} to redirect to other mini-apps, and the navigation target will get the information of the source mini-apps (i.e., source mini-app ID and extra data) with  \texttt{wx.getLaunchOptions} that returns \texttt{referrerInfo} containing all these information. 
    % with extra data to perform complex actions.  
    \wechat had a built-in whitelist security mechanism that required every developer to declare up to 10 mini-apps of interest as the trust mini-apps, but this mechanism is discontinued after April 2020 \cite{wxdoc-navigate} , and hence it is for developers to check the mini-app navigation source since there is no longer built-in mechanism.
    % The developers can check which mini-app the user is navigating from by obtaining the \texttt{appId} parameter in the \texttt{referrerInfo} when the mini-app launches.
    \item \paragraph{Cross-User Authentication ({\blue{\ding{187}}})} The mini-apps can be shared to other users or groups as a clickable URL. Nowadays, to attract more fresh members, many mini-app developers may offer a special bonus or discount for mini-app users if they share their mini-apps to other users (e.g., a user may get a discount if new members register with his/her own promotion code). However, this may result in promotion abuse when an attacker acquires multiple accounts and re-shares the promotion code between accounts. To avoid this sharing to be abused,
    %o attract more users to use a mini-app, 
    % Generally, when a user finds a mini-app of interest, he or she can share the mini-app to his friends through a clickable URL. This is an effective way to popularize mini-apps. Therefore, developers may offer some bonuses (\eg, game currency) for the users who preformed the sharing, and the users who launched the mini-app through the shared URL. To avoid the mini-app sharing feature to be abused, 
    \wechat introduces a novel private sharing feature, where the mini-app only allows first-hand receivers to use the URL to enter the mini-app, whereas second-handed users (users receiving the re-shared invitation) cannot. To that end, while sharing the mini-app, the developers can first call API  \texttt{createActivityId} to create an Activity ID (\eg, an ID for sales promotion). The developer then invokes \texttt{wx.updateShareMenu} to specify the ID as private by setting \texttt{isPrivateMessage} as \texttt{true}.  
    Later, when the user launched the mini-app, the developer can then call \texttt{authPrivateMessage} to validate whether the ID matches the Activity, and whether the user that opens the mini-app is the first-hand user with privileges to perform further actions (\eg, obtaining the promotion code). If so, the  promotion code will be displayed to the user.    
    
    %shared mini-app contains the private messages. If so, the private message is not available to the second-hand users. 
    % For example, when some mini-app vendors offer special discount for a high-level user when he/she introduces new members to use their mini-apps or services, this feature will be useful to prevent malicious users from acquiring multiple account to repeatedly get the discounts to make profit. Developers can check whether the shared link is valid via \texttt{wx.authPrivateMessage}.
\end{itemize}


\subsection{\textbf{Security Measures at Mini-app Back-end}}
\label{subsec:secmeasures-back}


% \begin{figure}
%     \includegraphics[width=\linewidth]{image/dataflow.pdf}
%     \caption{Data flow of keys and encrypted data}  %\ZY{Will fix this figure later}
%     \label{fig:back-end}
% \end{figure}
As shown in \autoref{fig:allsecure},
There are two approaches for the mini-apps to use their back-end services: (1) a mini-app can use cloud-base back-end hosted in the server of \wechat, (2) a mini-app can access a back-end that are not hosted in the \wechat back-end (\ie, third-party back-end).  Therefore, the security measures at the back-ends can be grouped into two major categories, including the (1) security measures to protect the third-party back-end, and (2) security measures to protect the cloud base back-end.

%communication encryption, which prevents the communication from being intercepted by attackers.
%In this case, \wechat will work as a gateway to monitor and vet all the incoming and outgoing traffics.
%The mini-app mechanism relies heavily on network communications with \wechat servers and back-ends to process user data and provide various services. 


\paragraph{(1) Third-party Back-end Protection} When compared with the cloud base back-end, the third-party back-ends are less trusted as they are not hosted into the server of \wechat. Therefore, \wechat have adopted relatively 
sophisticated security measures for them. Specifically, the security measures at the third-party back-ends can be grouped into two categories, including (1) a built-in back-end white-list, which specify the trusted back-ends, (2) a built-in user authentication mechanism, which authenticates the users,  and (3) an add-on communication encryption, which prevents the communication from being intercepted by attackers. 

% \begin{itemize}[leftmargin=*]
% \item \paragraph{White-List (\ding{188})} \wechat enforced a built-in security measure, named back-end white-list mechanism, to make sure that a mini-app can only communicate with the trusted back-ends. That is, the domain names of the back-ends have to be submitted to \wechat for vetting through the configuration of back-end white-list. For example, \wechat does not allow the incoming and outgoing HTTP requests, and as such, the configured domain must use HTTPS to protect the communication. 
% %Developers can control which domain a mini-app can communicate any time. 
% Meanwhile, mini-app front-ends cannot communicate with the domain names reserved by \wechat (\eg, \url{api.weixin.qq.com}). 
% %{\red{This prevents the malicious front-ends from accessing sensitive data directly from \wechat server, since malicious users may be able to intercept the network packets.}}\ZY{Why?}


 

\ignore{
\subsection{Mini-app Security Model}
\label{sub:threat-model}
The mini-app front-ends are not trusted, and developer need to configure properly if they use third-party back-ends.ba

The mini-app framework supports not only native app features, but also web-app features. As a native app, the mini-app interacts frequently with users' devices, including data, media, devices, and peripherals. As a web-app, the mini-apps consist of front-ends (mainly written in JavaScript) and their corresponding cloud back-ends. Since the front-ends of mini-apps are distributed to users' devices, these front-ends can potentially be decompiled and examined, wechat clearly stated in their official documentations that the data sent from mini-app front-ends cannot be trusted and requires verification.

In our mini-app attack scene, we adopt the same threat model as stated in \wechat official documentations by assuming that the mini-app framework is secured and attackers cannot interfere with the mini-app framework, whereas the attackers can obtain and unpack the mini-app front-end packages. Generally, the attack scenes can be summarized into two categories:


\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item \textbf{Attack targeting mini-apps}. In this scenario, the attackers can exploit the vulnerable mini-app, manipulate network packages, and attack the victim mini-app back-ends for sensitive information or make profits.
    \item \textbf{Attack targeting users}. In this scenario, the attackers can lure victims to install malicious mini-apps or native apps that steals sensitive user information or interfere with vulnerable mini-apps installed on victims' phone.
\end{itemize}

For the rest of this paper including the comparison between mechanisms, tool design and evaluations, we will further investigate the mini-app security mechanisms based on this threat model.

}






==> paper/02_backgtound_backup2.tex <==
\section{Mini-app Security Mechanisms}
\begin{figure}
    \includegraphics[width=\linewidth]{image/arch.pdf}
    \caption{The Three Mini-app Layers}
    \label{fig:arch}
\end{figure}
\begin{table*}[h]
\small
\aboverulesep=0pt
\belowrulesep=0pt
\setlength\tabcolsep{2.5pt}
\begin{tabular}{c|l|ccccccc}
\toprule
% &permission management&user data access&peripheral device access&extended framework API&Cross-app redirection&Plugin Integration&Built-in Cloud Feature\\
\multicolumn{2}{c|}{}&mini-apps&browser extensions&Android apps&iOS apps&apps in sandbox&virtual machines\\ \midrule
\multicolumn{2}{c|}{installation source}&\wechat app&in-browser market&Google Play&App Store&---&---\\ \midrule
\multirow{3}{*}{host app}&permission management&\CIRCLE&\Circle&\CIRCLE&\CIRCLE&\Circle&\Circle\\
&sensitive user data access $^{*}$&\CIRCLE&\Circle&\CIRCLE&\CIRCLE&\Circle&\Circle\\
&peripheral device access&\CIRCLE&\Circle&\CIRCLE&\CIRCLE&\LEFTcircle&\LEFTcircle\\ \midrule
\multirow{2}{*}{front-end}&extended functional API&\CIRCLE&\LEFTcircle&\CIRCLE&\CIRCLE&\Circle&\Circle\\
&cross redirection&\CIRCLE&\CIRCLE&\CIRCLE&\CIRCLE&\LEFTcircle&\Circle\\ \midrule
\multirow{2}{*}{back-end}&built-in cloud feature&\CIRCLE&\Circle&\Circle&\Circle&\Circle&\Circle\\
&oficial network API domain&\CIRCLE&\Circle&\Circle&\Circle&\Circle&\Circle\\
\bottomrule
\end{tabular}
\caption{Comparison of features provided by each paradigm framework}
\label{tab:comparison}
\end{table*}
\subsection{The Mini-app Architecture}
As shown in \cref{fig:arch}, the architecture of \wechat mini-app framework consists of three layers: the host OS \ZY{OS? I think OS is not a part of the mini-app.}, the mini-app front-ends, and the mini-app back-ends.
\begin{itemize}[leftmargin=*]
    \item \paragraph{Host OS layer} The host app runs atop the host OS. It provides and manages various OS system resources to the mini-apps.
    \item \paragraph{Mini-app front-end layer} The front-end mini-apps are distributed in the form of .wxapkg files that consists of JavaScript (JS) code, \wechat Marking Language files (WXML, wechat version of HTML), and \wechat Style Sheets (WXSS, wechat version of CSS). This front-end runs in a JavaScript environment provided by the host app. In this sandbox-like environment, the mini-apps runs with their separate storage space, and provides various functionalities via mini-app APIs provided by the framework.
    \item \paragraph{Mini-app back-end layer} In most of the cases, there is a back-end server that processes network request and manages data generated by various users. This back-end can be a third-party server that runs \wechat server SDK, or a \wechat cloud base that provides cloud function feature.
\end{itemize}

\begin{table*}[]
    \centering
    \small
    \begin{tabular}{c|l|l|l}
    \toprule 
    Type&Mechanism&Built-in&Add-on\\ \midrule
    OS&Permission management&authorization&---\\ 
    OS&Storage management&isolation&---\\
    OS&Device management&---&configuration\\
    front-end&In-miniapp plugins&isolation&---\\
    front-end&Background mini-app&lifecycle handling&---\\
    front-end&Mini-app redirection&whitelist&checking\\
    front-end&Private sharing&---&checking\\
    % front-end&Background management&y&\\
    back-end&Domain whitelist&whitelist \& blacklist$^{*}$&---\\
    back-end&Cloud API token (appsecret)&generation \& validation&maintainence\\
    back-end&Data encryption/decryption&encryption&decryption\\
    back-end&Cloud function&maintainance \& decryption&---\\
    % &&&---\\
    \bottomrule
    \end{tabular}
    \caption{Miniapp Security Mechanisms}
    \label{tab:mechanisms}
\end{table*}
\subsection{Mini-app vs Existing Paradigms}

\ZY{I do not think this part is needed. First, it is not related to our paper. Second, Luyi also talked the similar content in their background. At that time, their reviewers may challenged the differences between the miniapps and existing paradigm, so they added that part. But, currently, since his paper has already been published, I do not think this part is still needed. I think we can put this part at the discussion section.}
\ZQ{maybe we can keep it, but the description has to be crystal clear, and also serve the purpose for this paper, particularly if we have some background knowledge to refer here. If no, then we can remove it}

\AY{I added this section just to describe that mini-apps have complex functionalities of both native app functionalities and unified cloud function.}
Similar to mini-app paradigm, there had been other approaches to allow applications running in a execution environment in a certain framework. Aside from classical native apps that run in OSes such as Android and iOS, there have been two other major paradigms that are similar to mini-app paradigm: the browser extension and the virtual machine. Virtual machines improves security by allowing Operating Systems to execute in a isolated software-simulated PC or mobile device, whereas ensuring that the virtual machines are unaware of the framework. Hence, this paradigm is widely used in security vulnerability analysis and education. On the other hand, the browser extension framework extends the functionality by allowing extensions to execute on top of the web browser. As such, these browser extensions can provide many functionalities that pure webpages cannot provide. For example, with browser extensions, users can schedule meeting, view movies, and even play games \cite{}.

As shown in \cref{tab:comparison}, we compared the mini-app paradigm with other five similar paradigms in terms of supported features provided for mini-apps or containers running within the frameworks. As we can see, different from sandboxes and virtual machines, \wechat mini-app extends the functionalities with mini-app APIs, which significantly extends the functionalities of mini-apps. Compared with mobile native apps such as Android and iOS apps, mini-app framework shares a lot of similarities in that it also integrates a set features such as permission management, sensitive user data access (e.g., user phone number), and cross-app redirection. However, different from the mobile native apps that merely provide basic network request APIs, mini-apps provides built-in cloud feature and a unified network API domain that provides various network APIs for third-party back-end servers. This enables \wechat to secure sensitive user information by enforcing additional security mechanisms such as data encryption and invoker verification.

\subsection{Mini-app Security Model}
\label{sub:threat-model}
The mini-app front-ends are not trusted, and developer need to configure properly if they use third-party back-ends.ba

The mini-app framework supports not only native app features, but also web-app features. As a native app, the mini-app interacts frequently with users' devices, including data, media, devices, and peripherals. As a web-app, the mini-apps consist of front-ends (mainly written in JavaScript) and their corresponding cloud back-ends. Since the front-ends of mini-apps are distributed to users' devices, these front-ends can potentially be decompiled and examined, wechat clearly stated in their official documentations that the data sent from mini-app front-ends cannot be trusted and requires verification.

In our mini-app attack scene, we adopt the same threat model as stated in \wechat official documentations by assuming that the mini-app framework is secured and attackers cannot interfere with the mini-app framework, whereas the attackers can obtain and unpack the mini-app front-end packages. Generally, the attack scenes can be summarized into two categories:


\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item \textbf{Attack targeting mini-apps}. In this scenario, the attackers can exploit the vulnerable mini-app, manipulate network packages, and attack the victim mini-app back-ends for sensitive information or make profits.
    \item \textbf{Attack targeting users}. In this scenario, the attackers can lure victims to install malicious mini-apps or native apps that steals sensitive user information or interfere with vulnerable mini-apps installed on victims' phone.
\end{itemize}

For the rest of this paper including the comparison between mechanisms, tool design and evaluations, we will further investigate the mini-app security mechanisms based on this threat model.
% \begin{itemize}
    % \item Credential maintainence. Although wechat provides a cloud function mechanism that makes the session-key management and data decryption fully transparent to developers to make the developement easier and more secure, there are still a large number of mini-app that uses third-party server for more versatile functionalities. Therefore, when the developers are configuring their third-party servers, they have to maintain these credentials properly and prevent sensitive information, especially appsecrets and session-keys from being leaked to the front-end.
% \end{itemize}


%To run mini-apps across platforms in the host apps, the host app integrates a JavaScript runtime with a set of mini-app specific JavaScript APIs. The mini-apps are developed in JavaScript language with multiple WXML (WeiXin Markup Language) and WXSS (WeiXin Style Sheet) files that are built upon HTML and CSS with mini-app specific features.

% The mini-apps are webapp packages with js, wxml, and wxss that run in mini-app framework. The framework handles both mini-apps, peripheral devices, and network communication.


==> paper/03_eval.tex <==
\section{Scope and Analysis Strategy}

%To understand the magnitude and the impacts of the pitfalls identified 

In this paper, we performed a security analysis on four leading mini-apps platforms, 
i.e.,  \wechat from Tencent Holdings Ltd, \alipay from Alibaba Group Holding Limited, \baidu from Baidu Inc, and \tik from ByteDance Ltd. Particularly, to study the security issues of platforms correspondingly,  we registered their accounts, downloaded their development tools and SDKs, built mini-apps followed their official document, and ran the mini-apps onto multiple platforms including iOS and Android.  

%measurement results    (\S\ref{subsec:basic} and \S\ref{subsec:pitfalls}). Further,  as comparison, we also investigated other forms of ``Light Apps'', including Android Bundle from Google, Instant App from Google, iMessage App from Apple, as well as the popular web extensions, namely Chrome Extension and Firefox Extension (\S\ref{subsec:comparison}). We hope our research could shed light on the current security status regarding the mini-app paradigm as well as the novel conception of ``Light Apps''. 
%We compare the architecture of mini-app and that of others and discuss






\begin{table*}[h]
\resizebox{2\columnwidth}{!}
{
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Host App}} & \multirow{2}{*}{\textbf{Mini-app Name}} & \multicolumn{2}{c}{\textbf{Size}}          & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Background \\ Services Supported?\end{tabular}}}    & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Individual Developer \\ Supported?\end{tabular}}}  & \multicolumn{3}{c}{\textbf{Supported Platform}}   & \multirow{2}{*}{\textbf{Package Encryption}} & \multicolumn{3}{c}{\textbf{Entries}}                            \\ 
                                   &                                         & \textbf{One package} & \textbf{Entire Miniapp} &                                                                                                      &                                                                                                    & \textbf{Android} & \textbf{iOS} & \textbf{Windows}& & \textbf{QR code} & \textbf{Hyperlink} & \textbf{Mini-app Store} \\ \cmidrule(r){1-13}  
Wechat                             & Mini-program                            & 2M                   & 20M                     & \tickNo                                                                                                    & \tickYes                                                                                                & \tickYes                & \tickYes      & \tickYes        & \tickYes                & \tickYes                & \tickYes                  & \tickYes                       \\
Alipay                             & Tinyapp                                 & 2M                   & 8M                      & \tickNo                                                                                                   & \tickYes                                                                                                  & \tickYes                & \tickYes     & \tickNo         & \tickNo                & \tickYes                & \tickYes                  & \tickYes                       \\
Baidu                              & Smart (AI) Mini program                      & 2M                   & 8M                      & \tickNo                                                                                                     & \tickNo                                                                                                 & \tickYes                & \tickYes          & \tickNo   & \tickNo                & \tickYes                & \tickYes                  & \tickYes                       \\
Tiktok                             & Microapp                                & N/A                  & 4M                      & \tickNo                                                                                                    & \tickYes                                                                                                & \tickYes                & \tickYes         & \tickNo    & \tickNo                & \tickYes                & \tickYes                  & \tickYes                       \\ \bottomrule
\end{tabular}}
\vspace{2mm}
\caption{Comparison of mini-apps across platforms} 
\label{tab:compare:platfroms}
\end{table*}
 
 
%\subsection{Scope}
%\label{subsec:scope}



%Note that, in this paper, we also investigated other forms of ``Light App'' from tech giants such as Google and Apple (e.g., Android Bundle, Google Instant App, Apple iMessage App) as comparison. We will not group those forms of apps as mini-apps, since the architectures and frameworks of those apps are significantly different from that of mini-apps. For example, Android Bundle and Google Instant uses the APIs provided from Android OS instead of using in-app APIs, and they run directly onto the OS (although they rely on a specific app to run). Please refer to \S\ref{subsec:comparison} for more details.

 

\begin{table*}[h]
\resizebox{2\columnwidth}{!}
{
\begin{tabular}{cccccccccccccccc}
\hline
\multicolumn{3}{c}{\multirow{3}{*}{\textbf{Available APIs}}}                          & \multirow{3}{*}{\textbf{\begin{tabular}[l]{@{}c@{}} Involving\\ Attacks\end{tabular}}} & \multicolumn{3}{c}{\textbf{WeChat}}                                                                                 & \multicolumn{3}{c}{\textbf{Alipay}}                                                          & \multicolumn{3}{c}{\textbf{Baidu}}                                                               & \multicolumn{3}{c}{\textbf{TickTok}}                                                           \\ \cline{5-16} 
\multicolumn{3}{c}{}      &                                                                                       & \begin{tabular}[c]{@{}c@{}}Enabled? \\(31/32)   \end{tabular}            & \begin{tabular}[c]{@{}c@{}}SDK Version \\ (2.14.1)\end{tabular} &  \begin{tabular}[c]{@{}c@{}}$\sum$ API \\(867)    \end{tabular}                  &  \begin{tabular}[c]{@{}c@{}}Enabled? \\(26/32)       \end{tabular}          & \begin{tabular}[c]{@{}c@{}}SDK Version\\ (2.6.0)\end{tabular} &  \begin{tabular}[c]{@{}c@{}}$\sum$ API \\(234)    \end{tabular}    & \begin{tabular}[c]{@{}c@{}}Enabled? \\(23/32)       \end{tabular}                   & \begin{tabular}[c]{@{}c@{}}SDK Version\\  (3.260.6)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\sum$ API \\(373)    \end{tabular}  & \begin{tabular}[c]{@{}c@{}}Enabled? \\(20/32)   \end{tabular}             & \begin{tabular}[c]{@{}c@{}}SDK Version\\  (1.66.0)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\sum$ API \\(155)    \end{tabular}\\ \hline
\multirow{28}{*}{Front-end} & \multicolumn{2}{c}{UI Rendering}                         & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.9.6                                                           & 70                       & \tickYes &  1.13.0                                       &  27  & \tickYes  & \multicolumn{1}{l}{}                                            &    65  & \tickYes & 1.0.0                                          &  25   \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Data Caching}                         & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.9.6                                                           & 10                       & \tickYes & -                                                             &   10  & \tickYes  & -                                                                &   10  & \tickYes & 1.0.0                                                           &   10  \\ \cline{2-16} 
                            & \multirow{6}{*}{Media}              & Map                 & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.9.6                                                           & 23                       & \tickYes & 1.23.0                                                        &  18   & \tickYes  & -                                                                &   6  & \tickYes & 1.63.0                                                          &  2   \\ \cline{3-16} 
                            &                                     & Image               & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.2.0                                                           & 6                        & \tickYes & 1.4.0                                                         & 5    & \tickYes  & 3.110.3                                                          &   6  & \tickYes & 1.0.0                                                           &    5 \\ \cline{3-16} 
                            &                                     & Video               & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.2.0                                                           & 18                       & \tickYes & 1.10.0                                                        &  1   & \tickYes  & -                                                                &   26  & \tickYes & 1.0.0                                                           &   6  \\ \cline{3-16} 
                            &                                     & Audio \& Recorder   & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.9.6                                                           & 115                      & \tickYes & 1.23.4                                                        &   7  & \tickYes  & -                                                                &   52  & \tickYes & 1.0.0                                                           &   8  \\ \cline{3-16} 
                            &                                     & Camera              & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.6.0                                                           & 9                        & \tickYes & -                                                             &   1  & \tickYes  & 3.15.104                                                         &   9  & \tickYes & 1.78.0                                                          &   4  \\ \cline{3-16} 
                            &                                     & Rich text           & \multicolumn{1}{l}{}                                                                 & \tickYes & 2.7.0                                                           & 13                       & \tickNo  & N/A                                                           &   N/A  & \tickNo   & N/A                                                              &  N/A   & \tickNo  & N/A                                                             &   N/A  \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Location}                             & \ding{195}                                                           & \tickYes & 2.8.0                                                           & 7                        & \tickYes & 1.1.1                                                         &  3   & \tickYes  & 3.150.1                                                          &  7   & \tickYes & 1.0.0                                                           &    3 \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Data Encryption}                      & \multicolumn{1}{l}{}                                                                 & \tickYes & 2.3.1                                                           & 1                        & \tickYes & -                                                             &    1 & \tickYes  & -                                                                &  1   & \tickNo  & N/A                                                             &   N/A  \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Contact \& Phone Call}                & \ding{195}                                                           & \tickYes & 1.2.0                                                           & 2                        & \tickYes & 1.4.0                                                         &   5  & \tickYes  & -                                                                &  2   & \tickYes & 1.0.0                                                           &    2 \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Canvas}                               & \multicolumn{1}{l}{}                                                                 & \tickYes & 2.7.0                                                           & 64                       & \tickYes & -                                                             &    56 & \tickYes  & -                                                                &  46   & \tickYes & 1.0.0                                                         &    15 \\ \cline{2-16} 
                            & \multicolumn{2}{c}{File}                                 & \ding{194}                                                           & \tickYes & 2.11.0                                                          & 39                       & \tickYes & 1.4.0                                                         &  6   & \tickYes  & 3.130.1                                                          &   35  & \tickYes & 1.15.0                                                          &   35 \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Cross-app Channel}                    & \ding{196},\ding{197}                               & \tickYes & 1.3.0                                                           & 2                        & \tickYes & 1.13.0                                                        &  2   & \tickYes  & 1.10.8                                                           &   2  & \tickYes & 1.15.0                                                          &   2  \\ \cline{2-16} 
                            & \multicolumn{2}{c}{In-App Channel}                       & \ding{198}                                                           & \tickYes & 1.9.6                                                           & 6                        & \tickYes & 1.4.0                                                         &   6  & \tickYes  & 3.60.2                                                           &   5 & \tickYes & 1.0.0                                                           &   5  \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Shareable UI}                         & \ding{198}                                                           & \tickYes & 1.2.0                                                           & 5                        & \tickYes & 1.7.0                                                         &   2  & \tickYes  & -                                                                &   3 & \tickYes & 1.5.0                                                           &   3 \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Accessibility}                        & \multicolumn{1}{l}{}                                                                 & \tickYes & 2.13.0                                                          & 2                        & \tickNo  & N/A                                                           &  N/A   & \tickNo   & N/A                                                              & N/A  & \tickNo  & N/A                                                            &    N/A  \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Payment}                              & \ding{195}                                                           & \tickYes & 1.0*                                                            & 11                       & \tickYes & -                                                             &   13   & \tickNo  & N/A                                                                &    N/A & \tickYes & -                                                               &   1  \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Gait \& Sports}                       & \ding{195}                                                           & \tickYes & 1.2.0                                                           & 1                        & \tickYes & 1.17.1                                                        &   1  & \tickNo   & N/A                                                              &   N/A  & \tickNo  & N/A                                                             &   N/A    \\ \cline{2-16} 
                            & \multicolumn{2}{c}{Embedding Advertisement}              & \multicolumn{1}{l}{}                                                                 & \tickYes & 2.0.4                                                           & 21                       & \tickNo  & N/A                                                           &   N/A  & \tickNo   & N/A                                                              &  N/A   & \tickYes & 1.57.0                                                          &    13 \\ \cline{2-16} 
                            & \multirow{3}{*}{Peripheral}         & Bluetooth           & \ding{192},\ding{193}                               & \tickYes & 2.10.3                                                          & 48                       & \tickYes & -                                                             &  28   & \tickNo   & N/A                                                              &  N/A   & \tickNo  & N/A                                                             &     N/A  \\ \cline{3-16} 
                            &                                     & Wifi                & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.6.0                                                           & 10                       & \tickNo  & N/A                                                           &   N/A  & \tickNo   & N/A                                                              &   N/A  & \tickYes & 1.0.0                                                           &     1 \\ \cline{3-16} 
                            &                                     & NFC                 & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.7.0                                                           & 79                       & \tickNo  & N/A                                                           &   N/A  & \tickNo   & N/A                                                              &  N/A   & \tickNo  & N/A                                                             &   N/A    \\ \cline{2-16} 
                            & \multirow{5}{*}{Sensors \& Devices} & Battery             & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.2.0                                                           & 2                        & \tickYes & -                                                             &   2  & \tickYes  & 3.30.2                                                           &   2  & \tickNo  & N/A                                                             &   N/A    \\ \cline{3-16} 
                            &                                     & Compass             & \ding{195}                                                           & \tickYes & 1.1.0                                                           & 4                        & \tickYes & 1.9.0                                                         &   2  & \tickYes  & 3.30.2                                                           &    3 & \tickYes & 1.2.0                                                           &  3   \\ \cline{3-16} 
                            &                                     & Gyroscope           & \ding{195}                                                           & \tickYes & 2.3.0                                                           & 4                        & \tickYes & 1.9.0                                                         &   2  & \tickNo  & N/A                                                          &  N/A   & \tickNo  & N/A                                                             &    N/A  \\ \cline{3-16} 
                            &                                     & Accelerometer       & \ding{195}                                                           & \tickYes & 1.1.0                                                           & 4                        & \tickYes & 1.9.0                                                         &   2  & \tickYes  & 3.30.2                                                           &   3  & \tickYes & 1.0.0                                                           &   3  \\ \cline{3-16} 
                            &                                     & Vibration           & \multicolumn{1}{l}{}                                                                 & \tickYes & 1.2.0                                                           & 7                        & \tickYes & 1.9.0                                                         &  3   & \tickYes  & -                                                                &   2  & \tickYes & 1.0.0                                                           &  2   \\ \cline{2-16} 
                            & \multicolumn{2}{c}{AI Services}                          & \multicolumn{1}{l}{}                                                                 & \tickNo  & N/A                                                             & \multicolumn{1}{c}{N/A} & \tickNo  & N/A                                                           &   N/A  & \tickYes  & 3.20.11                                                          &   29  & \tickNo  & N/A                                                             &     N/A  \\ \hline
  \multirow{4}{*}{Back-end} & \multicolumn{2}{c}{Trust domain Policy}                  & \ding{194}                                                           & \tickYes & 1.1.0                                                           & 51                       & \tickYes & -                                                             &   14  & \tickYes  & -                                                                &   30  & \tickYes & -                                                               &   8  \\ \cline{2-16} 
                            & \multirow{3}{*}{Cloud Base}         & File Storage        & \ding{194},\ding{198}                               & \tickYes & 1.1.0                                                           & 4                        & \tickYes & -                                                             &    2 & \tickYes* & N/A                                                              &    5 & \tickNo  & N/A                                                             &   N/A  \\ \cline{3-16} 
                            &                                     & Database Access     & \ding{194},\ding{198}                               & \tickYes & 1.1.0                                                           & 227                      & \tickYes & -                                                             &   15  & \tickYes* & N/A                                                              &  23   & \tickNo  & N/A                                                             &    N/A \\ \cline{3-16} 
                            &                                     & Customized Function & \ding{194},\ding{198}                               & \tickYes & 1.1.0                                                           & 1                        & \tickYes & -                                                             &   1  & \tickYes* & N/A                                                              &   1  & \tickNo  & N/A                                                             &     N/A \\ \hline
\end{tabular}}
\vspace{2mm}
\caption{Comparison of major mini-apps APIs and SDKs across platforms. Current SDK version is given in the brackets. 
%\ding{192} Fake Peripheral; \ding{193} Peripheral Data Unauthorized Access; \ding{194} Network Isolation Escape; \ding{195} Collusion Attack; \ding{196}  Mini-app Launching Hi-Jack; \ding{197}  MitM attacks against Cross Mini-apps Communication; \ding{198} Session Riding;  
``-'' means we can not find the references available.  ``\tickYes*'' means the referred API is currently in an internal testing stage.  } 
\label{tab:compare:api}
\end{table*}



\subsection{Basic Comparison of Four Platforms}
\label{subsec:basic}

With the public official documents and our programming practices,  we are able to compare the mini-app platforms from multiple dimensions, 
and obtain many insights on the approaches that how the host app manage resources, and secure the mini-apps, including (I) basic profiles (e.g., name, size), and (II) available APIs and SDKs.
%(e.g., whether a vulnerable API exists on a specific platform).



\textbf{(I) Comparison of basic profiles}. As shown in \autoref{tab:compare:platfroms}, we compare the mini-apps from different platforms:

\begin{itemize}
\item \textbf{Name}. We found the mini-apps platforms trended to give mini-apps different names, but all the names intended to convince the users that their mini-apps had relatively small size. \looseness=-1 

\item \textbf{Size}. Different apps have different size limitation. We found all the platforms excepted \tik supported a sub-package loading feature, where the developer can divide one mini-app into multiple pages and the user can load all or some of the packages depending on which functionalities they intended to access. Particularly, we found that \wechat allowed the total size of all subpackages of a mini-app to reach 20 MB.

\item \textbf{Background Services}. Mini-apps from all platforms were not allowed to run in the background for a long time. The platforms only allowed the miniapp to run for a specific period of time (e.g., 5 mins for \baidu and \tik). When time is up or the mini-app occupies too much system resources, the host app would terminate the mini-app automatically. 

         
\begin{table*}[h]
\resizebox{1.3\columnwidth}{!}
{
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Host App}} & \multicolumn{4}{c}{\textbf{Role}}                                                                                                                                             & \multicolumn{2}{c}{\textbf{Policy}}   & \multicolumn{3}{c}{\textbf{Resources}}                                                                           \\ \cmidrule(l){2-10} 
                                   & \textbf{Admin}    & \textbf{Creator}  & \textbf{\begin{tabular}[c]{@{}c@{}}User\\ (logged)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}User\\ (unlogged)\end{tabular}} & \textbf{Read}     & \textbf{Write}    & \textbf{Files}    & \textbf{Database} & \textbf{ Customized   Functions } \\ \cmidrule(r){1-10}
\wechat                             & \tickNo & \tickYes & \multicolumn{2}{c}{\tickYes}                                                                                                 & \tickYes & \tickYes & \tickYes & \tickYes & \tickYes                                                        \\
\alipay                             & \tickYes & \tickYes & \multicolumn{2}{c}{\tickYes}                                                                                                 & \tickYes & \tickYes & \tickYes & \tickYes & \tickNo                                                        \\
\baidu                              & \tickNo & \tickYes & \tickYes                                                & \tickYes                                                  & \tickYes & \tickYes & \tickYes & \tickYes & \tickNo                                                        \\ \bottomrule
\end{tabular}}
\vspace{2mm}
\caption{Comparison of cloud base access control policy. \tik does not support cloud base currently.  } 
\label{tab:cloud:api}
\end{table*}

\item \textbf{Developers}. Different platforms had different regulations, specifying who and how can (to) be a developer. We found that \baidu has a relatively closed ecosystem, where only the enterprise developers were allowed to register as their developers. However,  all the platforms allowed a individual to apply a trial account to test on their development tools and SDK. For security concerns, the mini-app programmed by a test account were not allowed to be released.

\item \textbf{Supported OS}. All mini-apps were compatible to run on multiple OSes, including Android, iOS, and Windows, as shown in \autoref{tab:compare:platfroms}. Among them, \wechat mini-apps could run onto all the three platforms. Note that, although some host apps such as \wechat also had a macOS version, mini-apps that can run onto the macOS are currently not support at the time of writing, 


\item \textbf{Package Encryption}. We found that only \wechat supported the package encryption feature, where \wechat encrypted the mini-app packages running on Windows machines using AES-CBC and the encryption key was derived from the mini-app ID. This is because for mini-apps that run  on the mobile platforms such as Android and iOS, the corresponding packages containing the source codes and resources are all located at protected directory, which require the root privilege to be accessed. 
%It may require some efforts for a potential adversary to obtain the packages.
However, packages on a Windows machine can be easily accessed. If the encryption was not in position, it would be more trivial for adversary to reverse engineer the packages. 

\item \textbf{Entries}. An other observation was that all mini-apps from three the platforms supported multiple entries feature. That is, the mini-app can be launched through scanning QR code, clicking link or searching and opening it directly from mini-app store.

\end{itemize}





 \textbf{(II) Comparison of mini-apps APIs \& SDKs}. As shown in \autoref{tab:compare:api} (based on our best understanding), we group the major available APIs existing in different platforms into 32 categories, which fail into two main group, i.e., the front-end APIs and the back-end APIs:
 
 \textbf{Front-end APIs.} It can be observed that \wechat had more APIs (27 of 28 APIs) than others, while \tik had a relatively small API number (20 of 28 APIs). This is because \wechat have been developing the mini-app community for almost four years (since 2017), while \tik  started their mini-app products at 2019. This can also be observed and confirmed from the SDK version numbers.  For one specific platform, as the SDK version increased, more APIs with different functionalities were supported by the corresponding platforms. 
 We also observed that APIs that have access to system resources such as Bluetooth APIs,  File System APIs and location Services APIs  appeared relatively late. %(involved in Attack \ding{192} and \ding{193})
 %(involved in Attack \ding{194})
 %(involved in Attack \ding{195}) 
 Those APIs usually involved more security concerns, and it seemed that the designers of platforms all agreed that great caution should be exercised in dealing with sensitive resources. 
 %Sensor APIs such as Compass, Gyroscope and Accelerometer may be combined using Attack \ding{195} and abused to deploy user fingerprint attacks.  We found all platforms provided Cross-app channel APIs, in-App communication API, and Shareable UI APIs, these APIs may be vulnerable to Attack \ding{196}, \ding{197}, \ding{198}, where the attack manipulate the in-app or cross-app communicating channel. 
 %We have also observed that \tik does not provide an encryption API for data transmission, and each mini-app has to implement the encryption.   
 
 Each platform may have its unique features. For example, \wechat allowed the mini-app to access the accessibility services without permission checking process, and the accessibility services were believed to have major security impacts against the mobile platforms \cite{fratantonio2017cloak}. Fortunately, only a few methods are provided currently (checking whether the accessibility services are enabled or actively enabling a component of a mini-app to be accessed by the system Talkback service \cite{diaz2014accessibility}). We advocate that vendors should pay more attention when involving these dangerous APIs. For \wechat, we also found that it had a standalone SDK with well-designed document and APIs for achieving the securing payment \cite{wechatpay20}.  \wechat and \alipay allows the mini-app to access gait and sports data, which was believed to have privacy concern.
  %We believe all those sensitive information such as the payment history, contact information and sports data, may be subject to attack \ding{195}.
 \baidu provide an unique AI services feature, where their mini-apps can access their powerful AI interfaces such as speech recognition, image recognition and facial recognition. This is why they named their mini-apps as Smart (AI) mini-programs.   
 
 \textbf{Back-end APIs} It can be observed that all the four platforms supported the trust domain policy, where the host app back-end played the role of the gateway to filter out insecure network requests. These back-end APIs involved accessing of network resources, which may be subject to Attack \ding{194} (e.g., escaping network isolation) and \ding{198} (e.g., deleting file on cloud base). Specifically, the cloud base of \baidu (\baidu released the mini-app product at 2019) is under construction, and currently they released the internal testing APIs, which is similar to that of \wechat and \alipay. \tik currently does not support cloud base, and we infer that it is also because they had the support of mini-apps at 2019, and their cloud base may be in the developing process.

We found that each platform allowed the developer to customize the access control policy, specifying how the cloud resources can be accessed (e.g., if a record in a specific database can be accessed by a specific user).
We now compare the access control policies of the cloud base provided by each platform. As shown in \autoref{tab:cloud:api},  it can be observed that there are four roles available, including admin, who is the owner of the mini-app project, creator, who is creator of specific resources, and user, who consume the resources. We found that \baidu groups the users as the logged users and un-logged users, which is more fine grained and secure. \wechat could specify the access control for the defined cloud functions, while the other two did not support.   
 

==> paper/03_overview.tex <==

\section{The \textsf{Coffee} Attack}
\begin{figure*}
    \centering
    \includegraphics[width=.8\linewidth]{image/example.pdf}
    \caption{An example of session key leakage impact}
    \label{}
\end{figure*}
\subsection{Mini-app Security Model}
\label{sub:threat-model}
The mini-app front-ends are not trusted, and developer need to configure properly if they use third-party back-ends.ba

The mini-app framework supports not only native app features, but also web-app features. As a native app, the mini-app interacts frequently with users' devices, including data, media, devices, and peripherals. As a web-app, the mini-apps consist of front-ends (mainly written in JavaScript) and their corresponding cloud back-ends. Since the front-ends of mini-apps are distributed to users' devices, these front-ends can potentially be decompiled and examined, wechat clearly stated in their official documentations that the data sent from mini-app front-ends cannot be trusted and requires verification.

In our mini-app attack scene, we adopt the same threat model as stated in \wechat official documentations by assuming that the mini-app framework is secured and attackers cannot interfere with the mini-app framework, whereas the attackers can obtain and unpack the mini-app front-end packages. Generally, the attack scenes can be summarized into two categories:


\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item \textbf{Attack targeting mini-apps}. In this scenario, the attackers can exploit the vulnerable mini-app, manipulate network packages, and attack the victim mini-app back-ends for sensitive information or make profits.
    \item \textbf{Attack targeting users}. In this scenario, the attackers can lure victims to install malicious mini-apps or native apps that steals sensitive user information or interfere with vulnerable mini-apps installed on victims' phone.
\end{itemize}

For the rest of this paper including the comparison between mechanisms, tool design and evaluations, we will further investigate the mini-app security mechanisms based on this threat model.
\subsection{Insecure BLE Configuration}

\subsection{Unchecked Cross-miniapp Communication}

\subsection{Credential Leakage Exploitation}
Although the \wechat framework is supposed to secure the user data and communication well with all these various security mechanisms, we still found that there are concerning cases where developers expose their mini-app in danger with improperly used add-on security mechanism. In the example shown in fig., the mini-app user logs in and sends the login token to their third-party back-end server to exchange for session key. However, we observed that instead of maintaining the sensitive session key and only sending necessary information to the front-end, the back-end directly forwards the network packet from \wechat server, containing not only login results but also critical session key and encryption iv. Since this session key is the decryption key required for all encrypted data sent from \wechat server, and the encryption mechanism is publicized on \wechat official documentations, the attacker can arbitrarily capture and manipulate the encrypted data such as account details and \wechat sports data, even faking their identity. For example, in the figure shown above, we can easily decrypt the data with the session key obtained. As a result, we get to know the structure of user login information, and are able arbitrarily to fake our identity or bypass the login mechanism by modifying the phone number in this packet.

\paragraph{Key insight} \AY{This paragraph might be removed, just left here for reference} From this motivation example, we observe that although add-on mechanisms provide developers with versatility, there are still costs of such a freedom: the misused add-on security mechanisms may undermine the mini-app framework unexpectedly, making it vulnerable to \textsf{Coffee} attack. 
In this motivation example, \wechat directly lets developers using third-party back-end servers to fully control such a critical credential without further checking or warning to the developers, let alone managing these session keys for developers in the SDK, except for a sentence in the documentation specifying that developers should not disclose the session key. This eventually resulted in the unconscious leakage of critical credentials. Interested in the current situation of mini-app security mechanism usage and how the misuse and misconfiguration of add-on security mechanisms can undermine the framework security, in this paper, we focus on the security mechanisms that involves both built-in and add-on features, and provide a detailed analysis of these add-on security mechanism usage in the current mini-app ecosystem.




\paragraph{Motivating Example} 

% , whereas the developers are unable to verify the modified data.

% We then performed a proof-of-concept attack with this example in fig. We decrypted the data with the algorithm published on \wechat official documentation and found that the mini-app uses user phone number as login identifier. Moreover, we found that the mini-app leaked the manager account info, which can be used to obtain the administrative accounts. As a result, we logged in as the administrator merely by changing login request packets.




==> paper/03_overview_back.tex <==
\section{Built-in v.s. Add-on security}
The complexity of mini-app framework makes it challenging to design security mechanisms to protect user data and cloud communication from being intercepted and exploited. To achieve this goal, \wechat combined the built-in and add-on security mechanisms to balance the security and usability. To analyze the security of the mini-app framework, we first discuss the \wechat mini-app threat model in \cref{sub:threat-model} , and then compare the advantages and disadvantages of built-in and add-on mechanisms respectively in \cref{sub:build-in} and \cref{sub:add-on}.
% The reason why wechat has adopted such a complex security mechanism lies in the complex functionality involved in the mini-app paradigm. To gain an edge from native applications in terms of usability, funcitonality, and security, wechat is not merely a normal native application any more, but instead an OS-like ecosystem that involves both native OS resources and heterogeneous back-ends. On top of that, the requirement of using their own third-party servers from business vendors that would like to integrate their services into mini-apps requires wechat to support third-party back-ends and enforce data encryption, which elevated the challenge of securing the mini-app data while maintaining the versatile functionality. In this section, we discuss the threat model that wechat mini-app adopts as described in their official documentations when designing these mechanisms, and then provide a detailed comparison of wechat security mechanisms.

\subsection{The Threat Model of Mini-apps}

\subsection{The Dilemma of Built-in Mechanism}
\label{sub:build-in}
% In the wechat mini-app framework, the built-in mechanisms can be summarized into the following two mechanisms:
% \begin{itemize}
%     \item \paragraph{Non-interactive mechanism} These mechanisms are non-configurable and transparent to the developers: the developers cannot intefere or customize the mechanisms. The storage and plugin isolation and domain
%     \item \paragraph{Interactive mechanism}
% \end{itemize}

% The built-in security mechanisms of wechat mini-app includes isolation, lifecycle handling, whitelists, blacklists, permission authorization, and data encryption.
% \paragraph{Usability or security, that is a question} 
To ensure the safety of mini-apps running in \wechat, mandatory built-in mechanisms ensures that all the mini-apps running in the framework have enforced the necessary security protections. For example, each developers must request and authorize permissions when using specific system resources. Therefore, the OS resource will never be accessed if the permission is not granted. Secure as these built-in mechanisms are, however, they still suffer from disadvantages in two ways:
\begin{itemize}[leftmargin=*]
    \item \paragraph{Impairing usability} The built-in security mechanisms may require mandatory configuration from the developers, thus making the development process more complex. For example, in an earlier stage of mini-app framework, all developers are required to configure a navigation mini-app id list. As such, navigation to mini-apps that are not in this white list will not be allowed. This mechanism is initially designed to prevent unexpected navigation if malicious attackers hijacks the mini-app by hooking mini-app interfaces. However, when developers need to redirect to additional mini-apps, they have to re-configure the mini-app ids in their configuration files, re-compile the mini-app, and make users to update the mini-apps. This had raised complaints about the usability of mini-app frameworks among developers in the forum. As a result, \wechat removed the requirement of mini-app navigation configuration starting from 2018.
    \item \paragraph{Limiting functionality} Built-in security mechanisms may limit the functionalities of mini-apps. For example, although \wechat provided a `cloud function' feature to let users easily communicate with cloud back-ends without knowing the login authentication and data decryption mechanisms, they still allow developers to use third-party back-ends. Since there is a great amount of companies that wish to make use of their own back-end servers to link user account info and data with other platforms (e.g., PC app, Android app, etc.), it is not practical for \wechat to force all mini-app developers to use cloud function features, otherwise the mini-app loses its edge against native apps for the service providers due to the limited functionalities.
\end{itemize}

% \paragraph{Usability or security, that is a question} Due to the complexity of mini-app functionality that involve host OS, front-end, and back-ends including wechat clouds and third-party clouds, designing a security mechanism that achieves balance between the emerging functionality requirements and the imminent security requirements is a challenging task, since the wechat framework is facing a bilateral dilemma: the wechat framework can control everything and make every security mechanisms totally transparent to developers, but this will undoubtedly limit the functionality of mini-apps significantly, contradicting their initial motivation of providing a more versatile and convenient native-like experiences for developers and users; on the other hand, the wechat framework cannot simply let developers control the security mechanisms, since the developers can be evil or unconscious about the severe impact of security vulnerabilities, and hence the security of mini-app ecosystem will be significantly undermined in either way.

% \paragraph{Built-in and add-on: answer to the dilemma} 
To solve this dilemma, \wechat combines built-in and add-on mechanism. The built-in mechanisms are mandatory to the developers to make sure every mini-app running in the framework have enforced the security mechanisms, such as isolation, white lists, and permission managements. On top of that, \wechat also provides various optional add-on mechanisms for developers if they want to expand the functionalities of their mini-app and enforce additional security mechanisms, such as device configuration and session key management in third-party servers. Such a combination of built-in and add-on mechanisms achieves a balance by providing the capability of extending the security of mini-apps, whereas ensuring that basic security mechanisms are transparent to developers and cannot be interfered.


\subsection{The Cost of Add-on Freedom}
\label{sub:add-on}
There is no doubt that the add-on security mechanisms enforced atop built-in mechanisms are supposed be enhancing the framework security. 
% , rather than potentially undermining the security. 
However, we are surprised to find that it is not always true, 
% not all add-on security mechanisms enhance the framework security,
especially when they are misused by developers, which is inevitable: instead of merely making add-on configuration ineffective, the misuse of add-on security may leak critical information that undermines the entire security mechanism of mini-app framework.

\paragraph{Motivating Example} Although the \wechat framework is supposed to secure the user data and communication well with all these various security mechanisms, we still found that there are concerning cases where developers expose their mini-app in danger with improperly used add-on security mechanism. In the example shown in fig., the mini-app user logs in and sends the login token to their third-party back-end server to exchange for session key. However, we observed that instead of maintaining the sensitive session key and only sending necessary information to the front-end, the back-end directly forwards the network packet from \wechat server, containing not only login results but also critical session key and encryption iv. Since this session key is the decryption key required for all encrypted data sent from \wechat server, and the encryption mechanism is publicized on wechat official documentations, the attacker can arbitrarily capture and manipulate the encrypted data such as account details and \wechat sports data, even faking their identity. For example, in the figure shown above, we can easily decrypt the data with the session key obtained. As a result, we get to know the structure of user login information, and are able arbitrarily to fake our identity or bypass the login mechanism by modifying the phone number in this packet.

% , whereas the developers are unable to verify the modified data.

% We then performed a proof-of-concept attack with this example in fig. We decrypted the data with the algorithm published on \wechat official documentation and found that the mini-app uses user phone number as login identifier. Moreover, we found that the mini-app leaked the manager account info, which can be used to obtain the administrative accounts. As a result, we logged in as the administrator merely by changing login request packets.

\paragraph{Key insight} From this motivation example, we observe that although add-on mechanisms provide developers with versatility, there are still costs of such a freedom: the misused add-on security mechanisms may undermine the mini-app framework unexpectedly, making it vulnerable to \textsf{Coffee} attack. 
In this motivation example, \wechat directly lets developers using third-party back-end servers to fully control such a critical credential without further checking or warning to the developers, let alone managing these session keys for developers in the SDK, except for a sentence in the documentation specifying that developers should not disclose the session key. This eventually resulted in the unconscious leakage of critical credentials. Interested in the current situation of mini-app security mechanism usage and how the misuse and misconfiguration of add-on security mechanisms can undermine the framework security, in this paper, we focus on the security mechanisms that involves both built-in and add-on features, and provide a detailed analysis of these add-on security mechanism usage in the current mini-app ecosystem.


==> paper/03_problem.tex <==
\section{The \textsf{Coffee} Attacks}
\label{sec:overview}
As discussed in \S\ref{sec:back}, \wechat combines both the built-in and the add-on security measures to secure the mini-apps both at front-ends and back-ends: the built-in mechanisms are mandatory for all mini-apps (e.g., the mini-app isolation mechanism is enforced for every mini-app, and authorization scope is always required as long as the developer attempts to use corresponding resources), whereas the add-on security mechanisms involves developer implementations to make the mechanisms to be effective (e.g., the developers have to implement the data decryption of sensitive data with the session key of the user). Although these add-on mechanisms open up more versatility and freedom for developers, such as the free choice of implementing third-party servers, it is very likely for the framework to give too much freedom for the developers to maintain these essential mechanisms. To investigate the costs of such a freedom, we manually investigate all these four add-on security measures, and correspondingly, we identified four types of \textsf{Coffee} attacks, as summarized in the right part of \autoref{tab:mechanisms}. Among these four attacks targeting add-on mechanisms, three attacks are against the front-end mechanisms (\S\ref{subsec:coffee-front}), and one is against the add-on security mechanism enforced at the back-end (\S\ref{subsec:coffee-back}). 
 


%\subsection{Summary of Add-on Misuses and Attacks}
%\label{subsec:summaryofattacks}
%he mini-app framework supports not only native app features, but also web-app features. As a native app, the mini-app interacts frequently with users' devices, including data, media, devices, and peripherals. As a web-app, the mini-apps consist of front-ends (mainly written in JavaScript) and their corresponding cloud back-ends. Since the front-ends of mini-apps are distributed to users' devices, these front-ends can potentially be decompiled and examined, wechat clearly stated in their official documentations that the data sent from mini-app front-ends cannot be trusted and requires verification.
%We first compare the all the mis-use and attacks against the four different add-on security measures. Particularly, the objective of the attacker is to obtain the user's sensitive information, or intentionally modify and injected fake data into a vulnerable mini-app. We adopt the same threat model as stated in \wechat official documentations \cite{wechatkey20} by assuming that the mini-app framework is secured and attackers cannot interfere with the mini-app framework, whereas the attackers can obtain and unpack the mini-app front-end packages. In some of the attacks, we consider the attacker with his malicious native app or mini-app installed. The assumptions are practical, and previous efforts~\cite{lu2020demystifying} used the similar threat model.   
 
%We argue that a security measure ``must'' be positioned as built-in,  as long as it ``can'' be positioned as built-in. The add-on security measures may be useful only when the security measures cannot be a part of the framework. For example, in the traditional programming frameworks provided by OSes, user authentication cannot be included as one of the built-in security mechanisms, since the user information is maintained at the server of the native apps rather than the OS. In this case, the add-on security measure is the only option. However, in the context of the mini-apps, \wechat maintains the user database, and it has the capabilities of including user authentication as a built-in security measure. Therefore, \wechat integrates the user authentication as one of their built-in security measures. 
 
 
%In this section, we present the \textsf{Coffee} Attacks to show the grave consequences caused by the mis-configurations of the four add-on security mechanisms discussed in \S\ref{sec:back}. Particularly, we first show the insights and the threat model of our attacks (See \S\ref{subsec:threatmodel}), followed by three types of \textsf{Coffee} attacks against the front-end (See \S\ref{subsec:coffee-front}), as there are three add-on security measures can be deployed at front-end, and finally one type of \textsf{Coffee} attack against the add-on security measure deployed at the back-end (See \S\ref{subsec:coffee-back}). 
 


\ignore{
\begin{table*} 
    \centering
    \small
    \begin{tabular}{clll}
    \toprule 
    Type&Mechanism&Built-in&Add-on\\ \midrule
     Front-end&Permission management&authorization&N/A\\ 
     Front-end&Storage management&isolation&N/A\\
     Front-end&Device management&N/A&configuration\\
    Front-end&In-miniapp plugins&isolation&N/A\\
    Front-end&Background mini-app&lifecycle handling&N/A\\
    Front-end&Mini-app redirection&acceptlist&checking\\
    Front-end&Private sharing&N/A&checking\\
    % front-end&Background management&y&\\
    Back-end&Domain acceptlist&acceptlist \& blacklist$^{*}$&N/A\\
    Back-end&Cloud API token (appsecret)&generation \& validation&maintainence\\
    Back-end&Data encryption/decryption&encryption&decryption\\ 
    Back-end&Cloud function&maintainance \& decryption&N/A\\
    % &&&N/A\\
    \bottomrule
    \end{tabular}
    \caption{Summary of Mini-app Security Mechanisms}
    \label{tab:mechanisms}
\end{table*}

}

%\subsection{Insight and Threat Model}
%\label{subsec:threatmodel}







 
 %For example, the essential \texttt{Appsecret} is totally left for the developers to maintain but without any mechanisms to manage their usages to prevent them being leaked. As such, when developers misuse the mechanisms, they may impair the framework security, and unconsciously expose their mini-app in danger. 





%\paragraph{Threat Model and Assumptions} 
%The mini-app framework supports not only native app features, but also web-app features. As a native app, the mini-app interacts frequently with users' devices, including data, media, devices, and peripherals. As a web-app, the mini-apps consist of front-ends (mainly written in JavaScript) and their corresponding cloud back-ends. Since the front-ends of mini-apps are distributed to users' devices, these front-ends can potentially be decompiled and examined, wechat clearly stated in their official documentations that the data sent from mini-app front-ends cannot be trusted and requires verification.
%The objective of the attacker is to obtain the user's sensitive information, or intentionally modify and injected fake data into a vulnerable mini-app. We adopt the same threat model as stated in \wechat official documentations \cite{wechatkey20} by assuming that the mini-app framework is secured and attackers cannot interfere with the mini-app framework, whereas the attackers can obtain and unpack the mini-app front-end packages. In some of the attacks, we consider the attacker with his malicious native app or mini-app installed. The assumptions are practical, and previous efforts~\cite{lu2020demystifying} used the similar threat model.  



%Generally, the attack scenes can be summarized into two categories:
%\begin{itemize}[leftmargin=*]
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\setlength{\parskip}{0pt}
%    \item \textbf{Attack targeting mini-apps}. In this scenario, the attackers can exploit the vulnerable mini-app, manipulate network packages, and attack the victim mini-app back-ends for sensitive information or make profits.
 %   \item \textbf{Attack targeting users}. In this scenario, the attackers can lure victims to install malicious mini-apps or native apps that steals sensitive user information or interfere with vulnerable mini-apps installed on victims' phone.
%\end{itemize}

%For the rest of this paper including the comparison between mechanisms, tool design and evaluations, we will further investigate the mini-app security mechanisms based on this threat model.

\subsection{\textsf{Coffee} Attacks against Front-end}
\label{subsec:coffee-front}

%Android and iOS implement the security levels differently, as shown in \ref{tab:permission}.  Android provides all the three security levels for apps to customize their services, but iOS, however, only provides two primary security levels for iOS apps, and the strongest security level is not provided. We found the platforms of mini-apps such as \wechat followed the iOS's practice, in which only two security levels are provided. Since the strongest security level is defined to defend unauthorized services access attacks, the absent of the security level 3 will position the mini-apps running on Android devices in the risk of unauthorized services access attacks. 

In total, there are three add-on security measures of \wechat mini-apps that can be enforced at the front-end: the configurable services protection, cross-mini-app authentication, and cross-user sharing protection. However, if developers mis-use or mis-configure these add-on security measures, they may instead undermine the security of mini-apps. In this section, we introduce three attacks against these security mechanisms in details, including (1) unauthorized access attacks against configurable services protection, (2) fake message injection attack against cross-mini-app authentication and (3) private sharing abusing against the cross-user sharing protection. 

\paragraph{(1) Unauthorized Access Attacks}\AY{Was it peripheral communciation encryption stuff? The unauthorized access looks a bit weird isn't it} When mini-apps access peripheral devices such as Bluetooth devices, the developers can configure whether to enable the device encryption by setting 
% The attacks work against configurable services protection. Recall that 
% configurable device encryption requires the developers to manually set 
the parameter \texttt{readEncryptionRequired} and \texttt{writeEncryptionRequired} as \texttt{true} or \texttt{false}. 

When a mobile work as a central, it can communicate with other IoT devices such as smart-lights and Blood pressure monitors that have limited resources. These devices may not support the Bluetooth encryption. Therefore, the services on these devices may be unprotected for compatibility. However, when the mobile works as the peripheral, only other smartphones or laptops (\ie, centrals) can communicate with it, and all these devices should have the support of Bluetooth encryption. \wechat blindly followed the practice of IoT devices, and downgraded its security proprieties.

However, such a security mechanism should have been designed as an built-in security measure rather than a add-on security measure. That is, the encryption should be enforced. 
To understand this, we first explain why services are unprotected in some cases.
   

We make the following assumptions for this attack: (1) we assume the a mobile running a mini-app that forces the mobile to work as the peripheral, and the services on the mobile is misconfigured (\ie, \texttt{readEncryptionRequired} or \texttt{writeEncryptionRequired} are set as \texttt{false}). For concise, we denote this device as the peripheral. (2) Another mobile, worked as the central, is supposed to communicate with the peripheral. (3) 
The attacker is in the range of the two communicating devices and wait for a moment where the central and the peripheral get disconnected, but they intend to initiate new session. Such a moment can be easily identified, since the Bluetooth is a wireless communication technology, and before the connection is established, the central device usually sends out discovery requests.\looseness=-1


We now demonstrate how to exploit the mis-configurations of developers to deploy unauthorized access. In particular, the attacker collects the identifier of the victim central (i.e., Bluetooth MAC address), which goes over the air, and uses an attack device to impersonates the victim central. Next, the fake central establishes a connection with the victim peripheral. In the regular case, one peripheral is supposed to connect only one central at a time, and consequently, the peripheral is currently not available for other centrals. The fake central can now send the crafted data to the victim mini-app or receive sensitive information from the mini-app, since the communication requires no encryption. 
 
\paragraph{(2) Fake Message Injection Attacks}  The attack works against the cross-mini-app communication protection mechanism. As discussed, one mini-app can invoke  \texttt{wx.navigateToMiniprogram()} to deliver messages to other mini-apps, where the mini-app ID is attached for the receiver to verify whether the message is from a trusted mini-app. We argue that this security measure should have been designed as the built-in security measure. Indeed, the cross-mini-app authentication was a built-in feature, which allowed a mini-app to specify up to 10 mini-apps into an accept-list, and only the mini-apps in the accept-list could communicate with the mini-app. However, such a built-in security mechanism was discontinued since April 2018, and now developers have to implement the cross-mini-app communication themselves to prevent malicious mini-apps from injecting data into their mini-apps. However, not all developers are aware of the risks, and implement the cross-mini-app authentication. \looseness=-1

In our attack, we assume that the victim mini-app uses the cross-mini-app communication channel provided by \wechat to obtain the messages that sent from other mini-apps; However, the victim mini-app does not implement a mini-app ID checking mechanism to authenticate the source. To deploy the attack, the attacker first creates a malicious mini-app, and then uses the mini-app to invoke \texttt{wx.navigateToMiniprogram()} to launch and inject crafted data to the victim mini-app. Since the mini-app does not implement the cross-mini-app authentication, it will not able to identify whether the message is from a benign mini-app or a malicious one. Consequently, the victim mini-app will accept the inject message. This attack can have grave consequence to the victim mini-app. Indeed, according to our experiment, even a test version of the mini-app (a mini-app that has not upload onto the \wechat mini-app market for vetting) can call \texttt{wx.navigateToMiniprogram()}, which lows the bar for attackers significantly. 
%hence it is for developers to check the mini-app navigation source since there is no longer built-in mechanism.

\paragraph{(3) Private Sharing Abusing} This attack works against the cross user sharing protection. Recall that to prevent the mini-app sharing from abusing, the developer must first call \texttt{updateShareMenu} to specify the mini-app can only be shared once while initiating the mini-app sharing. Latter, when the shared mini-app is launched by a user, the developer then is required to check whether the user is a second-hand user by using \texttt{authPrivateMessage}. Such a security measure should be positioned as a built-in one, as \wechat is aware of the life cycle of any shared mini-apps. That is, the Clickable URL of the mini-app is shared between \wechat users through the Chat window of \wechat and to launch these shared mini-apps, the user also relies on the running environment provided by \wechat. However, \wechat made the security measure as a built-in one, leading the private sharing abusing attack. Specifically, in this attack, we assume that the developer specified the private message, but did specified the \texttt{authPrivateMessage} to validate the accessibility of the message. As a result, the attacker can create multiple accounts and re-share the vulnerable mini-app between accounts to maximize the benefit. For example, the private message can be the Discount Code of a specific product of a distributor, the abusing of the private sharing will impair the profit of the product distributors.  
 
%\item For mini-app platform such as \wechat, which provides the active pairing policy, the mini-app may actively start the pairing process to go through the pairing (Step \ding{186}). Note that, for mini-apps developed using the API from \alipay, steps \ding{186} and \ding{187} are not needed. 
%\item Attacker can actively cancel the pairing process by sending an error code \texttt{PARING\_NOT\_SUPPORTED}. Since the mini-app does not have an interface to access the pairing result, there is no  

   

  


%whether or not the traffic is encrypted depends on the presence of the link key: when the mobile has paired with another device, the link key is generated and the traffic will be encrypted
 
  


\subsection{\textsf{Coffee} Attacks against Back-end}
\label{subsec:coffee-back}

%\subsection{Insecure BLE Configuration}


 

%To achieve a balance between functionality and security, the host app must design the security mechanisms carefully.

%Built-in mechanisms ensures that all the mini-apps running in the framework have enforced the necessary security protections. 


%The add-on security mechanisms, on the other hand, have to be taken care of carefully.


% whereas the developers themselves may not be aware of how essential the mechanism is.

% it is good for security. For example, since each developers must request and authorize permissions when using specific APIs, the API will never be invoked if the permission is not granted. 
% Secure as these built-in mechanisms are, however, they still suffer from disadvantages in two ways:
% \begin{itemize}[leftmargin=*]
%     \item \paragraph{Impairing usability} The built-in security mechanisms may require mandatory configuration from the developers, thus making the development process more complex. For example, in an earlier stage of mini-app framework, all developers are required to configure a navigation mini-app id list. As such, navigation to mini-apps that are not in this white list will not be allowed. This mechanism is initially designed to prevent unexpected navigation if malicious attackers hijacks the mini-app by hooking mini-app interfaces. However, when developers need to redirect to additional mini-apps, they have to re-configure the mini-app ids in their configuration files, re-compile the mini-app, and make users to update the mini-apps. This had raised complaints about the usability of mini-app frameworks among developers in the forum. As a result, \wechat removed the requirement of mini-app navigation configuration starting from 2018.
%     \item \paragraph{Limiting functionality} Built-in security mechanisms may limit the functionalities of mini-apps. For example, although \wechat provided a `cloud function' feature to let users easily communicate with cloud back-ends without knowing the login authentication and data decryption mechanisms, they still allow developers to use third-party back-ends. Since there is a great amount of companies that wish to make use of their own back-end servers to link user account info and data with other platforms (e.g., PC app, Android app, etc.), it is not practical for \wechat to force all mini-app developers to use cloud function features, otherwise the mini-app loses its edge against native apps for the service providers due to the limited functionalities.
% \end{itemize}
% \paragraph{The Cost of Add-on Freedom}
% There is no doubt that the add-on security mechanisms enforced atop built-in mechanisms are supposed be enhancing the framework security. 
% However, we are surprised to find that it is not always true, 
% especially when they are misused by developers, which is inevitable: instead of merely making add-on configuration ineffective, the misuse of add-on security may leak critical information that undermines the entire security mechanism of mini-app framework. \AY{Originally, the rest of this part is now in }


\begin{figure*}
    \centering
    \includegraphics[width=.8\linewidth]{image/example.pdf}
    \caption{An example of session key leakage impact}
    \label{fig:attackexample}
\end{figure*}

%The mini-app front-ends are not trusted, and developer need to configure properly if they use third-party back-ends.ba


%\subsection{Unchecked Cross-miniapp Communication}

%\subsection{Credential Leakage Exploitation}

\wechat has positioned one add-on security measures at the back-end, \ie, the communication encryption, where  \wechat distributes \texttt{Appsecret} to the developers, and requires the developers to maintain the \textsf{Appsecret} and handle the decryption. In this section, we demonstrate the impacts of mis-use the security measure by introducing our encryption communication manipulation attacks. 



\paragraph{(4) Encrypted Communication Manipulation Attacks} We argue that this security measures should be designed as the built-in security measure rather than an add-on one, since \wechat has the capabilities of integrating all the security related keys and functionalities as simple as a few APIs (like what they did in the user authentication, where only two built-in APIs, \ie, \texttt{wx.login} and  \texttt{wx.code2session}, need to be invoked). However, currently, \wechat directly lets developers using third-party back-end servers to maintain \texttt{Appsecret}, receive the session key,  and fully handle the traffic communication decryption without further checking or warning to the developers. This eventually resulted in the unconscious leakage of critical credentials. \looseness=-1 

In this attack, we assume that vulnerable mini-app either leaked  \texttt{Appsecret} or the session key: (1) \texttt{Appsecret} may be hard-coded into the source code of the vulnerable mini-app, and as a result, an attacker can extract the \texttt{Appsecret} from reverse engineering the mini-app. After obtaining \texttt{Appsecret}, the attacker can further fetch the session key by simply invoking  \texttt{code2session} API in a controlled account, as the API only accepts \texttt{Appsecret}, mini-app ID (known to all), and a login token (the attacker's login token). (2) The session key of the mini-app can be distributed to the front-end of the mini-app due to the misunderstanding of development documentation. For instance, the developer may implement an interface in the front-end to query the session key from their back-end. In this case, the attacker can obtain such a session key through network traffic eavesdropping in the controlled environment (\eg, the attacker's smartphone with the victim mini-app installed).  In the following, We  show two attack examples to demonstrate the potential impacts: 


\begin{itemize}
\item \paragraph{Communication Manipulation on User's Mobile} In this attack, we assume that a malicious app is co-located with \wechat, and the malicious app has the capabilities of modifying network requests sending out from the smartphone. For example, this can be achieved by implementing a VPN extensions or a MITM proxy such as \textsf{Burp Suite}~\cite{wear2018burp}. Since the session key is obtained by the attacker due to the mis-use of the add-on security measures, the attacker can arbitrarily decrypt and even manipulate the encrypted data transferred between the \wechat server and the mini-app. For example, it can extract the sensitive information such as user's telephone number.  
 

\item \paragraph{Communication Manipulation on Attacker's Mobile} Different from traffic eavesdropping and modification, this attack can be deployed in the controlled environment, where the attacker use his or her own device and account to poke the vulnerable back-end.  Similar to the prior case, when the victim mini-app sends out the network request that contains the sensitive information, the attacker can then intercept the request and modify the request using the session key. The impacts of this attack can be disastrous: For example, some mini-apps may give their users some bonus or profit based on the \wechat WeRundata, the manipulation of WeRundata from an attacker will undermine fairness. In some other cases, instead of using the built-in user authentication, mini-apps may use the telephone number of users to authenticate the user, as shwon in \autoref{fig:attackexample}. However, the telephone number is obtained through the cipher sent from the mini-app, and by decrypting and re-encrypting the cipher, the attacker can modify the telephone numbers sent to the back-end, and achieve arbitrarily log into the user's account.    
 

\end{itemize}



 

Note that although the built-in user authentication also involved the use of \texttt{Appsecret}, it is not subject to the attacks introduced above. Recall that when the user authentication occurs, the mini-app front-end invokes \texttt{wx.login}, and sends the token to the back-end. The back-end then invokes \texttt{wx.code2session}, which accepts \texttt{Appsecret}, the token and mini-app ID, to get the unique user identifier. Although \texttt{Appsecret} and mini-app ID is know to the attacker, the attacker cannot guess a valid token within 5 minutes (it is updated every 5 minutes), since the login token is associated with the specific user and the specific mini-app and is distributed from the \wechat server. User authentication is still secure even if  \texttt{Appsecret} is leaked due to the well-designed \texttt{wx.login} API, this example further proved that the use of built-in API can make the framework more secure.   

 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


%two built-in APIs (\ie, \texttt{wx.login} and \texttt{wx.code2session}) sequentially to obtain the unique user identifier.  




    









%Although the \wechat framework is supposed to secure the user data and communication well with all these various security mechanisms, we still found that there are concerning cases where developers expose their mini-app in danger with improperly used add-on security mechanism. In the example shown in fig., the mini-app user logs in and sends the login token to their third-party back-end server to exchange for session key. However, we observed that instead of maintaining the sensitive session key and only sending necessary information to the front-end, the back-end directly forwards the network packet from \wechat server, containing not only login results but also critical session key and encryption iv. Since this session key is the decryption key required for all encrypted data sent from \wechat server, and the encryption mechanism is publicized on \wechat official documentations, the attacker can arbitrarily capture and manipulate the encrypted data such as account details and \wechat sports data, even faking their identity. For example, in the figure shown above, we can easily decrypt the data with the session key obtained. As a result, we get to know the structure of user login information, and are able arbitrarily to fake our identity or bypass the login mechanism by modifying the phone number in this packet.

%From this motivation example, we observe that although add-on mechanisms provide developers with versatility, there are still costs of such a freedom: the misused add-on security mechanisms may undermine the mini-app framework unexpectedly, making it vulnerable to \textsf{Coffee} attack. In this motivation example, \wechat directly lets developers using third-party back-end servers to fully control such a critical credential without further checking or warning to the developers, let alone managing these session keys for developers in the SDK, except for a sentence in the documentation specifying that developers should not disclose the session key. This eventually resulted in the unconscious leakage of critical credentials. Interested in the current situation of mini-app security mechanism usage and how the misuse and misconfiguration of add-on security mechanisms can undermine the framework security, in this paper, we focus on the security mechanisms that involves both built-in and add-on features, and provide a detailed analysis of these add-on security mechanism usage in the current mini-app ecosystem.


%\subsection{Root Cause}
% \begin{figure*}
%     \centering
%     \includegraphics[width=.8\linewidth]{image/example.pdf}
%     \caption{An example of session key leakage impact}
%     \label{}
% \end{figure*}
% In the wechat mini-app framework, the built-in mechanisms can be summarized into the following two mechanisms:
% \begin{itemize}
%     \item \paragraph{Non-interactive mechanism} These mechanisms are non-configurable and transparent to the developers: the developers cannot intefere or customize the mechanisms. The storage and plugin isolation and domain
%     \item \paragraph{Interactive mechanism}
% \end{itemize}
% The built-in security mechanisms of wechat mini-app includes isolation, lifecycle handling, whitelists, blacklists, permission authorization, and data encryption.
% \paragraph{Usability or security, that is a question} 




==> paper/03_study_overview.tex <==



\section{Possible Attacks Analysis and Scope}
\label{sec:analysis}

%\input{table/attack-tbl}


Having presented the background of how various cryptographic keys (\autoref{tab:symbols}) are used to access the sensitive data, we then describe the possible attacks when the assumptions made by \wechat are violated. In particular, we discuss the possible attacks  with and without leaking the \appsecret (\S\ref{subsec:possibleattacks}). Afterwards, we discuss the scope of this work (\S\ref{subsec:scope}).  \looseness=-1

\subsection{Possible Attacks}
\label{subsec:possibleattacks}

%Since the front-end (including the front-end of mini-program and \wechat client) is not trusted and can be vulnerable to various attacks, we present the security analysis of the \wechat sever and the back-end of the mini-program. Particularly, we analyze under the current design of sensitive data access protocol, what type of attacks \wechat server and the back-end of a mini-program may be subject to. To this end, we analyze the usages of the three types of keys as shown in \autoref{tab:symbols}, and understand their design purposes. Specifically, we present the attacks in different cases by assuming the attacker can obtain some or all of the keys, as shown in \autoref{tab:attackspossible}:  
%Basically, both \appsecret and \token is used to fetch the \sessionkey, and therefore, they are all used to protect \sessionkey to be leaked or abused.


\paragraph{(I) With the Leak of Master Key (\appsecret)} Since it is completely up to the developers to manage the \appsecret, not all of them will follow \wechat's development guidelines. Consequently, developers can hardcode \appsecret in the mini-programs, allowing them to be reverse engineered. With the leaked \appsecret, attackers can 
%
%We then assume that an attacker has the leaked \appsecret, and in such a case, the attacker can always manipulate his or her own data, since the attacker can always obtain the cipher of the his sensitive data, and can
always obtain the \sessionkey using the leaked \appsecret to encrypt and decrypt the data, thereby breaking both confidentiality and integrity (the details will be discussed next in \ref{sec:attacks}). 
 
\ignore{ 

\noindent\fbox{%
\centering
\vspace{1mm}
    \parbox{0.46\textwidth}{%
    \vspace{1mm}
    \textbf{The attacker uses \appsecret to query \sessionkey, and manipulate predictable  data} 
    \\   \hdashrule[0.5ex]{0.46\textwidth}{1pt}{1pt}
    The attacker can deploy Account Hijack Attacks since the mini-program's back-end uses the predictable  data to retrieve user accounts, and attacker cant decrypt/re-encdrypt the data.   
     \vspace{1mm}
    }%
    \vspace{1mm}
}
 
} 
 
% \begin{enumerate}
%  \item {\bf Manipulating Predictable  Data.}  The predictable  data (\eg, users' phone numbers) can be used as the primary key in the mini-program's back-end to retrieve the user information, and if this data can be manipulated, the attacker mount attacks go beyond the data manipulation (described next).
%  %
%  To be more specific,  since the mini-program's back-end usually needs to maintain a database to keep user's record and this database needs to be indexed, the mini-program back-end could use predictable  data such as the phone number to index each user. With the leaked \appsecret, an attacker is able to obtain his/her \sessionkey, with which he or she is able to manipulate the predictable  data sent to the mini-program back-end server to retrieve the information. As such, by changing the predictable  data (\eg, the phone number) to a victim's, the attacker can retrieve the victim's information, leading to {\it \bf  account hijacking attacks}, particularly if the mini-program back-end does not perform the consistency check between the submitted predictable  data and the corresponding \sessionkey, which is very likely true given the unawareness of our attack at this moment. \looseness=-1
 
%  % all the users indexes (distributed  from \wechat) and their \sessionkey, we found the mini-program back-ends prefer to use the user's phone number to uniquely associate a particular user's account. This may be because the user usually has one phone number, but the user usually has more than one \wechat accounts. This practice indeed gives the chance for the attackers to hijack the user's mini-program accounts: the attacker can first obtain his own the encrypted data, and then decrypt the data to inspect the format of the message transferred between the back-end and the \wechat server, and final modify his own data to someone else's to trick the back-end of the mini-program into believing the session is created from the victim instead of the attacker. 
 
%  \item {\bf Manipulating Non-Predictable Data.} Unlike predictable data manipulation with which attackers can advantage of accessing other user's account if the data is used to index users, unpredictable data manipulation allows attacker to change his or her own data, thereby with limited impact. For instance, 
%   %The non-predictable data cannot be used by third-party mini-program servers to retrieve user's data, and therefore, the attacker can only manipulate his or her own data, which breaks the data integrity. For example, 
%  the attacker can change his or her own daily step counts to whatever value to cheat the mini-program server to earn some benefits such as rewards or coupons. However, when deployed with malware and populated to large amount of users, such {\bf data manipulation attack} can still be devastating to the mini-program developers, and also the victim's users. For instance, attackers can decrypt each individual's data, change it (e.g., changing a victim's shipping address to attacker's), and collect it using the installed malware.
 
%  %the server and earn the some benefits.  Moreover, if we assume that the attacker has the capabilities of tricking the a victim into installing f malware, the attacker can further break the  data integrity of the victim by manipulating the data sent from the victim mobile device with the malware installed. Therefore, this attack can also be used to collect the user's sensitive information.  
% \end{enumerate} 
 
 
 
 
%\paragraph{(1) Account Hijack Attacks} The predictable  data (\eg users' phone numbers)  can be used as the primary keys in the mini-program's back-end to retrieve the user information, and if the data can be manipulated, the attacker mount attacks go beyond the data manipulation. To be more specific,  although the mini-program's back-end usually maintains a database which records all the users indexes (distributed  from \wechat) and their \sessionkey, we found the mini-program back-ends prefer to use the user's phone number to uniquely associate a particular user's account. This may be because the user usually has one phone number, but the user usually has more than one \wechat accounts. This practice indeed gives the chance for the attackers to hijack the user's mini-program accounts: the attacker can first obtain his own the encrypted data, and then decrypt the data to inspect the format of the message transferred between the back-end and the \wechat server, and final modify his own data to someone else's to trick the back-end of the mini-program into believing the session is created from the victim instead of the attacker. 

\ignore{

\noindent\fbox{%
\centering
\vspace{1mm}
    \parbox{0.46\textwidth}{%
    \vspace{1mm}
    \textbf{The attacker uses \appsecret to query \sessionkey, and manipulate non-predictable  data } 
    \\   \hdashrule[0.5ex]{0.46\textwidth}{1pt}{1pt}
    The attacker can deploy data manipulation attacks since the  attacker can decrypt/re-encdrypt the data.   
     \vspace{1mm}
    }%
    \vspace{1mm}
}
 
%\wechat server will distribute a unique ID that is associated with a particular \wechat account to the mini-program's back-end for the  mini-program's back-end to easily map the user \sessionkey and , when the user log  
}


 

% \paragraph{(2) Attacks against Non-Predictable  Data} The non-predictable  data cannot be used by third-party servers to retrieve user, and therefore, the attacker can  only manipulate his or her own data, which breaks the data integrity. For example, the attacker can change his or her own daily step counts to whatever value to trick the server and earn the some benefits.  Moreover, if we assume that the attacker has the capabilities of tricking the a victim into installing f malware, the attacker can further break the  data integrity of the victim by manipulating the data sent from the victim mobile device with the malware installed. Therefore, this attack can also be used to collect the user's sensitive information.  
  




\paragraph{(II) Without Master Key (\appsecret)} Developers could be cautious about the \appsecret leakage, and there is no leak at all. Then, the attacker cannot use the \appsecret to retrieve his or her own \sessionkey, and what attacker intercepts is only the cipher-text of sensitive data sent by \wechat servers, and this cipher-text will be delivered to the mini-program back-end (through SSL/TLS). With only the cipher-text, attacker can only launch the replay attack. However, \wechat will refresh the \sessionkey very often. % (it expires within 2 minutes according to our experiment). 
Therefore, it will be hard for attacker to launch the replay attack.
However, it could still be possible that careless mini-program developers can accidentally send the \sessionkey obtained at the mini-program back-end to the mini-program front-end. If attackers obtain this \sessionkey, again, the attacker can launch the multiple attacks to break integrity and data confidentiality (which is similar to the case where \appsecret gets leaked), although this attack can last for a very short-period of time in a particular session and the attacker has to keep refreshing \sessionkey from the mini-program servers.

\subsection{Scope}
\label{subsec:scope}
 
While there are multiple attacks against the \wechat ecosystem and \wechat has introduced both encryption with the corresponding protocols and access control mechanisms to protect the sensitive data, we focus on the network communication of encrypted sensitive user data obtained from super app and sent to mini-program vendor back-ends,
% in this work we focus exclusively on understanding the protection with the cryptographic protocols, 
since the super app access control mechanism has been studied by Lu et al.~\cite{lu2020demystifying}. In this work, we do not aim at attacking data that are customized and encrypted by mini-program vendor themselves in that they are not super app user specific, neither do we aim at sabotaging the mini-program vendor back-ends rendering unable to provide service. % While there are multiple super apps that followed the similar protocols to share their sensitive data (e.g., \textsf{Baidu}, \textsf{QQ}), in this work, we particularly focus on \wechat given its popularity. \looseness=-1 

%We first assume that an attacker does not have a leaked \appsecret. In this case, the only key he or she can obtain is \token, which is distributed to front-end. Meanwhile, the attacker can also obtain the cipher of his or her own sensitive data, since the transmission of cipher always involve the untrusted mini-program's front-end. We now discuss the predictability of attacks as follows: 

\ignore{

\noindent\fbox{%
\centering
\vspace{1mm}
    \parbox{0.46\textwidth}{%
    \vspace{1mm}
    \textbf{Attacker only has Login Token (\token) } 
    \\   \hdashrule[0.5ex]{0.46\textwidth}{1pt}{1pt}
    The attacker may deploy cross-user access attacks by enumerating the token. However, this is not feasible due to \token is immune to brute force.
     \vspace{1mm}
    }%
    \vspace{1mm}
}

}



%\paragraph{(3) Cross-user Access Attacks} The login token \token is used to ensure the user to only obtain his or her own data, but not someone else's. To be more specific, every time the user attempts to access his or her data, the user first requires the \token from the \wechat server, and \wechat server then associates the user with a newly generated \token, and returns the \token to the user. That is, in the underlying implementation of \wechat, the \token is used by \wechat to uniquely map a particular user to his or her own data and \sessionkey. In this case, if an attacker (\eg, a malicious user or a malicious mini-program's back-end) intends to access the other users' sensitive data (\ie, unauthorized data access), the attacker has to obtain the \token belongs to the user. However, since \token is a 128 bits long value, and gets expired after 5 minuets, it would be impossible for the attackers to achieve so.  In such a way, \wechat protect its data to be crawled by the attacker arbitrarily.    

\ignore{

\noindent\fbox{%
\centering
\vspace{1mm}
    \parbox{0.46\textwidth}{%
    \vspace{1mm}
    \textbf{Attacker without Encryption Key (\sessionkey) } 
    \\   \hdashrule[0.5ex]{0.46\textwidth}{1pt}{1pt}
    The attacker may replay the encrypted data. However, this is not feasible, due to the use of Encryption Key (\sessionkey).
     \vspace{1mm}
    }%
    \vspace{1mm}
}

}

%  \paragraph{(4) Replay Attacks} Intuitively, if an attacker obtains some  encrypted data but cannot decrypt the data,  the attacker can choose to replay the encrypted data, and observe how the server respond. If this attack can be applied to \wechat, the attacker can then have a chance to manipulate the data records maintained by back-end of the mini-program. For example, the attacker (\eg, a malicious user) can keep a high daily step counts that he or she reached one day, and replay the encrypted step counts everyday to trick the mini-program's back-end into believing the attacker can maintain such high records everyday. However, this is impossible since the Encryption Key (\sessionkey) has a validation period (although such a period is app-specific). The \sessionkey used to encrypt the replayed data can get expired, and if so, the server will obtain a new \sessionkey. In this case, the \sessionkey used to decrypt the replayed data will be different, and the mini-program's back-end will not be able to decrypt the data. Such an attack fails. 

\ignore{

\noindent\fbox{%
\centering
\vspace{1mm}
    \parbox{0.46\textwidth}{%
    \vspace{1mm}
    \textbf{Attacker with leaked Encryption Key (\sessionkey) } 
    \\   \hdashrule[0.5ex]{0.46\textwidth}{1pt}{1pt}
    The attacker can deploy  Account Hijack attacks and data manipulation attacks using the leaked \sessionkey.
     \vspace{1mm}
    }%
    \vspace{1mm}
}

 }
 
 
%\paragraph{Account Hijack and Data Manipulation using \sessionkey} Although \sessionkey is not fixed and cannot be hard-coded in the mini-program's front-end, we interestingly found some developers may mistakenly implement a interface that is used to query the \sessionkey from the backend,  resulting in the leakage of the \sessionkey. Since the attacks that caused by the \sessionkey leakage are the same as the attacks caused by the \appsecret leakage. We will explain the two types of attacks in the following.   
 
%\paragraph{\ding{183} Replay Attacks} Intuitively, if an attacker obtains some  encrypted data but cannot decrypt the data,  the attacker can choose to replay the encrypted data, and observe how the server respond. If this attack can be applied to \wechat, the attacker can then have a chance to manipulate the data records maintained by back-end of the mini-program. For example, the attacker (\eg, a malicious user) can keep a high daily step counts that he or she reached one day, and replay the encrypted step counts everyday to trick the mini-program's back-end into believing the attacker can maintain such high records everyday. However, this is impossible since the Encryption Key (\sessionkey) has a validation period (although such a period is app-specific). The \sessionkey used to encrypt the replayed data can get expired, and if so, the server will obtain a new \sessionkey. In this case, the \sessionkey used to decrypt the replayed data will be different, and the mini-program's back-end will not be able to decrypt the data. Such an attack fails.  

\section{Attacks when with a leaked \appsecret}
\label{sec:attacks}


As discussed in the \S\ref{sec:analysis}, the \appsecret is a critical part in mini-program communication and if it is leaked, the attacker can manipulate the sensitive data arbitrarily, causing various attacks. However, given the significance of \appsecret, our preliminary investigation revealed that the super app dev tool as well as the market does not enforce checking of \appsecret leakage as our test app is still able to be uploaded to the market when we place the \appsecret directly in our front-end code package. Since the official website indicates that the online developer dashboard does not save the \appsecret generated for each mini-program, and it is the developers' responsibility to keep the \appsecret well, it is highly likely that the \appsecret exist in the front-end during development where developers forget to remove them during publishing. 

Motivated by the observation, in this section, we present possible attacks to explore the impacts and the consequences of \appsecret leakage. At a high level, we first discuss the threat model (\S\ref{subsec:threatmodel}) to outline  the assumptions we have made in the work,  followed by attack workflow (\S\ref{subsec:attackworkflow}), which explain how an attacker exploit a miniapp when its \appsecret gets leaked,  and finally the consequences of the attacks (\S\ref{subsec:attackvariations}), where we demonstrate the how the attacker can weaponize the attacks to manipulate the sensitive data for fun and profit.

% As evidenced by our investigation that \appsecret is possible to be leaked, in this section we would like to discuss the threat model, attack procedure, and categorization of the variations of the attack that can be utilized by attacker if mini-programs leak their \appsecret{s}. In the end of this section, we raise two research questions to be answered in the following sections to measure and exploit the leakage problem.
 
 \begin{figure}
    \centering
    
     \includegraphics[width=0.9\linewidth]{image/attack356.pdf}
    \caption{Attack workflow}
    \label{fig:attack}
    
\end{figure}


\subsection{Threat Model}
\label{subsec:threatmodel}

\paragraph{Threat Model} In the communication protocol between mini-programs and super app, there are mainly three parties: the vendor, the user, and the super app. The super app executes mini-program front-end, delivers encrypted sensitive data, and provides back-end for mini-program back-ends to query for \sessionkey. The vendor refers to the developer of mini-programs that has at least a front-end which resides in the user's super app, and a back-end server for receiving data sent from the mini-program front-end. Then, the user uses the mini-program and grants permissions for mini-programs to access the sensitive data. \looseness=-1

As such, in our threat model, an attacker acts as a mini-program user. If a \appsecret is leaked, the object of the attacker is to obtain the victim user's sensitive information from  the corresponding vulnerable mini-program server, or intentionally modify and inject fake data of a particular user into the server. To this end, we assume that the attacker can access and unpack the front-end mini-program package and can capture the network packet of a controlled device. Such a controlled device can be the attacker's device or a user's device, and if it is the user's device, the attacker may need to install a malware to achieve that. Please note that similar assumptions~\cite{lu2020demystifying} were made in previous efforts that work against the mini-programs.  Moreover, we assume that the back-end of the mini-program is secure (e.g., we cannot compromise the back-end of the mini-program by using SQL injection or web shell). 
%In some of our attacks, the attacker may need to install malware onto the user's mobile (similar assumptions~\cite{lu2020demystifying} were made in previous efforts that work against the mini-programs). 
We also assume that the super app as well as its back-end is secure: the attacker cannot interfere with the super app (such as by hooking app API, where the attacker's account gets banned quickly enough to thwart his effort according to our investigation), as well as the super app back-end. \looseness=-1
%\ZY{Here, I think we need to also discuss the whether the back-end of the mini-program is secure? } 



%{\color{purple}How to derive the sabotaging} 

\ignore{
Meanwhile, as outlined in \autoref{tab:attackspossible}, attacks with and without leaking of \appsecret are all possible, we focus on systematically study \appsecret leaks (the first row of \autoref{tab:attackspossible}), understand its prevalence, root-cause, consequences, and meanwhile design countermeasures. We do not aim to detect the vulnerabilities and attacks in the last row of \autoref{tab:attackspossible} (namely on the \sessionkey leakage), since the \sessionkey is dynamically generated and developers can also have very diversified ways of leaking the \sessionkey to the front-end. We leave the study with this attack to future work. \looseness=-1
}
% As discussed in the background section, the \appsecret plays a critical role in the communication between mini-programs and the super app server. If the \appsecret gets leaked, all the sensitive data encrypted by the \sessionkey generated with \appsecret and user's login token will be obtained by the attacker, and thus the encrypted data can be easily decrypted or even be manipulated arbitrarily, causing various security problems. As such, in this section, we first discuss the threat model in which the parties involved with the communication between front-ends and back-ends of mini-programs are identified. Then, we provide a systematic categorization of attack variations that may be generated due to the \appsecret leakage of mini-programs.

\subsection{The Attack Workflow}
\label{subsec:attackworkflow}

Since the attacker in our threat model can obtain the mini-program front-end and control the network packets sent from a controlled device, the attacker can unpack the mini-program and identify how to trigger the sensitive data communication to retrieve or manipulate the data. As such, the attack workflow consists of two main steps after the attacker unpacks the mini-program front-end package as shown in \autoref{fig:attack}: 

\paragraph{(I) Obtaining Attacker's Encryption Key (\sessionkey)} To start the attack, assume an attacker ${Eve}$, he needs to first get his own \token, denoted  {\tt LT}$_{eve}$, 
from the \wechat server (\textbf{Step \ding{182}}). Next, he provides the leaked \appsecret, the mini-program ID (easily obtained in the meta-data of a mini-program), and {\tt LT}$_{eve}$ to the \wechat server (\textbf{Step \ding{183}}). Since \appsecret,  {\tt appID}, and {\tt LT}$_{eve}$ are all valid, the \wechat server will send his \sessionkey (\ie, {\tt EK}$_{eve}$) as what it does typically for the mini-program's back-end to ${Eve}$. Note that prior to this login, the server might already have a copy of {\tt EK}$_{eve}$ if $Eve$ has logged in before the mini-program server. Also, if \wechat server has refreshed the {\tt EK}$_{eve}$,  ${Eve}$ will get a new one, and the mini-program back-end will detect the {\tt EK} change as well  (at \textbf{Step \ding{187}}) and request for this new {\tt EK}$_{eve}$ from the \wechat server by asking $Eve$ to provide his $LT_{eve}$ again (details are omitted here for brevity). Therefore, it does not matter whether the mini-program server has a copy of {\tt EK}$_{eve}$ or not. \looseness=-1

\paragraph{(II) User Sensitive Data Retrieval and/or Manipulation} In this stage, the attacker ${Eve}$ first initiates a sensitive data query request (\eg, \texttt{getPhonenumber}), and requires the \wechat client to get his or her own data (\textbf{Step \ding{184}}). The \wechat client then sends the request to its server. \wechat sever then retrieves the data, encrypts the requested data (\eg, $Eve$'s Phone number $D_{eve}$) (\textbf{Step \ding{185}}), and finally returns the cipher (\ie, $D_{eve}^\prime$) back to the attacker ${Eve}$. At this point, the attacker could drop the cipher and  
then intentionally fabricates fake data. However, since the attacker does not know the format of the data transferred,  the attacker has to first decrypt the cipher to inspect the packets format, and then create the fake data (\textbf{Step \ding{186}}). However, if attackers already know the format of the to-be-manipulated data, {\bf Step \ding{184}-\ding{186}} can be omitted. Next, the attacker then manipulates the data, and re-encrypts the fake data using the same \sessionkey (\textbf{Step \ding{187}}).
%For example, ${Eve}$ can change his phone number to Alice's (\ie, $D_{Alice}$). Since mini-program's backend have the same \sessionkey as the attacker, it can decrypt the cipher and obtains the modified data (\ie, phone number $D_{Alice}$) (\textbf{Step \ding{188}}). If there is no consistency check between the phone number and the \sessionkey (likely true at this moment), the attacker can break into Alice's account.

\subsection{The Attack Consequences}
\label{subsec:attackvariations}

{In the threat model, we have discussed the two potential attack targets, the mini-program users and the mini-program vendors, that may be attacked if \appsecret is leaked. We also discussed that the goal of attack is to obtain the \sessionkey to retrieve of manipulate the sensitive data sent between mini-program front-end and back-ends. As such, in this section, we systematically categorize the attack variations with respect to the attack targets and attack goals. 
As shown in \cref{tab:attack_cat}, the attack target is either the users or vendors. As to the attack goal, we use the CVSS 3.1 scoring system~\cite{CVSS} that is widely used in industry and academia, which contains three types of attack impact: confidentiality, integrity, and availability. However, as we discussed in the attack scope that we do not aim at sabotaging the mini-program back-ends, the availability is not our attack goal and is thus out of scope. Meanwhile, since we focus on super app specific sensitive data, the confidentiality attack against vendor is out of scope too because they are customized by mini-program vendors instead of super app. As such, there are three types of variations of attack:}\looseness=-1

% we focus on the sensitive data of users in super app. As such, the confidentiality of data from vendor is out of our scope, and the attack goal of availability attack.

% As discussed in the Background section, the \appsecret is used to encrypt sensitive information related to the super app. These sensitive info are automatically encrypted by the super app to prevent malicious attacker from eavesdropping them. As such, the leakage of the encryption key \appsecret will void the security mechanism of the super app, causing a series of security problems. As such, in this part, we categorize and evaluate the potential impacts due to \appsecret leakage according to the goal and the target of the attack. The attack goal, refers to the desired impact the attacker aim to cause. According to the CVSS 3.1 scoring system~\cite{CVSS} which is widely adopted by industry and academia, the attack impact is categorized into confidentiality, integrity, and availability. Since our work does not aim to attack the vendors' back-end servers rendering them unavailable, we only focus on the former two categories. The attack target, as discussed in the threat model section, are either the victim user or the mini-program vendors in this paradigm. However, since all the sensitive data are related to the mini-program users themselves, when launching confidentiality attacks, non-mini-program encrypted data generated by vendors are out of our scope
% As such, the potential attack variations of attack are shown in \cref{tab:attack_cat}:
\paragraph{(I) Integrity Attack Against Users for Arbitrary Log In}
The integrity attack of sensitive data against users we identified is related to the predictable type of sensitive data mini-programs use as account identifier, e.g., the phone number. In mini-programs, the predictable data (\eg users' phone numbers) is widely used to provide quick registration service to new users in that the user only needs to click on a button and approve the usage of their phone number. Moreover, large vendors that have their own database also use this feature to link the mini-program user to their account information from other consoles (\eg Android apps and iOS apps) since the phone number are tied to super app account. 

However, with the leaked \appsecret, an attacker can obtain the \appsecret to manipulate the predictable data, making the attacker able to login to other users' account to perform malicious behaviors. For instance, he or she can use the discount offers or even free offers given to high-value customers, especially for some hotels or markets that give high-value customers large discounts. The attacker may be able to redeem for a free night for a luxury hotel if the victim has such offer in his or her account. While these attacks can be targeted (i.e., the attacker knows the phone numbers of the victim user before launching the attacks), it is also possible that an attacker can enumerate the phone number to launch the attack at scale. What makes it even worse is that the limited enumeration space of these predictable data that make the attack easier.
% the attacker may be able to get the sensitive information of victim's address, identity information such as name and ID, and order information that may contain home address. Besides, financial losses may be caused to the user or vendor if the attacker uses discount offers given to the victims (especially when some hotels and shops give high-value users large discounts or even free offers). The privacy leakage may also be conbined with other
For example, the 10-digit phone number consists of 3-digit area code, 3-digit central office code, and 4 digits of another enumerable code. As such, the enumeration space of phone number is quite small. \looseness=-1
% Meanwhile, since there are a log of real-world contact phone numbers that can be fetched elsewhere on shops, offices, and websites, it is even easier for attackers to pick up phone numbers of their interest. Similarly, the phone number can also be directly obtained via confidentiality attack if the victim has a malware monitoring network traffic as discussed.


% \paragraph{Integrity attack against vendor: arbitrary log in}
% The integrity attack against vendor is mostly related to predictable data. In mini-programs, the predictable data (\eg users' phone numbers) is widely used to provide quick registration service to new users in that the user only needs to click on a button and approve the usage of their phone number. Moreover, large vendors that have their own database also use this feature to link the mini-program user to their account information from other consoles (\eg Android apps and iOS apps) since the phone number are tied to super app account. However, with the leaked \appsecret, an attacker can obtain the \appsecret to manipulate the predictable data, making the attacker able to login to other users' account. After the attacker modifies the logged in phone number with \appsecret, he/she can launch various attacks. For instance, he/she can use the discount offers or even free offers given to high-value customers, especially for some hotels or markets that give high-value customers large discounts. For instance, an attacker may be able to redeem for a free night for a luxury hotel if the victim has such offer in his/her account. The problem of predictable data integrity attack is concerning in that these data are much more easily enumerated. For example, the 10-digit phone number consists of 3-digit area code, 3-digit central office code, and 4 digits of another enumerable code. As such, the enumeration space of phone number is quite small. Meanwhile, since there are a log of real-world contact phone numbers that can be fetched elsewhere on shops, offices, and websites, it is even easier for attackers to pick up phone numbers of their interest. Similarly, the phone number can also be directly obtained via confidentiality attack if the victim has a malware monitoring network traffic as discussed.

\paragraph{(II) Integrity Attacks Against Vendors for Cashback-for-Free}
The integrity attack against vendors is mostly related to unpredictable data that can be used to churn the benefits. In the new mini-program paradigm, one of the major difference from traditional e-commerce paradigm is that the social relationships can be used more efficiently to promote the providers' services. Residing in the social super apps, mini-program vendors seek to exploit the benefits of access to user social relationship such as friends and groups by attracting users to use their service with gifts and urging them to share the mini-program to groupchats, or even directly giving users money for their sharing behavior. As such, mini-programs may give users benefits (e.g., cashback, coupons) if the user help them promote their service to their own social relations (e.g., groupchats). A mini-program may directly give users benefits immediately after a user shares the mini-program to groupchat (where the groupchat ID can be found with share info), or attract users to play some game (such as achieving certain amount of walking with werun data) and then redeem the benefit after sharing the mini-program. However, if the encrypted werun data or share info from super app is manipulated by attackers, these benefits or even red packet money can be easily churned at a large scale. \looseness=-1

% As such, there are mainly two ways for users to get cashback with their social relationships. One is direct approach in which the mini-program directly gives a certain amount of money for each group the user shares to, using the share info data and group enter info data that returns the groupchat ID a user shares the app to or enters the mini-program from. The other is indirect approach in which the mini-program let user participate a certain event, such as using WeRun data to give gifts to users achieving 8000 steps of sports a day in a week), and letting users to share the mini-program to redeem the benefit.

% However, since the \appsecret may be leaked to the front-end, the encrypted could be modified. This may introduce financial losses to mini-program vendors in that the users may be using this feature to cheat. For instance, a user can repeatedly share the mini-program to a same group whereas changing the group ID in the network packet each time to abuse the sharing-for-money system, and an attacker can also abuse the werun data to quickly churn benefits across a large amount of similar mini-programs for free gifts.

\paragraph{(III) Confidentiality Attack against Users for Information Stealing} The leaked \appsecret may allow attackers to eavesdrop the encrypted sensitive data sent to mini-program back-end provided that the victim has network packet capturing malware installed on it. The impacts to the privacy leakage may vary according to the type of data leaked to attacker: the predictable data (\eg phone number) is critical to user privacy under mobile computing era because it is not only tied to the user's physical device but also are widely used by mini-programs to perform quick registration or link the user account on other terminals (e.g., iOS apps or Android apps). As such, if the phone number is eavesdropped, there can be a serious problem in that the attacker may use the phone number to perform traditional attacks such as targeted impersonation attack, or further combine with integrity attack to log in to the victim's account to achieve more security impacts. This can be further combined with other types of sensitive data fetched from super app, for instance, attackers may get to know the social relationships of a specific user by eavesdropping the phone number and the group ID the user shares to or enters mini-program from. Moreover, by knowing the \textsf{WeRun} data (i.e., the daily steps), the attacker can further infer the user's status on a specific date. For example, if the daily step is a few, the user is likely to be at home (the home address is also one type of the sensitive data). \looseness=-1

% \paragraph{Confidentiality attack against unpredictable data: replay attack}\AY{Even if the attacker does not attack another victim, it is still possible for attackers to attack mini-program vendors just by reading the con}


\begin{table}[]
    \centering
    \begin{tabular}{r|l|l}
    \toprule
    Impact/Target & User & Vendor\\ \midrule
    Integrity & Var. I Arbitrary Log-in& Var. II Cashback-for-free\\
    Confidentiality& Var. III Privacy Leakage & Out-of-scope \\
 \bottomrule
    \end{tabular}
    \caption{Summary of Attacks Powered by \appsecret Leakage}
    \label{tab:attack_cat}
\end{table}


% As such, we arrange the following sections of the paper by first quantifying how ubiquitous is the \appsecret leakage among over 3.6 million mini-programs we collected, and then with a detailed discussion about the attacks and their variations against such a vulnerability. In the end, we provide case studies to show the real-world impact, as well as a discussion section to analyze the potential reason and countermeasures of the \appsecret leakage problem.


==> paper/03_threat.tex <==

\subsection{Assumptions and Scope}
 
In this paper, we mainly describe the security issues caused by the design shortcomings of the mini-app APIs and mechanisms. Therefore, for a specific vulnerable platform (e.g.,\wechat, \alipay), since all the mini-apps are programmed using the same APIs provided by the host app, all mini-apps that use the referred API or mechanism are subject to the attacks introduced in our paper. All the attacks are validated on our own mini-app, and we did not deploy any attacks against mini-apps from other vendors for ethics concerns. 
 

The attackers, whose goal is to break the enforced isolation mechanism or access the sensitive data (e.g., system resources, user private information), can be group into two categories: ($i$) a outsider attacker without his malicious mini-app hosted, using on the shortcomings to deploy attacks against the mini-apps remotely (e.g., unauthorized access via Bluetooth) and ($ii$) a insider attacker with his malicious mini-app hosted on the victim host app (or malware installed on the smartphone), leveraging the design shortcomings to break the isolation and collect data.  


 
\subsection{Hardware Management}

\subsubsection{Observation and Root Causes} The mini-apps are designed to run on multiple platforms including iOS and Android. However, different platforms may have different security requirements and security polices, and the designer must handle the platforms' inconsistency. When that happens, we found that the designer usually trades off the security for compatibility. For example, Bluetooth pairing is the key negotiation process for two Bluetooth devices to achieve communication confidentiality and authentication. iOS devices adopt the passive pairing policy, which is less secure. While Android uses the active pairing for stronger security. We found the in-app APIs regarding Bluetooth pairing trend to implement the passive pairing for compatibility, downgrading the security policy of Android devices.  
 


\subsubsection{Absence of Secure Peripheral Management}  

Peripherals such as keyboards and mouses provide features to facilitate system use. While the functionalities of the peripherals to extend is countless, the methods for a peripheral to connect with a OS is limited, such as the Universal Serial Bus (USB) for wired connection, and Bluetooth for wireless connection. Compared with USB, which is subject to various limitations (requiring a wire to connect; less mobility), Bluetooth is more ubiquitous. Especially, the Low energy version, which is called Bluetooth Low Energy (BLE), has became the widely used standard for connecting peripherals. Consequently, being a OS-like entity for mini-apps, the host app implements and offers interfaces for mini-app to support various Bluetooth peripherals.


To be more specific, Bluetooth peripherals rely on pairing process for connecting the mini-app securely, where the smartphone running the mini-app and the BLE peripheral negotiate a common cryptographic key for securing the later communication. During the pairing process, the two devices first exchanges pairing features  (e.g., having a display or a keyboard), then use the exchanged features to determine an appropriate pairing method, complete the authentication process, and ultimately derive the key. Note that, the key is transparent to the upper layer apps including the host app and mini-apps. As long as the key is in position, the traffic is encrypted by the underlying OS. 
 
%The host app is responsible for managing the Bluetooth peripherals securely. 
 
%Specifically, to demonstrate the outsider attacking scenario, we use Bluetooth Low Energy (BLE) as an exemplary example. BLE has been widely used in many IoT applications such as home entertainment, health care and retail. To communicate with each other, the peripheral device (e.g., Bluetooth blood pressure monitor) provides services, and a central device (e.g., smartphone) can send a read or write request to access those services. The capabilities of being a central or a peripheral depends on implementation. For example, the smartphone can also work a peripheral if a peripheral app is installed and running on the smartphone. 
 

\textbf{Pitfall \#1: No Active Pairing Policy.} Since pairing is an advanced feature, which is not enabled by default. The approach for an native app to initiate the pairing process is implement differently across the system. According to \textsf{Accessory Design Guidelines for Apple Devices} \cite{Appleguidelines}, iOS devices adopt the passive pairing policy, where the apps running on a iPhone passively wait for feedback from the peripheral to determine whether or not to initiate the pairing process. If iOS does not receive any pairing attempts (e.g., an error code indicating the communication need to be encrypted) from the peripheral, the pairing process will not be initiated and the communication continues in plain-text. As a result, iOS does not provide any APIs for pairing.   Different from iOS, Android devices adopt an active pairing policy for stronger security, where an app running on Android smartphone can actively invoke the pairing process by calling the method \texttt{createBond()}. 

The inconsistency between Android devices and iOS regarding the pairing process confuses the designer of mini-apps, and as a result, among all the investigated mini-app platforms, only \wechat provided the \textsf{wx.makeBluetoothPair(.)} (and the API only works on an Android device), other platforms such as \alipay trends to follow iOS's practice for compatibility.


\textbf{Pitfall \#2: No API to Access Pairing Results.}
Pairing may fail due to various reasons (e.g., the user cancels the pairing process), and it is important for apps (or mini-apps) to know whether the pairing has been successfully processed. 
For example, apps and their peripheral may exchange sensitive information, and the data transmission should occur when the link is encrypted. 


%multiple outcomes can be resulted in such as pairing failed, pairing succeeded with a high security level (i.e., security level 2) or pairing succeeded with a low security level (i.e., security level 1)

%When the peripheral and the devices running the mini-app finish the pairing process,

Since pairing is a time consuming process which may involve the user's interactions (e.g., inputting the \textsf{PIN}), it may be not possible for apps to know the pairing result immediately. As a result, Android provides multiple asynchronous approaches for an app to know the pairing results before data transmission.  ($i$) An Android app can invoke \texttt{getBondState()} to know the pairing status including pairing in progress (\texttt{BOND\_BONDING}), pairing succeeded (\texttt{BOND\_BONDED}) or pairing failure (\texttt{BOND\_NONE}). ($ii$) An Android app can register intents \texttt{ACTION\_BOND\_STATE\_CHANGED} and
\texttt{ACTION\_PAIRING\_REQUEST} to get notified when pairing process is completed. As comparison, iOS, unfortunately, does not provide any approaches for an app to know the pairing results. Again, the mini-apps platforms such as \alipay followed the iOS practice and no platforms currently support an approach for the mini-app to know the pairing result before the data transmission. 
 
%For example, when two pairing devices use \textsf{Passkey Entry}, OS delivers the app a intent with a message \texttt{PAIRING\_VARIANT\_PIN}, and the pairing method \textsf{Passkey Entry} satisfies the security level 2. 



%Recall that \wechat provides an API \texttt{makeBluetoothPair(.)} to actively start pairing. However, according to our experiment, the API fails to notify the mini-apps of the pairing results. In particular, the method only allow mini-apps to register a callback to monitor if the pairing will begin, which is similar to \texttt{createBond()} of Android. There is no asynchronous framework available for mini-apps to get notified when the pairing finishes and whether the two pairing devices are successfully paired.  

%According to Google's official document,  the method returns true if the pairing will begin, and returns false if errors occur. The app can register for \texttt{ACTION\_BOND\_STATE\_CHANGED} intents to know the pairing result. 

%``\textit{If, for security reasons, the accessory requires a bonded relationship with the Central, the Peripheralshould reject the request using the Insufficient Authentication error code, as appropriate. As a result, the device (Apple device) may proceed with the necessary security procedures}''. It can be observed that iOS strictly follow the passive pairing policy, and therefore, no pairing related functions are provided in their official API \cite{CoreBluetooth}. 



%there are two pairing policies for a smartphone to pair with a peripheral \cite{ble5.0}: ($i$) Active policy: the smartphone can actively send a pairing request to the peripheral device, and the two devices enter the pairing process. ($ii$) Although the peripheral cannot initiate the pairing, it can notify the central to start the pairing process. Specifically,  if the peripheral attempts to achieve the secure communication, the peripheral can send an error message (e.g., \texttt{Insufficient\_Encryption}) to notify the central devices to initiate the pairing process. When the central receives the error message, it can respond the peripheral pairing request and then the two devices go through the pairing process. We refer this type of pairing policy passive policy. In the passive policy, if the central does not receive any error codes from the peripheral, the pairing process will not be initiated and the communication continues in plain-text.    
  
\textbf{Attack \# 1: Fake Peripheral Attacks.} We now demonstrate how to exploit the two design shortcomings to deploy fake peripheral attacks against mini-app. As shown in \autoref{fig:bleattack}, before our attacks, we assume that the victim peripheral paired with the a victim smartphone, where the victim mini-app is hosted. The Bluetooth traffic is supposed to be encrypted each time of the communication. 

The attacker is in the range of the two communicating devices and wait for a moment where the central and the peripheral get disconnected, but they intend to initiate new session. For example, a Bluetooth smart light user enters his home, launches the corresponding mini-app and the mini-app starts to scan the devices around. Such a moment can be easily identified, since the BLE is a wireless communication technology, and all the traffic such as the scanning requests goes in plain-text over the air and sniffable before the connection is established. 

\begin{figure}  
\centering
\includegraphics[width=0.7\columnwidth]{image/bleattack.pdf}\\
%\vspace{-2mm}
\caption{Fake peripheral attack against the mini-apps} 
%\vspace{-3mm}
\label{fig:bleattack}
\end{figure}

\begin{enumerate}
\item The attacker collects the identifier of the victim peripheral (i.e., Bluetooth MAC address), which goes over the air, and impersonates as the victim peripheral to establish a connection with the victim smartphone (Step \ding{182}). In the regular case, one smartphone is supposed to connect only one peripheral at a time, and consequently, the smartphone is currently not available for the victim peripheral. 
\item The mini-app on the smartphone is launched and the victim smartphone attempts to start encryption using the key that is negotiated with the victim peripheral  (Step \ding{183}). 
\item The attacker does not have the key for encryption, and therefore, responds the victim central a \texttt{PIN\_OR\_KEY\_MISSING} error (Step \ding{184}).  This is a widely used trick to attack against Bluetooth devices \cite{bledowngrade20,Blesa20}. 
\item According to the current practice, Android OS will delete the key when receives the error code (Step \ding{185}). At this point, if there is no attacker present, either the peripheral or the central is supposed to initiate the pairing process for communication security. However, the peripheral currently is the attacker that will not start pairing, and for mini-app platforms such as \alipay, they do not provide APIs for the victim mini-app to start the pairing either. As a result, the communication continues in plaintext (Shortcoming \#1). Meanwhile, there is no way for mini-app to know whether the link is secure (Shortcoming \#2).  
%\item For mini-app platform such as \wechat, which provides the active pairing policy, the mini-app may actively start the pairing process to go through the pairing (Step \ding{186}). Note that, for mini-apps developed using the API from \alipay, steps \ding{186} and \ding{187} are not needed. 
%\item Attacker can actively cancel the pairing process by sending an error code \texttt{PARING\_NOT\_SUPPORTED}. Since the mini-app does not have an interface to access the pairing result, there is no  

\item The attacker can now send the crafted data to the victim mini-app or receive sensitive information from the mini-app (Step \ding{186}), since the communication requires no authentication. This may cause grave consequences to the mini-apps running on the Android devices. For example, the mini-app can be a client of a Blood pressure monitor, and in that case, the attacker may inject false blood pressure measurement, misguiding the doctors.    
 

% The app is supposed to re-initiate the pairing process and


\end{enumerate}

   
\subsubsection{Insufficient Security Level for Soft-Defined Peripheral} 

Android and iOS also allow the smartphone to work as a peripheral device, which provides services for other devices. For compatibility concerns,  the communication media is also BLE, which is supported by most devices. For example, since Android 4.3 (API level 18), Android have introduced the built-in support for apps to become a BLE peripheral. The applications of the feature can be multiple, and one exemplary application is to allow the smartphone to become the Bluetooth Human Input Devices (e.g., a mouse or a keyboard), where a user can pair his smartphone with a Bluetooth-enabled devices such as a smart TV to use the smartphone as a mouse or keyboard to control the connected devices. 
  
In particular, when the smartphone works as a peripheral,  it can require a minimal security level (also known as permission), which specifies how services on the peripheral can be accessed. When the security level of the link status is less than the required security level, the data access should be rejected by the device. The security levels are determined by the pairing method, as shown in \autoref{tab:seclevel}. This is because in some of the pairing methods, an out of band channel or a user is involved, and such a engagement improves the security of the pairing process. For example, in the \textsf{Passkey Entry}, a user is required to approve the pairing request by inputting the displayed \textsf{PIN}, and such a interaction assists the pairing devices to complete the authenticate process. Therefore, pairing method such as \textsf{Passkey Entry} or \textsf{Numeric Comparison} can defend against Man-in-the-Middle (MitM) attacks or unauthorized data access.  Alternatively,  \textsf{Just Works} does not require either the approval from a user or a trust out of band channel to be involved, and it is subject to various Bluetooth attacks. 

%For example, when the smartphone works as a mission critical application such as a BLE keyboard, the soft-defined keyboard can enforce the highest security level (i.e., level 3) for the keystroke data to be transferred over the air, and reject the access request when the security level of the pairing method is not suffice. 


%Recall that in the pairing process, the two devices determine an appropriate pairing method based on the available pairing features (e.g., keyboard and display) of the pairing devices. 

\begin{table}[h]
\resizebox{1\columnwidth}{!}
{
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Pairing Methods}          & \textbf{Required Features}              & \textbf{Security Levels \cite{5.0}}    \\ \midrule
\textsf{Plaintext}          & No requirements                                    & 1                \\
\textsf{Just Works}         & No requirements                                      & 2                  \\
\textsf{Passkey Entry}      & Display and Keyboard                    & 3 \\
\textsf{Numeric Comparison} & Display and Keyboard (or Yes/No button) & 3 \\
\textsf{Out of Band}        & Out of Band Channel                     & 2 or 3 $\dagger$ \\ \bottomrule
\end{tabular}
}
\caption{Pairing method and security levels. The greater the number is, the more secure of the security level is. $\dagger$: The security level of OOB depends on whether the used out of band channel is secure.    }
\label{tab:seclevel}
\end{table}


\begin{table*}[h]
\resizebox{1.6\columnwidth}{!}
{
\begin{tabular}{@{}lllc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Android} $\dagger$} & \multicolumn{1}{c}{\textbf{iOS}}             & \textbf{Mini-app}      & \textbf{Security Level} \\ \midrule
\textsf{PERMISSION\_READ}                     & \textsf{CBAttributePermissionsReadable}              & \textsf{readable}               & 1                       \\
\textsf{PERMISSION\_WRITE}                    & \textsf{CBAttributePermissionsReadable}               & \textsf{writeable}              & 1                       \\
\textsf{PERMISSION\_READ\_ENCRYPTED}          & \textsf{CBAttributePermissionsReadEncryptionRequired} & \textsf{readEncryptionRequired} & 2                       \\
\textsf{PERMISSION\_WRITE\_ENCRYPTED}         & \textsf{CBAttributePermissionsReadEncryptionRequired} & \textsf{readEncryptionRequired} & 2                       \\
\textsf{PERMISSION\_READ\_ENCRYPTED\_MITM}    & N/A                                          & N/A                    & 3                       \\
\textsf{PERMISSION\_WRITE\_ENCRYPTED\_MITM}   & N/A                                          & N/A                    & 3                       \\ \bottomrule
\end{tabular}
}
\caption{Comparison of the supported security levels across different OS.  $\dagger$: Other than the listed security levels, Android defines security levels that are not in the specification, and those informal security levels are out of our focus.  }
\label{tab:permission}
\end{table*}
 
%The peripheral, which provides data services for the centrals to consume (i.e., read or write), can protect the services at a fine-grained granularity, according to BLE specification \cite{5.0}.
%Other than the regular role (i.e., a central),
 

\textbf{Pitfall \#3: Insufficient Security Level}. Android and iOS implement the security levels differently, as shown in \ref{tab:permission}.  Android provides all the three security levels for apps to customize their services, but iOS, however, only provides two primary security levels for iOS apps, and the strongest security level is not provided. We found the platforms of mini-apps such as \wechat followed the iOS's practice, in which only two security levels are provided. Since the strongest security level is defined to defend unauthorized services access attacks, the absent of the security level 3 will position the mini-apps running on Android devices in the risk of unauthorized services access attacks. 


\textbf{Attack \# 2: Peripheral Data Unauthorized Access Attacks.} In this attack, we assume the a Android phone running a peripheral mini-app, denoted as victim soft-defined peripheral, which defined services that use the highest security level the mini-app may support (i.e., security level 2).  An other device, which attempts to connect the victim soft-defined peripheral, is denoted as the victim central. We assume the attacker is in the range of the two communicating devices, and selects the moment that the two communicating devices intend to communicate. \looseness=-1   

%The attack set up is similar to the spoofing attacks against the mini-app central. Again, we assume the victim central and the victim peripheral (which is a smartphone running the peripheral mini-app) paired before the attack, and The services on the peripheral is in The attack   

First, the attacker pretends to be the victim central and connects to the victim soft-defined peripheral. Then, the attacker initiates a services access request to the peripheral. When receives the request, the peripheral notice that the link is not encrypted, but the services provided require a security level 2. As a result, the peripheral rejects the request using a error code \textsf{INSUFFICIENT\_ENCRYPTION}, which notify the ``central'' (which is the attacker) to start a pairing process. The attacker actively pair with the peripheral using \textsf{Just works}, which does not require the involvement of the user. Since the services only require security level 2 to access, the attacker can access all the services on the peripheral. The attack may result sensitive data leakage against the soft-defined peripheral. For example, the soft-defined peripheral can be a keyboard, which 
  
%Two pairing devices relay on the pairing request and pairing response to exchange the supported pairing features, and select 
  

\subsection{Resource Management and Data Isolation}

   
\subsubsection{Observation and Root Causes}  As discussed in \S\ref{sec:back}, the host app of mini-apps intends to provide a stronger security by aggressively integrating multiple resource isolation mechanisms. For example, a mini-app platform usually implements the network resources isolation, which requires all the network resources to be accessed when 
receives the approvals from the platform. However, to design an isolation mechanism requires significant efforts to understand security issues, and it cannot be easily achieved. Different from the local resources, which is stateful and the OS remembers which app has access to which resources, the network resources requests usually send through the network protocols such as HTTP or HTTPS, which is stateless. It is extremely challenge for the host to trace each request and force the isolation mechanism.  
Another observation is that different mini-apps (or build-in components) may have different isolation levels regarding different resources. However, two mini-apps can build a cross-app channel for communication, which may blur the security boundary of the isolation. 




\subsubsection{Escape of Network Resource Isolation} Recall that the mini-app host enforces the network resources isolation, where the mini-apps can only access the cloud base provided by the host app or the trusted domains vetted by the host app. If the mini-apps attempts to access a domain that are not fall into these two categories, the network request will be rejected the host app server, which server as a gateway, immediately. The network resource isolation is a mandatory for all the mini-apps that are publicly accessible.   

 
 \begin{figure}[h]  
\centering
\includegraphics[width=0.7\columnwidth]{image/remoteattack.pdf}\\
%\vspace{-2mm}
\caption{Escape of network resource isolation} 
%\vspace{-3mm}
\label{fig:escape}
\end{figure}

\textbf{Pitfall \#4: Inconsistency of Network Resource Isolation.} Other than the mini-apps, the host app also integrate multiple build-in components such as the document viewers and basic web bowers (e.g., \wechat integrates 
QQ Browser). Different from the hosted mini-apps, these build-in components are considered trust by default, and they can access all the network resources including these website using HTTP without any changes. However, one mini-app can use the provided interfaces to communicate with those build-in components without require the grant from the user.   




\textbf{Attack \#3: Network Isolation Escape}. In this attack, a malicious mini-app is hosted onto the host app, and its goal is to escape the network isolation, accessing the malicious back-end. As demonstrated in \autoref{fig:escape}, the mini-app is suppose to communicate with the mini-app back end, which is located in the cloud base of the host app,  and the getaway of the host app will reject any network requests other than these sending to the mini-app back-end. 


To go around the mechanism, the mini-app can load a document locally (or download the document from the back-end), which contains a malicious hyperlink. Then the mini-app invokes the API \texttt{openDocument()}, which will open the build-in document viewer for the malicious mini-app. The enter process from downloading the document to opening the document, no user action is required and no prompt is directed to the user. Therefore,  the attack can be deployed stealthily. Meanwhile, since the document viewer does not have restrictions regarding the network resources, it is able to launch the website when a user hit the link.  

To lure a careless user to press the link, the  malicious developer can forage products promotions or some other text descriptions of user's interest close to the link. 
Among all the platforms we have tested, only \wechat can defend against this type of attack. Hyperlinks in the document viewer of \wechat is un-clickable. 
The impact of our attack can be disastrous. There are numerous exploits that can be unitized by just clicking the crafted link. the exploit can be used to install spyware \cite{hackphone1clickwhatsapp}, or even worse, take the full control of the smartphone by remotely executing the malicious code \cite{hackphone1click}.  

 

%The mini-apps are designed to run on multiple platforms including iOS and Android. However, different platforms may have different security requirements and security polices, and the designer must handle the platforms' inconsistency. When that happens, we found that the designer usually trades off the security for compatibility. For example, Bluetooth pairing is the key negotiation process for two Bluetooth devices to achieve communication confidentiality and authentication. iOS devices adopt the passive pairing policy, which is less secure. While Android uses the active pairing for stronger security. We found the in-app APIs regarding Bluetooth pairing trend to implement the passive pairing for compatibility, downgrading the security policy of Android devices.  
 
\subsubsection{Insecure Cross-app Channel} Similar to the Android permission mechanism, the mini-app permissions are requested by a specific mini-app individually. When the user grant the access, the mini-app has the fully access of the system resources unless the user manually revoke the access. A mini-app without user's permission does not have the access to the sensitive resources. However, there is a way for mini-apps to communicate with each other, which blurs the security boundary of the isolation and involves novel threats.     

 \textbf{Pitfall \#5: Privacy Leakage Across Mini-apps}.  The host app allows two mini-apps to communicate with each other, which may leak sensitive data from one app to another. Specifically, if two mini-apps want to exchange data, they can use APIs specified by the host app to build a channel. For example,  as shown in
 \autoref{list:navigate}, in \tik, one mini-app, assumed $mini_{A}$, can launch and deliver messages to 
another mini-app, assumed $mini_{B}$, by initiating the API named \textsf{navigateToMiniProgram(Object msg)}, where the Object is the message the $mini_{A}$ intends to deliver. The message contains the unique identifier of $mini_{B}$ (i.e., \textsf{tt2d495bf4b2xxxxxx} in \autoref{list:navigate}), and the $mini_{B}$ can use an API named \textsf{navigateBackMiniProgram(Object msg)} to respond $mini_{A}$. However, the exchanged message may contain sensitive data such as location data, and the mechanism can be abused to deploy collusion attacks.
  
 \vspace{2mm}
\begin{lstlisting} [caption={}, basicstyle=\footnotesize\ttfamily,  xleftmargin=.05\textwidth ]
 tt.navigateToMiniProgram({
  appId: "tt2d495bf4b2xxxxxx",
  extraData: {
    longitude: 39,
    latitude: -86
  },
  success: function (e) {
    // data transmission succeeded
  },
  fail: function (e) {
    // data transmission failed
  },
});
\end{lstlisting} 
\begin{lstlisting} [caption={Cross-miniapp channel (TickTok)   },label={list:navigate},basicstyle=\footnotesize\ttfamily,  xleftmargin=.05\textwidth ]
//code fragment to receive data
var options = tt.getLaunchOptionsSync();

var lo=options.referrerInfo.extraData.longitude;
var la=options.referrerInfo.extraData.latitude;

tt.navigateBackMiniProgram({
  extraData: {
    feed_back: "Location data received",
  },
});
\end{lstlisting} 
 \vspace{2mm}

 
\textbf{Attack \#4: Collusion Attacks.} The collusion attack can be deployed against the mini-app ecosystem. As shown in \autoref{fig:collusion},  $Miniapp_{1}$ has the access to the location services and $Miniapp_{2}$ has the access to the user's contact book. However, they do not have a back-end. To send out the user's privacy,  $Miniapp_{1}$ and $Miniapp_{2}$ can invoke  $Miniapp_{3}$, establishing a channel to deliver the sensitive information.  $Miniapp_{3}$, which does not have the access to location services and contact book, now obtains these information from the tunnel. Then,  $Miniapp_{3}$ transmit the sensitive information to a remote malicious back-end. %{\red TODO: We should have a more specific analysis regarding what information can be leaked in the evaluation. }


\begin{figure} [h]  
\centering
\includegraphics[width=0.8\columnwidth]{image/collusion.pdf}\\
%\vspace{-2mm}
\caption{Collusion attacks} 
%\vspace{-3mm}
\label{fig:collusion}
\end{figure}

Different from the legacy collusion attacks on Android system, which is subject to a strong assumption that two malicious app must be installed onto the smartphone at the same time, the collusion attacks in the context of mini-apps can be deployed easily. This is because the mini-apps are featured with installation-free and instant experiences. To be more specific, one miniapp can use the method \texttt{navigateToMiniProgram(.)} to actively invoke mini-apps during the life-cycle even if the targeted mini-app was not hosted on the smartphone before. For most of the platforms we have investigated such as \alipay, \tik and \baidu, the host app will host the mini-app automatically without prompting the user for consent.  


\subsection{Inter-Process Communication Management}

\textbf{Pitfall \#6: Vulnerable Cross-miniapp Channel.} The mini-apps relay on the channel established by the host app for communication, and the process is significantly different from that of legacy OS. In legacy OS, all the apps and their resources are co-located in the same physical machine, and OS can setup a tunnel for two apps for communication under its fully supervision (e.g., Intent mechanism \cite{cruz2018intent} of Android). However, in the context of mini-apps, the mini-apps are stored remotely on the back-end of the host app before running. Even if the mini-app was previously launched, the resources (e.g., JavaScript code and images) can be modified and re-uploaded by the developer. Therefore,  the establishment of the communicating tunnel is a joint work between the front-end and the back-end of the host app, where the network connection is involved. To be more specific, when $mini_{A}$ requires the host app to deliver a message to $mini_{B}$, the host app will first initiate a network request to the its back-end for updating, then synchronize the resources of $mini_{B}$, and ultimately launches $mini_{B}$ and deliver the message.  Unfortunately, we found the involvement of the remote server may enlarge the attack surfaces of the mini-apps,  since the network requests are not fully controlled by the host app.

  



%If this is the case, when one mini-app attempts to setup a channel to another mini-app for communication, the host app has to issue a request to the remote server for downloading resources (e.g., JavaScript code, images and layout files). Even if two mini-apps are  This may involve security issues, For example, a malware, which has the capabilities of modifying the network requests, may deploy various attacks against the mini-app platforms.  

\textbf{Attack \#5: Mini-app Launching Hi-Jack.} In this attack, we assume that the malicious app is co-located with the victim host app on the smartphone, and the malicious app has the capabilities of modifying network requests sending out from the smartphone. This can be achieved by implementing a VPN extensions. For example, in iOS, \textsf{NetworkExtension} framework \cite{iosnetworking} is available for developer to customize a VPN, which can take control of all network requests and responses. In our attacks, we use \textsf{HTTP Catcher} \cite{httpcatcher}, a web debugging proxy, to demonstrate the novel threat. The attack below is successfully validated on \baidu mini-app platform. 


 
 
\begin{figure} [h]  
\centering
\includegraphics[width=0.8\columnwidth]{image/hijack.pdf}\\
%\vspace{-2mm}
\caption{Mini-app launching hi-jack} 
%\vspace{-3mm}
\label{fig:hijack}
\end{figure}


The attack process is demonstrated in \autoref{fig:hijack}. Initially, $Miniapp_{1}$ requires the host app to launch a session with $Miniapp_{2}$ by calling \texttt{navigateToMiniProgram(Object msg)}, where the identifier of $Miniapp_{2}$ is included in the \texttt{msg} object. The host app send out the request (Step \ding{182}), but unfortunately, the request is intercepted by the attacker. The attacker modifies the identifier of $Miniapp_{2}$ to another identifier that belongs to $Miniapp_{3}$, and $Miniapp_{3}$ is an mini-app controlled by the attacker. The attacker then send the modified request to the back-end and goes offline (Step \ding{183}). The back end responds the host app the resources of $Miniapp_{3}$ (Step \ding{184}), and consequently, the malicious $Miniapp_{3}$ is hosted onto the user's smartphone and then launched by the host app (Step \ding{185}). To avoid being noticed by the user, the malicious app can also craft the UI of $Miniapp_{3}$ as same as $Miniapp_{2}$. Once the attack is deployed successfully, $Miniapp_{3}$ can lure the user to input sensitive information and send the information to its remote back-end. 


\textbf{Attack \#6: MitM attacks against Cross Mini-apps Communication.} This attack is the variant of mini-app launch hijack, where the attacker internally manipulate the exchanged messages between two mini-apps. Recall that the only official interface for two apps to establishing the communicating channel is \textsf{navigateToMiniProgram(Object msg)}, which all involve the interaction between the front-end and the back-end of the host app. The co-located malware can passively monitor or actively modify all the messages attached, and even control the receiver of the messages (by modifying the identifier of the receiver, which is also included in the exchanged message). 

\subsection{User Interface Management}

\textbf{Observation and Root Causes} For native apps that developed by \textsf{C/C++} or \textsf{Java}, the UIs are highly related to the running context and has a relatively closed ecosystem. For example, one can not extract a specific UI of an native app, share the UI to others, and require the UI to compatibly run on other users' OSes. However, the host apps rely on web programming technologies (e.g., \textsf{HTML}, \textsf{CSS} and \textsf{JavaScript}) to build the apps, and as a result, the mini-apps extend a shareable UI feature from web applications. To be more specific, a user can share a specific UI of a mini-app in the format of URL or QR code to his or her friends, like we usually share a web page in the format of hyperlink. A user who receives the URL/QR code, can open the URL in his or her web browser (Scanning the QR code will also open the web browser), and then the web browser will launch the corresponding app and jump to referred mini-app UI. However, such a shareable UI feature also brings new security risks to the mini-apps community, since there are numbers of attacks that targeted the shareable web pages now can also work against mini-apps. 

  
\textbf{Pitfall \#7: Vulnerable Shareable UI Feature and Inter-app Communication Mechanism} One notorious attacks against the shareable web pages is session riding attack. In this type of attack, a victim user is logged into the web site, denoted as victim web, with a valid credential. A outsider attacker craft a request (e.g., dropping all the databases) of victim website, and share the request to the victim user. Obviously, the user does not intend to drop any databases currently. However, when the user click the link, the request is submitted by the user and all the databases are purged, since the victim user sends the request using a valid credential. 

It can be observed that to deploy session riding-like attacks, other than the shareable UIs, the attacker has to attach parameters with the UI to craft requests. Fortunately, the mini-apps platforms also allow the extra parameters (i.e., request) to be attached with the shareable UI. Specifically, different from native apps, which usually rely on a inter-process communication framework to exchange information,  two UIs that belong to one mini-app can attach the parameters of interest as a part of the shareable UI in the format of URL. For example,  a key-value pair (e.g., \textsf{password=1234}) can be attached to a shareable UI (e.g., \textsf{/root/console}) in the format of \textsf{/root/console?password=1234}), and due to the feature of shareable UI, the UI with parameters attached can be forward from one user to another. Now, the attacker has all the conditions to deploy a session riding-like attacks. 

%use URL to transmit information of interest. Assume that a login UI (e.g., \textsf{/root/login}) attempts to deliver a key-value pair (e.g., \textsf{password=1234}) to another console UI (e.g., \textsf{/root/console}), the login UI can simply build a URL and invoke an API named \texttt{navigateTo(URL url)} to summit the key-value pair to the console UI (i.e., the URL to be build in our case is  \textsf{/root/console?password=1234}). 
\begin{figure} [h]  
\centering
\includegraphics[width=0.75\columnwidth]{image/csrf.pdf}\\
%\vspace{-2mm}
\caption{Session riding attacks} 
%\vspace{-3mm}
\label{fig:csrf}
\end{figure}


\textbf{Attack \#7: Session Riding Attacks against Mini-apps.} As shown in \autoref{fig:csrf}, we now introduce how to deploy the session riding attacks against Mini-apps.  Initially, an outsider attacker crafts a shareable UI with the specific request attached (e.g., deleting a record from database) in the format of hyperlink (Step \ding{182}), and then sends the hyperlink to a victim user (Step \ding{183}). The user clicks the hyperlink and the host app will be automatically launched, opening the corresponding mini-app (Step \ding{184}), navigating to the UI that attacker intend the user to launch. At the same time, since the mini-apps are designed to provide users instant experiences, the mini-app is usually implemented to automatically log the user in once the user open the app (Like Whatsapp or Slack will always remember user's logged in status unless the user logs out intentionally). Once the targeted UI is launched, the UI will summit the request to the back-end (Step \ding{185}) with the validated credential. As a result, the server will preform the unintended actions (Step \ding{186}).  

The above procedure is too abstract, and we now use \baidu as an exemplary example to demonstrate the novel threats. 
Assume that the targeted UI (named \textsf{delete}) of the victim \baidu mini-app to access is located at \textsf{root} folder of the mini-app, i.e., \textsf{root/delete}. The \textsf{delete} UI accepts one parameter transmit from other UIs, and the parameter is an integer, representing the index of a specific record existing in the remote database. When  \textsf{delete} UI receives the index from other UIs, it sends the index automatically to the remote back-end to remove to corresponding record in the database. We assume the attacker attempts to delete the first record in the database, and therefore, the attacker should trick the user to launch the \textsf{delete} UI with \textsf{id=1} attached, i.e., \textsf{root/delete?id=1}. However, knowing the above URL is not enough for the session riding, since this is only a part of the URL, and the attacker also need to know the other building materials (e.g., domain names and Restful API) to craft the complete URL, which is acceptable for the host apps. 

To obtain other materials, we analyzed the URL, which represents the targeted shareable UI (i.e., \textsf{root/delete}), generated by the original host app. We found that when the attacker attempts to share the targeted UI with others, \baidu returns the attacker a randomized URL (e.g, \url{http://mbd.baidu.com/ma/s/rnJizCl23}), which hides the relative path of the targeted UI, and obfuscates the relationship between the path and other building materials. Fortunately, we are able to obtain the unprotected URL through scanning the QR code generated by the host app, and the original URL is in the following format \url{https://mbd.baidu.com/ma/landingpage?t=smartapp_share&appid={APPID}&url=root/delete&from={USERID}&token_ext=y4iFNuW0}, where \texttt{appid} is the identifier of the victim mini-app, \texttt{url} is the referred shareable UI,  and \texttt{from} is the identifier of the forwarder (i.e., the attacker in this case). 


It can be observed from the link that a token is also appended towards the end of the URL, and according to our experiment, the request will be rejected if the token is not in position. However, we found that \baidu has a security vulnerability regarding the token generation. That is, the token is just a token without binding the content of the request. As a result, the attacker can modify the URL and embed the parameters to build the request. The crafted URL is ultimately in the format of \url{https://mbd.baidu.com/ma/landingpage?t=smartapp_share&appid={APPID}&url=root/delete?id=1&from={USERID}&token_ext=y4iFNuW0}. When the user receives the link and opens it, as discussed earlier, the data record will be deleted. Similar to the session riding attacks in the web security, the session riding attacks against mini-apps can also cause catastrophic consequences. The user can be trick into deleting valuable data (as demonstrated), leaking privacy and credentials being manipulated remotely \cite{zeller2008cross}. 

  


%\subsection{Removal of Security-related APIs}

%\textbf{Observation and Root Causes}. As discussed in \S\ref{sec:back}, the host app of mini-apps intend to provide instant experience by aggressively simplifying original APIs. However, to design an OS requires significant efforts to understand security issues, and the designing procedures may cause confusion regarding how to simplify APIs. Consequently, the designer of a mini-app ecosystem may mistakenly remove the security related APIs, if the designers are not aware of the security impacts, leading to various attacks against the mini-apps as well as OS. Note that, the  shortcoming is different from the first one, in that 
  
%providing multiple features including storage-saving, cross platform and back-end resources isolation. %However, these features   

 





%\textbf{Inconsistency of Platforms }



==> paper/04-crawler.tex <==

%\subsection{Crawler} 



%To collect a data set for our analysis, we first need to design and implement a crawler that can automatically download the mini-apps from the \wechat server. 


Similar to web crawlers, which contain a keyword-based searching component and an output parsing and indexing component, our mini-app crawler has two such components. 
%
%Specifically, 
%Similar to legacy web crawlers and the existing mini-app crawler (\ie, {\sf Mini-crawler}), which contain a keyword-based searching component and an output parsing and downloading component, our mini-app crawler also has two such components. 
To be more specific, our crawler is built on top of the {\sf Mini-crawler} by reusing and upgrading its mini-app searching component, and re-designing and implementing the mini-app downloading component. In the following, we present how we build these two components.

 

% There are some efforts that were made to understand the the novel paradigm. For example, Zhang et al. ~\cite{ourfancywork} developed an approach to download mini-apps when given mini-app ids by hooking and invoking Android \wechat APIs for mini-app downloading. However, hooking is considered malicious behavior by \wechat, and the accounts are under the risk of being banned by \wechat once the host app detects the hooking process. Consequently, premium accounts are required to avoid the account being blocked. Our work, however, utilizes the redirection functionality of mini-apps to improve the durability of downloading. 

% (\S\ref{subsubsec:search}), and the downloading component (\S\ref{subsubsec:downlaod}). 

%corresponding to two important steps, including a meta data collector to search mini-apps (\eg, ratings and mini-app IDs) based on the fed keywords(\S\ref{subsubsec:search}), and a mini-app downloader to download the packages of mini-apps from \wechat server (\S\ref{subsubsec:downlaod}). 

\paragraph{(I) Mini-app Searching}
\label{subsubsec:search}
%\AY{No such section any more. No searching, just crawling.}\ZY{We still need this. Otherwise, how could you obtain the metadata?}
%Similar to web crawler, we need to first locate the URLs that can allow us query the mini-apps. However, 
Unlike Google Play which provides a web portal (an URL) to easily search Android apps, \Tencent does not provide such a web portal and instead all the mini-apps must be queried inside the \wechat app. Therefore, similar to the {\sf Mini-crawler}, which used the in-app searching interface to query mini-apps, \ie, the \texttt{innersearch} API (as presented in \autoref{tab:inner:apis1}), our crawler also used this API,
%we have to first locate the URLs if there is any inside the \wechat app. By manually launching the mini-app query interface and intercepts all the networking APIs invoked by \wechat, we successfully locate an \texttt{innersearch} API, as presented in \autoref{tab:inner:apis1}.
%This API %is an in-app interface for \wechat users to query the mini-apps, which 
which takes parameters including the searched keywords, \texttt{timestamp}, \texttt{client\_version}, \texttt{cookie}, and so on, and returns a list of the matched mini-apps with their {\tt appID}, {\tt label}, {\tt rating}, and so forth.


% However, we only need to take care the keywords, \texttt{timestamp}, and the \texttt{cookie} fields. 
% %
% %
% %
% %keywords  user's inputs as the keywords, and returns a list of mini-apps that contained the searched keyword in their names. We reverse engineered the traffic between \wechat server and client, and identified such the inner interface used by \wechat as shown in \autoref{tab:inner:apis1}. By default, we found that other than the user's inputs, the API accepts many inputs such as \texttt{timestamp}, \texttt{client\_version} and so forth. However, we only care about two of them, since others will not have no impacts on the query results. The two inputs are \textit{cookie} and a \texttt{query}. Specifically, \texttt{query} is the keyword that is used to retrieve mini-apps.  
% %

% Dealing with keywords and \texttt{timestamp} is trivial once we learnt their format. However, {\tt cookie} is a tricky field since it is distributed by \wechat servers to associate the users and gets expired every 2 hours, which can be observed by analyzing the traffic. In particular, every time when we perform an in-app mini-app query with \wechat, the \wechat server will re-send a fresh \textit{cookie} to the client. In the {\sf Mini-crawler}, such a {\tt cookie} is manually configured and updated, In our crawler, we have developed a script to automatically trigger the in-app query, and intercept the  \textit{cookie} sent from server, and then update it every 2 hours. In such a way, we can keep searching the mini-apps with arbitrary keywords without worrying about using any expired cookies.  \looseness=-1

\paragraph{(II) Mini-app Downloading}
\label{subsubsec:downlaod}
To download the mini-apps from \wechat, an intuitive way is to reverse engineer the \wechat protocol, locate the downloading interface, and extract it out for the downloading.  However, according to our analysis with \wechat app, we find that the downloading interface is significantly different from the aforementioned searching interface, which we cannot identify directly through the analysis of network traffic. Therefore, {\sf Mini-crawler} took an in-place API hooking inside \wechat instead of extracting the interface out to download the mini-apps. 
%
%is to reverse engineer \wechat and hook the download interface directly. 
However, the practice has one major drawback:  \wechat considers the API hooking as a dangerous behavior, and the \wechat accounts used to download the mini-apps may suffer from the risks of being banned by \wechat. Therefore, {\sf Mini-crawler} requires multiple premium accounts to reduce this risk. % to improve the durability of downloading (the limitation is also confirmed in their paper).  
%


Fortunately, by going through all the \wechat mini-app appming APIs, we have identified one interesting mini-app API that can allow mini-app downloading  without using additional mechanism such as API hooking, as shown in the 2nd API in \autoref{tab:inner:apis1}. In particular, this API is named \breakabletexttt{wx.navigateToMiniapp}, which is used by specific mini-apps for the purpose of navigating to other mini-apps. It takes a mini-app ID along with a version (release vs. debug) as parameters,  downloads the corresponding mini-app package, and opens it inside a mini-app.  We therefore developed a special mini-app using the \breakabletexttt{wx.navigateToMiniapp}, and use it to continuously download the mini-apps of our interests by feeding the mini-app IDs, perfectly serving our mini-app downloading needs. 
Moreover, we have also identified an API (the 5th API in \autoref{tab:inner:apis1}) that allows us to collect the developer information if it is available \cite{developinfo21} and the update date of the mini-app, which is  not covered and implemented by {\sf Mini-crawler} either.  Note that we will also release the source code of our crawler in Github.

\vspace{-2mm}
\subsection{\appsecret Leakage Inspector} 
\label{subsec:keyleak}

The miniapp analyzing script is quite straightforward to implemcom. As discussed, the \appsecret is a 256-bit string of hexadecimal digits. {To reduce the false-negative of \appsecret leakage, we would like to collect as many these 256-bit strings as possible first, and then validate the strings with the \wechat server to filter out all non-\appsecret strings.} Particularly,  we use a regular expression approach with a particular pattern of 32-bytes hex-string in the form of \texttt{[a-f0-9]\{32\}} to search the possible \appsecret in the code of miniapp, and use the 3rd API presented  in \autoref{tab:inner:apis1} to confirm the validity of \appsecret. %\ZY{Only the first one is used to confirm the validity of \appsecret. The second one is used to get \sessionkey, which is used in our attacks.}
This API is used to fetch the \textsf{AT} (which only accepts miniapp ID and the \appsecret) to perform the validation. When the fed \appsecret is correct, the API returns the actual \textsf{AT}. Otherwise, it returns an error code.   
Since this validation process is done with the \wechat server, we can ensure there is no false positive of \appsecret detection. We also scanned the decomplied code to determine which sensitive data or paid services (e.g., \texttt{getPhoneNumber} is used to get the user's phone number) are used by the vulnerable miniapp.  

\begin{table}[]
\scriptsize
 \belowrulesep=0pt
 \aboverulesep=0pt
 \setlength\tabcolsep{2pt}
\begin{tabular}{llcc}\toprule
 {\textbf{API}} &  {\textbf{Description}}    \\
 \midrule


\textbf{{{Mp.wx.qq.com/wxa-cgi/innersearch}}}    &   mini-app Searching API      \\
   \textbf{Parameters}   &       \\  
\SFviii   \texttt{query}    &   A keyword to search the mini-apps         \\  
%\SFviii Language & \texttt{obj.lang} & \tickNo    &  \tickYes     \\
\SFviii \texttt{client\_version}       &   The \wechat client version    \\ 
\SFviii \texttt{time}       & The timestamp of this query     \\ 
\SFviii  \texttt{cookie} &  \wechat client token     \\
\SFii~ ... & Other omitted parameters\\
\textbf{Return value} &  %The  mini-app metadata  
\\
\SFviii  \texttt{appID}     & The app ID of the mini-app       \\
\SFviii   \texttt{label}     & The category of the mini-app    \\
\SFviii  \texttt{rating}   &  The user rating of the mini-app    \\
\SFii~... & Other omitted fields in the return value\\
%\SFii Profile & A\_A1\_A\_A & a\_a1\_a   &      \\
%~~~\SFii Nick name   & A\_A1\_A\_B & a\_a1\_b   &      \\
  \midrule

\textbf{Wx.nativgateTomini-app()}        &    mini-app Downloading API    \\  
   \textbf{Parameters}   &       \\  
\SFviii\texttt{appID}        &  The app ID of the mini-app          \\  
\SFii\texttt{version}    &  The version (released or debug)       \\ 
\textbf{Return value}    &  The packed file of the mini-app     \\  \midrule

 \textbf{Api.weixin.qq.com/cgi-bin/token}     & A \appsecret Validation API    \\
    \textbf{Parameters}   &       \\  
\SFviii  \texttt{appID}      &   The app ID of the mini-app     \\
\SFviii \texttt{secret}    &  A \appsecret      \\
\SFii\texttt{grant\_type}   &  The access type  \\
\textbf{Return value}    &   An access token or error message   \\

\midrule

 \textbf{Api.weixin.qq.com/sns/jscode2session}      & \appsecret Validation API (\texttt{getEK()})    \\
    \textbf{Parameters}   &       \\  
\SFviii  \texttt{appID}      &   The app ID of the mini-app     \\
\SFviii \texttt{secret}    &  The Master key (\appsecret)      \\
\SFii\texttt{jscode}   &   A login token (\token) \\
\textbf{Return value}    &  The encryption key (\sessionkey)  \\
 
\midrule

 \textbf{Mp.weixin.qq.com/mp/waverifyinfo}      & Developer Information Downloading API   \\
    \textbf{Parameters}   &       \\  
\SFviii  \texttt{appID}      &   The app ID of the mini-app     \\
\SFviii \texttt{deviceType}    &  The device type of mobile (e.g., Android)     \\
\SFii\texttt{netType}   &  Network Connection Information (e.g., WiFi) \\
\textbf{Return value}    &     \\  
\SFviii  \texttt{developerinfo}     & The developer information of the mini-app       \\
\SFii\texttt{updatedate} & The relase date of the mini-app\\
     
           
\bottomrule
\end{tabular} 
\caption{Summary of Five Important APIs Used by Our Tool.}
\label{tab:inner:apis1}

\end{table}
\hspace{-0.2in}



==> paper/04_EVALUATION_BACKUP.tex <==
% \section{Evaluation}
\label{sec:evaluation}
 

\subsection{Experiment Setup}

\paragraph{Mini-program Crawling} The first step of our analysis is to crawl the mini-programs. To this end, we developed our own mini-program crawler by extending the existing open source \textsf{Mini-Crawler}~\cite{ourfancywork}. 
%
%In our evaluation, we would like to measure the impacts the of our finding by scanning how many mini-programs had leaked their \appsecret{s}. As discussed earlier, we can use the \wechat mini-program searching API and downloading API to collect the mini-programs, and to ensure better representativeness and coverage of the mini-programs, we used the methods introduced in  \textsf{Mini-Crawler}~\cite{ourfancywork} to generate the keywords and search the available mini-programs. To be more specific, 
In particular, to generate the keywords for searching the mini-programs, we first used the $1,000$ most commonly used Chinese characters as the seed keywords to download the mini-programs as our primary dataset, and then we further extract the names and descriptions from the collected mini-programs as the keywords to expand the keywords-list, which eventually contained 414,020 keywords. Next, we used the expanded keyword-list to search the mini-programs again, and the crawled mini-programs
formed our final dataset. 



\paragraph{Dataset Description} With our mini-program based crawler,  we have collected \totalanalyzedapps mini-programs. It has been reported that there are around 2 million mini-programs in \wechat market~\cite{WeChatMi59:online}. Therefore, we believe our dataset includes the majority of the mini-programs. In total, the collected mini-programs took up \totaldisk of disk space. 
%After we have unpacked them, we obtained \totalfiles and among all the files, \totaljsfiles are JavaScript files, which may contain the leaked \appsecret{s}. 
According to the metadata of these mini-programs, we further classify them into 21 categories based on 
%The collected mini-programs are categorized in \wechat mini-program market based on 
their primary functionalities such as `Business' and `Education', as reported in the first column of ~\autoref{tab:vuln_cat_score}. %We have observed that there are 21 categories in total, which covers many aspects of our daily life.  
According to the data presented in the 9th column, the categories with the most mini-programs are the shopping (\shoppingapps, \shoppingappsratio), lifestyle (\lifestyleapps, \lifestyleappsratio), and tools (\toolapps, \toolappsratio). 


Interestingly, we also found that about a third of the mini-programs (658,689 out of 1,921,084) have their ratings (from score 0.0 to 5.0), according to the last row of \autoref{tab:vuln_cat_score}. Note that unlike Google Play store with which we can easily know the popularity of an app based on the accumulated downloads, \Tencent does not provide such metadata. However, we can use the rating of a mini-program to reflect an approximated popularity of a mini-program, since the rating of a mini-program is only available when enough users have used and rated the mini-programs~\cite{ourfancywork}. %, and therefore, ratings of a mini-program can serve an important metric to reflect the popularity of a mini-program. \looseness=-1
%As shown in the table,  \ZY{WHICH} category has the most rated mini-programs. 

%Overall, we believed our dataset is representative. 

% \begin{table}[h]
% \begin{tabular}{lll}
% \hline
% \multicolumn{1}{|l|}{Category} & \multicolumn{1}{l|}{Number of Mini-programs} & \multicolumn{1}{l|}{Number of Rated Mini-programs} \\ \hline
% \multicolumn{1}{|l|}{}         & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                              \\ \hline
%                               &                                              &                                                   
% \end{tabular}
% \end{table}

% approximately \ZY{XX\%} mini-programs fail into the category \ZY{shopping}
%Other than analyzing the collected mini-programs from the JavaScript code, we also analyzed the these mini-programs by parsing the collected meta data. \ZY{We can put the statistics of the collected mini-programs in the first paragraph of the evaluation, which can be considered as a part of the description of our data-set collection. } 

%Recall that the rating and the category  of a mini-program can be found in the meta data, and therefore, we plot the heat-map based on the categories and the ratings of our collected mini-programs, where the x-axis is the categories that the mini-program belong to and the y-axis is the ratings of these mini-programs. \ZY{The heatmap is no longer needed. Instead, we present the statistics of vulnerable mini-programs} The more mini-programs fall into a specific category with a specific rating, the darker the color of the cell that represents the category with the rating will be. As shown in \cref{fig:heatmap_all_scores}, \AY{aside from the mini-programs that have been rated, there are still a portion of mini-programs not being rated. 



%This is because the rating will only show if enough users have rated the mini-program, otherwise, \wechat will only show `insufficient rating user in the metadata page'. In total, we found \numwithscore mini-programs that have ratings, where the mean value of these mini-programs are \meanscores, and \numwithscorefive mini-programs are rated 5.0 scores. 
% the mini-programs can either be rated or not rated. This is because the rating of a mini-program is displayed only when enough people rate the mini-program. 
% It can be observed from \autoref{fig:my_label} that aside from the mini-programs that currently do not have the ratings (only enough people rate the mini-program, most of these rated mini-programs a relatively high rating~\cite{ratings}). 
% For example, the mean value of these mini-programs are  [\ZY{}], and  [\ZY{}] with the rating of 5.0.
%\AY{Interestingly, for categories with more rated mini-programs, we find that games are usually rated lower, while the mini-program in categories of education, shopping, life-style, and tools usually have higher ratings.}


\paragraph{Machine Configuration} To extract and analyze these mini-programs, we used two desktops running Ubuntu 18.04 with 2 cores 4 threads, Intel Core i5-5300 (2.30 GHz) CPUs and 8 GB RAM. We opened 16 threads in each desktop to maximize the extraction and analysis speed. % \ZQ{confusing} \ZY{Rewritten the sentence}
% \sout{We use a client-server mode to run our analysis, where the server machine is responsible for assigning the tasks and collecting the results, and the client machine is responsible for the analysis.} 




%Since the similar mini-programs tend to have the similar names and descriptions to profile their functionalities, if we collect one mini-program with specific functionalities, the method allows us to collect more mini-programs with .        

 

%\AY{It has been reported that there are over 2 million mini-programs in \wechat market~\cite{WeChatMi59:online}. To do so, we collected mini-programs with our crawler based on the metadata collected from \wechat mini-program searching API. In total, we collected \totalapps mini-programs during the past year for our evaluation.} 
% \sout{We could have downloaded all of them for the analysis, but we feel we do not have to do so, since there could be many unpopular apps, similar to the apps in the Google Play. Therefore, we decide to crawl only the popular apps. However, there is no ranking of the mini-programs, and we can only search them using keywords. To search for popular mini-programs, we first obtain the company name from the list of Fortune 500~\cite{fortunechina}. With these company names, we first perform word segmenting with Chinese word segmentation tool \texttt{jieba}~\cite{jieba}, and then use the TF-IDF algorithm~\cite{ramos2003using} to extract the keywords from the two lists, and in total we collected 774 keywords. We feed these 774 keywords into our mini-crawler, and eventually collected \totalapps mini-programs in a one week period with one \wechat account. \looseness=-1 }




%This is because when processing the unpacked JavaScript code, our tool only matched the 32-bit string pattern to search for the possible \appsecret{s} and API usage without involving any other sophisticated program analysis.


%based on all our 493 collected keywords for analysis.
 
% \paragraph{Vulnerability Detection} It is straightforward to detect the vulnerability. First, we detect whether or not a mini-program has invoked the APIs (\ie, \texttt{getPhoneNumber}) that can fetch the encrypted sensitive data from the \wechat server, as our attack works against the data encryption mechanism; If so, we then further detect whether the mini-program has the \appsecret leakage. To be more specific, we tackle (1) Sensitive API Invocation Detection and (2) Master key \appsecret Leakage Detection:      

% \begin{itemize}
% \item \paragraph{(1) Sensitive API Invocation Detection} we utilize \texttt{esprima} to generate the Abstract Syntax Tree (AST) of the mini-programs and perform a static analysis for function invocation in the JavaScript file. As shown in \cref{tab:api}, each encrypted user information (in the \textbf{E} column) is associated with a mini-program API. As such, we can detect whether a mini-program accesses an encrypted user information by detecting whether the corresponding API is being invoked. Note that there is one special case: \texttt{getPhoneNumber}. To protect user privacy, this API is can not be invoked in the code, but invoked when the user actively clicks a WXML button with \texttt{openType="getPhoneNumber"}, so as to make sure the user is aware of the requirement of his/her phone number. As such, to cover all the APIs associated with encrypted data, we also parses the WXML files to detect the usage of the user phone number.

% \item \paragraph{(2) Master key \appsecret Leakage Detection}

% For detecting the leakage of  \appsecret, as it has a fixed format (\ie, it is a 32-byte long hex string), the most intuitive way to detect \appsecret leakage is to grep the decomplied JavaScript code using regular expression (\ie, \texttt{[a-f0-9]\{32\}}). However, such a method is subject to false alerts, since many strings in a mini-program have the same format (\ie, some online databases used the 32-bytes hex string as the primary key). Fortunately, we have identified an access token query API (\ie,  \url{https://api.weixin.qq.com/cgi-bin/token?grant_type=client_credential&appid=APPID&secret=MK}) provided by \wechat server, which can assist us to verify the correctness of \appsecret. Specifically, the API is designed for the third-party developers to query an access token (Note that the access token is different from login token \token), with which the third-party developers can then initiate the network requests to the \wechat server for some of the services (\eg, binding the mini-program with the vendor's official \wechat account). The API takes two parameters: the publicly accessible mini-program ID and the mini-program \appsecret, and returns the access token when the two parameters are matched.  Therefore, in our analysis, we first collect all specious strings from the decomplied mini-programs, and then feed those strings to the access token query API to check whether the \appsecret is valid.
% \end{itemize}


% \begin{table}[]
%     \centering
%     \scriptsize
%     \aboverulesep=0pt
%     \belowrulesep=0pt
%     \setlength\tabcolsep{4pt}

%     \begin{tabular}{c|r|r|r|r|r|r}
%     \toprule
%  \multirow{2}{*}{Category}&\multicolumn{2}{c|}{Rated}&\multicolumn{2}{c|}{Unrated}&\multicolumn{2}{c}{Total} \\ \cmidrule{2-7}
%          &\# apps&\% apps&\# apps&\% apps&\# apps&\% apps\\ \midrule
         
% business&1,544&0.08\%&77,160&3.80\%&78,704&3.87\%\\
% education&13,779&0.68\%&206,686&10.18\%&220,465&10.85\%\\
% entertainment&3,290&0.16\%&18,967&0.93\%&22,257&1.10\%\\
% finance&737&0.04\%&2,470&0.12\%&3,207&0.16\%\\
% food&3,947&0.19\%&106,506&5.24\%&110,453&5.44\%\\
% games&19,340&0.95\%&67,629&3.33\%&86,969&4.28\%\\
% government&1,535&0.08\%&26,208&1.29\%&27,743&1.37\%\\
% health&1,684&0.08\%&22,896&1.13\%&24,580&1.21\%\\
% images&1,163&0.06\%&4,958&0.24\%&6,121&0.30\%\\
% job&2,274&0.11\%&18,305&0.90\%&20,579&1.01\%\\
% lifestyle&12,280&0.60\%&311,038&15.31\%&323,318&15.92\%\\
% reading&944&0.05\%&6,678&0.33\%&7,622&0.38\%\\
% shopping&23,163&1.14\%&724,332&35.66\%&747,495&36.80\%\\
% social&3,054&0.15\%&17,004&0.84\%&20,058&0.99\%\\
% sports&1,572&0.08\%&12,371&0.61\%&13,943&0.69\%\\
% tool&20,891&1.03\%&209,959&10.34\%&230,850&11.37\%\\
% traffic&3,014&0.15\%&30,505&1.50\%&33,519&1.65\%\\
% travelling&607&0.03\%&7,767&0.38\%&8,374&0.41\%\\
% uncategorized&11&0.00\%&44,949&2.21\%&44,960&2.21\%\\
% Total&114,829&5.65\%&1,916,388&94.35\%&2,031,217&100.00\%\\


% \bottomrule
%     \end{tabular}
%     \caption{Category distribution of mini-programs\AY{200w}}
%     \label{tab:miniapp_category}
% \end{table}
 
 
 
  %\AY{In general, there are two questions to answer for coffee attack vulnerability detection. (1) is the appsecret of the mini-program leaked? (2) what kind of encrypted information does the mini-program access?}

 
%  \wechat have more than one million mini-programs available, and they did not provide 


% to generate our keyword database, which allows us to query and fetch mini-programs from \wechat. To be more specific, 



%  we use NLP techniques to generate the keyword for query. First, we used \texttt{Jieba} to perform Chinese word segmentation. Then, we used TFIDF algorithm to extract the keywords of these company names. After deduplication, we finally have a list of 493 keywords. As such, we used the 493 keywords to query the \wechat mini-program API, and collected 8,824 mini-programs for analysis

 
%  To investigate the impact of our discovered problem and attacks, we need to collect a set of mini-programs and detect the th



% We


% To collect the mini-programs, 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\scriptsize
% \tiny
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
\centering
\begin{tabular}{l|r|r|r|r|r|r|r|r|r}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Category}}} & \multicolumn{3}{c|}{\textbf{Rated}}                                                                                & \multicolumn{3}{c|}{\textbf{Unrated}}                                                                              & \multicolumn{3}{c}{\textbf{Total}}                                                                                \\ \cline{2-10} 
\multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{\textbf{\# Vuln}} & \multicolumn{1}{c|}{\textbf{\# App}} & \multicolumn{1}{c|}{\textbf{\%}}  & \multicolumn{1}{c|}{\textbf{\# Vuln}} & \multicolumn{1}{c|}{\textbf{\# App}} & \multicolumn{1}{c|}{\textbf{\%}} & \multicolumn{1}{c|}{\textbf{\# Vuln}} & \multicolumn{1}{c|}{\textbf{\# App}} & \multicolumn{1}{c}{\textbf{\%}} \\ \hline
business&146&7,178&2.03\%&470&65,924&0.71\%&616&73,102&0.84\%\\
education&1,735&95,220&1.82\%&1,825&115,715&1.58\%&3,560&210,935&1.69\%\\
e-learning&36&1,699&2.12\%&157&5,440&2.89\%&193&7,139&2.70\%\\
entertainment&134&7,114&1.88\%&115&13,782&0.83\%&249&20,896&1.19\%\\
finance&20&984&2.03\%&52&2,020&2.57\%&72&3,004&2.40\%\\
food&671&42,881&1.56\%&905&62,981&1.44\%&1,576&105,862&1.49\%\\
games&756&34,259&2.21\%&972&48,074&2.02\%&1,728&82,333&2.10\%\\
government&237&8,848&2.68\%&374&17,423&2.15\%&611&26,271&2.33\%\\
health&185&7,785&2.38\%&253&15,566&1.63\%&438&23,351&1.88\%\\
job&158&9,109&1.73\%&160&10,561&1.52\%&318&19,670&1.62\%\\
lifestyle&2,048&103,530&1.98\%&2,751&203,443&1.35\%&4,799&306,973&1.56\%\\
photo&21&1,972&1.06\%&15&3,758&0.40\%&36&5,730&0.63\%\\
shopping&3,250&210,436&1.54\%&4,005&495,334&0.81\%&7,255&705,770&1.03\%\\
social&141&8,561&1.65\%&175&10,626&1.65\%&316&19,187&1.65\%\\
sports&103&5,568&1.85\%&108&7,678&1.41\%&211&13,246&1.59\%\\
tool&2,454&95,255&2.58\%&2,673&123,324&2.17\%&5,127&218,579&2.35\%\\
traffic&289&14,794&1.95\%&259&17,121&1.51\%&548&31,915&1.72\%\\
travelling&56&3,216&1.74\%&80&4,729&1.69\%&136&7,945&1.71\%\\
uncategorized&1&280&0.36\%&2&38,896&0.01\%&3&39,176&0.01\%\\ \midrule
Total&12,441&658,689&1.89\%&15,351&1,262,395&1.22\%&27,792&1,921,084&1.45\%\\ \bottomrule

\end{tabular}
\caption{Distribution of the vulnerable mini-programs for each category based on whether they are rated. %\ZQ{elearning. Please change Appendix as well} %ratings and categories of vulnerable mini-programs 
} 
    \label{tab:vuln_cat_score} 

\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_score_ratio.pdf}
    \caption{The heatmap of the vulnerable mini-programs w.r.t. their categories and ratings}
    \label{fig:vuln_miniapp_cat_score_ratio}
\end{figure}



\begin{figure*}[htb]
    % \begin{minipage}[t]{.3\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{image/vuln_miniapp_cat_score_absolute.pdf}
    %     \subcaption{}\label{fig:vuln_miniapp_cat_problem_unrated_absolute}
    % \end{minipage}
    % \hfill

    \hfill
    % \begin{minipage}[t]{.33\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{image/vuln_miniapp_cat_problem_rated_absolute.pdf}
    %     \subcaption{}
    % \label{fig:vuln_miniapp_cat_problem_rated_absolute}
    % \end{minipage}  
     \begin{minipage}[t]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/vuln_miniapp_cat_problem_rated_ratio.pdf}
        \subcaption{}
    \label{fig:vuln_miniapp_cat_problem_rated_ratio}
    \end{minipage}
    \hfill
    % \begin{minipage}[t]{.3\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{image/vuln_miniapp_cat_problem_unrated_absolute.pdf}
    %     \subcaption{}
    % \label{fig:vuln_miniapp_cat_data_problem_unrated_absolute}
    % \end{minipage}
    % \hfill
    \begin{minipage}[t]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/vuln_miniapp_cat_problem_unrated_ratio.pdf}
        \subcaption{}
    \label{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated}
    \end{minipage}  
    
    \caption{The heatmap of the vulnerable mini-programs w.r.t. their categories and accessed data.}  
    \label{fig:heatmap}
    
\end{figure*}




% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_score_absolute.pdf}
%     \caption{Amount of vulnerable mini-programs w.r.t. scores}
%     \label{fig:vuln_miniapp_cat_problem_unrated_absolute}
% \end{figure} %1
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_score_ratio.pdf}
%     \caption{Ratio of vulnerable mini-programs w.r.t. scores}
%     \label{fig:vuln_miniapp_cat_problem_unrated_ratio}
% \end{figure} %2
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_problem_rated_absolute.pdf}
%     \caption{Amount of rated vulnerable mini-programs w.r.t. accessed data}
%     \label{fig:vuln_miniapp_cat_problem_rated_absolute}
% \end{figure} %3
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_problem_rated_ratio.pdf}
%     \caption{Ratio of rated vulnerable mini-program distribution w.r.t. accessed data}
%     \label{fig:vuln_miniapp_cat_problem_rated_ratio}
% \end{figure} %4
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_problem_unrated_absolute.pdf}
%     \caption{Amount of unrated vulnerable mini-programs w.r.t. accessed data}
%     \label{fig:vuln_miniapp_cat_problem_unrated_absolute}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_problem_unrated_ratio.pdf}
%     \caption{Ratio of unrated vulnerable mini-programs w.r.t. accessed data}
%     \label{fig:vuln_miniapp_cat_problem_unrated_ratio}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \begin{table*}[]
% \scriptsize
% % \tiny
% \belowrulesep=0pt
% \aboverulesep=0pt
% % \setlength\tabcolsep{1.5pt}
%     \centering
%     \begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
% \toprule
% \multirow{3}{*}{\bf Category}&\multicolumn{9}{c|}{\bf User Information}&\multicolumn{6}{c}{\bf Social Information}\\ \cmidrule{2-16}
% % &\multicolumn{3}{c}{\bf Address}\\ \cmidrule{2-22}
% &\multicolumn{3}{c|}{\textbf{phone number}}&\multicolumn{3}{c|}{\textbf{\texttt{werun} data}}&\multicolumn{3}{c|}{\textbf{user info}}&\multicolumn{3}{c|}{\textbf{share info}}&\multicolumn{3}{c}{\textbf{promoting messages}}\\ \cmidrule{2-16}
% % &\multicolumn{3}{c|}{\textbf{group chat info}}&\multicolumn{3}{c}{\textbf{address}} \\ \cmidrule{2-22}
% &\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app\\ \midrule
% %& \# vuln&\# app&\% app&\# vuln&\# app&\% app\\ \midrule
% business&13&2,832&0.46&6&299&2.01&7&5,790&0.12&36&3,696&0.97&0&21&0.0\\
% education&17&2,569&0.66&28&1,225&2.29&12&1,926&0.62&594&31,500&1.89&0&189&0.0\\
% entertainment&4&355&1.13&1&167&0.6&5&654&0.76&85&3,238&2.63&0&11&0.0\\
% finance&0&81&0.0&2&35&5.71&3&94&3.19&7&282&2.48&0&0&0.0\\
% food&13&1,637&0.79&4&526&0.76&0&903&0.0&138&19,859&0.69&0&122&0.0\\
% games&1&70&1.43&4&267&1.5&0&57&0.0&481&19,787&2.43&0&5&0.0\\
% government&10&647&1.55&7&249&2.81&11&478&2.3&36&2,545&1.41&0&8&0.0\\
% health&7&574&1.22&8&313&2.56&11&672&1.64&41&2,917&1.41&0&8&0.0\\
% images&0&48&0.0&1&46&2.17&3&121&2.48&5&774&0.65&0&3&0.0\\
% job&2&239&0.84&0&83&0.0&5&318&1.57&26&2,361&1.1&0&6&0.0\\
% lifestyle&46&4,207&1.09&14&955&1.47&23&3,465&0.66&497&36,614&1.36&0&187&0.0\\
% reading&1&199&0.5&5&64&7.81&3&249&1.2&19&1,164&1.63&0&5&0.0\\
% shopping&70&13,518&0.52&41&2,746&1.49&20&8,209&0.24&1,169&84,442&1.38&0&1,505&0.0\\
% social&0&130&0.0&7&200&3.5&1&172&0.58&63&2,395&2.63&1&13&7.69\\
% sports&2&242&0.83&40&2,338&1.71&3&383&0.78&23&2,782&0.83&0&6&0.0\\
% tool&31&2,150&1.44&52&2,371&2.19&22&2,451&0.9&464&22,474&2.06&0&114&0.0\\
% traffic&6&346&1.73&2&418&0.48&3&226&1.33&26&4,004&0.65&0&25&0.0\\
% travelling&2&184&1.09&0&171&0.0&1&171&0.58&7&1,034&0.68&0&6&0.0\\
% uncategorized&0&9&0.0&0&2&0.0&0&1&0.0&1&32,902&0.0&0&32,834&0.0\\


% % total&225&30,037&0.75&312&12,540&2.49&317&26,125&1.21&5,461&276,245&1.98&3&34,935&0.01&0&0&0.00&0&0&0.00\\ 
% \bottomrule




% \bottomrule
%     \end{tabular}
%     \caption{\AY{This table equals the union of previous two tables} Mini-programs and accessed sensitive information (Note that we have not found cases requiring user address or group messaging information, so the data is removed from the table).}  
%     \label{tab:apis}

% \end{table*}


%\AY{In our paper, we are interested in two types of mini-programs: (1) the mini-programs that have been developed by IT companies that migrated their native apps into \wechat mini-program platform (e.g., mini-programs developed by Tencent and Baidu). (2) the mini-programs developed by . As such, we obtained the list of top IT companies from the report of Chinese IT companies (2020) published by Internet Society of China \cite{isc}. For the list of top commercial companies, we obtained the keyword list from Fortune China \cite{fortunechina}.}

% \AY{With the company list obtained, we use NLP techniques to generate the keyword for query. First, we used \texttt{Jieba} to perform Chinese word segmentation. Then, we used TFIDF algorithm to extract the keywords of these company names. After deduplication, we finally have a list of 493 keywords. As such, we used the 493 keywords to query the \wechat mini-program API, and collected 8,824 mini-programs for analysis.}
% \subsection{Vulnerability Detection}
% \AY{In general, there are two questions to answer for coffee attack vulnerability detection. (1) is the appsecret of the mini-program leaked? (2) what kind of encrypted information does the mini-program access?}





%\paragraph{Vulnerability}

% 
% \paragraph{Data Set} We collected our mini-programs from \wechat app via its built-in mini-program searching functionality. In \wechat app, users can either install a mini-program by clicking on a link shared by other user, or manually use keyword to search for a specific mini-program. To obtain a list of mini-programs to be downloaded, we reverse engineered \wechat, investigated the workflow of the search interface, and collected the metadata of $510,000$ mini-programs containing mini-program IDs, descriptions, and extra category info. Then, we created a crawler that runs on mobile phones to automatically download mini-programs. In average, our tool $3,000$ mini-programs a day. We used two mobile phones to work together, and eventually we obtained \totalnum mini-program packages for analysis.    

% We implemented \textsf{CoffeCAN} in JavaScript with \texttt{esprima}\cite{esprima} to generate AST of mini-program source code, and Python to support multi-process processing. We performed our analysis on two Linux computers, each of which has 8 cores, Intel Core i7-8700 (3.20 GHz) CPUs and 16 GB RAM. It took 10 days for us to finish the analysis of the \totalnum mini-programs. 




\subsection{Evaluation Result}

It took \totaltime for our analysis tool to finish the extraction and analysis with the crawled mini-programs. %, and we successfully extracted and analyzed all the mini-programs with our tool. %
The most time consuming overhead is on the mini-program unpacking and code extraction, which takes an average of \totalavg seconds, whereas scanning the code to detect the hexstrings and APIs costs just several mini-seconds.
%
%the average time spent on scanning the mini-program code for vulnerability detection is \anaavg seconds.
With these tested mini-programs, we have identified \sessionstrings unique 32-byte hexstrings from the unpacked mini-program code, and with \numofsecrethour hours' \appsecret online validation, we have detected \leakedapps mini-programs (\leakedratio) that have leaked their \appsecret{s}, as reported in the last row of \autoref{tab:vuln_cat_score}.
%
%

Next, we seek to draw some observations and insights from the vulnerable mini-programs. Since the information we have for each mini-program can include (i) the category it belongs to; (ii) whether it is rated or not, if so, the specific rating score; (iii) the privacy sensitive information it accesses (e.g., \texttt{weRunData}, \texttt{phoneNumber}); (iv) the corresponding developer's information such as the company name if it is available; and (v) when the mini-program was last updated;  we then look into these five dimensions to better understand the distribution of the vulnerable mini-programs.


\ignore{
To gain a better understanding of the \appsecret exposure, we have conducted analysis over the \leakedapps vulnerable mini-programs, through which we have  further obtained more insights from them such as (I) the distribution 
of the ratings of the vulnerable mini-programs
(II) distribution of the categories of the vulnerable mini-programs,  (III) the distribution of the sensitive information these vulnerable mini-programs accessed, (IV) the distribution of the developer information of these vulnerable mini-programs, and (V) the distribution of vulnerable mini-program registration and updating date. 
}


%in the following sections, we first discuss the distribution of mini-programs we collected with respect to their categories and scores, followed by detailed discussion on vulnerable mini-programs, including the the sensitive information collected by these vulnerable mini-programs, categories of these vulnerable mini-programs, and finally the vulnerabile mini-programs developed by large companies.


%After analysis, we have collected 
%With the \leakedapps vulnerable mini-programs, we  

%Then, with the \wechat network APIs, we implemented a python tool to query the results from \wechat server and executed the script with \numofsecretthread threads. 

%\AY{Among the mini-programs, we collected The experiment run for \numofsecrethour hours, and as a result, we  among the \totalanalyzedapps mini-programs that have been successfully unpacked. 






% \sout{Among all our \totalapps collected mini-programs, our tool successfully unpacked \totalanalyzedapps mini-programs. Among these \totalanalyzedapps mini-programs, our tool identified \leakedapps mini-programs that had leaked their {\tt MK}s. In the following, we describe how we reached these results. In particular, we first discuss the performance of our tool (\S\ref{subsubsec:tool}), followed by the statistics of all our collected mini-programs (\S\ref{subsubsec:dataset}),  the statistics of these vulnerable mini-programs (\S\ref{subsubsec:flaws}).}\sout{, and finally the statistics of the vulnerable mini-programs from  the top fortune 500  Companies (\S\ref{subsubsec:top}).  }

% \begin{figure} 
% \centering
% \begin{minipage}[t]{0.495\linewidth}
% \includegraphics[width=\linewidth]{image/stat_x_time.pdf}
% \caption{Distribution of mini-program extraction time}
%  \label{fig:stat_exec}
% \end{minipage}
% % \hspace{1mm}
% \begin{minipage}[t]{0.495\linewidth}
% \includegraphics[width=\linewidth]{image/stat_analyze_time.pdf}
% \captionsetup{justification=centering}
% \caption{Distribution of mini-program analyze time}  
%  \label{fig:stat_analyze}
%  \
% \end{minipage}
% % \begin{minipage}[t]{0.495\linewidth}
% % \includegraphics[width=\linewidth]{image/stat_size.pdf}
% % \captionsetup{justification=centering}
% % \caption{Distribution of mini-program Size}  
% %  \label{fig:stat_ast}
% % \end{minipage}
% % \begin{minipage}[t]{0.495\linewidth}
% % \includegraphics[width=\linewidth]{image/stat_loc.pdf}
% % \caption{Distribution of mini-program line of codes}
% %  \label{fig:stat_loc}
% % \end{minipage}
% % \hspace{1mm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{image/all_miniapp_cat_score.pdf}
%     \caption{Heatmap of collected mini-programs, w.r.t. scores and categories} %\ZY{Black-white}
%     \label{fig:heatmap_all_scores}
%     \
% \end{figure}

%\texttt{WXUnpacker}~\cite{decomplier}

%The results of our extraction are shown as green lines in \autoref{fig:stat_exec} through \autoref{fig:stat_ast}. As shown in the figures, we observed that the extraction time elapsed to extract a mini-program package scatters from 10 seconds to 1 minutes, whereas the analysis time are relatively shorter (90\% of the mini-programs are analyzed within 5 seconds). The mini-programs we collected ranges from 12 to 20,045 lines of code, with the AST nodes ranging from 47 to 21,224. This indicates that we have collected not only tiny mini-programs with limited functions but also heavy mini-programs that provide complex functionalities. These



%\ZQ{fix this paragraph}




 

 

 

%As shown in the figures, compared with normal mini-programs, mini-programs that leaked \appsecret on average take less time to extract and to analyze, and contains less lines of codes and AST nodes. 








% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{image/company.pdf}
%     \caption{Relationships between developers and mini-programs \ZQ{This figure doesn't contribute much interesting knowledge and can be removed}}
%     \label{fig:developers}
% \end{figure}

% \begin{figure} 
% \centering
% \begin{minipage}[t]{0.463\textwidth}
% \includegraphics[width=\textwidth]{image/miniapp_cat_score.pdf}
% \caption{Heatmap of distribution in scores and categories among all mini-programs}
%  \label{fig:heatmap__all_score}
% \end{minipage}
% % \hspace{1mm}
% \begin{minipage}[t]{0.533\textwidth}
% \includegraphics[width=\textwidth]{image/miniapp_cat_prob.pdf}
% \captionsetup{justification=centering}
% \caption{Heatmap of user information access among all mini-programs}  
%  \label{fig:heatmap_all_access}
% \end{minipage}
% \end{figure*}
% \begin{figure*} 
% \centering
% \begin{minipage}[t]{0.463\textwidth}
% % \includegraphics[width=\textwidth]{image/miniapp_cat_score.pdf}
% \caption{Heatmap of distribution in scores and categories among vulnerable mini-programs}
%  \label{fig:heatmap_vuln_score}
% \end{minipage}
% \hspace{1mm}
% \begin{minipage}[t]{0.533\textwidth}
% \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_prob.pdf}
% \captionsetup{justification=centering}
% \caption{Heatmap of user information access among vulnerable mini-programs}  
%  \label{fig:heatmap_vuln_access}
% \end{minipage}
% \end{figure}
% \begin{figure} 
% \centering
% \includegraphics[width=\linewidth]{image/redirection_appsecret_string.pdf}
% \caption{Relationship of confirmed miniapps that leak appsecret as String variables}
%  \label{fig:redirection_appsecret}
% \end{figure}


% \begin{table}
%     \centering
%     \scriptsize
%     \aboverulesep=0pt
%     \belowrulesep=0pt
%     \begin{tabular}{r|l|l}
%     \toprule
% {\bf \# App}&\bf Domain&\bf Servive\\ \midrule
% 34&apis.map.qq.com&Tencent Map\\ 
% 14&api.map.baidu.com&Baidu Map\\ 
% 13&pingtas.qq.com&Tencent mini-program Analytics\\ 
% 11&wx.qlogo.cn&Tencent Avatar Logo\\ 
% 10&restapi.amap.com&AutoNavi Map\\ 
% 8&webim.tim.qq.com&Tencent Web Messaging\\ 
% 7&log.aldwx.com&Third-party mini-program Analyics\\ 
% 6&api.mch.weixin.qq.com&Tencent Payment\\ 
% 5&api.aikst.cn&mini-program Template Provider\\ 
% 5&yun.tim.qq.com&mini-program Third-paty Back-end\\ 
% 4&sandcash.mixienet.com.cn&mini-program Third-paty Back-end\\ 
% 4&thirdwx.qlogo.cn&mini-program Template Provider\\ 
% 4&tcb-api.tencentcloudapi.com&Tencent Cloud Base\\ 
% 4&wxapp.yz168.cc&mini-program Third-paty Back-end\\ 
% 3&glog.aldwx.com&Third-party mini-program Analyics\\ 
% 3&api.q.qq.com&Tencent Server API\\ 
% 3&www.hhhkd.top&mini-program Third-party Back-end\\ 
% 3&tongji.dcloud.io&Third-party mini-program Analytics\\ 
% 3&aip.baidubce.com&Baidu Cloud API\\ 
% 3&iploc.ywdier.com&Third-party mini-program Back-end\\ \bottomrule

%     \end{tabular}
%     \caption{Top 20 communication domains configured by vulnerable mini-programs\AY{Not Up To Date}}
%     \label{tab:vuln_domain}
% \end{table}



% In this paper, we mainly investigate two types of vulnerabilities: the appsecret leakage, and the session key leakage. For appsecrets, the 32-bit hex string can be leaked as hard-coded strings, or as part of the parameter of network URLs. To model the potential leakage of session keys, we investigate them from two aspects: on one hand, we investigate the network URL associated with user login and login token to find whether there are sensitive third-party network APIs that are potentially leaking session key. On the other hand, we track the network request APIs associated with sensitive APIs related to encrypted data: since the decryption are only supposed to be performed at back-end, if an API associated with encrypted data does not send their data to the back-end, then the mini-program may be processing the data at the front-end and the session key is being potentially leaked.

% \paragraph{(II) Vulnerable mini-programs and information accessed} 


% As shown in \cref{fig:heatmap_score}, in general, most of the vulnerable mini-programs are not being scored yet, indicating that they are fresh-created mini-programs or mini-programs not being used by a large amount of people. During our inspection, most of these mini-programs not being scored are regional lifestyle or shopping mini-programs, such as local hair saloons and local supermarket. Aside from these mini-programs, most of the affected and scored mini-programs are over 4.0 points, which indicates that the appsecret leakage may also affect very highly rated mini-programs. As to the categories, we discover that most of the mini-programs associated with appsecret leakages are education, games, lifestyle, shopping, and sports mini-programs. Interestingly, these mini-programs are much more likely to be associated with sensitive user data, such as user phone number to register account, and user sports data. 

% From the figure, we discovered that most of the popular mini-programs are shopping mini-programs, whereas the majority of the rest of the mini-programs are associated with shopping activities as well (e.g., the first food mini-program is actually a wine shop). This means many of these mini-programs with appsecret leakage are associated with actions such as shopping, payment, and coupon, which may be dangerous since the attacker can manipulate encrypted data to make profits or steal user information.


% \begin{table}
% \centering
% \scriptsize
% \aboverulesep=0pt
% \belowrulesep=0pt
% \begin{tabular}{c|c|c|c}
% \toprule
% \bf Developer&{\bf \# App}&\bf Avg. Ratings&\bf Type\\ \midrule
% \multirow{12}{*}{Yunlei}&Nanyang Transportation&4.7&Traffic\\ 
% &Xiangtan Transportation&-&Traffic\\ 
% &Transportation Code&4.5&Traffic\\ 
% &Shangqiu Transportation&4.7&tool\\ 
% &Enshi Transportation&4.7&Traffic\\ 
% &Ezhou Transportation&4.7&Traffic\\ 
% &Huaihua Transportation&4.8&Traffic\\ 
% &Jingzhou Transportation&4.7&Tool\\ 
% &Qianjiang Transportation&4.7&Traffic\\ 
% &Suzhou Transportation&4.7&Traffic\\ 
% &Yangzhou Transportation&4.7&Tool\\ 
% &Yichang Transportation&4.7&Tool\\ \cmidrule{1-1}
% \multirow{4}{*}{Nestle}&We Proudly Serve&4.6&Food\\ 
% &DolceGusto Member Center&4.6&Food\\ 
% &Nestle Member Club&4.4&Lifestyle\\ 
% &Nestle Customer Center&3.5&Shopping\\ \cmidrule{1-1}
% \multirow{3}{*}{Tencent}&Tencent Everyday Battle Chess&3.7&Games\\ 
% &Cool Run Everyday&3.5&Games\\ 
% &Tencent Billiards&4&Games\\ \cmidrule{1-1}
% \multirow{2}{*}{Shizhidong}&Fresh Graduate Jobs&-&Job\\ 
% &Graduate Job Hunting&-&Job\\ \cmidrule{1-1}
% \multirow{2}{*}{\tabincell{c}{Xindong\\Shikong}}&King of Music Guessing&3.4&Entertainment\\ 
% &Gala of Poetry&-&Tool\\ \cmidrule{1-1}
% \multirow{2}{*}{Hengzhao}&Chengtian Water Dispenser&4&Government\\ 
% &Yusheng Cloud Payment&4.1&Tool\\ \cmidrule{1-1}
% \multirow{2}{*}{Xingyi}&Traffic Rule Break Platform&4.6&Government\\ 
% &Traffic Rule Break Inquiry&4.7&Government\\ \cmidrule{1-1}
% \multirow{2}{*}{Juhe Zaisheng}&Juhe Yishoutang&-&Lifestyle\\ 
% &Juhe Yishouke&-&Lifestyle\\ \cmidrule{1-1}
% \multirow{2}{*}{Luyi Huadeng}&Luyi Huadeng&-&Shopping\\ 
% &Luyi Huadeng Photoelectricity&-&Shopping\\ \cmidrule{1-1}
% \multirow{2}{*}{Jiadianwang}&Changsha Electrial Appliances&-&Shopping\\ 
% &Shenzhen Electrial Appliances&-&Shopping\\ 
% \bottomrule
% \end{tabular}
% \caption{Developers with at least two vulnerable mini-programs}
% \label{tab:vuln_dev}
% \
% \end{table}




%vulnerable mini-programs from top companies and finally the (IV) distribution of vulnerable mini-programs from top Companies. 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_score.pdf}
%     \caption{Heatmap of vulnerable mini-programs, w.r.t. scores and categories\AY{200w}} %\ZY{Black-white}
%     \label{fig:heatmap_all_scores}
%     \
% \end{figure}
 
\paragraph{(I) Statistics of the Vulnerable Mini-programs w.r.t Their Categories} Almost all (97.96\%) mini-programs have been classified into a specific category in the \wechat mini-program store, as shown in \autoref{tab:vuln_cat_score}.
We can observe from the last column that 
%also presents the distribution of categories of all the identified vulnerable mini-programs, and from the distribution, we can observe that 
the percentage of the vulnerable mini-programs in each category are diversified, ranging from 0.01\% to 2.89\%, indicating that the \appsecret leakage problem is a system wide problem regardless of the mini-program categories, though some categories (e.g., e-learning, finance, and government) contain slightly higher percentage of vulnerable mini-programs. 

\ignore{
%
For instance, we can notice from \autoref{tab:vuln_cat_score}, we also discovered most of \appsecret leakages occur in reading mini-programs (193 out of 7,139, 2.70\%), followed by the finance mini-programs (72 out of 3,004, 2.40\%). 
Among all the rated mini-programs, the category with the most vulnerable mini-programs is government mini-programs (237 out of 8,848, 2.68\%).
Among all the unrated mini-programs, again, the category with the most vulnerable mini-programs is reading mini-programs (157 out of 5,440, 2.89\%). The results are worrisome. For example, many of these finance and reading mini-programs (e.g., buying online reading materials) are often involved with payment procedures, and the \appsecret leakage over these mini-programs can have serious impacts (\eg, an attacker can hijack the victim's account and shop for free). The \appsecret leakage occur in the government mini-programs may damage the reputation of government.\looseness=-1 
}

%As also shown in \autoref{fig:heatmap} (a) and \autoref{fig:heatmap} (b), from the perspective of categories distribution, we know that mini-programs under the category education, food, games, lifestyle, shopping, reading and  are with more vulnerable mini-programs 


%Due to the similar reason,  education, We can observe the mini-programs with high scores tend to be more vulnerable. \ZY{May need to fix this when data is ready} Although these mini-programs may provide satisfactory services to their users, they are still place their user sensitive data in danger. 

 
 
\paragraph{(II) Statistics of the Vulnerable Mini-programs w.r.t Their Ratings} As mentioned earlier, the rating of a mini-program could partially reflect its popularity and quality. %Among the total \totalanalyzedapps mini-programs, only one third of them appear to be more popular apps and they have the corresponding ratings with score from 0 to 5. 
Intuitively, the more popular a mini-program is, the less vulnerable it should be. However, as presented in \autoref{tab:vuln_cat_score}, 1.89\% of the rated mini-programs are actually vulnerable, whereas only 1.22\% of the unrated ones are. Therefore, we cannot simply link the vulnerability ratio with the popularity of the mini-programs, and we have to zoom in the ratings with other dimensions to draw insights. \looseness=-1

%
%\autoref{tab:vuln_cat_score} presents the distributions of ratings of mini-programs (The detailed distribution of the ratings of mini-programs can be found \autoref{tab:vuln_cat_score-full}  in of Appendix A). As shown in the table, 65.71\% identified mini-programs are not yet scored, due to the lack of enough rated users. These mini-programs are likely to be unpopular or with relatively lower quality. Among them, 1.22\% are vulnerable. With all mini-programs with ratings,  1.89\% of the mini-programs are vulnerable.  Although these mini-programs are popular,  they may still expose sensitive data in danger in that the \appsecret{s} are leaked. \looseness=-1

%However, if we zoom in the ratings with the specific category of the mini-programs, we 

To this end, we associate the ratings with the corresponding mini-app category, and plot a heatmap 
%
  %We have also plot the heatmaps 
based on the categories and the ratings of the detected mini-programs, as shown in \autoref{fig:vuln_miniapp_cat_score_ratio}, where the x-axis represents the specific category, and y-axis represents the percentage of the mini-programs in the corresponding rated mini-programs category, for each rating rage such as [0.0-0.9] and [1.0-1.9].
%
%\autoref{fig:vuln_miniapp_cat_problem_unrated_ratio} uses the categories as the x-axis and the percentage of vulnerable mini-programs in the mini-programs of a specific category with a specific rating as the y-axis, and
The higher the percentage is, the darker the color of that cell will be. % that represents the category with the rating will be. 
We can observe that the mini-programs with lower ratings tend to have a higher percentage of vulnerable mini-programs. This is reasonable, as the developers of mini-programs with higher ratings may spend more efforts on security and privacy to stay competitive, and maintain their advantages. Note that we also present the specific values of the ratings, the number of the vulnerable mini-programs, and its percentages among the rated mini-programs in \autoref{tab:vuln_cat_score-full} in Appendix for readers of interests. \looseness=-1
  
  
 % As shown in \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio}, the x-axis is the categories that the mini-program belong to and the y-axis is the ratings of these mini-programs. The more mini-programs fall into a specific category with a specific rating, the darker the color of the cell that represents the category with the rating will be. Similarly, \autoref{fig:heatmap} (b) uses the categories as the x-axis and the percentage of vulnerable mini-programs in the mini-programs of a specific category as the y-axis, and higher of the percentage is, the darker the color of the cell that represents the category with the rating will be.\autoref{fig:vuln_miniapp_cat_problem_unrated_ratio}



%vulnerable mini-programs with high ratings is more than the number of vulnerable mini-programs with low ratings. According to our analysis, this is because the number of mini-programs with higher ratings is greater than the number of the mini-programs with the lower ratings. However, as shown in \autoref{fig:heatmap} (b), we observe 









%However, in the rated mini-programs, we found that \ZY{XXX\%} of the mini-programs are rated a higher score (from 2.5 to 5.0). Although these mini-programs may provide satisfactory services to users, they may still expose their data in danger in that the \appsecret{s} are leaked.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{image/all_miniapp_cat_score.pdf}
%     \caption{Heatmap of collected mini-programs, w.r.t. scores and categories} %\ZY{Black-white}
%     \label{fig:heatmap_all_scores}
%     \
% \end{figure}



%\ZY{Pls do not forget to patch the numbers}

\paragraph{(III) Statistics of the Vulnerable Mini-programs w.r.t Their Accessed Sensitive Data} Recall that according to different sensitive information the mini-program accessed, the attacker can deploy different attacks against the mini-programs, and therefore, we present the statistics of different sensitive data these mini-programs accessed based on the API used. We identified that there have been multiple mini-programs that accessed various sensitive data including phone number, we run data, user information, mini-program share information, and private forwarding message, whereas we did not identify any cases accessing the user address and group enter info. 
%
%
Similar to how we plot \autoref{fig:vuln_miniapp_cat_score_ratio}, 
%Instead of using the rating range to plot \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio}, 
we use the accessed sensitive data in the y-axis to plot  \autoref{fig:vuln_miniapp_cat_problem_rated_ratio} and \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated}, where \autoref{fig:vuln_miniapp_cat_problem_rated_ratio} shows the distribution of the vulnerable mini-programs in the rated category and \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated} shows the unrated category. Note that the detailed distributions of the sensitive data access of rated mini-programs, unrated mini-programs, and all mini-programs can be found in \autoref{tab:apis-rated}, \autoref{tab:apis-unrated} and \autoref{tab:apis} in Appendix, respectively.

%what we have done in the analysis of distribution of ratings, we have also plot the heatmaps based on the categories and the access sensitive data of our collected mini-programs. To be more specific, \autoref{fig:vuln_miniapp_cat_problem_rated_ratio} uses the categories as the x-axis and the percentage of rated vulnerable mini-programs that access the specific type of data in the mini-programs of a specific category as the y-axis, while \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated} uses the percentage of unrated vulnerable mini-programs that access the specific type of data in the mini-programs of a specific category as the y-axis (The detailed distributions of sensitive data access of rated mini-programs, unrated mini-programs and all mini-programs can be found in \autoref{tab:apis-rated}, \autoref{tab:apis-unrated} and \autoref{tab:apis} of our Appendix A).  




%the distribution of sensitive information the mini-program accessed from perspective of the numbers and the percentage of the vulnerable mini-programs in both rated mini-programs (\autoref{fig:heatmap} (c) and \autoref{fig:heatmap} (d)) and un-rated mini-programs (\autoref{fig:heatmap} (e) and \autoref{fig:heatmap} (f)).  

%\autoref{fig:heatmap} (c) and \autoref{fig:heatmap} (d) present the distribution of the numbers of rated vulnerable mini-programs that access the sensitive information.

\begin{table}[]
\scriptsize
 \belowrulesep=0pt
 \aboverulesep=0pt
 \setlength\tabcolsep{3pt}
    
        \resizebox{0.485\textwidth}{!}{ 
\begin{tabular}{l|r|r|r|r|r|r}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Associated\\  Apps\end{tabular}}}                   & \multicolumn{2}{c|}{\textbf{Rated}}             & \multicolumn{2}{c|}{\textbf{Unrated}}           & \multicolumn{2}{c}{\textbf{Total}}             \\ \cmidrule{2-7}
 & \textbf{\# Companies} & \textbf{\# Apps} & \textbf{\# Companies} & \textbf{\# Apps} & \textbf{\# Companies} & \textbf{\# Apps} \\ \hline
>=20&0&0&7&162&7&162\\
19&0&0&4&76&4&76\\
18&0&0&3&54&3&54\\
17&0&0&0&0&0&0\\
16&0&0&2&32&2&32\\
15&1&15&1&15&2&30\\
14&0&0&1&14&1&14\\
13&1&13&1&13&2&26\\
12&1&12&5&60&6&72\\
11&2&22&3&33&5&55\\
10&0&0&4&40&4&40\\
9&3&27&6&54&9&81\\
8&1&8&9&72&10&80\\
7&1&7&21&147&22&154\\
6&1&6&21&126&21&132\\
5&6&30&41&205&46&235\\
4&5&20&113&452&118&472\\
3&20&60&226&678&245&738\\
2&91&182&956&1,912&1,038&2,094\\
1&1,525&1,525&17,044&17,044&18,569&18,569\\ \hline
Total&1,658&1,927&18,468&21,189&19,966&23,116\\
 \bottomrule


\end{tabular} 
}
    \caption{Numbers of vulnerable mini-programs associated with the same software development company.} 
    \label{tab:company}
\end{table}

A number of interesting observations can be drawn from these two figures. In particular, among the rated vulnerable mini-program category (\autoref{fig:vuln_miniapp_cat_problem_rated_ratio}), the government and entertainment mini-programs tend to access \texttt{PhoneNumber} most often. According to our analysis, these mini-programs usually use the users' phone numbers to authenticate users. %as their identifiers.  to provide the user services. 
%
As a result, these mini-programs could suffer from account hijack attacks.  
%
%We also find that the image mini-programs usually access the \texttt{Userinfo}, since the user information include the user's avatar, and these image mini-programs intend to load and beatify the user's avatar.   \ZQ{This explanation is very weak}
%
Also, we notice that social mini-programs usually access the promoting messages (by using \texttt{authPrivate}), which allows the mini-programs to promote products effectively on social networks. These information can be manipulated or collected by the attackers. 
In unrated vulnerable mini-program category (\autoref{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated}), we notice that
%We also observed that in \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated},  
most of the vulnerable mini-programs tend to use \textsf{WeRunData}, and finance category has the higher percentage to be vulnerable than other categories. % is used mostly by the unrated mini-programs across the categories. 
An investigation of why so many vulnerable mini-programs use \textsf{WeRunData} reveals that this data is often used to attract and reward users (e.g., when they daily step count reached certain threshold). However, with the leaked \appsecret, an attacker can arbitrarily modify the \textsf{WeRunData} of the corresponding mini-programs to easily gain fun and profit.

%one of the promotion means to attract their users, where the mini-programs providers will reward their users with coupons, as long as their daily step count reached the conditions. our attacks can work against these mini-programs by arbitrarily modifying  the \textsf{WeRunData} 


\ignore{
As shown in \autoref{fig:vuln_miniapp_cat_problem_rated_ratio}, in all vulnerable rated mini-programs, we seek to make some interesting discoveries. 
For example, we found that 

government mini-programs and entertainment mini-programs accessed \texttt{PhoneNumber} most often. According to our analysis, these mini-programs usually use the users' phone numbers as their identifiers to provide the user services. 
As a result, attackers may deploy account hijack attacks against them.  
We found that the image mini-programs usually access the \texttt{Userinfo}, since the user information include the user's avatar, and these image mini-programs intend to load and beatify the user's avatar.  Social mini-programs usually access the promoting messages (by using \texttt{authPrivate}), which allows the mini-programs to promote products effectively on social networks. These information can be manipulated or collected by the attackers.  We also observed that in \autoref{fig:vuln_miniapp_cat_problem_unrated_ratio-unrated},  \textsf{WeRunData} is used by the most of the unrated mini-programs across the categories. Interestingly, we found that \textsf{WeRunData} is usually served as one of the promotion means to attract their users, where the mini-programs providers will reward their users with coupons, as long as their daily step count reached the conditions. However, our attacks can work against these mini-programs by arbitrarily modifying  the \textsf{WeRunData}. 
}


%(c) and \autoref{fig:heatmap} (e),  share info is used most often by both rated and unrated vulnerable the mini-programs, and this is because the number of mini-programs that access this type of sensitive data is also the most when compared with the mini-programs that access other types of sensitive data. As shown in \autoref{fig:heatmap} (d), the percentage of rated vulnerable mini-programs that access the phone numbers stays relatively high. The phone number can be used to mount account hijack attacks, which can cause grave consequences against the mini-programs. The percentage of unrated vulnerable mini-programs that access \textsf{WeRunData} most often. The \textsf{WeRunData} data can be used to mount the data manipulation attacks. From the perspective of categories, we also obtained a lot of insights. For example,  Social  mini-programs also used   \textsf{WeRunData} very often, as the users of these mini-programs can show off their daily step counts to their friends. 
%  Finance mini-programs used \textsf{WeRunData} most often, since many mini-programs usually use a publicity stunt ``financial management''  attract their users by rewarding their users with coupons, as long as their daily step count reached the conditions. 


%and \ZY{HEATMAP4}, we can observe that for the rated mini-programs, the \texttt{WeRun} information (\werunratio) is used most often, followed by sharing information (\shareratio), user profile (user account information) (\profileratio), and phone numbers (\phoneratio). The distribution of unrated mini-programs are similar, which can be observed from \ZY{HEATMAP6} and \ZY{HEATMAP5}.


 


%The statistics of sensitive data access are also shown in \autoref{tab:apis-rated} (Rated mini-programs) and \autoref{tab:apis-unrated} (Unrated mini-programs). It can be observed that for the rated mini-programs, the \texttt{WeRun} information (\werunratio) is used most often, followed by sharing information (\shareratio), user profile (user account information) (\profileratio), and phone numbers (\phoneratio)
%\ZY{Use the 2w vulnerable mini-programs to compute the ratio, not the 200w.}\AY{This is NOT 200w. This is the total amount of mini-programs that accessed corresponding API, which makes well more sense than using total 2w as base number...}. \ZY{We are presenting the distribution of Sensitive Information Collected by Vulnerable Mini-programs. Not the distribution of mini-programs that access APIs. Therefore, I still think we should use the 2w vulnerable apps. }
%If the phone number is accessed by vulnerable mini-programs, attackers can fake their identity by changing the phone number in the encrypted data sent to mini-program cloud database. For share information, the attacker can fabricate the group id he shares the message to, so as to make profit by fooling the mini-program that gives user rewards for each separate group the user shares the mini-program to.
%Recall that in \S\ref{tab:wechatdata},  mini-programs can access up to seven types of sensitive data. However, in our experiment, we have not found any mini-programs that use group chat info and the user's addresses.  Our \autoref{tab:apis} only contains the information that is used by the mini-programs. This might be explained by \wechat's recent updates on deprecating these legacy APIs for developers:\AY{as the corresponding APIs are deprecated and removed from the documentations, the developers removed the APIs from their mini-programs.} \ZY{Then we should not explain them at all from the very beginning. How do you think?}


%\item \textbf{Distribution of Types of Sensitive Information Collected by One Vulnerable Mini-programs.}We have already known that the distribution of sensitive data collected by the vulnerable mini-programs (i.e., which type of  sensitive data is commonly used by the most of the vulnerable mini-programs). However, a mini-program may access multiple types of sensitive data, and we would like to measure how many types of sensitive data a single mini-program may access in the regular case. This is because the type of information reflects the attack surfaces of a mini-program (e.g., phone number can be used to deploy account  hijacking  attacks and \texttt{WeRun} can be used to deploy data manipulation attacks). \sout{To our surprise,  there are \noaccess vulnerable mini-programs that did not access any sensitive data.} \ZY{I don't know if it is a good idea to present the dataset here. The reviewers may argue against us that most of our ``vulnerable'' mini-programs are not ``vulnerable'' at all. I was thinking, for example, in the 4w vulnerable mini-programs, only 200 mini-programs does not invoke the APIs. Now, this becomes more than 80\% of our collected mini-programs, which is not good. }\AY{As we get rid of the histogram, we no longer need to mention this one.}

 
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_problem_count.pdf}
%     \caption{Types of sensitive data accessed by each vulnerable mini-program\AY{200w}}
%     \label{fig:dev_figure}
% \end{figure}

% \begin{table}[]
%     \centering
%         \scriptsize
%     \belowrulesep=0pt
%     \aboverulesep=0pt
%     \begin{tabular}{r|r|r}
%     \toprule
%         \# Associated apps & \# Developers &\# Total apps\\
%         \midrule
%         >=20&7&162\\
% 10-19&35&488\\
% 2-9&1,633&4,287\\
% 1&18,178&18,178\\
% personal&4,676&4,676 \\
% \midrule
% Total&24,529&27,791\\\bottomrule
%     \end{tabular}
%     \caption{Amount of vulnerable mini-programs associated with a company or personal developer}
%     \label{tab:company}
% \end{table}


 




% As shown in the table, the user information (\eg, user's avatar and gender) gets used most often (\inforatio). The attacker can use the leaked \appsecret and malware to steal the sensitive information from a victim. Aside from the user information, the second most used sensitive information is phone numbers. With the leaked \appsecret, the attacker can manipulate the phone number, and deploy the account hijack attacks against these mini-programs. We currently have not found any mini-programs used the social information or shipping addresses.

\paragraph{(IV) Statistics of the Vulnerable Mini-programs  w.r.t Their Developers} 
%As  mentioned  earlier,   not all developer information that is available, and at the time of writing, we have collected \ZY{XXX} records of the developer information, through which we can better understand why there are so many vulnerable mini-programs. Intuitively,  one sloppy 
Next, we aim to understand how many developers have produced the vulnerable mini-programs, and how often they made these mistakes. 
%
%One developer may make the same mistake more than once (e.g., developing multiple mini-programs with \appsecret leakage), and therefore, we would like to investigate how many vulnerable mini-programs may be associated with the same developer in general. 
However, in the meta-data of the mini-programs, \Tencent does not provide the individual developer's personal information, and instead \Tencent just uses a string ``individual developer'' to label all the developer information of the mini-programs that are produced by the individual developers. Therefore, in the following, other than 4,676 mini-programs that have been developed by the individual developers, we present the  %cannot determine whether two mini-programs with the same information (both labeled `individual developer'') are developed by the same individual developer. Therefore, we 
%only present the distributions 
statistics of the vulnerable mini-programs that are produced by the corresponding companies. 


In particular, we have collected the developer information of the companies of the vulnerable mini-programs if they are available, and \autoref{tab:company} shows the statistics based on how many mini-programs have been associated with the same company. We can notice that the majority of the companies developed just a single vulnerable mini-program, and but sometimes one company can produce multiple vulnerable mini-programs (e.g., a company called `Suzhou Yutianxia' has produced 30 vulnerable mini-programs according to the data we have). % vulnerable mini-programs associated with a single company may reach up to 30 (by a company called `Suzhou Yutianxia'). 
%
%One reason we found is these companies tend to use templates to quickly generate the mini-programs
%{According to our manual analysis, we have noticed that these companies usually use the code templates to quickly generate the mini-programs, and these templates may be problematic, which requires the \appsecret to be hardcoded into the mini-programs. This may be why they have developed so many vulnerable mini-programs.} \ZY{Need to be confirmed by Allen} 
Interestingly, we also found that the mini-programs produced by companies with multiple vulnerable ones tend to be unrated. For example, as shown in the first row of \autoref{tab:company}, there are seven companies, each of which has developed more than 20 vulnerable mini-programs, and none of these mini-programs are rated. 

%As discussed, the companies with rated mini-programs intend to stay competitive, and value the security and privacy.   


Surprisingly, we also found that not only small companies produce vulnerable mini-programs, but also large software vendors, even including \Tencent itself. %  such mistake, large software vendors also leak their \appsecret{s} in their mini-programs in a row. 
%
For instance, we noticed \Tencent has released  277 mini-programs, but 14 of them (5 rated, and 9 unrated) are actually vulnerable. These mini-programs are likely developed from different departments of \Tencent. % A deep investigation with these mini-programs reveals that these mi
There are also several other well-known companies that have vulnerable mini-programs. For instance, we we have found 7 vulnerable mini-programs from L'oreal Hong Kong, 6 from Jing Dong, and 6 from Nestle China. These data just again confirms that it is a system wide problem.


\ignore{

As shown in \autoref{tab:companydeveloper} in our Appendix A, we have listed 40 the companies that have leaked their \appsecret(s) (ranked by the number of vulnerable mini-programs programmed by the company).  
%
It can be observed that in these vulnerable mini-programs, 14 are from Tencent. In fact, in our experiment, we also observed that 7 mini-programs are from L'oreal, 6 mini-programs are from Jing Dong, and 6 mini-programs are from Nestle. These companies are not listed due to the page limit. The companies, however, may develop many mini-programs other than the vulnerable ones. Based on our manual efforts and our collected mini-program developer information, we also found that for the large companies, they usually occasionally make mistakes. 

For example, Tencent has released  277 mini-programs, and only 14 are vulnerable. However, as mentioned earlier, ``Suzhou Yutianxia'' have developed 30 mini-programs, and we have not collected any non-vulnerable mini-programs in our dataset.   
}
% In \ZY{TABLE}, we also collected the non-vulnerable mini-programs from these companies (based on \ZY{XXX} collected developer information records), and calculate the ratio of the vulnerable mini-programs in all their developed mini-programs.  It can be observed that in general, larger companies made few mistakes when compared with the small companies. 

%developer inforamtion by associating the mini-programs with the same company together.   

%For a company that developed vulnerable mini-programs, we search all the mini-programs that have developed by these companies in the developer information, and group them by two categories, i.e., the rated mini-programs and the unrated mini-programs.  \autoref{tab:company} shows the results.  Overall, we found that \ZY{XXX} companies developed vulnerable mini-programs, and among them, \ZY{XXX} have developed more than one vulnerable mini-programs. Interestingly, we found a company named  `Suzhou Yutianxia' has developed 30 mini-programs.   


%developed more than one vulnerable mini-programs. Next,

%Overall, the companies that developed rated mini-programs have made fewer mistakes when compared with the companies that developed unrated mini-programs. As discussed, these companies with  

%We found that the number of vulnerable mini-programs associated with a single company may reach up to 30 (by a company called `Suzhou Yutianxia'),  and the developer with multiple vulnerable mini-programs are usually software outsourcing companies. We also observed that the rated mini-programs has fewer rated 

%For the rated mini-programs, this number becomes \ZY{XXX} and there are XXX unrated mini-programs can be associated with one developer. 




% Interestingly, we identified that not only large vendors make such mistake, invididual or small companies will also likely to expose their \appsecret{s} in multiple mini-programs.
% For instance, as reported in \autoref{tab:vuln_dev},  we found that Hubei Yulei incorporation has released 12 mini-programs and all of them are vulnerable.

%{As discussed in previous sections, a developer may develop multiple mini-programs with \appsecret leakage. As such, we investigated how many vulnerable mini-programs may be associated with a specific developer. As shown in \cref{fig:}, we found that although many vulnerable mini-programs are associated with a single developer, there are still many developers that developed multiple vulnerable mini-programs in a row --- and we even found that there are two developers developed 7 vulnerable mini-programs. This indicates that the \appsecret leakage may be propagated by a sloppy developer into multiple mini-programs, which threatens the mini-program ecosystem.}
% developers Interestingly, we identified that not only large vendors make such mistake, invididual or small companies will also likely to expose their \appsecret{s} in multiple mini-programs. For instance,} as reported in \autoref{tab:vuln_dev}, % and make the same mistake (\ie, the \appsecret leakage) more than once. 
% we found that Hubei Yulei incorporation has released 12 mini-programs and all of them are vulnerable, although these mini-programs may have different functionalities (\eg, some of them are traffic mini-programs and others are the tools). \looseness=-1  


% \begin{table}[]
% \scriptsize
%  \belowrulesep=0pt
%  \aboverulesep=0pt
%  \setlength\tabcolsep{1.5pt}
% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Associated\\  apps\end{tabular}}}} & \multicolumn{3}{c|}{\textbf{Rated}}                                                                                                                                                                                    & \multicolumn{3}{c|}{\textbf{Unrated}}                                                                                                                                                                                 & \multicolumn{3}{c}{\textbf{Total}}                                                                                                                                                                                   \\ \cline{2-10} 
% \multicolumn{1}{|c}{}                                                                                        & \multicolumn{1}{c|}{\textbf{\# Comp}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Vuln \\ apps\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Total \\ apps\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\# Comp}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Vuln\\ apps\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Total \\ apps\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\# Comp}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Vuln\\ apps\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Total \\ apps\end{tabular}}} \\ \hline
% \textbf{{[}20,)}                                                                                              &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \textbf{{[}15,20)}                                                                                            &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \textbf{{[}10,15)}                                                                                            &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \textbf{{[}6,9)}                                                                                              &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \textbf{{[}2,5)}                                                                                              &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \textbf{1}                                                                                                    &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \textbf{Total}                                                                                                &                                       &                                                                                       &                                                                                        &                                       &                                                                                      &                                                                                        &                                       &                                                                                      &                                                                                        \\ \hline
% \end{tabular}
% \end{table}


\paragraph{(V)  Statistics of Vulnerable Mini-program w.r.t Their Latest Update} The meta-data of a mini-program contains the latest updated timestamp. Therefore, we can use this information to understand how long this \appsecret leakage vulnerability has lived. 
%
%Finally, we would like to understand the relationship between the latest update date and the vulnerable mini-programs. 
%(i.e., the \appsecret leakage become more serous or it is mitigated across time, and whether the identified problem has been existed long ago) . 
To this end, we first collected the timestamp of the latest update of all of the vulnerable mini-programs,  then grouped them together based on their latest update month, and finally count the numbers of vulnerable mini-programs in each group. \autoref{fig:company-vuln} shows this result. We can observe that (1) this vulnerability has been there since the first date when \Tencent introduced the mini-program into \wechat (e.g., a mini-program named WuiGuang Calendar that was released January 2017 has leaked the \appsecret and it never gets updated); (2) Both rated and unrated vulnerable mini-programs have long lived, and there is no strong correlation between their distributions; and (3) The number of vulnerable mini-programs introduced (or updated) in each month reached the peak in January 2019 and had started to decline since then. 

%many of the rated and unrated mini-programs that updated long time ago  are still vulnerable (e.g., an mini-program named GuiGuang Calendar that was  released January, 2017 leaked the \appsecret), which indicates that the \appsecret leakage problem exist across time regardless of the ratings of mini-programs. 
%We also observed that for both of the rated and unrated mini-programs, 
%the emergence of vulnerable mini-programs grew rapidly in the first years, with the monthly growth up to around 200 mini-programs.  
%(i.e., the \appsecret leakage become more serous or it is mitigated across time, and whether the identified problem has been exist ) in the very beginning of \wechat mini-program paradigm, the problem of leaked \appsecret{s} increased drastically. This is likely because the amount of mini-programs started to increse. We also observed that with the quarter increased vulnerable mini-programs reached top in the second quarter of 2018 (2018-04 to 2018-06), the amount of added vulnerable mini-programs is constantly on the decrease. This reflects more and more developers started to value the mini-program security. 



%\ZY{I don't fully understand why we present both the distribution of registration date and the updating date. The registration should be enough, right? Why we need the updating date and what is the difference? Or, should we only present the updating date? I am confused here. May be we should somehow differentiate them and better motivate it.  }
%(I would take some time looking for the potential reason for it. Is it update of mechanism? or the review process?) \ZY{I will fix this after you updated the data}

% \item {\bf Distribution of Vulnerable mini-programs from the Fortune 500 Companies} 
% \label{subsubsec:top}
% \AY{To identify problems related with high-profile companies, we first generated a dictionary containing keywords from the Fortune top 500 companies. Then, we matched the mini-program names to filter out mini-programs we are interested in, both for all mini-programs and mini-programs identified to contain \appsecret exposure. In total, \topcompanyapps mini-programs are identified, with \topcompanyappsvuln of them are vulnerable. With these data, we present the distribution of vulnerable mini-programs and the ratio of all related mini-programs in \cref{fig:company-vuln}. As shown in the figure, }

 

% \begin{figure*}
%     \centering
% \begin{minipage}{0.48\linewidth}
% \includegraphics[width=\linewidth]{image/reg_histo.pdf}
%     \caption{Distribution of vulnerable mini-programs with respect to the registration dates}
%     \ZY{The color does not look good}
% \end{minipage}
%     \begin{minipage}{0.48\linewidth}
% \includegraphics[width=\linewidth]{image/upd_histo.pdf}
%     \caption{Distribution of vulnerable mini-programs with respect to the most recent update dates(barchart with rated/unrated)}
% \end{minipage}
%     \label{fig:company-vuln}
% \end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/upd_histo.pdf}
    \caption{The number of the vulnerable mini-programs with respect to their most recent update dates %(barchart with rated/unrated)}
    }
    %\ZY{The color does not look good}\AY{will change to a lighter color, in blue and orange}}
    \label{fig:company-vuln}
\end{figure}


%that are possibly used to register account or create orders. This is surprising since the mini-program developers involved with such important functionalities overlooked the explicit warning in the \wechat official documentations of not leaking these \appsecret, and proceed to exposing their \appsecret to the front-end. Besides, it is also interesting that although the documentation indicates that the involved mini-program will be taken off the market if \appsecret leakage is detected, there are still over 2.1\% of the mini-programs that leaked \appsecret but still appear on the market. This indicates that the mini-program vetting and \appsecret leakage checking process of mini-program framework still needs to be improved.



%in different categories may access different kinds of user information. For example, there are more shopping and lifestyle mini-programs that access phone number and user information, since the mini-programs often require user information to perform purchasing and payment. For weRunData, however, most of the mini-programs that access these information are sports and tool mini-programs. For example, we found a mini-program that require wechat sports data to monitor whether a user is sticking to the fitness plan, and a mini-program called `earn scores' to earn scores by walking and completing tasks for purchasing presents.

 


% Aside from 2 mini-programs that does not access any sensitive encrypted information, the mini-programs accessed various information including phone number, user info, share info, and weRun data. The functionalities of these mini-programs cover a wide fields, ranging from online shopping and membership to travelling and sports. As mentioned in previous texts, most of these vulnerable mini-programs are associated with online shopping and membership coupons, which can be potentially exploited by attackers to make profit if they require user information or phone number for logging in. Besides, we also found that membership mini-programs may require user share info for which \wechat group chat the user is being navigated from. These membership mini-programs may motivate existing members to share their mini-programs to attract more fresh users, and may give special discount or coupons for them. As such, these mini-programs may also be vulnerable since attackers can modify the group information in the share info. 




 
 

 






% %\subsection{Case Studies}
% \paragraph{Account Hijacking} Vulnerable mini-programs that access user phone number to register or log in user accounts are subject to account hijacking attacks, where attackers use the \appsecret to query session key for modifying login information to fake themselves as arbitrary account. In this paper, we have demonstrated this attack in \cref{sub:attack}: since the attackers can trigger user log in access either via re-entering the mini-program or by hooking and executing \texttt{wx.login} API, the attackers can immediately trigger user login to get the login token to refresh the \appsecret when \appsecret is updated. Among the \leakedapps vulnerable mini-program, one-third (51) are associated with this sensitive information, and the affected mini-programs are not limited to shopping. Aside from shopping mini-programs, we also found \appsecret leakage with phone number access among education, travelling, and public transportation mini-programs (e.g., bus e-cards). As such, the mini-program developer should be careful with the \appsecret and phone number access to avoid their mini-programs from being exploited by malicious users, which may cause loss of the company or user privacy.

% \paragraph{User Information Manipulation} Aside from phone numbers, a number of mini-programs require user information, such as the user account nickname, avatar, and region, to identify users. However, if the \appsecret is leaked, the attacker can change his or her user information, such as user nickname, gender, or user region, to perform phishing attack on other users with fake identity. We noticed that, among the vulnerable mini-programs, aside from shop mini-programs, there are games and lifestyle mini-programs. For game mini-programs that require two or more players (e.g., Tencent Battle Chess), attackers can approach other users with fake identity and avatars to scam the victim for money, although the account information in the mini-programs are believed to be verified by \wechat. 
% % For lifestyle mini-programs, we found a group mini-program that can be used to launch a lottery draw or reward point collection activity where users can receive profits or gifts. If the account information is modified, this may also

% \paragraph{User Sports Data Manipulation} The user sports data may also leak the user privacy if improperly used by mini-programs, or used to cheat in sports ranking activities. For example, we observed a mini-program developed by Behang University that integrates a daily sports ranking among other users. Some colleges or classes may require the students to perform certain sports exercises, give awards to top runners or pose punishments on last runners, the users can use the leaked appsecret to modify his/her sports data to cheat. Aside from cheating, we also observed that many mini-programs advocating `low carbon lifes' or `citizen excercises' give users score points if he/she achieves certain amount of sport activity (e.g., a certain amont of footsteps walks everyday) which can be used for getting gifts. Although we have not found \appsecret leakage in these case yet, but if the \appsecret is leaked, the mini-programs can be abused by manipulating the sports data sent to the server.

%\paragraph{(III) Vulnerable mini-programs from top companies} 

% which is surprising because the documentation of \wechat mini-program has warned the developers not to leak these \appsecret in the official documentation, but the developers still insisted on leaking these essential \appsecret. Since the \appsecret serves as a master password to verify the identity of mini-program owner, this leakage makes the mini-programs vulnerable to various Coffee attacks.


% On top of the mini-program scores, we also grouped the affected mini-programs according to accessed user information in \cref{fig:heatmap_vuln}. We found that a majority of mini-programs that leaked appsecrets are associatede with user's phone number access. This is likely because of the phone number is used by mini-programs to register and log in user account. For example, when entering Nestle member center, the mini-program will ask the user for his/her personal information access. Then, the mini-program will promt the user to log in or register to receive discounts or send promotions to the new user.


% We first captured all string values that appear in the form of 32-bit hex string, and then we send this value and the corresponding mini-program ID to \texttt{api.weixin.qq.com/cgi-bin/token} to validate whether the string value is a real appsecret. 



% \paragraph{(III) Redirected mini-programs} Interestingly, aside from the mini-program credential leakage, we also observed that these vulnerable mini-programs are redirecting to other mini-programs. If the account info can be fabricated in the vulnerable mini-program, then the victim being redirected to may suffer from the attack too if extra data is being attached and processed during the redirection. 

% \paragraph{mini-programs that are being redirected by large amount of mini-programs} As shown in \cref{fig:redirection_appsecret} and \cref{fig:redirection_key}, we observed that there are large clusters where multiple mini-program redirect to a center mini-program. For instance, in the top left of \cref{fig:redirection_appsecret}, there are 118 vunerable mini-program being redirected to by \AY{Miniapp A}, which itself does not leak appsecret. Similarly, in \cref{fig:redirection_key}, there are three massive clusters with over 200 mini-programs. This may be mini-programs that are using a same set of mini-program template or third-party cloud service that leaked the appsecret in the template or the session key in their session key network request. As such, the credential leakage may be propagated via copy-paste or mini-program template. In the next section, we will explain more details about the implication of these cases with real world cases.

% \paragraph{mini-programs that redirect to each other} As shown in \cref{fig:redirection_appsecret}, we observed that there are some small clusters where mini-programs redirects to each other. For example, in the middle of \cref{fig:redirection_appsecret}, there is a cluster where 11 vulnerable mini-program redirects to each other. As shown in \cref{tab:appsecret}, this cluster belongs to the 10 mini-programs with 11 referrers that appear very similar in the mini-program name and the Javascript code. Therefore, it is very possible that all the 11 mini-programs are developed by a same vendor, and the vendor is possibly developing many duplicated mini-programs to escape from mini-program auditing and management.


% \AY{EVALUATION DATA}

% Normally, the session key is generated by the back-end with login token returned by \texttt{wx.login}, and this session key is used for decryptions of user sensitive data. Therefore, since the session key cannot be leaked to the front-end, all sensitive encrypted data has to be sent back to the back-end. To investigate the potential leakage, we investigate three problems in this section. Our study shows that there is a concerning amount of mini-programs that are highly possible to either leak the session keys via sensitive network URLs, or process encrypted data with leaked session key because there is no associated network requests found after sensitive encrypted data is being acquired.




% \begin{table*}[]
% \scriptsize
% \belowrulesep=0pt
% \aboverulesep=0pt
% \setlength\tabcolsep{1.5pt}
%     \centering
%     \begin{tabular}{c|c|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
%     \toprule
%      \multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\rot{business}}&\multicolumn{1}{c|}{\rot{education}}&\multicolumn{1}{c|}{\rot{entertainment }}&\multicolumn{1}{c|}{\rot{finance}}&\multicolumn{1}{c|}{\rot{food}}&\multicolumn{1}{c|}{\rot{game}}&\multicolumn{1}{c|}{\rot{government}}&\multicolumn{1}{c|}{\rot{health}}&\multicolumn{1}{c|}{\rot{images}}&\multicolumn{1}{c|}{\rot{job}}&\multicolumn{1}{c|}{\rot{lifestyle}}&\multicolumn{1}{c|}{\rot{reading}}&\multicolumn{1}{c|}{\rot{shopping}}&\multicolumn{1}{c|}{\rot{social}}&\multicolumn{1}{c|}{\rot{sports}}&\multicolumn{1}{c|}{\rot{tool}}&\multicolumn{1}{c|}{\rot{traffic}}&\multicolumn{1}{c|}{\rot{travelling}}\\ \hline
%      \multirow{11}{*}{\rot{back-end}}&\multirow{9}{*}{\tabincell{c}{session\\key}}&\texttt{login}&14,744&48,810&3,622&1,526&34,422&21,140&11,416&9,956&454&6,164&86,823&2,426&132,115&6,486&3,849&33,303&10,124&1,166\\\cline{3-21}
%   &&\texttt{getUserInfo}&11,332&38,231&3,248&1,164&26,322&23,203&8,489&7,307&380&4,972&64,401&1,314&9,5916&5,522&3,180&29,032&7,678&955
% \\\cline{3-21}
%       &&\texttt{getUserProfile}&30&86&30&4&40&8&28&45&2&56&197&5&265&18&6&47&18&1\\\cline{3-21}
%       &&\texttt{getUserInteractiveStorage}&&&&&&\\\cline{3-21}
%      &&\texttt{getWeRunData}&161&280&42&23&120&105&102&81&5&21&226&17&609&62&1040&428&34&6\\\cline{3-21}
%      &&\texttt{getGroupEnterInfo}&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\\\cline{3-21}
%      &&\texttt{getShareInfo}&&&&&&\\\cline{3-21}
%      &&\texttt{chooseInvoice}&4&3&0&0&0&0&3&1&0&0&9&0&3&0&2&16&1&0\\\cline{3-21}
%      &&\texttt{request}&&&&&&\\\cline{2-21}
%      \bottomrule
%     \end{tabular}
%     \caption{Security-related APIs and Values\AY{Will fix that later}}
%     \label{tab:apis}
% \end{table*}

% \begin{table}[]
%     \centering
%     \scriptsize
%     \begin{tabular}{r|c|c}
%     \toprule
%     \# of mini-program a specific mini-program redirects to& \# app & \% app\\
%  >10&50&0.02\\
% 9&25&0.01\\
% 8&31&0.01\\
% 7&29&0.01\\
% 6&262&0.10\\
% 5&599&0.23\\
% 4&613&0.23\\
% 3&2920&1.11\\
% 2&34055&12.89\\
% 1&225612&85.40\\
% total&264196&100.00\\\bottomrule
%     \end{tabular}
%     \caption{Amount of mini-programs each mini-program redirects to\AY{Would like to remove}}
%     \label{tab:redirection}
% \end{table}


% \section{Case Study and Root Causes}
% \subsection{Coffee Attack}
 





==> paper/04_design.tex <==
\section{Detection}
The add-on security measures may unconsciously introduce various vulnerabilities that make mini-apps are subject to \textsf{COFFEE} attacks. To measure and understand the impact of the \textsf{COFFEE} attacks, we design and implement our detection tool, named \textsf{COFFEE} atta\textsf{C}k \textsf{AN}alyzer (\textsf{COFFEECAN}), to perform a large-scale analysis of mini-app vulnerabilities. In the following, we will explain how \textsf{COFFEECAN} detects the vulnerabilities that may lead  \textsf{COFFEE} attacks by using concerted examples as shown in \autoref{fig:code}.
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{image/code.pdf}
    \caption{Examples of codes related to Coffee attack}
    \label{fig:code}
\end{figure*}
%  \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/tool.pdf}
%     \caption{The CoffeeCAN workflow \ZY{TODO}}
%     \label{fig:tool}
% \end{figure}
\subsection{Detecting Bluetooth Mis-configuration}
\paragraph{Example I: Bluetooth Mis-configuration} As shown in Case 1 of \autoref{fig:code}, when configuring Bluetooth peripheral servies with \texttt{addService(service)} (line 21), developers can enable or disable Bluetooth encryption with the parameters \breakabletexttt{writeEncryptionRequired} and the parameter \breakabletexttt{readEncryptionRequired} of \texttt{service} parameter by setting them to \texttt{true} or \texttt{false} (line 18-19). To detect the values set to these two parameters, the most intuitive way is to locate the \texttt{service} parameter when \texttt{addService} is invoked, and use a simple string marching of the two parameters \breakabletexttt{writeEncryptionRequired} and  \breakabletexttt{readEncryptionRequired} in the de-complied JavaScript code. However, this approach practice is not feasible when applied to heavily obfuscated mini-app front-ends. For example,  a developers may 
not directly define a \texttt{service} object and pass it to \texttt{addService}. Instead, the developer may give the object a random name (\eg, \texttt{bleservice} in line 16 of our example), and locate the variable not close to the API \texttt{addService}. 

%but define them as an arbitrary variable (\texttt{bleservice} in line 16) and refer to it.

\paragraph{Our Approach} We perform a data flow tracking on top of the control flow obtained from the Abstract Syntax Tree (AST). To keep tracking the all the declared variables, we assign each function expression node in the AST with additional information such as what variables are declared in the function, what other functions get called within the function,  and what the parameters are passed into those called functions. For instance, when traversing code fragments of 
\texttt{addService} at line 02, we observed two declared variables: \texttt{a} at line 05, and \texttt{bleservice} at line 16. We also observed two functions get called: \texttt{b["a"]} at line 09, with an object as parameter, and \texttt{addService} at line 21, with a parameter \texttt{bleservice}. Since \texttt{addService} is the API of interest, we then examine the structure of referred \texttt{bleservice} declared in line 16, and associate the values of its parameters through searching of the AST. Finally, we discover that both the two parameters of \texttt{bleservice} are set to \texttt{false}, which indicates that this mini-app contains Bluetooth mis-configuration that makes it vulnerable to \textsf{COFFEE} attack.

% Our idea is to use the backward slicing to traverse the data flow graph of mini-app, where data dependencies are inferred from the program states and the generated data flow graphs. To that end, we first identify the names of security-related APIs, and then traverse from their successors (e.g., the code fragments that use the return values of the API) 
\subsection{Detecting Missing Verification}
\paragraph{Example II: Cross-User or Cross-Mini-app missing Verification} As discussed in \S\ref{sec:back}, there are two types of verification in general: the cross-miniapp redirection verification to identify which mini-app the current mini-app is redirected to, and the cross-user sharing verification to check whether the current user has privileges. As shown in Case 2 of \autoref{fig:code}, when entering mini-apps (i.e., in the \texttt{onShow} function at line 01), the developers can check whether the user that enters the mini-app is the first-hand user by invoking \textsf{authPrivateMessage} at line 04. If so, \textsf{authPrivateMessage} enters the \texttt{success} branch at line 06. Similarly, developers can check whether the mini-app is being redirected to from a trusted mini-app by getting the \texttt{appId} from \texttt{referrerInfo}. To detect cross-user verification is similar to detecting Bluetooth mis-configuration, as we only identify the invocation of \textsf{authPrivateMessage}. However, we observed that the verification process in the real world can be more sophisticated due to the obfuscation or programming practice. For instance, in line 11 of, aside form checking \texttt{appID}, the developer also performed a series of null checking of \texttt{onShow} function argument \texttt{t}, \texttt{referrerInfo} as well as \texttt{scene} (the scene value is associated a set of conditions of mini-app launch, e.g., 1038 refers to the launch via a cross-user redirection). We have to resolve the relationship of these checking processes. 


%, when the user is launching the mini-app via secret sharing feature.


%\paragraph{(1) Missing cross-user sharing verification} The developers can send private sharing link by calling \texttt{updateShareInfo} and setting the \texttt{isPrivateMessage} parameter to \texttt{true}, and then check whether the user that enters the mini-app is the first-hand user by invoking \textsf{authPrivateMessage} that returns the verification result. As such, identifying the cross-user sharing verification is similar to that of finding misconfigurations in Bluetooth. For mini-apps that issue secret sharing, we can find the invocation of \texttt{updateShareInfo} and examine whether the parameter is \texttt{true} via data flow tracking. For whether the mini-app performs verification, we can check whether the \texttt{authPrivateMessage} is invoked.

%\paragraph{(2) Missing cross-miniapp redirection verification} As shown in case 2 of \autoref{fig:example}, when entering mini-apps (i.e., in the \texttt{onShow} function at line 01), the developers can check whether the mini-app is being redirected to from a trusted mini-app by getting the \texttt{appId} parameter from the object \texttt{referrerInfo}. However, we observed that the cross-miniapp checking in the real world may be more complex. For instance, in line 11, aside form the \texttt{appID} checking, the developer performed a series of null checking of \texttt{onShow} function argument \texttt{t}, \texttt{referrerInfo} as well as \texttt{scene} (the scene value is associated a set of conditions of mini-app launch, e.g., 1038 refers to the launch via a cross-user redirection).

\paragraph{Our Approach} Fortunately, we observe that although the cross-mini-app verification may occur in various AST nodes (\eg, in \texttt{if} statements, \texttt{for} statements,  \texttt{loop} statement), they all involve logical expressions with \texttt{==} or \texttt{in} operator, since the verification has to be performed by comparing the variable of interest (e.g., \texttt{appId}) with one or multiple mini-app ID strings. Therefore, to detect the occurrences of the validation, we can  we analyze each logical expression involving \texttt{referrerInfo} since it indicates the mini-app used information from the mini-app referrer, and then check if there is a \texttt{==} or \texttt{in} operator associated with \texttt{appId} and one or multiple mini-app ID string.



%when the code fragment is represented as the Abstract Syntax Tree (AST), the data to be verified is one leaf node of the AST, by analyzing the AST, we can easily determine whether verification is involved.  Therefore, to detect the occurrences of the validation, we can first use the solution introduced in \textbf{S1} to identify the API of interest, and then parse the relationship between the APIs using their Abstract Syntax Tree (AST) representations.  

%Although the verification may occur in various AST nodes (in if statements, for loops, while loops, etc), they all involve logical expressions with \texttt{==} or \texttt{in} operator, since the verification has to be performed by comparing the \texttt{appId} with one or multiple mini-app ID strings. As such, to identify the mini-app redirection checking in the complex real-world cases,

\subsection{Detecting Key Leakage}

\paragraph{Example III: Key leakage}
 In general, there are two types of keys can be leaked, \ie, \texttt{Appsecret} and session key.  
\texttt{Appsecret} can be considered as the master key of the mini-app ecosystem,  which can be used to fetch a valid session key. Developers may hard-coded these \texttt{Appsecret} into front-end due to the misunderstanding of the official document, as shown in Case 3 of \autoref{fig:code} (line 03).  Session key is used to encrypt the sensitive data transferred between the mini-app front-end and its back-end. Although the session key will be updated every time the user logins the back-end of the mini-app, some developers may mistakenly implement a interface that is used to obtain a session key at the front-end of the mini-app, resulting in the leakage of the session key, as shown in Case 3 of \autoref{fig:code} (line 03). Therefore, our tool must handle these two types of keys. For the \texttt{Appsecret}, as it has a fixed format (\ie, it is a 32-digits long string containing the hexadecimal digits), the most straightforward way to detect of \texttt{Appsecret} the leakage is to grep the decomplied JavaScript code and uses the regular expression to match it. However, such a method is subject to false alert, since many strings in a mini-app have the same format (\ie, the index of online database).  For the session key leakage, we have to design a way that can automatically identify the customized interfaces, which can be challenging, as different developers can have different programming practice and gives the interface various names and parameter lists.    


%In general, there are two types of keys that can be leaked: \texttt{appsecret} and session key.  \texttt{appsecret} can be considered as the master key of a mini-app that is used to verify the identify of network API invoker whenever a \wechat API is invoked (e.g., the \texttt{code2session} API that returns user session key with user login token). Session key, on the other hand, is a global encryption key used to encrypt the sensitive data transferred between the mini-app front-end and its back-end (e.g., user account information).

\paragraph{Our Approach} As discussed earlier, there are two types of keys that can be leaked from the front-end of the mini-app, \ie,  \texttt{Appsecret} and the key session-key. Overall, we statically collect all the suspicious values and dynamically verify them to confirm whether they are the real keys. Specifically, we use the following methods when identifying different keys:    
\begin{itemize}[leftmargin=*]
\item \paragraph{Appsecret} \texttt{Appsecret} is a 32-bit hex string assigned to each mini-app as the master key, and the method that searching all strings that are 32-bit long is subject to mis-match issues, since not all these strings are the  \texttt{Appsecret}s. To address that, we first collect all specious strings, and then feed these strings to the network API \texttt{/cgibin/token}. This is a network API used by the back-end server to get the token for invoking all \wechat network APIs, and takes two parameters: the mini-app ID and the mini-app appsecret. As such, we can check whether the appsecret is valid by checking whether the network API returns valid results showing the token required.
\item \paragraph{Session Key} To detect session key is more complicated, as a developer may define many network interfaces at the front end, and any of these interfaces  can be the mis-used one that returns the session key to the front end. However, the login token is associated with the mini-app ID and the user ID, and updates every 5 minutes. Therefore, it is impossible to obtain the login token. We observed that all the session key acquisition process begins with the \texttt{wx.login} API that returns user login token for back-end to get session key. As such, to identify potential session key leakage via static analysis, we first identify the invocation of \texttt{wx.login}, and then track the function calls and values involved in the \texttt{.then()} function and the \texttt{success} or \texttt{fail} callback functions. To this end, our tool investigates two problems: (1) what are the URLs a mini-app network request is sent to? (2) what is the mini-app action that follows user login? 
\begin{itemize}[leftmargin=*]
\item 
\paragraph{(1) Network URLs} Since session keys has to be leaked via network request, we can collect all URL strings in the mini-app front-end code. Then, to analyze these URL strings, we use word segmentation, an NLP technique used to split long english strings, into english keyword list. For example, the \texttt{Getsessionkey} URL will be splitted into \textit{get}, \textit{session}, and \textit{key}. Then, with the session URL keyword list of all mini-app packages in the dataset is obtained, we perform a manual analysis to understand the functionalities of these third-party URLs, and identify potential leakages of session key for suspected URLs such as \texttt{Getsessionkey} as shown at line 05 in \autoref{fig:code}.

% \begin{itemize}
%     \item \paragraph{The URLs that resemble the official API.} In \wechat, mini-app front-ends cannot directly communicate with the \breakabletexttt{api.weixin.qq.com} domain, which indicates that it cannot directly invoke \texttt{jscode2session} via \texttt{wx.request}. However, we observed there are many cases where developers just duplicated the official \texttt{jscode2session} with a similar API name (e.g., \texttt{/code2session}) and directly forwards the return value as it is to their front-end, even when the session key should have been filtered out.
%     \item \paragraph{The URLs that directly returns the session key.} Unlike the APIs that duplicate \wechat \texttt{jscode2session} and forwards the entire return value as it is, other developers may directly leak the session key to the front-end via getter API (e.g., \texttt{Getsessionkey} in line 05 as shown in \autoref{fig:code}). Therefore
% \end{itemize}

\item 
\paragraph{(2) Function calls} Aside from \texttt{wx.login} API that is associated with network requests which may potentially leak session keys, we observe that there are a set of mini-app APIs (e.g., \texttt{getWeRunData}) which returns encrypted data. Since the session key is supposed to be maintained by the back-end, the front-end cannot read these data, and therefore the front-end \textit{has} to send this encrypted data back to their back-ends. Therefore, for all these APIs associated with sensitive data, we examine whether there are network request APIs in the \texttt{.then()} function and callback functions as well. If there is no network request associated with network request, the mini-app may potentially perform the decryption in the front-end.
\end{itemize}



%To address this challenge, we introduced static analysis. Our observation is that to fetch the session key, \textsf{code2session} will be invoked eventually, and the three inputs are required (\ie, \texttt{Appsecret}, token, and the mini-app). Among these inputs, the token is returned from the API \texttt{wx.login}. Therefore, we can track the propagation of the return value of \texttt{wx.login} to identify whether the mini-app uses the token to further fetch the session key. However, the regular use of \texttt{wx.login} will also involve the use of sending login token to the back-end, which may brings the false alerts. To address this, we have another observation: the leakage of session key due to the misunderstanding of their official document, and when this occurs, the developer usually used session key to decrypt the sensitive data at front-end, instead of decrypting the data at back-end. Therefore, if we also observe that (i) a mini-app sends the token to back-end, (ii) the mini-app never sends the cipher of sensitive data to the back-end; the mini-app is performing the decryption at front-end      
\end{itemize}


% \paragraph{(1) appsecret leakage} Since appsecrets are 32-bit hex strings, the most straightforward way to detect \texttt{appsecret} leakage is to find all the strings in this format among the decomplied JavaScript code. However, such a method is subject to false positives, since many other strings appear in a same format (e.g., the cloud database token). To identify the appsecrets out of the 32-bit hex strings, we send these strings to the network API \texttt{/cgibin/token}, a \wechat network API used by the back-end server to get back-end API token for invoking all \wechat network APIs, to the \breakabletexttt{api.weixin.qq.com/} domain. Since this API only takes the mini-app ID and the appsecret as argument, we can verify whether a suspected string is mini-app appsecret by checking whether the network API returns the API token, or just error message.

% \paragraph{(2) session key leakage}
% Session keys are dynamically generated when user logs in the mini-app. When a user logs in, instead of directly returning the session key for the untrusted front-end to send back to back-end server, the mini-app host app generates a login token, which will be sent to back-end and then invoke \texttt{jscode2session} to eventually get session key with appid, appsecret, and login token. Since the session key is used to decrypt all sensitive data sent from the host app, this session key is not supposed to be leaked. However, we still observed some developers that leaks the session key to the front-end to handle decryption. For example, in \autoref{fig:code}, the developer sends the login token back to \texttt{/wxapp/Getsessionkey} with appsecret and login code, and then the back-end leaks the session key to the front-end in line 08.

% It is challenging to identify the session key leakage for two reason. First, the session key can be leaked via an arbitrary third-party network API implemented by the developer, and hence it is unlike \wechat back-end APIs that have fixed URL names. Second, since the network APIs are implemented by third-party developer themselves, we cannot infer session key leakage from the properties of the return value, e.g., \texttt{session\_key} in line 08, since different developer may return session key in different object structure.



%In our study, we focus on the security mechanism usage of developers, including the built-in mechanism permission authentication and aforementioned add-on mechanisms. Note that since our analysis is based on distributed mini-app packages, the non-interactive built-in mechanisms (i.e., isolation, encryption, and decryption) and mechanisms configured outside mini-app packages (i.e., white lists) are out of our scope. To do so, we first categorized the usage conditions of security mechanisms, and then present the design of \textsf{MiniLyzer}.
% that involve add-on security mechanisms from the developers, categorize the configuration and usage into four conditions, and then design our analysis tool based on this categorization.



==> paper/04_design_back.tex <==

\section{Detection}

As the add-on security measures may unconsciously introduce various \textsf{Coffee} attacks against the mini-apps, we would like to measure the impact of the \textsf{Coffee} attacks by preforming a Large-Scala scanning over the released mini-apps. To this end, in this section, we design and implement our detection tool, named   \textsf{Coffee} atta\textsf{C}k \textsf{AN}alyzer (\textsf{CoffeeCAN}), that can determine whether a mini-app is vulnerable. In this section, we first demonstrate a motivating example (\S\ref{subsec:example}) that includes all the aforementioned cases to show how to identify these mis-use; Then we discuss the design challenges and our insights (\S\ref{subsec:challengesandinsights}); Finally, we explain the current design of our \textsf{CoffeeCAN} (\S\ref{subsec:desgin}). 
 
%In our study, we focus on the security mechanism usage of developers, including the built-in mechanism permission authentication and aforementioned add-on mechanisms. Note that since our analysis is based on distributed mini-app packages, the non-interactive built-in mechanisms (i.e., isolation, encryption, and decryption) and mechanisms configured outside mini-app packages (i.e., white lists) are out of our scope. To do so, we first categorized the usage conditions of security mechanisms, and then present the design of \textsf{MiniLyzer}.
% that involve add-on security mechanisms from the developers, categorize the configuration and usage into four conditions, and then design our analysis tool based on this categorization.
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{image/code.pdf}
    \caption{An excerpted example of mini-app vulnerable to Coffee attack \ZY{TODO}}
    \label{fig:example}
\end{figure*}

\subsection{Motivating Example}
\label{subsec:example}










\subsection{Design Challenges and Insights}
\label{subsec:challengesandinsights}


\paragraph{Challenges} Based on the above motivating example, we can notice that to detect mini-apps that are subject to \textsf{Coffee} attacks, we must correctly recognize the APIs and parameters to determine whether there are some mis-configurations (\ie, detecting misuse of Bluetooth device communication encryption), then recognize whether there are the validation processes that authenticates a user or a mini-app (\ie, detecting misuse of cross mini-app communication or cross-user sharing), and finally identify the potential leakages (\ie, the misuse of communication encryption). More specifically, we have to address the following challenges: 


\begin{itemize}[leftmargin=*]
\item \paragraph{C1. Recognizing the mis-configuration of API} 
In the case of Bluetooth device communication encryption, the developers can enable or disable Bluetooth encryption with  \texttt{addService(service)}, in which the parameter \breakabletexttt{writeEncryptionRequired} and the parameter \breakabletexttt{readEncryptionRequired} of \texttt{service} are set to \texttt{true} or \texttt{false}.  The most intuitive way is to use simple string marching to search strings such as \breakabletexttt{writeEncryptionRequired} and  \breakabletexttt{readEncryptionRequired} in the de-complied JavaScript byte-code, and then reorganize the \texttt{Boolean} value attached. However, such a practice is not feasible, as in the context of JavaScript, the JavaScript code can be heavily obfuscated. As shown in \autoref{fig:example}, the \texttt{Boolean} attached with  \breakabletexttt{writeEncryptionRequired} can be renamed to an un-recognizable value, and be placed far from the \breakabletexttt{writeEncryptionRequired}, which cannot be handled by simple String matching.  \looseness=-1
\item 
\paragraph{C2. Identifying the mis-use of verification processes} When entering mini-apps, the developers can check whether the mini-app is being redirected to from a trust mini-app by getting the \texttt{appId} parameter from the object \texttt{referrerInfo}. For secret sharing, the developers can also check whether the user that enters the mini-app is the first-hand user by invoking and inspecting the return value of \breakabletexttt{wx.authPrivateMessage}. However, in addition to identifying the configuration values (\ie, whether an mini-app invokes the API with specified parameter), which faces \textbf{C1},  we also have to deal with the relationship between the these APIs. For example, as shown in \autoref{fig:example}, in the validation processes, the mini-app must first get the value of interest (\eg, \texttt{appId} contained in \texttt{referrerInfo}), and then check whether the the value is in a pre-defined list. The verification expression can be implemented in various ways, and in \autoref{fig:example}, we can observe the developer used both ternary operator and equality operators to represent the checking logic, which cannot be easily identified. 

\item 
\paragraph{C3. Determining the potential leakage} In general, there are two types of keys can be leaked, \ie, \texttt{Appsecret} and session key.  
\texttt{Appsecret} can be considered as the master key of the mini-app ecosystem,  which can be used to fetch a valid session key. Session key is used to encrypt the sensitive data transferred between the mini-app front-end and its back-end. Although the session key will be updated every time the user logins the back-end of the mini-app, some developers may mistakenly implement a interface that is used to obtain a session key at the front-end of the mini-app, resulting in the leakage of the session key. Therefore, our tool must handle these two types of keys. For the \texttt{Appsecret}, as it has a fixed format (\ie, it is a 32-digits long string containing the hexadecimal digits), the most straightforward way to detect of \texttt{Appsecret} the leakage is to grep the decomplied JavaScript code and uses the regular expression to match it. However, such a method is subject to false alert, since many strings in a mini-app have the same format (\ie, the index of online database).  For the session key leakage, we have to design a way that can automatically identify the customized interfaces. However, different developers can have different programming practice and gives the interface various names and parameter lists.    

\end{itemize}
 

\paragraph{Insights} Consequently, we propose three solutions to deal with the challenges. First, we use the backward slicing programming slicing to correctly track the API parameters, so that we can determine whether there are mis-configurations (\eg, Bluetooth encryption APIs). Second, we use Abstract Syntax Tree (AST) to handle the relationship between the APIs for verification process detection. Finally, we satanically collect the values that looked appear to be \texttt{Appsecret} or session key interfaces, and then dynamically verify them using the related APIs that provided by \wechat.  

\begin{itemize}[leftmargin=*]
\item \paragraph{S1. Using Backward slicing to track API of interest and its parameters} Recall that in the analysis of API of interest and its parameters, heave code obfuscation can be applied,  where the name of   parameters cannot be easily identified. Our idea is to use the backward slicing to traverse the data flow graph of mini-app, where data dependencies are inferred from the program states and the generated data flow graphs. To that end, we first identify the names of security-related APIs, and then traverse from their successors (e.g., the code fragments that use the return values of the API) 
%forwardly and the code fragments that refers the target API 
backwardly to track the propagation of the parameters of interest. \looseness=-1

\item \paragraph{S2. Using Abstract Syntax Tree (AST) to identify the verification process} Recall that the verification process may appear in various statements such as \texttt{IF} statements and \texttt{FOR} statements, and the name of the variables can also varies from mini-app to mini-app due to the code obfuscation and the programming practices of the developers. Fortunately, we observe that all the verification processes involved the similar logical expressions: when the code fragment is represented as the Abstract Syntax Tree (AST), the data to be verified is one leaf node of the AST, by analyzing the AST, we can easily determine whether verification is involved.  Therefore, to detect the occurrences of the validation, we can first use the solution introduced in \textbf{S1} to identify the API of interest, and then parse the relationship between the APIs using their Abstract Syntax Tree (AST) representations.  

\item \paragraph{S3. Statically identifying suspicious values and dynamically verifying keys for analyzing potential leakage} As discussed earlier, there are two types of keys that can be leaked from the front-end of the mini-app, \ie,  \texttt{Appsecret} and the key session-key. Overall, we statically collect all the suspicious values and dynamically verify them to confirm whether they are the real keys. Specifically, we use the following methods when identifying different keys:    
\begin{itemize}
\item \paragraph{Appsecret} \texttt{Appsecret} is a 32-bit hex string assigned to each mini-app as the master key, and the method that searching all strings that are 32-bit long is subject to mis-match issues, since not all these strings are the  \texttt{Appsecret}s. To address that, we first collect all specious strings, and then feed these strings to the network API \texttt{/cgibin/token}. This is a network API used by the back-end server to get the token for invoking all \wechat network APIs, and takes two parameters: the mini-app ID and the mini-app appsecret. As such, we can check whether the appsecret is valid by checking whether the network API returns valid results showing the token required.

\item \paragraph{Session Key} To detect session key is more complicated, as a developer may define many network interfaces at the front end, and any of these interfaces  can be the mis-used one that returns the session key to the front end. However, the login token is associated with the mini-app ID and the user ID, and updates every 5 minutes. Therefore, it is impossible to obtain the login token. To address this challenge, we introduced static analysis. Our observation is that to fetch the session key, \textsf{code2session} will be invoked eventually, and the three inputs are required (\ie, \texttt{Appsecret}, token, and the mini-app). Among these inputs, the token is returned from the API \texttt{wx.login}. Therefore, we can track the propagation of the return value of \texttt{wx.login} to identify whether the mini-app uses the token to further fetch the session key. However, the regular use of \texttt{wx.login} will also involve the use of sending login token to the back-end, which may brings the false alerts. To address this, we have another observation: the leakage of session key due to the misunderstanding of their official document, and when this occurs, the developer usually used session key to decrypt the sensitive data at front-end, instead of decrypting the data at back-end. Therefore, if we also observe that (i) a mini-app sends the token to back-end, (ii) the mini-app never sends the cipher of sensitive data to the back-end; the mini-app is performing the decryption at front-end      
\end{itemize}


%In general, although the token is sent to the back-end, the mini-app should not expect the  , we can use static analysis to filter the      



%Recall that \textsf{code2session} accepts three parameters including a mini-app ID, a {\red{login}} token, and the \texttt{Appsecret}, and returns the session key and user identifier when the parameters are correct. (we used our own login token and update the token periodically to ensure the validity of the token)

 


%The appsecret is a 16-bit hex string assigned to each mini-app as a secret key. To avoid missing suspected appsecrets, we record every 16-bit hex strings in the mini-app as suspected appsecrets first. To verify whether the hex string is a real mini-app appsecret, we found a network API that requires both the mini-app id and mini-app secret to get a token from the \wechat server by the back-ends. Since we have the hex string and know the mini-app id, we can verify the hex string by checking whether the response from \wechat server returns an error message or directly returns the token.


\end{itemize}
 
 

 



% is generated when a user logs in, and is used in all sensitive data encryption.  


 

%Being the decryption key that is fetched by \texttt{Appsecret}  


%in a variety of encryption communications between the front-end and back-ends, including user session tracking, network API invoking, and signature verification. Since the \wechat platform will not maintain the appsecrets for developers, developers have to maintain it well, otherwise the developers will have to make the \wechat framework to generate a brand new one. However, if the developer is sloppy enough to believe that front-end packages is well encrypted and decide to let the front-end to maintain the appsecret, then this leaked appsecret may be exploited by attackers.


%As shown in the figure, this checking process may appear in various statements

%To detect this usage, we not only need to track the control flow, but also need to track the parameter parsed into the corresponding API.
% These two parameters are optional and are by default true if the developers choose not to configure them. However, if these parameters are set to false, the communication of Bluetooth devices may be less secure and prone to potential security problems.

% \paragraph{RQ1: Is device misconfigured?}

%\subsubsection{Entry checking} When entering mini-apps, the developers can check whether the mini-app is being redirected to from a valid mini-app by getting the \texttt{appId} parameter from the object \texttt{referrerInfo}. For secret sharing, the developers can also check whether the user that enters the mini-app is a valid target of the secret sharing by invoking \texttt{wx.authPrivateMessage}. As shown in the figure, this checking process may appear in various statements such as If statements and For statements, but they all involve logical expressions. Therefore, to detect this type of mechanism usage, we can parse the AST and identify the value in both sides.


% If the developers forget to check the mini-app or user source of navigation and executes with the extra data,
% the mini-app may be attacked by unexpected users or from unexpected mini-apps. Similarly, if the developer forget to check the private message while the secret sharing mechanism is issued, then the mechanism may become ineffective due to this mismatching.

% \paragraph{RQ2: Is mini-app redirection checking missing?}

% \paragraph{RQ3: Is private sharing checking missing?}

%\subsubsection{Credential maintenance} In our paper, we focus on the mini-app framework security, and therefore the developer-defined credentials such as administrative usernames and passwords are out of scope. 


%In general, there are two mini-app related credentials: the cloud API token, and the decryption key.

%\paragraph{Cloud API token} The cloud API token, appsecret, is a type of critical information maintained by each mini-app, since it involves in a variety of communications between the front-end and back-ends, including user session tracking, network API invoking, and signature verification. Since the \wechat platform will not maintain the appsecrets for developers, developers have to maintain it well, otherwise the developers will have to make the \wechat framework to generate a brand new one. However, if the developer is sloppy enough to believe that front-end packages is well encrypted and decide to let the front-end to maintain the appsecret, then this leaked appsecret may be exploited by attackers.

% \paragraph{RQ4: Is appsecret leaked?}

%\paragraph{Data encryption key} The data encryption key, session key, is generated when a user logs in, and is used in all sensitive data encryption. Therefore, similar to appsecret, the developers using third-party back-ends have to maintain the session key properly, or otherwise any leakage to the front-end may grant the attackers capabilities of various man-in-the-middle attacks.

% \paragraph{RQ5: Is session key leaked?}

\subsection{Current Design of \textsf{CoffeeCAN}}
\label{subsec:desgin}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/tool.pdf}
    \caption{The CoffeeCAN workflow \ZY{TODO}}
    \label{fig:tool}
\end{figure}

\AY{Part of this section will be truncated. Will refer to this part after tables in Evaluation are done.}
As shown in \autoref{fig:tool}, our \textsf{CoffeeCAN} has three major components, including a (1) Data Flow Analyzer to preform the backward slicing program analysis, (2) Authentication Detector to search all validation processes of interest using AST, and (3) Leakage Tester to collect and validate all the potential key leakage. In the following, we present the detailed design of each component: 



\paragraph{(1) Data Flow Analyzer}  Data Flow Analyzer is used to identify whether an API is invoked with correct parameters by first recognizing the API of interest, then constructing a data dependence graph backwardly to identify the parameters of the API, and finally inspecting the value of the parameters to determine whether it is mis-configured. In the following, we use the case of detecting Bluetooth Configurable Service mis-use to demonstrate our principles. First, we can easily identify the API \texttt{addService}, which accepts the parameter that may be mis-configured. Second, we construct a data dependence graph backwardly. We define the API \texttt{addService} as the source and all the declared variables as the sinks.  
In JavaScript, if the API would like to use the declared variable, the declared variables can either be a local variable or a global variable. For local variable, it can only be found in the current JavaScript that the API is co-located with. For the global variable, the variable can either be found at the current JavaScript file or a Public modules. Our tool handles both.  We records all the declared variables, and explore the possible connections between the identified declared variables and the API of interest (\ie, \texttt{addService} in this case). For example, in our case, we identified a declared variable named \texttt{service} is passed into the API \texttt{addService}. Similarly, we can also use the same method to confirm \texttt{readEncryptionRequired} is set to \texttt{false}, and conclude that this mini-app is subject to unauthorized data access.   

%The above case demonstrate how to identify the parameters that need to be fed in the API of interest.  Other than that, in some other case of 

Other than the parameters of an API, the return value of an API can also be used to determine whether there are mis-configurations. For example, as shown in \autoref{fig:example}, the return value of \texttt{wx.login} is used to fetch the session key, which will result in the session key leakage. Therefore, we would like to track the propagation of the return value of a specific API. Different from C and Java languages, to use the return values of APIs, the successors has to be invoked synchronized, \ZY{Two questions: (1) what do you mean by synchronized? You have never explained. (2) What the method you used to detect the return value mis-use? I cannot find any explanations. I only find how they work. } Otherwise the successor APIs will only receive ``undefined'' value since it is invoked before the return value of the previous API is returned. To perform synchronized function invocation, Javascript also has three conditions
\begin{itemize}[leftmargin=*]
    \item \paragraph{Sequential expression (line 25)}. Javascript functions can be invoked sequentially by commas. If functions are invoked with these commas, then the functions can only be invoked after the previous function has finished.
    \item \paragraph{\texttt{.then() (line 29)} member function}. If the developers wants to make use of the return value of the previous function, they can use the \texttt{\.then()} member function by declaring the successor function in the \texttt{then()} member. The successor function will be invoked with the return value after the previous function finishes.
    \item \paragraph{Callback function (line 27)}. If the developers want to let the previous function to execute the successor function, which is often the case in mini-apps because the mini-app framework takes care of most of the processing, the developers can similarly declare the successor function via function constructor. \wechat mini-app framework APIs often come with a \texttt{success} and a \texttt{fail} callback (and sometimes a \texttt{complete} callback that will be invoked after either \texttt{success} and \texttt{fail} finishes). Developers can perform any operations as they wish by using this feature.
\end{itemize}


%  \begin{figure*}
%      \centering
%      \includegraphics[width=\linewidth]{image/AST.pdf}
%      \caption{An example of AST}
%      \label{fig:AST}
%  \end{figure*}

%are effective at function level, indicating that only global variables exported from public modules or in the current JavaScript file and the local variables defined in the current function body can be referred to in a function declaration. 


%Therefore, we can track the identified variable declaration by extending each function declaration node by recording all declared variables, declared functions, and invoked functions together with the referred variable name. For example, the function declares a variable called \texttt{service}, and calls the function \texttt{addService()}. The invocation of \texttt{addService} involves the argument \texttt{service}, and the declaration of \texttt{service} involves the property that we are interested in: \texttt{readEncryptionRequired}. If this property is set to \texttt{false}, then this may be a vulnerable configuration. tracking the propagation of the corresponding parameters. In general, the parameters are represented as JSON objects, and these 
 




%This JSON object may either be predeclared and referred to in the argument, or directly declared as the function argument. 
% merely tracking the control flow is not enough, in that the values of the function parameters may not always be directly declared in the arguments: they may also refer to a predefined global or local variable. 
% As such, we track the data flow of the function parameter if the parameter is a object reference, or directly analyze the declared object in the API.
% we still need to track the function parameter and investigate if the variable is being configured correctly. To do this, data flow analysis had been a widely-adopted tool. However, we cannot directly perform dynamic analysis in the mini-apps since running mini-apps require the support of \wechat framework and \wechat account, which is strictly being monitored and managed to defend against malicious behaviors. Therefore, we perform a static data flow analysis based on the AST.
%To track the data flow of configuration APIs, we define the security related APIs as source (e.g., \texttt{addService(service)}, and the variable declarations of the parameter as sink (e.g., \texttt{service}). We observe that, 

%, we have to first use backward slicing to identify the API of interest, and then track the parameters of the target API and further inspect these identified parameters. Specifically, our Control Flow Analyzer includes two steps: 

%\begin{itemize}[leftmargin=*]
%\item \paragraph{Step I - Parameter Identification}  To identify configuration APIs such as BLE configuration API, aside from tracking the control flow to locate the API invocation, we also need to track the data flow in the function parameters, since the configurations of BLE devices are parsed to the API as a JSON object.

%\item \paragraph{Step II - API Identification} 
% % Javascript adopts a different programming mode to support synchronized execution,and there are three different conditions where a function is called, as shown in \autoref{fig:example}: {(1) Call expression (line 17)}. Similar to other languages, Javascript functions can be directly called after being declared with \texttt{function} declarator; {(2) Member expression (line 18)}. Javascript functions can be a member method of any object. In mini-app framework, most of the functions are called as a member method of \texttt{wx} object. {(3) Function constructor (line 20)}. Callback functions in javascripts are parsed to the original function as a parameter of property of param object through function constructor. Since we focus on mini-app specific APIs related to the add-on security mechanisms, we do not include the first direct function define-call condition, since all the mini-app specific APIs appear as the member of \texttt{wx} class, or are invoked as function parameter.

%\AY{Because wechat mini-app APIs are invoked as members of \texttt{wx}, therefore, we directly match the function name. Although this is simple, }




%\end{itemize}




 
 
 

%\subsubsection{Control Flow Tracking} The first step to analyze the security mechanism usage is to figure out what APIs are invoked, and what APIs are associated with these security mechanisms. 

% of analyzing the source code of mini-apps is tracking the mini-app control flow.
%To do so, a widely adopted approach is static analysis, with which the tool traverses the control flow graph of mini-app source code. Hence, we first identify the invocation of security-related APIs, and then traverse their successors (e.g., the APIs that use the return values of the API) to track the propagation of the security-related APIs.



%\subsubsection{Function Parameter tracking}

% Then, we examine each variable declarations: if the declaration is a basic type such as boolean and integer, we record the corresponding values. If the declared variable is an object, we examine the properties and the corresponding values. If an object is associated to a vulnerable configuration (e.g., \texttt{readEncryption} is set to \texttt{false}), and the corresponding function call is associated with this insecure variable configuration (e.g. \texttt{addService)}, then this usage is considered insecure.




\paragraph{(2) Authentication Detector} In the Authentication Detector, we used the AST to represent the sophisticated logic expressions, and determine whether there are verification involved. Again, we use the example in \autoref{fig:example} to demonstrate the principles. The verification expression is \breakabletexttt{t.scene \&\& 1038==t.scene \&\&  "wxff60d952b9\\494209"  ==  (t.referrerInfo \&\& t.referrerInfo.appId ? t.referrerInfo.appId : "" )}, which can be broken into 9 independent expressions, as shown in \autoref{fig:AST}. Our Data Flow Analyzer can quickly identify the parameter need to be checked (\ie, \texttt{t.referrerInfo.appId}), which located at the seventh and eighth leaf node of the AST. To resolve the relationship between the nodes of the AST, (1) we first track back to the parent of the leaf node and checks whether the parent is an 
equality operator. (2) If so, we further checks if there are correct appId (\ie, appIds usually are usally in the format of ``wx********'') in the other sibling nodes. \ZY{I think we need an algorithm here.}



 


%To further determine if the mini-app verify the source 

%We then assume the parameter need to be checked (\ie, \texttt{t.referrerInfo.appId}) as one, while others as 

%In this case, if its parent is \texttt{"||"} or \texttt{"&&"}, one of the possible the representations of its parent must be \texttt{t.referrerInfo.appId}.    


%Start from any of the leaf node that equals the parameter need to be check (\eg, the seventh one), we can trace its parent   

    

% t.scene && 1038==t.scene && 35"wxff60d952b9494209"==(t.referrerInfo&&36t.referrerInfo.appId?t.referrerInfo.appId:"")


When entering mini-apps, developers can get the source mini-app of navigation or the share ticket (a signature of a sharing action) that can be used to verify whether the current user is eligible for using the current mini-app. Therefore, we covered both of these two cases.


\begin{itemize}[leftmargin=*]
\item \paragraph{Case I: Cross-Mini-app Authentication Process Detection} To check the source mini-app of navigation, the developer need to get the \texttt{appId} from the \texttt{referrerInfo}, which is obtained with \texttt{getLaunchOption} or \texttt{getEnterOption} API. Also, the developers have to process the \texttt{referrerInfo} object to get the \texttt{extra} data for information of the redirection. As such, we consider an API is related to mini-app navigation if the mini-app uses the \texttt{extra} param of \texttt{referrerInfo}. To check whether the source mini-app id is being checked, we parse the AST of logical expressions (e.g., line foo in figure bar), and check if there is a binary expression \texttt{==} between \texttt{referrerInfo.appId} and a mini-app id string, or if there is a JS-specific \texttt{in} operator associated with \texttt{referrerInfo.appId} if the developer has a set of mini-app whitelists.

\item 
\paragraph{Case II: Cross-User Authentication Detection} When the developer uses private message checking, he/she first sets \texttt{isPrivateMessage} parameter to \texttt{true} when user shares the mini-app via \texttt{wx.openShareMenu()}. When checking the validity of current user, the devloper invokes \texttt{wx.authPrivateMessage()} with the share ticket generated when the mini-app is being shared. Therefore, if a mini-app contains the sharing API with private message parameter enabled, we consider it associated with private sharing. Then, we investigate whether the developer checks the message sharing with corresponding API invocation.
\end{itemize}

 

\paragraph{(3) Leakage Tester} As shown in table foo, there are two types of sensitive credentials that we are interested in: the API invocation token appsecrets and the decryption key session-key.
\begin{itemize}[leftmargin=*]
\item 
\paragraph{Appsecrets Leakage Detection} The appsecret is a 32-bit hex string assigned to each mini-app as a secret key. To avoid missing suspected appsecrets, we record every 32-bit hex strings in the mini-app as suspected appsecrets first. To verify whether the hex string is a real mini-app appsecret, we found a network API that requires both the mini-app id and mini-app secret to get a token from the \wechat server by the back-ends. Since we have the hex string and know the mini-app id, we can verify the hex string by checking whether the response from \wechat server returns an error message or directly returns the token.

\item 
\paragraph{Session Key Leakage Detection} For session keys, we identify potential session key leakage with static analysis by detecting network APIs associated with sensitive APIs and identifying suspicious strings that may refer to network API URLs: 

\begin{itemize}[leftmargin=*]
    \item \paragraph{Network request APIs} In mini-apps, since the session keys are supposed to be maintained by back-ends and shall never be leaked to the front-end, when the sensitive data is obtained from host app, the developers can only send the encrypted data to their back-end for decryption, which will involve a network request API such as \texttt{wx.request}. Therefore, if a mini-app API is invoked but without any network request API associated, the mini-app either decrypts the data in the front-end which means the session key is leaked, or the mini-app does not use the sensitive data at all, which is a improper over-requisition of sensitive data. 
    \item \paragraph{Network URL strings} The session key can only be fetched when a user login token is generated, and can only be leaked through network communication with the back-end server, since the API domain of \wechat official is forbidden in front-ends. Therefore, whenever there is a \texttt{wx.login()} API that generates user login token, we investigate whether the successor API invocation involves network API, and then we identify the string values that appear to be URL paths and then manually examine these string values. For example, if there is a URL path of \texttt{code2session}, this is likely to be leaking session key since the \wechat \texttt{code2session} API returns session key info, and the third-party server is highly possible to be merely duplicating this API and just forwards the session key info back to front-end to circumvent the blacklist of \wechat API domain enforced in the front-end.
\end{itemize}

\end{itemize}




% Validation. We found that there is a wechat network API used by the back-end servers to obtain API invocation token.







% \paragraph{Structure recovery}

% \paragraph{Semantic recovery}

==> paper/04_measurement.tex <==


  
 
 
 

\begin{table}[h]
\resizebox{0.8\columnwidth}{!}
{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Data \& Resources} & \textbf{Type} & \textbf{\wechat}                        & \textbf{\alipay}                        & \textbf{\baidu}                         & \textbf{\tik}                                \\ \midrule
\textbf{\textcircled{\tiny{1}} User profile}      & A             & \tickYes                & \tickYes                & \tickYes                & \tickYes                \\
\textbf{\textcircled{\tiny{2}} Gait \& Sports}    & A             & \tickYes                & \tickYes                & \multicolumn{1}{c}{N/A} & \multicolumn{1}{c}{N/A} \\
\textbf{\textcircled{\tiny{3}} In-App Contact}    & A             & \multicolumn{1}{c}{N/A} & \tickYes                & \multicolumn{1}{c}{N/A} & \multicolumn{1}{c}{N/A} \\
\textbf{\textcircled{\tiny{4}} Billing Address}   & A             & \tickNo                 & \tickYes                & \tickYes                & \multicolumn{1}{c}{N/A} \\
\textbf{\textcircled{\tiny{5}} Invoice}           & A             & \tickNo                 & N/A                 & \tickYes                & \multicolumn{1}{c}{N/A} \\
\textbf{\textcircled{\tiny{6}} Location}          & S             & \tickYes                & \tickYes                & \tickYes                & \tickYes                \\
\textbf{\textcircled{\tiny{7}} Phone number}      & S             & \tickYes                & \tickYes                & \tickYes                & \multicolumn{1}{c}{N/A} \\
\textbf{\textcircled{\tiny{8}} System Contact}    & S             & \tickYes                & \tickYes                & \tickYes                & \tickYes                \\
\textbf{\textcircled{\tiny{9}} Audio Record}          & S             & \tickYes                & \multicolumn{1}{c}{NA} & \tickYes                & \tickYes                \\
\textbf{\textcircled{\tiny{10}} Photo \& Video}    & S             & \tickYes                & \tickYes                & \tickYes                & \tickYes                \\
\textbf{\textcircled{\tiny{11}} Camera}            & S             & \tickYes                & \tickYes                & \tickYes                & \tickYes                \\
\textbf{\textcircled{\tiny{12}} Bluetooth}         & S             & \tickYes                & \tickYes                & \multicolumn{1}{c}{N/A} & \multicolumn{1}{c}{N/A} \\ \bottomrule
\end{tabular}}
\vspace{2mm}
\caption{Comparison of sensitive data protected by each platform. ``A'' means app-specific data, while ``S'' means the system resources. ``\tickYes'' means the sensitive data is protected while ``\tickNo'' means not. ``N/A'' means the sensitive data can not be accessed by the platform.    } 
\label{tab:scope}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[h]
\resizebox{1.6\columnwidth}{!}
{
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Attacks}                                                                                       & \textbf{Pitfalls} & \textbf{Adversary} & \textbf{\begin{tabular}[c]{@{}c@{}}  Sensitive data \end{tabular}} & \textbf{Wechat} & \textbf{Alipay} & \textbf{Baidu} & \textbf{TikTok} \\ \midrule
\textbf{Fake Peripheral}                                                                               &   \ding{182},\ding{183}   &         O           &          \textcircled{\tiny{12}}                                 &       \tickNo      &      \faAndroid   &       N/A    &         N/A          \\ \midrule
\textbf{Peripheral Data Unauthorized Access}                                                           &        \ding{184}            &       O            &         \textcircled{\tiny{12}}                                                                         &        \faAndroid       &       N/A            &       N/A          &         N/A         \\ \midrule
\textbf{Network Isolation Escape}                                                                      &        \ding{185}           &         I           &            -                                                                &         \tickNo     &            \faAndroid,\faApple     &        \faAndroid,\faApple         &      \faAndroid,\faApple            \\ \midrule
\textbf{Collusion Attack}                                                                              &           \ding{186}         &          I          &   \textcircled{\tiny{1}}, \textcircled{\tiny{2}}, \textcircled{\tiny{3}}, \textcircled{\tiny{4}}, \textcircled{\tiny{6}}, \textcircled{\tiny{7}}, \textcircled{\tiny{8}}                                                                         &           \faAndroid,\faApple         &        \faAndroid,\faApple            &    \faAndroid,\faApple               &    \faAndroid,\faApple        \\ \midrule
\textbf{Mini-app Launching Hi-Jack}                                                                    &       \ding{187}           &        I            &      \textcircled{\tiny{1}}, \textcircled{\tiny{2}}, \textcircled{\tiny{3}}, \textcircled{\tiny{4}}, \textcircled{\tiny{6}}, \textcircled{\tiny{7}}, \textcircled{\tiny{8}},   \textcircled{\tiny{9}}, \textcircled{\tiny{10}}, \textcircled{\tiny{11}}                                                                              &            \tickNo      &        \tickNo          &          \faAndroid,\faApple       &              \tickNo    \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}MitM attacks against Cross Mini-apps Communication\end{tabular}} &    \ding{187}           &            I        &              \textcircled{\tiny{1}}, \textcircled{\tiny{2}}, \textcircled{\tiny{3}}, \textcircled{\tiny{4}}, \textcircled{\tiny{6}}, \textcircled{\tiny{7}}, \textcircled{\tiny{8}},  \textcircled{\tiny{9}}, \textcircled{\tiny{10}}, \textcircled{\tiny{11}}                                                                   &      \tickNo           &          \faAndroid,\faApple         &            \faAndroid,\faApple      &       \tickNo           \\ \midrule
\textbf{Session Riding}                                                                                &       \ding{188}            &          O          &  \begin{tabular}[c]{@{}c@{}}\textcircled{\tiny{1}}, \textcircled{\tiny{2}}, \textcircled{\tiny{3}}, \textcircled{\tiny{4}}, \textcircled{\tiny{6}}, \\ \textcircled{\tiny{7}}, \textcircled{\tiny{8}}, \textcircled{\tiny{9}}, \textcircled{\tiny{10}}, \textcircled{\tiny{11}}, \textcircled{\tiny{12}}     \end{tabular}                                                           &            \tickNo      &           \faAndroid,\faApple        &       \faAndroid,\faApple       &       \tickNo          \\ \bottomrule
\end{tabular}}
\vspace{2mm}
\caption{Attack and pitfalls against mini-app platforms. \ding{182} No Active Pairing Policy; \ding{183} No API to Access Pairing Results; \ding{184} Insufficient Security Level For Peripheral;
\ding{185} Inconsistency of Network Resource Isolation; \ding{186} Privacy Leakage Across Mini-apps; 
\ding{187} Vulnerable Cross-miniapp Channel; \ding{188} Vulnerable Shareable UI Feature and Inter-app Communication Mechanism. ``O'': Outsider adversary; ``I'': Insider adversary; \textcircled{\tiny{1}} --\textcircled{\tiny{12}} represent sensitive data (See \autoref{tab:scope}); \tickNo: Not vulnerable. \faAndroid: mini-app running on Android is vulnerable. \faApple: mini-app running on iOS is vulnerable. }  %\red{Need to do some experiments and then update the result to the paper} 
\label{tab:attack}
%  \faAdjust: The host app running on one specific OS (e.g., Android or iOS) is vulnerable. \faAndroid,\faApple : The host app running on both OS are vulnerable. 
\end{table*}

  
%\subsection {Attack Measurement Result}
%\label{subsec:pitfalls}
%We deployed the attacks discussed in \S\ref{sec:threat} on different platforms. 

\textbf{Sensitive Data}. Recall one goal of the attacker is to access the sensitive information. Therefore, before we launch our attack, we like to understand what kind of sensitive information can be leaked and how severe the impact can be. To that end, we  examined the in-app permission checking list to confirm whether specific resources (including system resources such as Bluetooth and app-specific resources such as in-app contact list) are protect by the host app. 

As shown in \autoref{tab:scope}, we compare the sensitive data protected by each platform, and specific sensitive data is under protection means the host app will prompt the user for consent before the mini-app can access the resource. It can be observed that sensitive data can be grouped into two categories, i.e., ($i$) App specific data (\textcircled{\tiny{1}} -- \textcircled{\tiny{5}}). We found the app-specific data trended to be more sensitive when compared with the system resources. For example, all the platforms supported the mini-apps to access the user profile, which contains name (or nick name), gender and residential area. Mini-apps of \alipay can access in-app contact information of \alipay (friends list). Due to the fact that \alipay is a digital wallet, the contacts and the associated account likely to have financial transitions, and the contact information is more sensitive. Billing address and invoice are also involved in financial transitions. However, not all platforms treated these information cautiously.  ($ii$) System resources (\textcircled{\tiny{6}} -- \textcircled{\tiny{12}}). It can be observed that the sensitive system resources trended to be protected more carefully. This may be because they followed the major OS's implementations (e.g., Android). Moreover, recently, an escalate privilege flaw regarding the system resources was reported \cite{lu2020demystifying} and most of the platforms had fixed the flaw accordingly.    

\textbf{Attack Result}. We deployed our attacks against the different host apps (platforms). Specifically, all the attacks discussed were tested on a Google Pixel 4 running Android 10 and an iPhone running iOS 14.2. We did not test the attacks on Windows machine, since only \wechat supported to run mini-apps on a Windows machine.  Since our attacks also involved the peripheral security, we used \textsf{CC2640R2F} \cite{CC2640} launchpad to work as the fake peripheral. We used \textsf{Adafruit Bluefruit LE Sniffer} \cite{Adafruit} to collect the Bluetooth information of interest.  \autoref{tab:attack} present the attack result. 

\begin{itemize}
\item \textbf{Fake Peripheral}. In this attack, an outsider attacker pretends to be the fake peripheral and attempts to connect to a  \textit{Android} phone running vulnerable mini-app for unauthorized data access. We did not test the attack on iOS, since the threat model of iOS is different (iOS cannot defend against such attack). \wechat was not subject to the fake peripheral attack, this is because \wechat provided a pairing API only for the Android platform to balance the security and compatibility. \alipay was subject to fake peripheral attack. \baidu and \tik did not support to communicate with a Bluetooth peripheral and therefore, and therefore they were not subject to the fake peripheral attack.  

\item \textbf{Peripheral Data Unauthorized Access}. In this attack, an outsider attacker attempts to access sensitive data from a soft-defined peripheral (i.e., an Android phone running vulnerable mini-app). Again, this attack only works against Android phone. At the time of testing, only \wechat supported the software-defined peripheral feature, and it was subject to the attack. \wechat had not provided the highest security level for an Android phone exclusively at the time of writing.  

\item \textbf{Network Isolation Escape}. In this attack, an insider attack lures a user to click a hyperlink embed in a PDF document and if the user click the link, the network requests without vetting are sent out.   According to our experiment, only \wechat can defend against the attack, since \wechat used a special document viewer for the document opened by the mini-app, and all the link embedded in the document will become un-clickable. 


 \item \textbf{Collusion Attack}. In this attack, a malicious mini-app (i.e., insider attacker) with the access to sensitive resources conspires with an other mini-app with network access to steal sensitive information. Since the cross-app channel only allowed text to be transferred, figures, audios and videos are not vulnerable to the attack. According to our experiment, although no platform can defend against the attack, \wechat is more secure when compared with others. Before the establishment of the cross-app channel, 
\wechat displayed an innocuous dialog box and showed a message such as ``Launching Miniprogram X'', where X is the name of the mini-app to be communicate with. Only if the user pressed ``yes'', the communication can then be established. However, in this case, even if the sensitive information were transferred, no warnings were directed to the user during the process. Therefore, it is not easy for users to identify the potential threat. For other platforms, the channel can be established without prompting the user.  
 
 \item \textbf{Mini-app Launching Hi-Jack.} In this attack, an insider attacker (which is a network proxy app) modifies the network requests sent from the mini-app cross-app channel to hijack session, 
 launching a malicious mini-app instead of the app that the user intends to launch. The launched malicious mini-app can be designed to steal sensitive data (although the user consent is required), and therefore, particular resources can be vulnerable to the attack. 
 \wechat and \tik encrypted the requests, and we can not identify and modify the requests.  \alipay also protected the message integrity. Therefore, our attack cannot work against them. 
 
 \item \textbf{MitM attacks against Cross Mini-apps Communication}. Similar to mini-app launching hijack, the goal of the attacker is to monitor or modify the messages exchanged in the cross-app channel. Since two victim mini-apps may exchange sensitive data using the cross-app channel, the exchanged data can be in grave danger. Again, our attack failed in the context of \wechat and \tik. However, since \alipay only protected the message integrity instead of encrypting it, we can monitor the message exchanged between two \alipay mini-apps. \looseness=-1
 
\item \textbf{Session Riding Attack}. 
In this attack, an outsider attacker forces an end user to execute unwanted actions through the shareable UI. According to our experiment, \alipay and \baidu were subject to the attack. However, \wechat and \tik specified only particular UIs are shareable, and they also enforced token to protect the UI path or parameters to be modified. Therefore, mini-apps running on \wechat and \tik are not vulnerable to our attacks.  

\end{itemize}



 


%{\textbf{TODO: In the second round of my proofreading, I will analyze the different platforms regarding resource management, peripheral management, UI management and  network management.   }}
 


%Due to the same reason, 




 



==> paper/05_eval.tex <==
\section{Evaluation}

\begin{table*}[]
\footnotesize
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
    \centering
    \begin{tabular}{c|c|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
    \toprule
     \multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\rot{business}}&\multicolumn{1}{c|}{\rot{education}}&\multicolumn{1}{c|}{\rot{entertainment }}&\multicolumn{1}{c|}{\rot{finance}}&\multicolumn{1}{c|}{\rot{food}}&\multicolumn{1}{c|}{\rot{game}}&\multicolumn{1}{c|}{\rot{government}}&\multicolumn{1}{c|}{\rot{health}}&\multicolumn{1}{c|}{\rot{images}}&\multicolumn{1}{c|}{\rot{job}}&\multicolumn{1}{c|}{\rot{lifestyle}}&\multicolumn{1}{c|}{\rot{reading}}&\multicolumn{1}{c|}{\rot{shopping}}&\multicolumn{1}{c|}{\rot{social}}&\multicolumn{1}{c|}{\rot{sports}}&\multicolumn{1}{c|}{\rot{tool}}&\multicolumn{1}{c|}{\rot{traffic}}&\multicolumn{1}{c|}{\rot{travelling}}\\ \hline
     \multirow{7}{*}{\rot{front-end}}&\multirow{3}{*}{\tabincell{c}{device\\configuration}}&\texttt{openBluetoothAdapter}&530&269&16&11&49&51&198&132&2&2&779&1&649&17&86&511&222&11\\\cline{3-21}
     &&\texttt{createBLEPeripheralService}&&&&&&\\ \cline{3-21}
     &&\texttt{addService}&&&&&&\\ \cline{2-21}
     &\multirow{2}{*}{\tabincell{c}{cross-miniapp
    \\redirection}}&\texttt{navigateToMiniProgram}&&&&&&\\\cline{3-21}
     &&\texttt{referrerInfo.appId}&&&&&& \\\cline{2-21}
     &\multirow{2}{*}{\tabincell{c}{cross-user\\sharing}}&\texttt{updateShareMenu}&&&&&&\\\cline{3-21}
     &&\texttt{authPrivateMessage}&&&&&& \\\cline{1-21}
     \multirow{11}{*}{\rot{back-end}}&\multirow{9}{*}{\tabincell{c}{session\\key}}&\texttt{login}&14,744&48,810&3,622&1,526&34,422&21,140&11,416&9,956&454&6,164&86,823&2,426&132,115&6,486&3,849&33,303&10,124&1,166\\\cline{3-21}
  &&\texttt{getUserInfo}&11,332&38,231&3,248&1,164&26,322&23,203&8,489&7,307&380&4,972&64,401&1,314&9,5916&5,522&3,180&29,032&7,678&955
\\\cline{3-21}
      &&\texttt{getUserProfile}&30&86&30&4&40&8&28&45&2&56&197&5&265&18&6&47&18&1\\\cline{3-21}
      &&\texttt{getUserInteractiveStorage}&&&&&&\\\cline{3-21}
     &&\texttt{getWeRunData}&161&280&42&23&120&105&102&81&5&21&226&17&609&62&1040&428&34&6\\\cline{3-21}
     &&\texttt{getGroupEnterInfo}&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\\\cline{3-21}
     &&\texttt{getShareInfo}&&&&&&\\\cline{3-21}
     &&\texttt{chooseInvoice}&4&3&0&0&0&0&3&1&0&0&9&0&3&0&2&16&1&0\\\cline{3-21}
     &&\texttt{request}&&&&&&\\\cline{2-21}
     &\multirow{2}{*}{\tabincell{c}{cloud function}}&\texttt{calFunction}&&&&&&\\\cline{3-21}
     &&\texttt{CloudID}&&&&&&\\
     \bottomrule
    \end{tabular}
    \caption{Security-related APIs and Values\AY{Let's get some cell coloring trick!}}
    \label{tab:apis}
\end{table*}

% \begin{table*}[]
% \footnotesize
% \belowrulesep=0pt
% \aboverulesep=0pt
% \setlength\tabcolsep{2pt}
%     \centering
%     \begin{tabular}{c|c|l|r|r|r|r|r|l}
%     \toprule
%      Layer&Category&Name&\# app&\% app&avg. LOC&avg. node&avg. var&Description\\ \midrule
%      \multirow{7}{*}{front-end}&\multirow{3}{*}{device 
%      configuration}&\texttt{openBluetoothAdapter()}&&&&&&initialize bluetooth adapter\\
%      &&\texttt{createBLEPeripheralService()}&&&&&&initialize BLE peripheral service\\ 
%      &&\texttt{addService()}&&&&&&BLE peripheral security configuration\\ \cmidrule{2-21}
%      &\multirow{2}{*}{cross-miniapp redirection}&\texttt{navigateToMiniProgram()}&&&&&&initialize navigation to another mini-app\\
%      &&\texttt{referrerInfo.appId}&&&&&&used to check redirection source\\\cmidrule{2-21}
%      &\multirow{2}{*}{cross-user sharing}&\texttt{updateShareMenu()}&&&&&&initialize mini-app sharing\\
%      &&\texttt{authPrivateMessage()}&&&&&&verify valid user for private sharing\\\cmidrule{1-21}
%      \multirow{7}{*}{back-end}&\multirow{5}{*}{session key}&\texttt{login()}&&&&&&returns user token for session key acquisition\\
%      &&\texttt{getWeRunData()}&&&&&&returns encrypted data that requires session key to decrypt\\
%      &&\texttt{getGroupEnterInfo()}&&&&&&returns encrypted data that requires session key to decrypt\\
%      &&\texttt{getShareInfo()}&&&&&&returns encrypted data that requires session key to decrypt\\
%      &&\texttt{request()}&&&&&&related to sending token and receiving session key\\\cmidrule{2-21}
%      &\multirow{2}{*}{cloud function}&\texttt{calFunction()}&&&&&&used to call cloud functions\\
%      &&\texttt{CloudID()}&&&&&&used to obtain sensitive data from \wechat cloud\\
%      \bottomrule
%     \end{tabular}
%     \caption{Security-related APIs and Values}
%     \label{tab:apis}
% \end{table*}




\begin{table}[]
    \centering
    \aboverulesep=0ex
    \belowrulesep=0ex
    \footnotesize
    \setlength\tabcolsep{3.5pt}
    % \setlength\tabcolsep{1pt}
    % \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l|r|r|r|r|r|r|r|r}
    
    % Category &\tabincell{c}{insecure\\redirection\\target} &\tabincell{c}{redirected\\to insecure\\target}&\tabincell{c}{appsecret\\leakage\\as string}&\tabincell{c}{appsecret\\leakage\\in URL}&\tabincell{c}{session\\key\\leakage}&\tabincell{c}{frontend\\-maintained\\sensitive data}\\\midrule
    \toprule
    \multirow{2}{*}{category}&\multicolumn{2}{c|}{\tabincell{c}{unchecked\\redirection}}&\multicolumn{2}{c|}{\tabincell{c}{appsecret\\leakage(string)}}&\multicolumn{2}{c|}{\tabincell{c}{appsecret\\leakage (URL)}}&\multicolumn{2}{c}{\tabincell{c}{session key\\leakage}}\\ \cmidrule{2-9}
    &\# app&\% app&\# app&\% app&\# app&\% app&\# app&\% app\\\midrule
    % category & \tabincell{c}{missing\\redirection\\checking}  & \tabincell{c}{appsecret\\leaked as\\string} & \tabincell{c}{appsecret\\leaked in\\URL} & \tabincell{c}{session key\\leaked in\\URL}\\ \midrule
    
business&116&0.21&52&0.37&5&0.93&171&0.34\\
education&5,034&9.03&1,490&10.68&66&12.24&6,254&12.45\\
entertainment&385&0.69&117&0.84&5&0.93&541&1.08\\
finance&165&0.30&81&0.58&3&0.56&145&0.29\\
food&5,962&10.69&858&6.15&26&4.82&4,879&9.71\\
game&1,965&3.52&848&6.08&19&3.53&1,726&3.44\\
government&1,200&2.15&1,368&9.81&57&10.58&2,712&5.40\\
health&1,318&2.36&357&2.56&16&2.97&945&1.88\\
images&27&0.05&3&0.02&1&0.19&103&0.20\\
job&231&0.41&178&1.28&9&1.67&1,359&2.70\\
lifestyle&7,421&13.31&2,814&20.17&123&22.82&10,824&21.54\\
reading&133&0.24&855&6.13&2&0.37&245&0.49\\
shopping&27,933&50.10&3,011&21.59&131&24.30&11,074&22.04\\
social&379&0.68&171&1.23&6&1.11&1,524&3.03\\
sports&413&0.74&134&0.96&5&0.93&859&1.71\\
tool&1,900&3.41&1,271&9.11&55&10.20&5,337&10.62\\
traffic&1,074&1.93&305&2.19&9&1.67&1,397&2.78\\
travelling&104&0.19&35&0.25&1&0.19&151&0.30\\
total&55,760&100.00&13948&100.00&539&100.00&50,246&100.00\\


\midrule

 \bottomrule
    \end{tabular}
    % }
    \caption{Affected mini-apps w.r.t. mini-app category. M: missing redirection checking, AS: appsecret leaked as string variable, AU: appsecret leaked in URL, S: session key leakage, F: frontend-maintained sensitive data}
    \label{tab:eval-overview}
\end{table}
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%     vulnerability&insecure&secured&total&\%\\
%     absent checking&55,780&88&55,868&99.8\\
%     redirection victim&15,211&43,276&57,487&26.5\\
%     unchecked secret sharing&&&&\\\bottomrule \toprule
%     direct appsecret leakage&15,211&&&2.98\\
%     appsecret leakage in URL&1,266&&&0.25\\
%     session key leakage&101,029&&&19.8\\
%     \end{tabular}
%     \caption{Temporal table of all statistics}
%     \label{tab:my_label}
% \end{table}
\subsection{Experiment Setup}

\paragraph{Data Set} We collected our mini-apps from \wechat app via its built-in mini-app searching functionality. In \wechat app, users can either install a mini-app by clicking on a link shared by other user, or manually use keyword to search for a specific mini-app. To obtain a list of mini-apps to be downloaded, we reverse engineered \wechat, investigated the workflow of the search interface, and collected the metadata of $250,000$ mini-apps containing mini-app IDs, descriptions, and extra category info. Then, we created a crawler that runs on mobile phones to automatically download mini-apps. In average, our tool $3,000$ mini-apps a day. We used two mobile phones to work together, and eventually we obtained \totalnum mini-app packages for analysis.    


We implemented \textsf{CoffeCAN} in JavaScript with \texttt{esprima}\cite{esprima} to generate AST of mini-app source code, and Python to support multi-process processing. We performed our analysis on two Linux computers, each of which has 8 cores, Intel Core i7-8700 (3.20 GHz) CPUs and 16 GB RAM. It took 10 days for us to finish the analysis of the \totalnum mini-apps. 
% We implemented our analyzer based on Javascript, \texttt{esprima}, and Python for multi-processor support. 



%To collect the \wechat mini-apps, we reveres engineered  first acquired a mini-app ID list that contains 205,000 mini-apps via keyword searching in the \wechat mini-app discovery page. With the mini-app ID list collected, we then implemented a mini-app that reads the ID list and use the mini-app API \texttt{navigateToMiniProgram()} to trigger mini-app redirection, and developed a Python script based on \texttt{selenium} to confirm the cross mini-app redirection and eventually download mini-apps. We had implemented our crawler and performed the mini-app collection lasted for the last 15 months, and we finally collected 200,000 mini-apps in total, since there are mini-apps that are being removed from the market during the collection process.



% \paragraph{Experiment Setup}
% In total, among the mini-apps, we analyzed xxx LOC, xxx sensitive API invocations, xxx variable declarations, xxx logical expressions, and confirmed xxx appsecrets out of xxx interested credential-like string values. In the following sections, we will present our analyisis results with respect to the vulnerabilities that occur in the mini-app ecosystem.

\subsection{Evaluation Result}
In total, \texttt{CoffeeCAN} parsed \AY{TBD} apps, \AY{TBD} lines of code, with \AY{TBD} AST nodes and \AY{TBD} variable declarations. As shown in \cref{tab:apis}, for Bluetooth usage, \AY{TBD} mini-apps accessed bluetooth adapter, \AY{TBD} mini-apps created BLE peripheral services, and \AY{TBD} mini-apps use \texttt{addService} to configure their peripheral services. For cross-miniapp redirection, \AY{TBD} mini-apps issued cross-miniapp redirection to an external mini-app, but there are only \AY{TBD} mini-apps that used \texttt{referrerInfo} to perform their actions based on information from the redirection source mini-app. In terms of cross-user sharing, we only found \AY{TBD} and \AY{TBD} mini-apps that issued mini-app sharing and secret sharing verification respectively. This is partly because the API \texttt{authPrivateMessage} is relatively newly introduced into the mini-app framework in version 2.13.0 (September 2020).~\cite{secretsharing}. For back-end mechanisms, we found that there is a large percentage (\AY{TBD}) of mini-apps that involved \texttt{login} to obtain user login token and prepare for obtaining user sensitive data. Similarly, there are \AY{TBD} mini-apps that used network request API to communicate with their back-ends. Aside from third-party back-ends, there are also a large amount of mini-apps (\AY{TBD} and \AY{TBD}) that used \wechat cloud function feature \texttt{callFunction} to use cloud functions and  \texttt{CloudID} to obtain data from the cloud respectively.

In total, \textsf{CoffeeCAN} identified 55,760 mini-app with unchecked redirection, 13,948 appsecrets leaked as string values, 539 appsecrets leaked in URLs, and 50,246 potential session key leakages. With these preliminary data obtained, we further examine the existence and the impact of vulnerabilities in these mini-apps against \textsf{Coffee} attack. Note that unlike traditional app markets such as Google Play, \wechat mini-apps do not have a summary of total installation amount. Hence, to model the popularity (as well as the impact) of a specific mini-app A, we use the amount of referrers, i.e., the amount of external mini-apps that redirect to this specific mini-app A as the metric to evaluate mini-app popularity. In the following subsections, we examine the existence of these four following vulnerabilities: (1) mis-configuration of Bluetooth service protection, (2) misuse of cross-mini-app communication, (3) misuse of cross-user sharing, and (4) the leakage of Appsecrets and session keys. \looseness=-1


\paragraph{(1) Device mis-configuration}
For device configuration, we mainly focus on three APIs. The \texttt{openBluetoothAdapter()} API is invoked whenever a mini-app uses Bluetooth related functionality, which is used to identify mini-app associated with Bluetooth usage. The \texttt{createBLEPeripheralSever()} API is invoked when a mini-app would like to set the user's device as peripheral device, and therefore is used for identifying mini-apps that assign itself as peripheral service. And the \texttt{addService()} API is invoked when developer configures security mechanism adopted for the device, i.e., whether the encryption of read or write is turned on. The result is presented in {\red{XXXX}}

%\paragraph{(2) Mini-app redirection}  If a mini-app uses the \texttt{referrerInfo} to execute according to the navigation source mini-app metainfo including the mini-app IDs, extra data, and URL params, the mini-app should verify whether the navigation is issued from an expected mini-app either by comparing it with a certain mini-app ID using \texttt{==} operator (e.g., \texttt{\{wxid\}==referrerInfo.appId}) or with a list of mini-app using \texttt{in} operator (e.g., \texttt{referrerInfo.appId in wxidlist}). As discussed in \AY{label}, the redirection target mini-app that does not enforce source mini-app checking can be vulnerable in both attack scenes: the attackers can either attack the `target' (i.e., the vulnerable mini-app) with malicious mini-apps or directly attack the `source' (i.e., the victim that redirects to a vulnerable attack) and make profit.

% As show in table, we are surprised to find that only a tiny portion of mini-apps have enforced such a checking, leaving 10.94\% of the mini-apps investigated does not perform such a checking.


\paragraph{(2) Cross Mini-app communication mis-configuration} As shown in \autoref{tab:eval-overview}, we discovered that there are over 10\% of the investigated mini-app did not perform entry checking of navigation sources before using the \texttt{referrerInfo} to perform actions with the redirection info of the source mini-apps. These mini-apps can be targets of Coffee attacks, since the extra data can be intercepted, modified, and sent from unexpected sources (e.g., a malicious mini-app). We observed a concerning situation from the table in that most of the mini-apps with unchecked redirection are shopping mini-apps, which are heavily involved with financial-related activities, such as coupon offering, discount activities, and payment. This absent checking may eventually result in payment bypassing, or financial shuffling (repeated discount aquisition).

To understand the behavior of these mini-apps, we present the top 20 affected mini-apps with respect to the amount of referrers in \cref{tab:unchecked}. As shown in the table, the services provided by most popular vulnerable mini-apps cover a wide category: there are 3 online shops, 3 tool mini-apps, 3 social mini-apps, 3 lifestyles mini-apps associated with daily actions (e.g., searching for express delivery info), 2 health mini-apps, and even a popular mini-app associated with government affairs. Therefore, the attackers may perform a mini-app version of Intent injection attack that exploits the mini-app to make profit. For instance, if a shop mini-app as mentioned before may post coupons on other mini-apps as advertisement to attract users, where the coupon info (e.g., the discount) is carried in the extra data. If the shop mini-app does not perform entry checking, attackers can develop a malicious mini-app to issue modified coupon (e.g., modify the discount to 100\% off) info to make profit. 

% and can affect up to thousands of victims. As shown in \autoref{}
% When mini-apps are set as redirection target by multiple mini-apps, the mini-app that does not perform redirection source checking can be vulnerable to malicious mini-apps that perform a mini-app version of Intent injection attack, since the target mini-app executes with the extra data regardless of the source mini-app. We grouped these vulnerable mini-apps according to their popularity (i.e., number of victims

% \paragraph{Finding 5} {\it Most of the mini-apps do not check the redirection sources} This reveals that the navigation
\begin{table}[]
    \centering
    \setlength\tabcolsep{3.5pt}

    \footnotesize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{r|c|c|c|l}
    \toprule
         \# referrer&category&appid&vendor&service  \\
         \midrule
10,664&plugin&wx56c8****&--&product sharing\\
1,136&tool&wx13e4****&Jing Dong&product sharing\\%
783&tool&wx18a2****&GeiZan&tips payment\\%
528&lifestyle&wxdfbe****&Zhuke&home decoration\\%
284&lifestyle&wx6885****&Qianhai Baidi&delivery inquiry\\%100
223&traffic&wxf0f2****&Qiankou&car service\\
201&lifestyle&wx7b88****&Yiqi&hair saloon\\%
177&Health&wxb032****&Tencent&medical service\\%
64&government&wxb66a****&Qiusheng&traffic service\\%
60&social&wx19ac****&Yingji&social game\\%
53&tool&wxda9c****&Yuandian&law library\\%
42&games&wx845a****&Zhangfeng&game center\\%
32&business&wx1810****&Chutou&payment\\%
30&job&wx1131****&Qianjin&job info\\%51
29&social&wxb036****&Wechat&social circles\\%
26&health&wx862d****&Jing Dong&medical service\\%
26&shopping&wxde8a****&Meituan&food finding\\%
25&shopping&wxb1f2****&Yanzhi Youwu&fashion goods\\%LOOK&
24&shopping&wx2184****&MengMilk&milk shop\\%
21&social&wx734c****&Dazhong Dianping&food finding\\%


    % wx56c8f077de74b07c&10,664&product sharing$^{*}$\\
    % wx13e41a437b8a1d2e&1,136&online shopping\\
    % wx18a2ac992306a5a4&783&tips payment\\
    % wxdfbe172ee4082058&528&home decoration\\
    % wx6885acbedba59c14&284&home delivery tool\\
    % wxf0f2bd1ead5f89e8&223&car membership\\
    % wx7b88ebd0567bdb12&201&hair saloon\\
    % wxb032bc789053daf4&177&health mini-app\\
    % wxb66a0b7859131c7d&64&traffic rule break inquiry\\
    % wx19ac3436ccf898ee&60&red packet\\
\bottomrule
    \end{tabular}
    \caption{Top-20 affected mini-app that does not perform entry checking\\$^{*}$The first one is a mini-app plugin}
    \label{tab:unchecked}
\end{table}

\begin{table}[]
    \centering
    \footnotesize
    \begin{tabular}{r|c|c}
    \toprule
    \# of mini-app a specific mini-app redirects to& \# app & \% app\\
 >10&50&0.02\\
9&25&0.01\\
8&31&0.01\\
7&29&0.01\\
6&262&0.10\\
5&599&0.23\\
4&613&0.23\\
3&2920&1.11\\
2&34055&12.89\\
1&225612&85.40\\
total&264196&100.00\\\bottomrule
    \end{tabular}
    \caption{Amount of mini-apps each mini-app redirects to}
    \label{tab:redirection}
\end{table}

\begin{table}[]
    \centering
    \footnotesize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{r|c|c|c|c}
    \toprule
         \# referrer&category & service & appid &secret  \\
         \midrule
118&food&wine shop&wxe89b****&ed02cc****\\
53&tool&law library&wxda9c****&944493****\\
42&games&game center&wx845a****&0df030****\\
11&shopping&jewelry shop&wxb482****&b2b326****\\
11&shopping&jewelry shop&wx1126****&ff5559****\\
11&shopping&jewelry shop&wx0d3b****&53f77c****\\
11&shopping&jewelry shop&wx473b****&60d3fe****\\
11&shopping&jewelry shop&wxf398****&e13dd2****\\
11&shopping&jewelry shop&wx88a8****&b910e8****\\
11&shopping&jewelry shop&wxda03****&d96c66****\\
11&shopping&jewelry shop&wxe4e7****&5c369a****\\
11&shopping&jewelry shop&wx404f****&5ee970****\\
11&shopping&jewelry shop&wxb84e****&2c3e30****\\
10&games&game center&wx324a****&b5ce11****\\
8&business&web shop&wx46ec****&1d8b08****\\
5&health&medicine shop&wx893d****&54fa16****\\
4&shopping&health food&wx8d67****&1bf08a****\\
4&traffic&house rent&wx0453****&671a11****\\
4&shopping&group shopping&wx6878****&4222bb****\\
4&traffic&traffic service&wx0392****&bc4aff****\\

\bottomrule
    \end{tabular}
    \caption{Top-20 mini-apps that leaked appsecret}
    \label{tab:appsecret}
\end{table}

\begin{table}[]
    \centering
    \footnotesize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
         category&name& vendor&U&AS&AU&S\\ \midrule
         wx1610****&games&ball game&\CIRCLE&\CIRCLE&\CIRCLE&\CIRCLE\\
wxb473****&shopping&online shop&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx71e8****&sports&jumping rope&\Circle&\CIRCLE&\CIRCLE&\CIRCLE\\
wx33df****&shopping&NESCAFE&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx788b****&games&air battle game&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx0868****&games&adventure game&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx8f83****&shopping&underwear shop&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wxa98c****&traffic&hotel&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx052a****&shopping&furniture shop&\Circle&\CIRCLE&\CIRCLE&\CIRCLE\\
wx1791****&shopping&online shop&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wxe704****&lifestyle&cosmetics shop&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx7717****&games&humorous game&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx899e****&lifestyle&car rent&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wxdfd3****&lifestyle&online shop&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wxecb3****&education&design class&\CIRCLE&\CIRCLE&\CIRCLE&\Circle\\
wxe46b****&shopping&coat shop&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx2be4****&education&software class&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx81a4****&education&daily clock in&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wx81ac****&games&humorous game&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
wxaa92****&tool&pet playground&\CIRCLE&\CIRCLE&\Circle&\CIRCLE\\
\bottomrule
    \end{tabular}
    \caption{Results of mini-apps involved with multiple vulnerabilities: U for missing redirection, AS for appsecret leakage as string, AU for appsecret leakage in URL, S for session key leakage, \CIRCLE for presence, and \Circle for absence}
    \label{tab:miniapp_problems}
\end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%       Mini-app Category & Consequence \\
%         financial & \\
%         food &\\
%         shopping &\\
%     \end{tabular}
%     \caption{Example consequences of mini-app absent checking}
%     \label{tab:my_label}
% \end{table}
% \begin{table}[]
%     \centering
%     \begin{tabular}{r|c|c}
%          \# mini-apps redirected to a vulnerable mini-app & value & \%  \\
% >7&40&\\
% 7&9&\\
% 6&2&\\
% 5&4&\\
% 4&14&\\
% 3&29&\\
% 2&88&\\
% 1&389&\\
% 0$^{*}$&55205&\\
%     \end{tabular}
%     \caption{Number of mini-apps redirected to mini-app with absent checking\\ \AY{Although there is a large number of mini-app is mapped to 0 redirections, they can highly possible to be redirected to dynamically.}}
%     \label{tab:my_label}
% \end{table}

\paragraph{(3) Misuse of cross-user sharing}
To our surprise, in our dataset, we did not find absent of cross user sharing verification, all 515 cases of mini-apps we identified that used \texttt{updateShareMenu} to issue secret sharing performed such checking. There are two possible reason for this absence of vulnerability cases. First, the private messaging feature is a feature that has been relatively newly introduced after September 2020, therefore, there has not been enough developers that are aware of this feature and utilize the secret sharing feature in their mini-apps. Second, compared with mini-app entry checking, the official documentation explicitly introduced the usage of \texttt{authPrivateMessage} API to the developer in the documentation related to such private message feature. Therefore, the developers are aware of the necessity of using this API to authenticate users that enters the mini-app via private message.
% To detect secret sharing usages, we first identify the mini-apps that use \texttt{updateShareMenu} and assigned the parameter \texttt{isPrivateMessage} as true. Then, we check whether the mini-app invokes \texttt{authPrivateMessage} to check whether the user launches the mini-app as first-hand user. In our experiment, we found that there is only a tiny portion of mini-apps that used the private message feature, and these developers have enforced the secret sharing checking. This is partly because the private message feature is relatively newly introduced in SDK 2.13.0 (September 2020), and our current dataset has not covered enough updated mini-apps. However, if the developer forgets to check the secret sharing feature, the mini-app will be exposed in the similar danger as absent redirection checking are.


\paragraph{(4) Appsecret leakage}
We have identified 13,948 and 539 mini-apps respectively that leaked their essential appsecret key in their front-end packages as string values or in URLs. This is surprising because  the documentation of \wechat mini-app has warned the developers not to leak these appsecrets. Since the appsecret serves as a master password to verify the identity of mini-app owner, this leakage of appsecret key can be extremely dangerous to the mini-app since attackers may now fake themselves as mini-app developers, and thus invoke various \wechat cloud APIs or modify sensitive decrypted data sent to the mini-app (e.g., user account information that contains phone number as login identifier). 

% We first captured all string values that appear in the form of 32-bit hex string, and then we send this value and the corresponding mini-app ID to \texttt{api.weixin.qq.com/cgi-bin/token} to validate whether the string value is a real appsecret. 

\paragraph{Appsecret leakage as string variables}  As shown in \cref{tab:eval-overview}, there is still a reasonable amount of 15,211 mini-apps that leaked the essential appsecret as string variable, hard-coded as string variables in their mini-app front-end packages. We sorted the mini-app according to amount of referrers in \cref{tab:appsecret}, and discovered that most of the popular mini-apps are shopping (12 cases), whereas the majority of the rest of the mini-apps are associated with shopping activities as well (e.g., the first food mini-app is actually a wine shop). These mini-apps involved with this leaked appsecret may face severe consequences, since the attacker may use this appsecret to attack the mini-app by faking their identities. Moreover, attackers may also use malicious native apps in victims' devices to hijack network communication, obtain the users' login token to acquire session keys, and then steal the intercepted sensitive data by decrypting them with the session key. Further, we are even more surprised to find that mini-apps developed by large vendors may make this mistake as well, for example, we found 2 mini-apps fron Tencent and 1 mini-app from Meituan that have leaked the appsecret in their mini-app.
% \ZY{Table? Data?}

\paragraph{Appsecret leakage in URL strings} On top of the appsecret directly leaked in the source code as string variables, we also found 539 cases of appsecret leakage in network URLs. These cases occur when the developers directly encode the entire URL request containing not only the API URL \texttt{jscode2session} but also parameters (i.e., mini-app ID and appsecret) into their code. These developers may have directly use the string in request URL for convenience or write them in code comments as remainders, but this practice eventually leaked the appsecrets and expose the mini-apps in danger.


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%          app name & category & consequence\\
         
%     \end{tabular}
%     \caption{Examples of appsecret leakage consequences}
%     \label{tab:my_label}
% \end{table}
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%     \toprule
%          value & \# mini-app\\ \midrule
%          1cdc05151d64f3a4a6ebd0e9de64422a&17477\\ 
% 900150983cd24fb0d6963f7d28e17f72&12184\\ 
% 64a7f2b033fb593a8598bbc48c3b8486&9287\\ 
% c476515b7257635068360f86bebfded5&7702\\ 
% f45474f4488f32afb482708a49c7ffad&4150\\ 
% a941f5923e72b27adc646f2193e76219&4085\\ 
% bd782dd159db94b096a2cbdac9184b46&3968\\ 
% 914e2186012c189a3675704f65e8a989&3831\\ 
% c45d2aa4a23822a0813eaf5de25b7c2c&2902\\ 
% 89f5bc2d5c9b4c68b3c03aaad4d0af4f&2888\\ 
% \bottomrule
%     \end{tabular}
%     \caption{Most popular non-appsecret strings\AY{Leave here for now, redact after the paper is stable}}
%     \label{tab:my_label}
% \end{table}

\paragraph{(5) Session key leakage} CoffeeCAN identified 50,246 cases of potential session key leakage, both for suspected URL strings related to session keys and for mini-app APIs associated with sensitive data that with network-related APIs missing. We grouped the URLs and API usages, manually inspected these URLs, and presented the top URLs and API usages in \cref{tab:url} and \cref{tab:api} respectively.
% Normally, the session key is generated by the back-end with login token returned by \texttt{wx.login}, and this session key is used for decryptions of user sensitive data. Therefore, since the session key cannot be leaked to the front-end, all sensitive encrypted data has to be sent back to the back-end. To investigate the potential leakage, we investigate three problems in this section. Our study shows that there is a concerning amount of mini-apps that are highly possible to either leak the session keys via sensitive network URLs, or process encrypted data with leaked session key because there is no associated network requests found after sensitive encrypted data is being acquired.

\paragraph{Sensitive URLs}
In \cref{tab:url}, the first column shows the associated URL, followed by the URL type and number of mini-apps affected. In general, there are two types of sensitive URLs: duplication of wechat official API, or self-implemented session key getter. 
\begin{itemize}[leftmargin=*]
    \item \paragraph{Duplication of wechat official API} As shown in the previous motivatin exeample, the mini-app obtained its session key by sending the user login token invoke third-party network API \texttt{/wechat/code2session}, which in fact is a duplication of the wechat official network API \texttt{/sns/jscode2session}. In such a case, the third-party server is duplicating the \wechat official network API in their own server, and instead of filtering out sensitive information, the server returns the data from \wechat server as it is to the front-end. 
    \item \paragraph{Self-implemented session key getter} On top of duplication of \wechat APIs, we found self-implemented network APIs can also leak session keys. In our study, we found that there is a high portion of APIs appear as session key getter, which potentially sends session keys to the front-ends, such as \texttt{/wxapp/getNewSessionKey}.
\end{itemize}

As shown in \autoref{tab:url}, 80\% of the top-related URLs are session key getters, and half of the top-hit URLs affect over one thousand mini-apps. Therefore, compared with \wechat network API duplication URLs, session key getters appear in a more versatile form. These network APIs can appear directly as a URL path \texttt{/wxapp/GetsessionKey}, or appear as a URL parameter \texttt{/bale/pay.php?do=getSession}. On the other hand, there are only 2 top-hit URLs fall into the \wechat API duplication category. Aside from the \texttt{/auth/jscode2session} that is likely to leak session key as the case shown in \cref{fig:code}, we are surprised to find that there are still some mini-apps that attempt to send requests directly to \wechat API domain \texttt{api.weixin.qq.com}, which is blocked by the mini-app framework to prevent leaking session keys to the front-end. A possible explanation is that the developer attempted to get session key from the \wechat domain, and forgot to remove this line of code when he/she finds it not feasible.


\paragraph{API usage related to sensitive data} In \autoref{tab:api}, we summarized the top 10 associated API invocations after mini-app obtains encrypted sensitive data. We observe from the table that the most popular APIs are setData, log, and request, which are associated with caching sensitive data, logging out sensitive data, and sending these data to the back-end. We also observed that many mini-apps that require sensitive data invoked cloud function APIs (i.e., callFunction and CloudID) to utilize \wechat's encapsulation of data decryption. Still, as shown in the table, there are in total 1,973 mini-apps involved with missing network request to send the sensitive data, and all of these mini-apps's are involved with \texttt{getWeRunData} that returns encrypted user sports data. This means that these mini-apps are potentially leaking session keys, storing them in the front-end, and using them to decrypt these sensitive data, which results in a session key leakage.


\begin{table}[]
    \centering
    \footnotesize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \setlength\tabcolsep{1.8pt}
    \begin{tabular}{c|c|c|r}
         \toprule
         { API name} & { API type}&{example} & { \# app} \\ \midrule
         setData&data caching&this.setData&2,042\\
        log&logging&console.log&1,612\\
        request&network request&wx.request&1,197\\
        showToast&logging&wx.showToast&636\\
        showModal&user interface&wx.showModal&521\\
        callFunction&cloud function&cloud.callFunction&487\\
        CloudID&cloud function&cloud.CloudID&479\\
        stringify&utility&JSON.stringify&442\\
        hideLoading&user interface&wx.hideLoading&385\\
        getStorageSync&data caching&wx.getStorageSync&378\\
          \bottomrule
    \end{tabular}
    \caption{Mini-app behavior related to sensitive data}
    \label{tab:api}
\end{table}
\begin{table}[]
    \centering
    \footnotesize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{l|c|r}
         \toprule
          URL & type & \# Mini-app  \\ \midrule
    api.weixin.qq.com/sns/jscode2session&D&2,533\\
     /admin/index.php?m=get\_session\_key&G&1,737\\
     /auth/jscode2session&D&1,284\\
     /wxapp/getNewSessionKey&G&1,097\\
     /wxapp/Getsessionkey&G&659\\
     /bale/pay.php?do=getSession&G&466\\
     /mini\_shop\_h5/Setting/get\_session\_key&G&332\\
     /login/getJcbWxSessionKey&G&280\\
     /entry/wxapp/GetSessionkey&G&209\\
     /weapp/member/get\_session\_key.json&G&169\\
          \bottomrule
    \end{tabular}
    \caption{Top URLs related to session key. G: session key getter; D: duplication of wechat official API}
    \label{tab:url}
\end{table}
% 7997 G
% 5741 D (2533 blackened)


==> paper/05_mitigation.tex <==
% From our study, we discover that the mini-apps may still be vulnerable in practice. A malicious attacker can still be able to download, decompile, analyze, and utilize the \textsf{Coffee} attack to exploit vulnerable mini-apps. Therefore, in this section, we present four ways to mitigate this problem, both from the front-ends and the back-ends.
%Although some threats are caused by the architecture of the mini-app from the high level (e.g., UI management), which requires the defense measure to be made  
% Since there are multiple attacks and each attack may vary from one platform to another, depending on the implementation, it is not piratical to design a defending framework that can work against all the current products. Therefore, in this section, we present design principles for protecting mini-apps regarding pitfalls we have identified in this paper.










 


    

 

%since the SDK encapsulates the network API within the SDK, the mini-app server SDK is able to manage the session keys obtained from the wechat server. Then, the SDK can block the network request containing session key, or immediately acquire a new session key after this session key is used. Similarly, the decryption of sensitive user data can also be automatically performed by the \wechat server SDK.

 
 
%has the interfaces of fetching    



%Similar to appsecrets, the leaked session key may cause numerous security problems. To prevent developers from leaking session keys to front-end, the mini-app should enforce the detection of session key leakage in their SDK. For example, since the SDK encapsulates the network API within the SDK, the mini-app server SDK is able to manage the session keys obtained from the wechat server. Then, the SDK can block the network request containing session key, or immediately acquire a new session key after this session key is used. Similarly, the decryption of sensitive user data can also be automatically performed by the \wechat server SDK.



%the mini-app frameworks should transform vulnerable fully-optional add-on mechanisms into mechanisms that at least involve part of built-in mechanisms. This can be done either by encapsulating mechanism implementation into a simple API for developers to invoke, or enforcing the mechanism as a built-in mechanism that is transparent to developers.
  







%Similar to appsecrets, the leaked session key may cause numerous security problems. To prevent developers from leaking session keys to front-end, the mini-app should enforce the detection of session key leakage in their SDK. For example, since the SDK encapsulates the network API within the SDK, the mini-app server SDK is able to manage the session keys obtained from the wechat server. Then, the SDK can block the network request containing session key, or immediately acquire a new session key after this session key is used. Similarly, the decryption of sensitive user data can also be automatically performed by the \wechat server SDK.




\ignore{
\textbf{Peripheral Management.} 
As reported in our paper, different platforms may have different security polices to deal with the peripheral that connects to it, which leads the corresponding APIs are also scientifically different. Therefore, finding an approach that can balance the security and the compatibility can be challenging.   \wechat have provided us a excellent practice, where \wechat provided different APIs for Android and iOS, and the mini-apps developers can choose to customize the security levels correspondingly according to the intended security requirement. Therefore, as mitigation, we argue all the manufactures should follow the practice of \wechat, enabling the most security option for the mini-app developers to protect the mission critical mini-apps.  

\textbf{Resource Management.} Resources, including local sensitive resources and network resources, should be better protected and isolated. 
Recall that the root cause of the network isolation escape or collusion attacks is that the OS fail to maintain the current status of the resources. Resources exchanged from two mini-apps with different privileges, blurring the security boundary of the resource isolation. Therefore, the ultimate defense is to design a stateful resource management mechanism within mini-app host app, allowing the mini-app host app to monitor and track the sensitive resource. When attacks occur, the host app could terminate the process and direct alerts to the end user.   

However, the above solution requires the refactoring of the entire mini-app architecture, where a state machine should be introduced and enforced, which may require significant implementation efforts. To mitigate the risk, manufactures may choose to give the end-user a chance to make decision in particular case, which can make the attack hard to be deployed. For example, when one mini-app attempts to deliver data to another app,  the host app can  prompt a dialog to the user for consent (e.g., Displaying ``$Miniapp_{1}$ attempts to transfer data to $Miniapp_{2}$''). Although currently, due to the absent of the state machine, the host app is still not able to know what kind of resource to be transmitted through cross-app channel, the dialog may raise alarms to the user, avoiding the sensitive data to be leaked without user's awareness.      

\textbf{Cross-app Communication Management.} In the context of mini-apps, for two mini-apps intend to communicate with each other, the host app will establish a network channel for them, instead of handling the data locally. Therefore, the long term defense is to clearly separate the cross-app communication channel from the network communication channel, forcing all the data exchanged under the protection of the host app, instead of going out to the network. This can ultimately prevent the attacks such as the MitM attacks. The short-term defense is to secure the network communication, enforcing data encryption and digital signature to protect the confidentiality and the integrity of the data transmitted. 
 


\textbf{UI Management.} The shareable UI is a hybrid solution, which extends the shareable features of the legacy web application, allowing the UI to run independently with the specific request attached. Due to the novel shareable feature,  session riding attacks can be deployed. Therefore, we should essentially limit the capabilities of UI sharing. For example, \wechat and \tik allowed the developer to customize whether a specific UI is shareable, and the solution can prevent the an attacker arbitrarily launch UIs according to his demand. However, this cannot eradicate the attack, and  we should also prevent an attacker to attach an unintended request with an UI by manipulating the link referring to the UI. To that end, we could ($i$) obfuscate the link and ($ii$) enforce the use of cryptography techniques such as digital signatures. All these techniques can prevent the attacker modify the link. 


 

%, and the designer must handle the platforms' inconsistency. When that happens, we found that the designer usually trades off the security for compatibility. For example, Bluetooth pairing is the key negotiation process for two Bluetooth devices to achieve communication confidentiality and authentication. iOS devices adopt the passive pairing policy, which is less secure. While Android uses the active pairing for stronger security. We found the in-app APIs regarding Bluetooth pairing trend to implement the passive pairing for compatibility, downgrading the security policy of Android devices.  
 
}

==> paper/06_casestudies.tex <==
 
 
  

 

%As discussed in \S\ref{subsec:attackworkflow}, there are two types of attacks against the vulnerable mini-programs. Based on their impacts and consequences, we further propose three different concrete attacks, i.e., (A1) account hijack attacks and (A2) promotion abuse (achieved through sensitive data manipulation as discussed in \S\ref{attack:data}), and (A3) services theft (achieved through services manipulation as discussed in \S\ref{attack:services}).


 
% The predictable  data (\eg, users' phone numbers) can be used as the primary key in the mini-program's back-end to retrieve the user information, and if this data can be manipulated, the attacker mount attacks go beyond the data manipulation (described next).
%  %
%  To be more specific,  s











%Leaking \texttt{MK} from mini-program code can lead to a variety of devastating attacks against both mini-program users and servers. For example, \textit{We Proudly Serve} from \textsf{Nestle} has leaked their \appsecret, and in our experiments,  we hijacked multiple accounts (we used our own accounts to demonstrate the impacts) by enumerating the phone numbers, we can harvest a large amount of \textit{We Proudly Serve}'s user information. We discovered that a banking mini-program (\textit{`Pinyue Benefit Center'}) from ICBC that uses the Werun data for promotion where users gain the `energetic value' with the steps they walked each day, and such a value can be used to redeem for gifts in the shop.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


% \begin{table*}[]

%     \centering
% \scriptsize
%     \aboverulesep=0pt
%     \belowrulesep=0pt
%     \begin{tabular}{r|l|l|l|l|l|l}
%     \toprule
%          {\bf Company Name} & \bf The mini-program Name& \bf Category & \textbf{Data} & \textbf{Attacks} \bf &\textbf{AppID}& \textbf{The Leaked \appsecret }\\
%          \midrule
% \multirow{17}{*}{Tencent}&AI Illustrator YUI&games&\ding{192}& A1 &wxaf3a********e7c8&77c8************************3bcd\\
% &Longzu Illusion Game&tool&\ding{192}& A1 &wxa565********5216&e31d************************8901\\
% &Pipixia Videos&entertainment&\ding{192},\ding{193}& A1, A2&wx8e41********8a4f&4614************************032c\\
% &Hispital Copay Platform&health&& &wx0646********5bbb&b9ff************************11eb\\
% &Tencent Billiard&entertainment&\ding{192}& A1 &wx2f7f********31ee&6de7************************596a\\
% &Moment Gallery&tool&\ding{192}& A1 &wx34ce********fef3&05de************************c88e\\
% &Health Data Assistant&education& & &wx6920********a49b&6201************************eda8\\
% &Personality Test&games&\ding{192}& A1 &wxfbe7********d8d0&a1d5************************9c2d\\
% &Everyday Cool Run&social&\ding{192}& A1 &wxcf75********f808&05b6************************1827\\
% &Financial Regulation Platform&tool&\ding{192}& A1 &wxebfa********c5c2&6a0f************************4a80\\
% &Campus Cloud Card&tool& & &wx626b********071b&07f9************************a0ad\\
% &Intelligent Welcoming Assistant&e-learning&\ding{194}& A2   &wxadc5********3159&260d************************c063\\
% &Click to earn&health&\ding{192}& A1 &wxa564********6246&d76d************************dfa6\\
% &Video Marking&games&\ding{192}& A1 &wxfd80********924f&f0f6************************27f7\\
% &Tencent Everyday Chess&games&\ding{192}& A1 &wx2225********fe10&27e2************************4163\\
% &Wepaytest&education&& &wx80f9********56c2&8e29************************75ba\\
% &Tuyan&games&\ding{193}& A2 &wx7edb********e67f&c3d6************************eadb\\ \cmidrule{1-7}
% \multirow{6}{*}{Nestle}&NESCAFE space&food&\ding{194},\ding{192}&   A1, A2 &wx33df********ccc1&8d39************************3490\\
% &Nestle Coffee Membership&tool&\ding{194},\ding{192}& A1, A2 &wx693d********d699&76ad************************c2bb\\
% &Yiyang Member Center&lifestyle&\ding{194},\ding{192}& A1, A2 &wx02a9********87b9&e5b0************************f4b5\\
% &Nestle Customer Service&food&\ding{194}& A2 &wx7cff********b6fe&c1c6************************054b\\
% &DolceGusto Member Center&shopping&\ding{194},\ding{192}& A1, A2 &wx0e08********cb22&c315************************f293\\
% &We Proudly Serve&shopping&\ding{194},\ding{192}& A1, A2 &wx1bb7********1204&c5bf************************4397\\ \cmidrule{1-7}
% \multirow{4}{*}{Sanofi}&Nutrition Nursing UAT&health&\ding{194},\ding{192}& A1, A2 &wx036f********29a1&d93e************************f757\\
% &Nutrition Nurses&business&\ding{194},\ding{192}& A1, A2 &wx4049********ee80&1e51************************62fc\\
% &Nutrition Nursing&business&\ding{194},\ding{192}& A1, A2 &wxaa42********74ee&1296************************ee5a\\
% &Nutrition NursesUAT&business&\ding{194},\ding{192}& A1, A2 &wxa0f4********58fa&a8d8************************bac3\\ \cmidrule{1-7}
% \multirow{4}{*}{China Unicom}&Failure report and Complaint&finance&\ding{194}& A2 &wx6d28********fd6e&9854************************0b25\\
% &Unicom Club&finance&\ding{194},\ding{192}& A1, A2 &wx2002********0de4&20d3************************0377\\
% &Henan 114 Move Car&tool&& &wxf332********4f01&13f3************************4771\\
% &Fengxingdong Cloud Shop&shopping&\ding{194}& A2 &wx4e5e********35be&1dca************************b8cd\\ \cmidrule{1-7}
% \multirow{3}{*}{Bank Of China}&BOC Virtual Bank&shopping&\ding{192}& A1 &wx3db9********36e1&7c58************************caff\\
% &Data Center Meetings&shopping&\ding{192}& A1 &wx1ce1********d65e&00e6************************6855\\
% &BOC Technical Summit&business&\ding{192}& A1 &wxd577********6d0d&1fab************************6b39\\\cmidrule{1-7}
% \multirow{3}{*}{Hitachi}&Hi Design Platform&tool&\ding{192}& A1 &wx3cb9********0d70&b876************************a82a\\
% &York Design&tool&\ding{192}& A1 &wx6e50********2d6e&3879************************3aab\\
% &AI sense&business&\ding{192}& A1 &wx7342********db84&7c3a************************a96b\\\cmidrule{1-7}
% \multirow{2}{*}{Shou Gang} &Cloud Security Community&tool&& &wx3571********b9b0&e76d************************a66f\\
% &\ding{192}rmation Collection System&lifestyle&& &wxf869********1d0b&4358************************0048\\\cmidrule{1-7}
% \multirow{2}{*}{China Mobile} &Mobile Cloud Calculator&finance&& &wx7c62********9ef2&fc29************************888d\\
% &Home Internet Assistant&finance&& &wx6ce5********bb8b&761b************************e0e4\\\cmidrule{1-7}
% \multirow{2}{*}{ICBC}&ICBC Intelligent Messaging&lifestyle&\ding{194}& A2 &wxae7a********3fe9&4def************************6dbc\\
% &Pinyue Benefit Center&traffic&\ding{192},\ding{193},\ding{195}& &wx1a6a********39f4&7889************************2a7b\\ \cmidrule{1-7}
% \multirow{2}{*}{Volkswagen}&Audi Sales Consultant&shopping&\ding{192}& A1 &wxa8d8********9b29&6849************************155c\\
% &Audi Online 4S Shop&shopping&\ding{192},\ding{193}& &wx46a6********c671&48ce************************103a\\

% %} 
% \bottomrule

%     \end{tabular}
%     \caption{The top-10 Fortune 500 companies that have the most number of mini-programs leaked the \appsecret. \ding{192} user info; \ding{193} shared info; \ding{194} phone number; \ding{195} werun data. Note that none of them used any paid services.  
%     }
%     \label{tab:appsecret}
%      \vspace{-0.2in}
% \end{table*}



==> paper/3_attack.tex <==




\section{(DEPRECATED SECTION)}

\input{table/attack-tbl}
Having presented the background of how various cryptographic keys (\autoref{tab:symbols}) are used to access the sensitive data, we then discuss our threat model and describe the possible attacks when the assumptions made by \wechat are violated. In particular, as shown in \autoref{tab:attackspossible}, we discuss the possible attacks with and without leaking the \appsecret. \looseness=-1






\AY{THE FOLLOWING SUBSECTION IS CURRENTLY DEPRECATED, LEAVING HERE FOR POTENTIALLY REUSABLE SNIPPETS}
\subsection{Attack Procedures}

 {According to how the mini-programs utilize the sensitive data, different mini-programs may expose themselves to different attacks when their \appsecret{s} are leaked. In general, we conduct two types of case studies corresponding to our two types of attacks to show how the attacker can manipulate the predictable data (one case study) and the non-predictable data (three case studies) to cause the serious impacts against their users. Particularly, we would like to present the implementation details in the first case study with other case studies briefly discussed, since the implementation processes of the later three case studies are similar to the first one.   }

\subsubsection{Manipulating  Predictable  Data (i.e., users’ phone numbers)} Recall that the  predictable  data  can be used as the primary key to retrive the user information, and if leaked, the attacker can mount the account hijacking attacks. Next, we present a concrete account hijacking attack 
against \texttt{Nestle (We Proudly Serve)} mini-program to further demonstrate the consequence of the attack.
While performing our attack, we first registered two accounts: a victim account and an attack account, with \wechat, and use the mini-program with these two accounts, as we must make sure we attack our own account, a community practice for the attack work.
As described in \S\ref{sub:overview:attack}, the attack involves two stages: (I) Obtaining attacker’s encryption key (\sessionkey), and (II) User phone number retrieval and manipulation.


\subsubsection{Manipulating  Non-Predictable  Data} We have already demonstrated how an attacker can mount account hijack attacks via the predictable data (i.e., phone number), and in the following, we would like to illustrate how the attacker can manipulate the non-predictable data. Particularly, we would like to demonstrate how an attacker can manipulate the WeRun and User Information.

\begin{itemize}
    \item  \textbf{\texttt{WeRun} Data Manipulation for Cheating and Profit.} {\texttt{WeRun} data contains the steps a user walks each day. Among the vulnerable mini-programs, we observed that some mini-programs use this feature to monitor the sports condition of users, such as universities (e.g., Beihang University)  that require minimal daily sports for students, and these daily sports will be used to grade the students. As a student,  he or she can follow the steps \ding{182}--\ding{188} that introduced in our previous case study to manipulate the daily step counts and achieve cheating.  
    Some mini-programs (e.g., Zhongchuang Steps \& Entertainment) %advocates users to protect the environment by allowing users to 
    reward their users based on the user's daily step counts. As such, a malicious user may also exploit the mini-programs by manipulating the steps to earn the rewards.} \looseness=-1
    \item \textbf{User Information Access for Account Information Stealing}  The \texttt{getUserProfile} API enables mini-program developers to acquire the basic account information such as avatars, gender, and nicknames. However, the information can also be collected by attacker if the \appsecret is leaked, since the attacker can use the steps \ding{182}--\ding{186} to decrypt the encrypted user information, and send the decrypted data to a remote server. For example, we confirmed that \texttt{Cool Run Everyday} from \Tencent themselves leaked their \appsecret, enabling attackers to collect sensitive the user information.

\end{itemize}





 
 \begin{figure}
    \centering
    
     \includegraphics[width=0.9\linewidth]{image/attack356.pdf}
    \caption{Attack workflow}
    \label{fig:attack}
    
\end{figure}



==> paper/4_details.tex <==
% \section{The Coffee Attacks}
% \subsection{Coffee Attack with Session Key}
% \begin{itemize}
%     \item User login
%     \item Token exchange
%     \item Session key interception
%     \item Data manipulation
% \end{itemize}
% \subsection{Coffee Attack with App Secret}
% \begin{itemize}
%     \item Appsecret leakage
%     \item User login
%     \item Token interception
%     \item Data manipulation
% \end{itemize}
% \subsection{Chained Coffee Attack}
% \begin{itemize}
%     \item Variant 1/2 exploitation
%     \item Mini-app redirection
% \end{itemize}

% \AY{EVALUATION PART.}


 

% Next, we perform a few case studies to demonstrate the impact of \appsecret leakage vulnerability. %for the vulnerable miniapps we collected  to show the significance of security impact of our findings. We could have analyze all of them, but we feel we do not have to do so, since there could be many unpopular apps, similar to the apps in the Google Play. Moreover, our evaluation has already demonstrated the impacts from the aggregation level.  As such, 
% Certainly we cannot access all of the vulnerable miniapps due to the sheer volumns, and we thus decide to mainly focus on the popular apps. To this end, we select the miniapps developed by high-profile companies (e.g., Fortune 500), and launch the attacks against them in a controlled environment using our own account.
% %
% However, not all the attacks can be launched on those  high-profile miniapps, since they may not use the resources of interest. For example, attacks against sensitive data for promotion abuse only work when the victim miniapp consumes share info or WeRun data. For those attacks that cannot be demonstrated with the high-profile miniapps, we use other miniapps we can find to show the attack consequences. 



\ignore{
\begin{table*}[]

    \centering
    \footnotesize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{r|l|l|l|l|l}
    \toprule
         {\bf Company Name} & \bf The Mini-app Name& \bf Service& \bf Accessed Data &AppID& The Leaked \appsecret \\
         \midrule
\multirow{6}{*}{Nestle (6)}&Nestle DolceGusto Member Center&info&Membership& &wx0e0801****0ccb22&c315d53c8559********41f3de23f293\\ 
&Nestle Customer Center&\ding{194}&Customer Service&wx7cfffc****2cb6fe&c1c6e1bb34eb********36d1bcc7054b\\ 
&Nestle Flagship Shop&info,share&Online Shopping&wx8ab43c****e821ec&6e288bfbb5f1********824f4e068246\\ 
&Nestle Ice Cream Happy Sharing&info&Online Shopping&wx856d1a****db51bb&cb63ec2b59f7********0591e9e4c7f9\\ 
&Nestle Coffee Member CLub&\ding{194},info&Membership&wx693d49****efd699&76addd6853c1********4b305403c2bb\\ 
&We Proudly Serve&\ding{194},info&Membership&wx1bb769****cd1204&c5bfc2f397b0********32a08c5a4397\\ \cmidrule{1-1}
\multirow{3}{*}{Tencent (3)}&Cool Run Everyday&info&Game&wxcf7574****9cf808&05b6705c4e49********e3ec6a8b1827\\ 
&Tencent Billiards&info&Game&wx2f7fda****d031ee&6de7dba82ea5********bde00af2596a\\ 
&Tencent Everyday Battle Chess&info&Game&wx222566****15fe10&27e2c95ee6d8********5c3b20004163\\ \cmidrule{1-1}
\multirow{2}{*}{China Telecom (2)}&China Telecom Guangdong Job Center&info&Job Hunting&wx387938****dac055&2ccc88b5eeed********37598daf73ce\\ 
&China Telecom 5G Membership&\ding{194}&Membership&wx77120a****c97e10&110cc0d6a8a1********b9e9b0a68920\\ \cmidrule{1-1}
\multirow{2}{*}{China Mobile (2)}&China Mobile 139 email&\ding{194},info&Email service&wxbb71dd****b241c6&6559cdb6a96d********922e08db1694\\
&Xinjiang Mobile Network Expert&\ding{194}&Network service&wx8d024d****26a222&c0c5547b955c********74224d5d01d9\\\cmidrule{1-1}
\multirow{2}{*}{China Post (2)}&China Post Car Holders&info&Car Service&wx3d12c0****6c8ac7&a9b39e4a8ad5********b7bfc9836596\\
&China Post Library&info&Library Management&wxf17464****fe7d1e&6a0fc5bec9bf********029b4b6426e3\\\cmidrule{1-1}
\multirow{2}{*}{HP (2)}&HP China Official Shop&\ding{194},info,share&Online Shopping&wxb3bd23****b71a8f&55f198de96ec********bd21da0fe699\\ 
&HP Shining SHop&-&Online Shopping&wx6cf02e****84cd25&00c3bd48f833********6905c9ed6382\\ \cmidrule{1-1}
\multirow{2}{*}{Mazda (2)}&Mazda 4S Shop&info&Car Service&wxbf3596****9ec33e&291282f1fe55********ffa69e1d2c6a\\ 
&Mazda Ningyuan Shop&info&Online Shopping&wx950114****73996b&67ae1eb49951********8fc318cca733\\ \cmidrule{1-1}
Ford (1)&Ford Automobile Price Lookup&-&Tool&wxf17f34****173dfc&8ee65b2c6d53********f127c469ca09\\ 
Hyundai \& KIA (1)&Hyundai - KIA Car Accessories&-&Online Shopping&wx37c559****09e679&ce6a4d07efc3********97cb6ac747a4\\ 
Hyundai (1)&Hyundai Accessories Shop&info&Online Shopping&wxc24f31****01bf6d&b80f9d1f7155********2f5c0d47f0aa\\ 
KIA (1)&Tianjin KIA Automobile&info&Onlien Shopping&wx04a75d****367052&bb9b8864fa93********f4d412fde1d2\\ 
Toyota (1)&Toyota Online Shop&\ding{194},werun,info&Online Shopping&wx4fc971****749395&45efd214ff5b********ea0ddff6d9cd\\ 
Volvo (1)&Volvo Repair&info&Car Service&wx64fd8c****7bb2f5&f6d06690b5c2********e452d4cf5557\\ 
Cisco (1)&Cisco Collaboration&info&Product Promotion&wx165c7b****78c840&7a137597d24e********f6aebcb3a5cc\\ 
Lenovo (1)&Lenovo Inteliggent Travelling&\ding{194},info&Tool&wxea9cc8****7eb436&1661322ad673********37efb8b9bf06\\ 
Huawei (1)&Huawei Companion Club&info&Membership&wx8ff299****09f4a3&49959a260a54********a3c2751d2f05\\ 
Bank of China (1)&BOC Virtual Bank&info&Virtual Bank&wx3db9d1****7e36e1&7c58efe92830********b0745088caff\\ 
China Life (1)&Salesperson account book&\ding{194}&Tool&wx1eb67a****4f0ab8&5fb5cdc6a6d5********4f3c529b780b\\
Ansteel Group (1)&Ansteel Milk Online Shop&info&Online Shopping&wx06ea38****742f29&6006c93fb84a********bfc98c141fbd\\
Pingan (1)&Pingan Free Insurance&info&Insurance Promotion&wx2880e1****da6a98&282d87d7bc8c********7592bb7dc2ac\\ 
Petro China (1)&Petro China Labor Security&-&Online Shopping&wx5e6e04****377ebc&3118d627c696********0b61769d781b\\ 
Sinopec (1)&Sinopec Gueizhou&\ding{194},info&Car Service&wx9a9515****883445&19450d6c760d********7f34d82deb4d\\ 
SinoPharm (1)&SinoPharm Engineering Hiring&info&Job Hunting&wxb77466****bcd35d&7e26b6075e97********5cfc3a1c3363\\ 
Bosch China (1)&Bosch China Hiring&info&Job Hunting&wx4cfc8d****e5e1c1&48487340a435********34b1cd8037fb\\ 
Nike (1)&Nike Fitness Center&info&Sports&wx081618****8041bc&095cb97dbbb4********2aba5f40b2da\\ 

%} 
\bottomrule

    \end{tabular}
    \caption{The list of the Fortune 500 companies whose mini-apps have leaked the \appsecret. \AY{Need update}
    }
    \label{tab:appsecret}
    
\end{table*}}

%\subsection{Vulnerable Miniapps from the Fortune 500 Companies} 
%\label{subsubsec:top}

% To identify who developed the vulnerable miniapps, we sampled 400 vulnerable miniapps from our dataset (approximately 1\%) and examined all of them, and we were surprised to find that there are 37 miniapps developed by the Fortune 500 companies

% % Note that although we have used the keywords generated from such as Fortune 500,some of the collected mini-apps are not from these companies. They are collected because their names also contained some of the generated keywords. Therefore, we manually examined all the \leakedapps vulnerable mini-apps and identified \companyapps mini-apps exactly from the world's top commercial companies.


\begin{table*}[]
    \centering
    \scriptsize
    \setlength\tabcolsep{2pt}
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
    \toprule
    \multirow{3}{*}{\bf Category}&\multicolumn{18}{c }{\bf Ratings distribution} \\ \cmidrule{2-19}
   &\multicolumn{3}{c|}{\textbf{1.0-1.9}}&\multicolumn{3}{c|}{\textbf{2.0-2.9}}&\multicolumn{3}{c|}{\textbf{3.0-3.9}}&\multicolumn{3}{c|}{\textbf{4.0-4.9}}&\multicolumn{3}{c|}{\textbf{5.0}}& \multicolumn{3}{c}{\textbf{Unrated}} \\ \cmidrule{2-19}
& \# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln\\ \cmidrule{1-19}
business&0&0&0.00&0&1&0.00&0&4&0.01&0&38&0.09&0&4&0.01&12&812&2.02\\
education&0&1&0.00&0&4&0.01&0&38&0.09&7&216&0.55&0&15&0.04&126&3,714&9.39\\
e-learning&0&0&0.00&0&2&0.00&0&4&0.01&0&11&0.03&0&1&0.00&37&118&0.38\\
entertainment&0&2&0.00&0&7&0.02&2&17&0.05&1&23&0.06&0&0&0.00&8&226&0.57\\
finance&0&0&0.00&0&2&0.00&0&2&0.00&0&11&0.03&0&0&0.00&0&82&0.20\\
food&0&0&0.00&0&1&0.00&0&2&0.00&0&49&0.12&0&2&0.00&16&1,795&4.43\\
games&0&0&0.00&18&23&0.10&63&124&0.46&9&37&0.11&0&0&0.00&161&294&1.11\\
government&0&0&0.00&0&2&0.00&0&7&0.02&0&48&0.12&0&1&0.00&24&645&1.64\\
health&0&0&0.00&0&1&0.00&0&3&0.01&0&49&0.12&0&2&0.00&4&510&1.26\\
photo&0&1&0.00&0&0&0.00&0&2&0.00&1&7&0.02&0&0&0.00&0&27&0.07\\
job&0&0&0.00&0&1&0.00&0&10&0.02&0&29&0.07&0&1&0.00&2&351&0.86\\
lifestyle&0&0&0.00&0&1&0.00&0&37&0.09&3&227&0.56&1&19&0.05&120&5,398&13.50\\
shopping&0&2&0.00&0&0&0.00&2&23&0.06&10&299&0.76&0&26&0.06&42&9,205&22.62\\
social&0&0&0.00&0&3&0.01&0&5&0.01&1&38&0.10&0&0&0.00&14&279&0.72\\
sports&0&0&0.00&0&0&0.00&0&2&0.00&0&33&0.08&1&6&0.02&7&213&0.54\\
tool&0&3&0.01&3&24&0.07&4&48&0.13&19&325&0.84&4&20&0.06&441&3,955&10.75\\
traffic&0&0&0.00&0&5&0.01&0&16&0.04&0&71&0.17&0&3&0.01&8&574&1.42\\
travelling&0&0&0.00&0&0&0.00&0&3&0.01&0&12&0.03&0&1&0.00&2&175&0.43\\
uncategorized&0&0&0.00&0&0&0.00&0&0&0.00&0&0&0.00&0&0&0.00&0&5&0.01\\
TOTAL&0&9&0.02&21&77&0.24&71&347&1.02&51&1,523&3.85&6&101&0.26&1,024&28,378&71.92\\

 
\bottomrule
% business&0&0&0&0&0&0&1&3&3&37&0&570&614\\
% education&0&0&0&2&1&4&8&34&75&145&0&3,290&3,559\\
% entertainment&0&0&1&1&2&6&9&10&14&16&0&188&247\\
% finance&0&0&0&0&0&1&0&2&6&4&0&59&72\\
% food&0&0&0&0&1&0&1&1&13&37&0&1,523&1,576\\
% games&0&0&1&3&23&68&135&182&51&12&0&1,252&1,727\\
% government&0&0&0&0&0&0&1&5&17&32&0&556&611\\
% health&0&0&0&0&1&0&1&4&4&36&0&392&438\\
% images&0&0&0&1&0&0&1&1&2&6&0&25&36\\
% job&0&0&0&0&0&1&4&6&14&13&0&280&318\\
% lifestyle&0&0&0&0&0&0&7&24&81&167&0&4,517&4,796\\
% reading&0&0&0&0&1&1&1&2&5&5&0&177&192\\
% shopping&0&0&0&1&1&0&5&20&95&239&0&6,887&7,248\\
% social&0&0&0&0&2&2&2&3&20&13&0&274&316\\
% sports&0&0&0&0&0&0&0&1&5&31&0&174&211\\
% tool&0&0&1&3&14&16&26&39&115&246&0&4,665&5,125\\
% traffic&0&0&0&0&1&4&4&13&26&50&0&449&547\\
% travelling&0&0&0&0&0&0&0&1&1&10&0&124&136\\
% uncategorized&0&0&0&0&0&0&0&0&0&0&0&3&3\\
    \end{tabular}
    \caption{Distribution of the detailed ratings of  miniapps} 
    \label{tab:vuln_ratings} 
    \vspace{-0.2in}
\end{table*}




==> paper/5_1_case_study.tex <==
\section{Case Study}
\subsection{Mini-app session key leakage}
In this section, we present two case studies vulnerable to Coffee attack to show how credential leakage can pose a threat to mini-apps.

\subsection{Mini-app appsecret leakage}

==> paper/5_evaluation.tex <==
% \section{Evaluation}

 
\begin{table*}[]
\scriptsize
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
    \centering
    \begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r   }
\toprule

\multirow{3}{*}{\textbf{Category}}&\multicolumn{12}{c|}{{\bf Sensitive Data}}&\multicolumn{9}{c}{\textbf{Paid Services}}\\\cmidrule{2-22}
% &\multicolumn{3}{c|}{Group Chat Info}&\multicolumn{3}{c}{Shipping Address}\\ \cmidrule{2-22}
&\multicolumn{3}{c|}{{\textbf{Phone number  }}}&\multicolumn{3}{c|}{{\textbf{User info  }}}&\multicolumn{3}{c|}{{\textbf{Share info  }}}&\multicolumn{3}{c|}{\textbf{{Werun info  }}}&\multicolumn{3}{c|}{{\textbf{AI  }}}&\multicolumn{3}{c|}{{\textbf{Security  }}}&\multicolumn{3}{c }{{\textbf{Location  }}}\\\cmidrule{2-22}
% \multicolumn{3}{c|}{\texttt{wx.authPrivateMessage}}&\multicolumn{3}{c|}{\texttt{wx.getEnterGroupInfo}}&\multicolumn{3}{c}{\texttt{wx.chooseAddress}}\\ \cmidrule{2-22}
&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln&\# ind.&\# com.&\% vuln\\ \midrule
business&0&242&0.59&8&644&1.59&0&49&0.12&0&9&0.02&0&5&0.01&10&855&2.12&0&0&0.00\\
education&1&775&1.90&114&3,065&7.78&15&635&1.59&0&33&0.08&0&6&0.01&132&3,957&10.00&0&1&0.00\\
e-learning&0&39&0.10&2&103&0.26&2&22&0.06&0&9&0.02&0&0&0.00&37&134&0.42&0&0&0.00\\
entertainment&0&42&0.10&6&234&0.59&3&74&0.19&0&2&0.00&0&0&0.00&11&268&0.68&0&0&0.00\\
finance&0&33&0.08&0&74&0.18&0&10&0.02&0&3&0.01&0&2&0.00&0&96&0.23&0&0&0.00\\
food&0&511&1.25&8&1,369&3.37&0&158&0.39&0&6&0.01&0&0&0.00&16&1,846&4.55&0&0&0.00\\
games&1&23&0.06&133&422&1.36&92&170&0.64&0&3&0.01&0&0&0.00&250&473&1.77&0&0&0.00\\
government&0&141&0.34&24&524&1.34&0&47&0.11&0&7&0.02&0&3&0.01&24&700&1.77&0&0&0.00\\
health&0&161&0.39&4&448&1.11&1&47&0.12&1&11&0.03&0&4&0.01&4&559&1.38&0&0&0.00\\
photo&0&2&0.00&1&32&0.08&0&4&0.01&0&1&0.00&0&0&0.00&1&36&0.09&0&0&0.00\\
job&0&101&0.25&1&275&0.68&0&36&0.09&0&1&0.00&0&2&0.00&2&390&0.96&0&0&0.00\\
lifestyle&5&1,440&3.53&93&4,183&10.46&4&590&1.45&0&22&0.05&0&9&0.02&124&5,658&14.14&0&1&0.00\\
shopping&0&1,885&4.61&41&7,174&17.65&6&1,434&3.52&1&65&0.16&0&9&0.02&52&9,504&23.38&0&1&0.00\\
social&1&55&0.14&13&282&0.72&0&62&0.15&0&6&0.01&0&3&0.01&15&320&0.82&0&0&0.00\\
sports&1&38&0.10&6&224&0.56&1&25&0.06&3&44&0.11&0&0&0.00&8&253&0.64&0&0&0.00\\
tool&8&761&1.88&181&3,332&8.59&33&432&1.14&8&43&0.12&0&17&0.04&466&4,327&11.72&2&2&0.01\\
traffic&1&161&0.40&6&465&1.15&0&33&0.08&0&2&0.00&0&4&0.01&8&665&1.65&0&1&0.00\\
travelling&0&31&0.08&1&137&0.34&0&12&0.03&0&0&0.00&0&0&0.00&2&191&0.47&0&0&0.00\\
uncategorized&0&0&0.00&0&3&0.01&0&1&0.00&0&0&0.00&0&0&0.00&0&5&0.01&0&0&0.00\\
TOTAL&18&6,441&15.80&642&22,990&57.81&157&3,841&9.78&13&267&0.68&0&64&0.16&1,162&30,237&76.81&2&6&0.02\\

\bottomrule
    \end{tabular}
    \caption{Statistics of the identified vulnerable mini-programs. Note that ``ind.'' represents individual developers and ``com.'' represents enterprise developers (i.e., by company). %\ZY{Maybe we can color the cells to make them look better?} \ZQ{Explain what does Ind and com mean in the table} 
    }  
    \label{tab:vuln_cat_full}
\vspace{-0.2in}
\end{table*}
 \section{Evaluation}
\subsection{Experiment Setup}
 
\paragraph{Dataset Collection} We build a mini-program crawler based on the Mini-Crawler (please see Appendix-\S\ref{subsec:crawler} for greater details) to download the mini-programs. To generate the appropriate keywords, we first used the $1,000$ most commonly used Chinese characters and $1,000$ most commonly used English words as seed keywords to search for and download the mini-programs as our primary dataset, and then we further extracted the names and descriptions from the collected mini-programs as keywords to expand the keywords-list, which eventually contained 414,020 keywords. Next, we used the expanded keyword-list to search the mini-programs again, and the crawled mini-programs
formed our final dataset. With our crawler,  we have collected \totalanalyzedapps mini-programs. It has been reported that there are around 4 million mini-programs in the \wechat market~\cite{wechat3M}. Therefore, we believe our dataset includes the majority of the mini-programs.
%According to the metadata of these mini-programs, we further classify them into 21 categories based on their primary functionalities such as ``Business'' and ``Education''. 
%According to the data presented in the 7th column, the categories with the most mini-programs are the shopping (\shoppingapps, \shoppingappsratio), tool (\toolapps, \toolappsratio), and education (\eduapps, \eduappsratio).  


  
%  super app --- seven in total (i.e.,\texttt{wx.getGroupEnterInfo},   \texttt{wx.chooseAddress},\texttt{wx.authPrivateMessage},\texttt{wx.\\getUserInfo}, \texttt{getPhoneNumber}, and \texttt{wx.getWeRunData}) among the mini-programs.  For instance, if a mini-program that leaks the \appsecret invokes \breakabletexttt{getPhoneNumber} API, this mini-program may be prone to both confidentiality attack (fetching the user's phone number) or integrity attack against vendors (arbitrary login due to predictable data manipulation.)
 
 


 \paragraph{Script and Machine Setup} The mini-program vulnerability analyzing script is quite straightforward to implement: since \appsecret is a 256-bit string of hexadecimal digits, we unpack the mini-programs and use a regular expression to search the unpacked mini-programs. Once we have identified such \appsecret-alike strings, we feed the string to the API that is used to fetch \textsf{AT}. Since the API only returns \textsf{AT} when the correct \appsecret is fed, we do not have false positive (Please refer to \S\ref{subsec:inspector} for more details). To run the script,   we used two desktops running Ubuntu 18.04, Intel Core i5-5300 (2.30 GHz) CPUs and 8 GB RAM. We opened 16 threads in each desktop to maximize the extraction and analysis speed.  

 
\subsection{Experiment Results}
%\subsection{Quantifying \appsecret with \wechat}
\label{sec:evaluation}





\subsubsection{Efficiency}

It took \totaltime for our analysis tool to finish the extraction and analysis with the crawled mini-programs. %, and we successfully extracted and analyzed all the mini-programs with our tool. %
The most time consuming process is on the mini-program unpacking and code extraction, which takes an average of \totalavg seconds, while scanning the code to detect the hexstrings and APIs costs just several milliseconds.
%
%the average time spent on scanning the mini-program code for vulnerability detection is \anaavg seconds.
With these tested mini-programs, we have identified \sessionstrings unique 32-byte hexstrings from the unpacked mini-program code, and with \numofsecrethour hours' \appsecret online validation, we have detected \leakedapps mini-programs that have leaked their \appsecret{s}. \looseness=-1
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/upd_histo.pdf}
%     \caption{The number of the vulnerable mini-programs fixed after our first report \AY{Need to update it}  \ZQ{maybe completely remove this?}%(barchart with rated/unrated)}
%     }
%     %\ZY{The color does not look good}\AY{will change to a lighter color, in blue and orange}}
%     \label{fig:company-vuln}
% \end{figure}
 


% \usepackage{multirow}





% \begin{table}[]
% \scriptsize
% % \tiny
% \belowrulesep=0pt
% \aboverulesep=0pt
% \setlength\tabcolsep{1.5pt}
% \centering
% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Category}}} & \multicolumn{3}{c|}{\textbf{Rated}}                                                                                & \multicolumn{3}{c|}{\textbf{Unrated}}                                                                              & \multicolumn{3}{c}{\textbf{Total}}                                                                                \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{\textbf{\# Vuln}} & \multicolumn{1}{c|}{\textbf{\# App}} & \multicolumn{1}{c|}{\textbf{\%}}  & \multicolumn{1}{c|}{\textbf{\# Vuln}} & \multicolumn{1}{c|}{\textbf{\# App}} & \multicolumn{1}{c|}{\textbf{\%}} & \multicolumn{1}{c|}{\textbf{\# Vuln}} & \multicolumn{1}{c|}{\textbf{\# App}} & \multicolumn{1}{c}{\textbf{\%}} \\ \hline
% business&146&7,178&2.03\%&470&65,924&0.71\%&616&73,102&0.84\%\\
% education&1,735&95,220&1.82\%&1,825&115,715&1.58\%&3,560&210,935&1.69\%\\
% e-learning&36&1,699&2.12\%&157&5,440&2.89\%&193&7,139&2.70\%\\
% entertainment&134&7,114&1.88\%&115&13,782&0.83\%&249&20,896&1.19\%\\
% finance&20&984&2.03\%&52&2,020&2.57\%&72&3,004&2.40\%\\
% food&671&42,881&1.56\%&905&62,981&1.44\%&1,576&105,862&1.49\%\\
% games&756&34,259&2.21\%&972&48,074&2.02\%&1,728&82,333&2.10\%\\
% government&237&8,848&2.68\%&374&17,423&2.15\%&611&26,271&2.33\%\\
% health&185&7,785&2.38\%&253&15,566&1.63\%&438&23,351&1.88\%\\
% job&158&9,109&1.73\%&160&10,561&1.52\%&318&19,670&1.62\%\\
% lifestyle&2,048&103,530&1.98\%&2,751&203,443&1.35\%&4,799&306,973&1.56\%\\
% photo&21&1,972&1.06\%&15&3,758&0.40\%&36&5,730&0.63\%\\
% shopping&3,250&210,436&1.54\%&4,005&495,334&0.81\%&7,255&705,770&1.03\%\\
% social&141&8,561&1.65\%&175&10,626&1.65\%&316&19,187&1.65\%\\
% sports&103&5,568&1.85\%&108&7,678&1.41\%&211&13,246&1.59\%\\
% tool&2,454&95,255&2.58\%&2,673&123,324&2.17\%&5,127&218,579&2.35\%\\
% traffic&289&14,794&1.95\%&259&17,121&1.51\%&548&31,915&1.72\%\\
% travelling&56&3,216&1.74\%&80&4,729&1.69\%&136&7,945&1.71\%\\
% uncategorized&1&280&0.36\%&2&38,896&0.01\%&3&39,176&0.01\%\\ \midrule
% Total&12,441&658,689&1.89\%&15,351&1,262,395&1.22\%&27,792&1,921,084&1.45\%\\ \bottomrule

% \end{tabular}
% \caption{Distribution of the vulnerable mini-programs for each category based on whether they are rated. %\ZQ{elearning. Please change Appendix as well} %ratings and categories of vulnerable mini-programs 
% } 
%     \label{tab:vuln_cat_score} 

% \end{table}


 
% \begin{figure}[htb]
   
%         \centering
%         \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_problem_rated_ratio.pdf}
%         \subcaption{}
%     \label{fig:vuln_mini-program_cat_problem_rated_ratio}
   
%     \caption{The heatmap of the vulnerable mini-programs w.r.t. their categories and accessed data.\AY{Change to table when data ready}}  
%     \label{fig:heatmap}
    
% \end{figure}




% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_score_absolute.pdf}
%     \caption{Amount of vulnerable mini-programs w.r.t. scores}
%     \label{fig:vuln_mini-program_cat_problem_unrated_absolute}
% \end{figure} %1
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_score_ratio.pdf}
%     \caption{Ratio of vulnerable mini-programs w.r.t. scores}
%     \label{fig:vuln_mini-program_cat_problem_unrated_ratio}
% \end{figure} %2
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_problem_rated_absolute.pdf}
%     \caption{Amount of rated vulnerable mini-programs w.r.t. accessed data}
%     \label{fig:vuln_mini-program_cat_problem_rated_absolute}
% \end{figure} %3
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_problem_rated_ratio.pdf}
%     \caption{Ratio of rated vulnerable mini-program distribution w.r.t. accessed data}
%     \label{fig:vuln_mini-program_cat_problem_rated_ratio}
% \end{figure} %4
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_problem_unrated_absolute.pdf}
%     \caption{Amount of unrated vulnerable mini-programs w.r.t. accessed data}
%     \label{fig:vuln_mini-program_cat_problem_unrated_absolute}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_problem_unrated_ratio.pdf}
%     \caption{Ratio of unrated vulnerable mini-programs w.r.t. accessed data}
%     \label{fig:vuln_mini-program_cat_problem_unrated_ratio}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \begin{table*}[]
% \scriptsize
% % \tiny
% \belowrulesep=0pt
% \aboverulesep=0pt
% % \setlength\tabcolsep{1.5pt}
%     \centering
%     \begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
% \toprule
% \multirow{3}{*}{\bf Category}&\multicolumn{9}{c|}{\bf User Information}&\multicolumn{6}{c}{\bf Social Information}\\ \cmidrule{2-16}
% % &\multicolumn{3}{c}{\bf Address}\\ \cmidrule{2-22}
% &\multicolumn{3}{c|}{\textbf{phone number}}&\multicolumn{3}{c|}{\textbf{\texttt{werun} data}}&\multicolumn{3}{c|}{\textbf{user info}}&\multicolumn{3}{c|}{\textbf{share info}}&\multicolumn{3}{c}{\textbf{promoting messages}}\\ \cmidrule{2-16}
% % &\multicolumn{3}{c|}{\textbf{group chat info}}&\multicolumn{3}{c}{\textbf{address}} \\ \cmidrule{2-22}
% &\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app\\ \midrule
% %& \# vuln&\# app&\% app&\# vuln&\# app&\% app\\ \midrule
% business&13&2,832&0.46&6&299&2.01&7&5,790&0.12&36&3,696&0.97&0&21&0.0\\
% education&17&2,569&0.66&28&1,225&2.29&12&1,926&0.62&594&31,500&1.89&0&189&0.0\\
% entertainment&4&355&1.13&1&167&0.6&5&654&0.76&85&3,238&2.63&0&11&0.0\\
% finance&0&81&0.0&2&35&5.71&3&94&3.19&7&282&2.48&0&0&0.0\\
% food&13&1,637&0.79&4&526&0.76&0&903&0.0&138&19,859&0.69&0&122&0.0\\
% games&1&70&1.43&4&267&1.5&0&57&0.0&481&19,787&2.43&0&5&0.0\\
% government&10&647&1.55&7&249&2.81&11&478&2.3&36&2,545&1.41&0&8&0.0\\
% health&7&574&1.22&8&313&2.56&11&672&1.64&41&2,917&1.41&0&8&0.0\\
% images&0&48&0.0&1&46&2.17&3&121&2.48&5&774&0.65&0&3&0.0\\
% job&2&239&0.84&0&83&0.0&5&318&1.57&26&2,361&1.1&0&6&0.0\\
% lifestyle&46&4,207&1.09&14&955&1.47&23&3,465&0.66&497&36,614&1.36&0&187&0.0\\
% reading&1&199&0.5&5&64&7.81&3&249&1.2&19&1,164&1.63&0&5&0.0\\
% shopping&70&13,518&0.52&41&2,746&1.49&20&8,209&0.24&1,169&84,442&1.38&0&1,505&0.0\\
% social&0&130&0.0&7&200&3.5&1&172&0.58&63&2,395&2.63&1&13&7.69\\
% sports&2&242&0.83&40&2,338&1.71&3&383&0.78&23&2,782&0.83&0&6&0.0\\
% tool&31&2,150&1.44&52&2,371&2.19&22&2,451&0.9&464&22,474&2.06&0&114&0.0\\
% traffic&6&346&1.73&2&418&0.48&3&226&1.33&26&4,004&0.65&0&25&0.0\\
% travelling&2&184&1.09&0&171&0.0&1&171&0.58&7&1,034&0.68&0&6&0.0\\
% uncategorized&0&9&0.0&0&2&0.0&0&1&0.0&1&32,902&0.0&0&32,834&0.0\\


% % total&225&30,037&0.75&312&12,540&2.49&317&26,125&1.21&5,461&276,245&1.98&3&34,935&0.01&0&0&0.00&0&0&0.00\\ 
% \bottomrule




% \bottomrule
%     \end{tabular}
%     \caption{\AY{This table equals the union of previous two tables} mini-programs and accessed sensitive information (Note that we have not found cases requiring user address or group messaging information, so the data is removed from the table).}  
%     \label{tab:apis}

% \end{table*}


%\AY{In our paper, we are interested in two types of mini-programs: (1) the mini-programs that have been developed by IT companies that migrated their native apps into \wechat mini-program platform (e.g., mini-programs developed by Tencent and Baidu). (2) the mini-programs developed by . As such, we obtained the list of top IT companies from the report of Chinese IT companies (2020) published by Internet Society of China \cite{isc}. For the list of top commercial companies, we obtained the keyword list from Fortune China \cite{fortunechina}.}

% \AY{With the company list obtained, we use NLP techniques to generate the keyword for query. First, we used \texttt{Jieba} to perform Chinese word segmentation. Then, we used TFIDF algorithm to extract the keywords of these company names. After deduplication, we finally have a list of 493 keywords. As such, we used the 493 keywords to query the \wechat mini-program API, and collected 8,824 mini-programs for analysis.}
% \subsection{Vulnerability Detection}
% \AY{In general, there are two questions to answer for coffee attack vulnerability detection. (1) is the appsecret of the mini-program leaked? (2) what kind of encrypted information does the mini-program access?}





%\paragraph{Vulnerability}

% 
% \paragraph{Data Set} We collected our mini-programs from \wechat app via its built-in mini-program searching functionality. In \wechat app, users can either install a mini-program by clicking on a link shared by other user, or manually use keyword to search for a specific mini-program. To obtain a list of mini-programs to be downloaded, we reverse engineered \wechat, investigated the workflow of the search interface, and collected the metadata of $510,000$ mini-programs containing mini-program IDs, descriptions, and extra category info. Then, we created a crawler that runs on mobile phones to automatically download mini-programs. In average, our tool $3,000$ mini-programs a day. We used two mobile phones to work together, and eventually we obtained \totalnum mini-program packages for analysis.    

% We implemented \textsf{CoffeCAN} in JavaScript with \texttt{esprima}\cite{esprima} to generate AST of mini-program source code, and Python to support multi-process processing. We performed our analysis on two Linux computers, each of which has 8 cores, Intel Core i7-8700 (3.20 GHz) CPUs and 16 GB RAM. It took 10 days for us to finish the analysis of the \totalnum mini-programs. 

%\paragraph{Overall Results} 

% \AY{Our collection of metadata took two months and we managed to collect the developer info for 31,608 mini-programs, with 30,435 mini-programs developed by large companies and 1,173 developed by individuals, as some of the mini-programs have been withdrawn from the market by the time we collect the metainfo.}
%\paragraph{Statistics of Vulnerable mini-programs} 

\subsubsection{Statistics of  Vulnerable Mini-Programs}

We seek to obtain some insights from the vulnerable mini-programs. The information we have for each mini-program includes (i) the category it belongs to;  (ii) the privacy resources it accesses (e.g., \texttt{weRunData}, \texttt{phoneNumber}); (iii) when the mini-program was last updated;   (iv) the difference between enterprise developers and individual developers; and (v) the rating of the vulnerable mini-programs. 
%, and (vi) the high profile mini-programs. 
In the following, we explain the results in greater details.\looseness=-1 

%\begin{enumerate} [label=(\Roman*)]
 
\smallskip \noindent \textbf{What are the categories of vulnerable mini-programs?} Almost all (96.21\%)  
mini-programs have been classified into a certain category in the \wechat mini-program store, as shown in \autoref{tab:vuln_cat_full}.
We observe that 
%also presents the distribution of categories of all the identified vulnerable mini-programs, and from the distribution, we can observe that 
the percentage of the vulnerable mini-programs in each category (the first column) and their accessed data (e.g., phone number, user info, share info, werun info) or services (e.g., AI, security, and location) are quite diversified, %, where for the categorized mini-programs the ratio ranges from \AY{ ?} to \AY{ ?}, 
indicating that the \appsecret leakage problem is a system wide problem regardless of the mini-program categories, though some categories (e.g., tool, government, and games) contain slightly higher percentage of vulnerable mini-programs.   Unfortunately, these mini-programs are critical to user's daily life, e.g., tool mini-programs usually provide convenient services such as QR code scanning when boarding a bus, government tools usually involve with user's real identify information and critical administrative services, and games often involve payment and in-game trading. 




\begin{figure*}
    \centering
        \includegraphics[width=.24\linewidth]{image/rating_date.pdf}
        \includegraphics[width=.24\linewidth]{image/dev_date.pdf}
        \includegraphics[width=.24\linewidth]{image/acc_date.pdf}
        \includegraphics[width=.24\linewidth]{image/cloud_date.pdf}
        \vspace{-0.15in}
    \caption{The trending of all vulnerable mini-programs w.r.t rating, developer, accessed resource type, and accessed data type.}
    \label{fig:trends}
\end{figure*}

%\vspace{-0.2cm} 

 
\smallskip \noindent \textbf{What are the accessed resources of vulnerable mini-programs?} {Recall that an attacker can launch different types of attack depending on the type of sensitive resources a mini-program accesses, }
% Recall that according to different sensitive resources a mini-program accessed, an attacker can launch different attacks against them, and therefore,
we also present the statistics of different sensitive data these mini-programs accessed in \autoref{tab:vuln_cat_full} based on the APIs used {to understand the potential impacts of \appsecret leakage among these vulnerable mini-programs}. We identify that \numaccesseddata mini-programs have accessed various sensitive data including phone number, werun data, user information, mini-program share information, %, and private forwarding message (we do not identify any cases accessing the promoting messages, and group chat info), 
and \numaccessedcloud accessed at least one cloud services. Interestingly, we also note that there are \nonaccessed vulnerable mini-programs that do not access any MK accessible resources at all. However, those mini-programs are potentially vulnerable, since they could be used to access the MK accessible resources in the future. In that case, we can break those mini-programs using the discussed methods.  %, and thus be subject to our attacks.   
% Similar to how we plot \autoref{fig:vuln_mini-program_cat_score_ratio}, we use the accessed sensitive data in the y-axis \autoref{fig:vuln_mini-program_cat_problem_rated_ratio} and \autoref{fig:vuln_mini-program_cat_problem_unrated_ratio-unrated}, where \autoref{fig:vuln_mini-program_cat_problem_rated_ratio} shows the distribution of the vulnerable m the rated category and \autoref{fig:vuln_mini-program_cat_problem_unrated_ratio-unrated} shows the unrated category.
%Note that the detailed distributions of the sensitive data access of rated mini-programs, unrated mini-programs, and all mini-programs can be found in \autoref{tab:apis-rated}, \autoref{tab:apis-unrated} and \autoref{tab:apis} in Appendix, respectively.

 
\smallskip \noindent \textbf{Who are the developers of vulnerable mini-programs?} Next, our aim is to understand who are the developers of these vulnerable mini-programs, %how many developers have produced the vulnerable mini-programs, 
and how often they made these mistakes. 
At a high level, there are two kinds of developers: individual developer and enterprise developers.
%
%One developer may make the same mistake more than once (e.g., developing multiple mini-programs with \appsecret leakage), and therefore, we would like to investigate how many vulnerable mini-programs may be associated with the same developer in general. 
{Compared with enterprises developers whose enterprise name and tax ID is shown in the metadata, \Tencent does not provide such info for mini-programs developed by individual developers, whereas the metadata page only shows `individual developer'.}
% the individual developer's personal information, and instead \Tencent just uses a string `individual developer' to label all the developer information of the mini-programs that are produced by the individual developers.
Therefore, in the following, other than 4,676 mini-programs that have been developed by the individual developers, we present the  %cannot determine whether two mini-programs with the same information (both labeled `individual developer'') are developed by the same individual developer. Therefore, we 
%only present the distributions 
statistics of the vulnerable mini-programs that are produced by the corresponding companies. 
%
In particular, we have collected the developer information of the companies of the vulnerable mini-programs if they are available, and \autoref{tab:company} shows the statistics based on how many mini-programs have been associated with the same company. We can notice that the majority of the companies developed just a single vulnerable mini-program, and but sometimes one company can produce multiple vulnerable mini-programs (e.g., a company called `Suzhou Yutianxia' has produced 30 vulnerable mini-programs according to the data we have).






\begin{table}[]
\scriptsize
 \belowrulesep=0pt
 \aboverulesep=0pt
 \setlength\tabcolsep{3pt}
    
        \resizebox{0.485\textwidth}{!}{ 
\begin{tabular}{l|r|r|r|r|r|r}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Associated\\  Apps\end{tabular}}}                   & \multicolumn{2}{c|}{\textbf{Rated}}             & \multicolumn{2}{c|}{\textbf{Unrated}}           & \multicolumn{2}{c}{\textbf{Total}}             \\ \cmidrule{2-7}
 & \textbf{\# Companies} & \textbf{\# Apps} & \textbf{\# Companies} & \textbf{\# Apps} & \textbf{\# Companies} & \textbf{\# Apps} \\ \hline
>=20&0&0&16&417&16&417\\
19&0&0&2&38&2&38\\
18&0&0&2&36&2&36\\
17&0&0&1&17&1&17\\
16&0&0&3&48&3&48\\
15&1&15&2&30&3&45\\
14&0&0&1&14&1&14\\
13&1&13&4&52&5&65\\
12&3&36&6&72&9&108\\
11&0&0&1&11&1&11\\
10&0&0&9&90&9&90\\
9&3&27&9&81&12&108\\
8&1&8&24&192&25&200\\
7&1&7&29&203&30&210\\
6&1&6&26&156&27&162\\
5&6&30&69&345&75&375\\
4&7&28&155&620&161&648\\
3&21&63&333&999&353&1,062\\
2&100&200&1,300&2,600&1,388&2,800\\
1&1,624&1,624&22,357&22,357&23,805&23,981\\
total&1,769&2,057&24,349&28,378&25,781&30,435\\

 \bottomrule


\end{tabular} 
}
    \caption{Numbers of vulnerable mini-programs associated with the same software development enterprises.} 
    \label{tab:company}
   
\end{table}

 

%\AY{(2) the amount of vulnerable mini-programs accessing sensitive data have been constantly at a higher amount compared with those do not access the sensitive data, and (3) vulnerable mini-programs not accessing any sensitive data raised rapidly from 2017 to 2019, and then constantly on the drop until 2021. This is even more surprising that although we noticed relevant reports of failure to publish mini-program due to \appsecret leakage from the platform in August 2019~\cite{report}, indicating the existence of \appsecret leakage detection mechanism by the super app platform, our result still indicate the existence of mini-programs leaking \appsecret even in 2021. This indicates that the super app platform is still using fully or hybrid manual checking process for mini-program vetting during publishing, whereas the detection mechanism could be improved significantly by an automatic solution.}

 
\smallskip \noindent \textbf{What are the lastest update of the vulnerable mini-programs?} The meta-data of a mini-program contains the latest updated timestamp. Therefore, we can use this information to understand how long this \appsecret leakage vulnerability has lived.  Moreover, we would like to understand how the vulnerable mini-program resources are accessed and the vulnerable mini-programs' ratings across the time. As such, we group the resources accessed, their ratings, and the developer information based on their latest update month. As shown in \autoref{fig:trends}, we have obtained the following observations:
%To this end, we first collected the timestamp of the latest update of all of the vulnerable mini-programs,  then grouped them together based on their latest update month, and finally count the numbers of vulnerable mini-programs in each group. 
  (i) \appsecret leakage vulnerability has been there since the first date when \Tencent introduced the mini-program into \wechat (e.g., a mini-program named WuiGuang Calendar released January 2017 has leaked the \appsecret and it never gets updated). (ii) As the time goes by, the number of vulnerable mini-programs decreased regardless of the data resource accessed and their ratings. However, the mini-programs 
developed by companies remain a major source of vulnerable mini-programs.


\smallskip \noindent \textbf{What are the ratings of the vulnerable mini-programs?} Unfortunately, compared with popular traditional platforms like Google Play, there is no total number of downloads in mini-program store. However, we can use another type of information to characterize mini-programs' popularity: the rating of a mini-program, which is only available when enough users have used and rated the mini-programs~\cite{ourfancywork}. Therefore, the rating could reflect the popularity of a mini-program, %the rated mini-programs will have significantly more downloads and users than the unrated ones. %Among the total \totalanalyzedapps mini-programs, only one third of them appear to be more popular apps and they have the corresponding ratings with score from 0 to 5. 
%Intuitively, the more popular a mini-program is, the less vulnerable it should be. However, as presented in \autoref{tab:vuln_cat_score-full}, \AY{?} of the rated mini-programs are actually vulnerable, whereas only  \AY{?} of the unrated ones are. Therefore, we cannot simply link the vulnerability ratio with the popularity of the mini-programs, and we have to zoom in the ratings with other dimensions to draw insights. \looseness=-1
%
%\autoref{tab:vuln_cat_score} presents the distributions of ratings of mini-programs (The detailed distribution of the ratings of mini-programs can be found \autoref{tab:vuln_cat_score-full}  in of Appendix A). As shown in the table, 65.71\% identified mini-programs are not yet scored, due to the lack of enough rated users. These mini-programs are likely to be unpopular or with relatively lower quality. Among them, 1.22\% are vulnerable. With all mini-programs with ratings,  1.89\% of the mini-programs are vulnerable.  Although these mini-programs are popular,  they may still expose sensitive data in danger in that the \appsecret{s} are leaked. \looseness=-1
%However, if we zoom in the ratings with the specific category of the mini-programs, we 
and we have associated the ratings with the corresponding mini-app category,   as shown in \autoref{tab:vuln_ratings}.
%
%\autoref{fig:vuln_mini-program_cat_problem_unrated_ratio} uses the categories as the x-axis and the percentage of vulnerable mini-programs in the mini-programs of a specific category with a specific rating as the y-axis, and
% that represents the category with the rating will be. 
We can observe that the mini-programs with lower ratings tend to have a higher percentage of vulnerable mini-programs. This is reasonable, as the developers of mini-programs with higher ratings may spend more efforts on security and privacy to stay competitive, and maintain their advantages.   \looseness=-1


% decreased significantly.
% \AY{Interestingly, we were also surprised to find out that although the problem of \appsecret leakage had been raised by developer as early as in 2019~\cite{}, the \appsecret leakage continues to exists even after 2021. This further demonstrated the surprising neglect of potential impacts brought about by \appsecret leakage among the mini-program community.}

%\end{enumerate}



%
%However, not all the attacks can be launched on those  high-profile mini-programs, since they may not use the resources of interest. For example, attacks against sensitive data for promotion abuse only work when the victim mini-program consumes share info or WeRun data. For those attacks that cannot be demonstrated with the high-profile mini-programs, we use other mini-programs we can find to show the attack consequences. 


 


\ignore{
To gain a better understanding of the \appsecret exposure, we have conducted analysis over the \leakedapps vulnerable mini-programs, through which we have  further obtained more insights from them such as (I) the distribution 
of the ratings of the vulnerable mini-programs
(II) distribution of the categories of the vulnerable mini-programs,  (III) the distribution of the sensitive information these vulnerable mini-programs accessed, (IV) the distribution of the developer information of these vulnerable mini-programs, and (V) the distribution of vulnerable mini-program registration and updating date. 
}


%in the following sections, we first discuss the distribution of mini-programs we collected with respect to their categories and scores, followed by detailed discussion on vulnerable mini-programs, including the the sensitive information collected by these vulnerable mini-programs, categories of these vulnerable mini-programs, and finally the vulnerabile mini-programs developed by large companies.


%After analysis, we have collected 
%With the \leakedapps vulnerable mini-programs, we  

%Then, with the \wechat network APIs, we implemented a python tool to query the results from \wechat server and executed the script with \numofsecretthread threads. 

%\AY{Among the mini-programs, we collected The experiment run for \numofsecrethour hours, and as a result, we  among the \totalanalyzedapps mini-programs that have been successfully unpacked. 






% \sout{Among all our \totalapps collected mini-programs, our tool successfully unpacked \totalanalyzedapps mini-programs. Among these \totalanalyzedapps mini-programs, our tool identified \leakedapps mini-programs that had leaked their {\tt MK}s. In the following, we describe how we reached these results. In particular, we first discuss the performance of our tool (\S\ref{subsubsec:tool}), followed by the statistics of all our collected mini-programs (\S\ref{subsubsec:dataset}),  the statistics of these vulnerable mini-programs (\S\ref{subsubsec:flaws}).}\sout{, and finally the statistics of the vulnerable mini-programs from  the top fortune 500  Companies (\S\ref{subsubsec:top}).  }

% \begin{figure} 
% \centering
% \begin{minipage}[t]{0.495\linewidth}
% \includegraphics[width=\linewidth]{image/stat_x_time.pdf}
% \caption{Distribution of mini-program extraction time}
%  \label{fig:stat_exec}
% \end{minipage}
% % \hspace{1mm}
% \begin{minipage}[t]{0.495\linewidth}
% \includegraphics[width=\linewidth]{image/stat_analyze_time.pdf}
% \captionsetup{justification=centering}
% \caption{Distribution of mini-program analyze time}  
%  \label{fig:stat_analyze}
%  \
% \end{minipage}
% % \begin{minipage}[t]{0.495\linewidth}
% % \includegraphics[width=\linewidth]{image/stat_size.pdf}
% % \captionsetup{justification=centering}
% % \caption{Distribution of mini-program Size}  
% %  \label{fig:stat_ast}
% % \end{minipage}
% % \begin{minipage}[t]{0.495\linewidth}
% % \includegraphics[width=\linewidth]{image/stat_loc.pdf}
% % \caption{Distribution of mini-program line of codes}
% %  \label{fig:stat_loc}
% % \end{minipage}
% % \hspace{1mm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{image/all_mini-program_cat_score.pdf}
%     \caption{Heatmap of collected mini-programs, w.r.t. scores and categories} %\ZY{Black-white}
%     \label{fig:heatmap_all_scores}
%     \
% \end{figure}

%\texttt{WXUnpacker}~\cite{decomplier}

%The results of our extraction are shown as green lines in \autoref{fig:stat_exec} through \autoref{fig:stat_ast}. As shown in the figures, we observed that the extraction time elapsed to extract a mini-program package scatters from 10 seconds to 1 minutes, whereas the analysis time are relatively shorter (90\% of the mini-programs are analyzed within 5 seconds). The mini-programs we collected ranges from 12 to 20,045 lines of code, with the AST nodes ranging from 47 to 21,224. This indicates that we have collected not only tiny mini-programs with limited functions but also heavy mini-programs that provide complex functionalities. These



%\ZQ{fix this paragraph}




 

 

 

%As shown in the figures, compared with normal mini-programs, mini-programs that leaked \appsecret on average take less time to extract and to analyze, and contains less lines of codes and AST nodes. 








% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{image/company.pdf}
%     \caption{Relationships between developers and mini-programs \ZQ{This figure doesn't contribute much interesting knowledge and can be removed}}
%     \label{fig:developers}
% \end{figure}

% \begin{figure} 
% \centering
% \begin{minipage}[t]{0.463\textwidth}
% \includegraphics[width=\textwidth]{image/mini-program_cat_score.pdf}
% \caption{Heatmap of distribution in scores and categories among all mini-programs}
%  \label{fig:heatmap__all_score}
% \end{minipage}
% % \hspace{1mm}
% \begin{minipage}[t]{0.533\textwidth}
% \includegraphics[width=\textwidth]{image/mini-program_cat_prob.pdf}
% \captionsetup{justification=centering}
% \caption{Heatmap of user information access among all mini-programs}  
%  \label{fig:heatmap_all_access}
% \end{minipage}
% \end{figure*}
% \begin{figure*} 
% \centering
% \begin{minipage}[t]{0.463\textwidth}
% % \includegraphics[width=\textwidth]{image/mini-program_cat_score.pdf}
% \caption{Heatmap of distribution in scores and categories among vulnerable mini-programs}
%  \label{fig:heatmap_vuln_score}
% \end{minipage}
% \hspace{1mm}
% \begin{minipage}[t]{0.533\textwidth}
% \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_prob.pdf}
% \captionsetup{justification=centering}
% \caption{Heatmap of user information access among vulnerable mini-programs}  
%  \label{fig:heatmap_vuln_access}
% \end{minipage}
% \end{figure}
% \begin{figure} 
% \centering
% \includegraphics[width=\linewidth]{image/redirection_appsecret_string.pdf}
% \caption{Relationship of confirmed mini-programs that leak appsecret as String variables}
%  \label{fig:redirection_appsecret}
% \end{figure}


% \begin{table}
%     \centering
%     \scriptsize
%     \aboverulesep=0pt
%     \belowrulesep=0pt
%     \begin{tabular}{r|l|l}
%     \toprule
% {\bf \# App}&\bf Domain&\bf Servive\\ \midrule
% 34&apis.map.qq.com&Tencent Map\\ 
% 14&api.map.baidu.com&Baidu Map\\ 
% 13&pingtas.qq.com&Tencent mini-program Analytics\\ 
% 11&wx.qlogo.cn&Tencent Avatar Logo\\ 
% 10&restapi.amap.com&AutoNavi Map\\ 
% 8&webim.tim.qq.com&Tencent Web Messaging\\ 
% 7&log.aldwx.com&Third-party mini-program Analyics\\ 
% 6&api.mch.weixin.qq.com&Tencent Payment\\ 
% 5&api.aikst.cn&mini-program Template Provider\\ 
% 5&yun.tim.qq.com&mini-program Third-paty Back-end\\ 
% 4&sandcash.mixienet.com.cn&mini-program Third-paty Back-end\\ 
% 4&thirdwx.qlogo.cn&mini-program Template Provider\\ 
% 4&tcb-api.tencentcloudapi.com&Tencent Cloud Base\\ 
% 4&wxapp.yz168.cc&mini-program Third-paty Back-end\\ 
% 3&glog.aldwx.com&Third-party mini-program Analyics\\ 
% 3&api.q.qq.com&Tencent Server API\\ 
% 3&www.hhhkd.top&mini-program Third-party Back-end\\ 
% 3&tongji.dcloud.io&Third-party mini-program Analytics\\ 
% 3&aip.baidubce.com&Baidu Cloud API\\ 
% 3&iploc.ywdier.com&Third-party mini-program Back-end\\ \bottomrule

%     \end{tabular}
%     \caption{Top 20 communication domains configured by vulnerable mini-programs\AY{Not Up To Date}}
%     \label{tab:vuln_domain}
% \end{table}



% In this paper, we mainly investigate two types of vulnerabilities: the appsecret leakage, and the session key leakage. For appsecrets, the 32-bit hex string can be leaked as hard-coded strings, or as part of the parameter of network URLs. To model the potential leakage of session keys, we investigate them from two aspects: on one hand, we investigate the network URL associated with user login and login token to find whether there are sensitive third-party network APIs that are potentially leaking session key. On the other hand, we track the network request APIs associated with sensitive APIs related to encrypted data: since the decryption are only supposed to be performed at back-end, if an API associated with encrypted data does not send their data to the back-end, then the mini-program may be processing the data at the front-end and the session key is being potentially leaked.

% \paragraph{(II) Vulnerable mini-programs and information accessed} 


% As shown in \cref{fig:heatmap_score}, in general, most of the vulnerable mini-programs are not being scored yet, indicating that they are fresh-created mini-programs or mini-programs not being used by a large amount of people. During our inspection, most of these mini-programs not being scored are regional lifestyle or shopping mini-programs, such as local hair saloons and local supermarket. Aside from these mini-programs, most of the affected and scored mini-programs are over 4.0 points, which indicates that the appsecret leakage may also affect very highly rated mini-programs. As to the categories, we discover that most of the mini-programs associated with appsecret leakages are education, games, lifestyle, shopping, and sports mini-programs. Interestingly, these mini-programs are much more likely to be associated with sensitive user data, such as user phone number to register account, and user sports data. 

% From the figure, we discovered that most of the popular mini-programs are shopping mini-programs, whereas the majority of the rest of the mini-programs are associated with shopping activities as well (e.g., the first food mini-program is actually a wine shop). This means many of these mini-programs with appsecret leakage are associated with actions such as shopping, payment, and coupon, which may be dangerous since the attacker can manipulate encrypted data to make profits or steal user information.


% \begin{table}
% \centering
% \scriptsize
% \aboverulesep=0pt
% \belowrulesep=0pt
% \begin{tabular}{c|c|c|c}
% \toprule
% \bf Developer&{\bf \# App}&\bf Avg. Ratings&\bf Type\\ \midrule
% \multirow{12}{*}{Yunlei}&Nanyang Transportation&4.7&Traffic\\ 
% &Xiangtan Transportation&-&Traffic\\ 
% &Transportation Code&4.5&Traffic\\ 
% &Shangqiu Transportation&4.7&tool\\ 
% &Enshi Transportation&4.7&Traffic\\ 
% &Ezhou Transportation&4.7&Traffic\\ 
% &Huaihua Transportation&4.8&Traffic\\ 
% &Jingzhou Transportation&4.7&Tool\\ 
% &Qianjiang Transportation&4.7&Traffic\\ 
% &Suzhou Transportation&4.7&Traffic\\ 
% &Yangzhou Transportation&4.7&Tool\\ 
% &Yichang Transportation&4.7&Tool\\ \cmidrule{1-1}
% \multirow{4}{*}{Nestle}&We Proudly Serve&4.6&Food\\ 
% &DolceGusto Member Center&4.6&Food\\ 
% &Nestle Member Club&4.4&Lifestyle\\ 
% &Nestle Customer Center&3.5&Shopping\\ \cmidrule{1-1}
% \multirow{3}{*}{Tencent}&Tencent Everyday Battle Chess&3.7&Games\\ 
% &Cool Run Everyday&3.5&Games\\ 
% &Tencent Billiards&4&Games\\ \cmidrule{1-1}
% \multirow{2}{*}{Shizhidong}&Fresh Graduate Jobs&-&Job\\ 
% &Graduate Job Hunting&-&Job\\ \cmidrule{1-1}
% \multirow{2}{*}{\tabincell{c}{Xindong\\Shikong}}&King of Music Guessing&3.4&Entertainment\\ 
% &Gala of Poetry&-&Tool\\ \cmidrule{1-1}
% \multirow{2}{*}{Hengzhao}&Chengtian Water Dispenser&4&Government\\ 
% &Yusheng Cloud Payment&4.1&Tool\\ \cmidrule{1-1}
% \multirow{2}{*}{Xingyi}&Traffic Rule Break Platform&4.6&Government\\ 
% &Traffic Rule Break Inquiry&4.7&Government\\ \cmidrule{1-1}
% \multirow{2}{*}{Juhe Zaisheng}&Juhe Yishoutang&-&Lifestyle\\ 
% &Juhe Yishouke&-&Lifestyle\\ \cmidrule{1-1}
% \multirow{2}{*}{Luyi Huadeng}&Luyi Huadeng&-&Shopping\\ 
% &Luyi Huadeng Photoelectricity&-&Shopping\\ \cmidrule{1-1}
% \multirow{2}{*}{Jiadianwang}&Changsha Electrial Appliances&-&Shopping\\ 
% &Shenzhen Electrial Appliances&-&Shopping\\ 
% \bottomrule
% \end{tabular}
% \caption{Developers with at least two vulnerable mini-programs}
% \label{tab:vuln_dev}
% \
% \end{table}




%vulnerable mini-programs from top companies and finally the (IV) distribution of vulnerable mini-programs from top Companies. 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{image/vuln_mini-program_cat_score.pdf}
%     \caption{Heatmap of vulnerable mini-programs, w.r.t. scores and categories\AY{200w}} %\ZY{Black-white}
%     \label{fig:heatmap_all_scores}
%     \
% \end{figure}

 
% A number of interesting observations can be drawn from these two figures. In particular, among the rated vulnerable mini-program category (\autoref{fig:vuln_mini-program_cat_problem_rated_ratio}), the government and entertainment mini-programs tend to access \texttt{PhoneNumber} most often. According to our analysis, these mini-programs usually use the users' phone numbers to authenticate users. As a result, these mini-programs could suffer from account hijack attacks. Also, we notice that social mini-programs usually access the promoting messages (by using \texttt{authPrivate}), which allows the mini-programs to promote products effectively on social networks. These information can be manipulated or collected by the attackers. 
% In unrated vulnerable mini-program category (\autoref{fig:vuln_mini-program_cat_problem_unrated_ratio-unrated}), we notice that  
% most of the vulnerable mini-programs tend to use \textsf{WeRunData}, and finance category has the higher percentage to be vulnerable than other categories. An investigation of why so many vulnerable mini-programs use \textsf{WeRunData} reveals that this data is often used to attract and reward users (e.g., when they daily step count reached certain threshold). However, with the leaked \appsecret, an attacker can arbitrarily modify the \textsf{WeRunData} of the corresponding mini-programs to easily gain fun and profit.


% \paragraph{(IV) Statistics of the vulnerable mini-programs w.r.t developers}


% ; and (3) The number of vulnerable mini-programs introduced (or updated) in each month reached the peak in January 2019 and had started to decline since then.{It is also surprising that the mini-program \appsecret leakage problem still exists even when we crawl the mini-programs between 2020 to 2021 since that we found that \appsecret leakage has been reported in online developer forum as early as in 2019, and mini-programs dating back to as early as in 2017 still exist on the market without being removed to protect their data security~\cite{officalbad}}




 



 



%that are possibly used to register account or create orders. This is surprising since the mini-program developers involved with such important functionalities overlooked the explicit warning in the \wechat official documentations of not leaking these \appsecret, and proceed to exposing their \appsecret to the front-end. Besides, it is also interesting that although the documentation indicates that the involved mini-program will be taken off the market if \appsecret leakage is detected, there are still over 2.1\% of the mini-programs that leaked \appsecret but still appear on the market. This indicates that the mini-program vetting and \appsecret leakage checking process of mini-program framework still needs to be improved.



%in different categories may access different kinds of user information. For example, there are more shopping and lifestyle mini-programs that access phone number and user information, since the mini-programs often require user information to perform purchasing and payment. For weRunData, however, most of the mini-programs that access these information are sports and tool mini-programs. For example, we found a mini-program that require wechat sports data to monitor whether a user is sticking to the fitness plan, and a mini-program called `earn scores' to earn scores by walking and completing tasks for purchasing presents.

 


% Aside from 2 mini-programs that does not access any sensitive encrypted information, the mini-programs accessed various information including phone number, user info, share info, and weRun data. The functionalities of these mini-programs cover a wide fields, ranging from online shopping and membership to travelling and sports. As mentioned in previous texts, most of these vulnerable mini-programs are associated with online shopping and membership coupons, which can be potentially exploited by attackers to make profit if they require user information or phone number for logging in. Besides, we also found that membership mini-programs may require user share info for which \wechat group chat the user is being navigated from. These membership mini-programs may motivate existing members to share their mini-programs to attract more fresh users, and may give special discount or coupons for them. As such, these mini-programs may also be vulnerable since attackers can modify the group information in the share info. 




 
 

 






% %\subsection{Case Studies}
% \paragraph{Account Hijacking} Vulnerable mini-programs that access user phone number to register or log in user accounts are subject to account hijacking attacks, where attackers use the \appsecret to query session key for modifying login information to fake themselves as arbitrary account. In this paper, we have demonstrated this attack in \cref{sub:attack}: since the attackers can trigger user log in access either via re-entering the mini-program or by hooking and executing \texttt{wx.login} API, the attackers can immediately trigger user login to get the login token to refresh the \appsecret when \appsecret is updated. Among the \leakedapps vulnerable mini-program, one-third (51) are associated with this sensitive information, and the affected mini-programs are not limited to shopping. Aside from shopping mini-programs, we also found \appsecret leakage with phone number access among education, travelling, and public transportation mini-programs (e.g., bus e-cards). As such, the mini-program developer should be careful with the \appsecret and phone number access to avoid their mini-programs from being exploited by malicious users, which may cause loss of the company or user privacy.

% \paragraph{User Information Manipulation} Aside from phone numbers, a number of mini-programs require user information, such as the user account nickname, avatar, and region, to identify users. However, if the \appsecret is leaked, the attacker can change his or her user information, such as user nickname, gender, or user region, to perform phishing attack on other users with fake identity. We noticed that, among the vulnerable mini-programs, aside from shop mini-programs, there are games and lifestyle mini-programs. For game mini-programs that require two or more players (e.g., Tencent Battle Chess), attackers can approach other users with fake identity and avatars to scam the victim for money, although the account information in the mini-programs are believed to be verified by \wechat. 
% % For lifestyle mini-programs, we found a group mini-program that can be used to launch a lottery draw or reward point collection activity where users can receive profits or gifts. If the account information is modified, this may also

% \paragraph{User Sports Data Manipulation} The user sports data may also leak the user privacy if improperly used by mini-programs, or used to cheat in sports ranking activities. For example, we observed a mini-program developed by Behang University that integrates a daily sports ranking among other users. Some colleges or classes may require the students to perform certain sports exercises, give awards to top runners or pose punishments on last runners, the users can use the leaked appsecret to modify his/her sports data to cheat. Aside from cheating, we also observed that many mini-programs advocating `low carbon lifes' or `citizen excercises' give users score points if he/she achieves certain amount of sport activity (e.g., a certain amont of footsteps walks everyday) which can be used for getting gifts. Although we have not found \appsecret leakage in these case yet, but if the \appsecret is leaked, the mini-programs can be abused by manipulating the sports data sent to the server.

%\paragraph{(III) Vulnerable mini-programs from top companies} 

% which is surprising because the documentation of \wechat mini-program has warned the developers not to leak these \appsecret in the official documentation, but the developers still insisted on leaking these essential \appsecret. Since the \appsecret serves as a master password to verify the identity of mini-program owner, this leakage makes the mini-programs vulnerable to various Coffee attacks.


% On top of the mini-program scores, we also grouped the affected mini-programs according to accessed user information in \cref{fig:heatmap_vuln}. We found that a majority of mini-programs that leaked appsecrets are associatede with user's phone number access. This is likely because of the phone number is used by mini-programs to register and log in user account. For example, when entering Nestle member center, the mini-program will ask the user for his/her personal information access. Then, the mini-program will promt the user to log in or register to receive discounts or send promotions to the new user.


% We first captured all string values that appear in the form of 32-bit hex string, and then we send this value and the corresponding mini-program ID to \texttt{api.weixin.qq.com/cgi-bin/token} to validate whether the string value is a real appsecret. 



% \paragraph{(III) Redirected mini-programs} Interestingly, aside from the mini-program credential leakage, we also observed that these vulnerable mini-programs are redirecting to other mini-programs. If the account info can be fabricated in the vulnerable mini-program, then the victim being redirected to may suffer from the attack too if extra data is being attached and processed during the redirection. 

% \paragraph{mini-programs that are being redirected by large amount of mini-programs} As shown in \cref{fig:redirection_appsecret} and \cref{fig:redirection_key}, we observed that there are large clusters where multiple mini-program redirect to a center mini-program. For instance, in the top left of \cref{fig:redirection_appsecret}, there are 118 vunerable mini-program being redirected to by \AY{mini-program A}, which itself does not leak appsecret. Similarly, in \cref{fig:redirection_key}, there are three massive clusters with over 200 mini-programs. This may be mini-programs that are using a same set of mini-program template or third-party cloud service that leaked the appsecret in the template or the session key in their session key network request. As such, the credential leakage may be propagated via copy-paste or mini-program template. In the next section, we will explain more details about the implication of these cases with real world cases.

% \paragraph{mini-programs that redirect to each other} As shown in \cref{fig:redirection_appsecret}, we observed that there are some small clusters where mini-programs redirects to each other. For example, in the middle of \cref{fig:redirection_appsecret}, there is a cluster where 11 vulnerable mini-program redirects to each other. As shown in \cref{tab:appsecret}, this cluster belongs to the 10 mini-programs with 11 referrers that appear very similar in the mini-program name and the Javascript code. Therefore, it is very possible that all the 11 mini-programs are developed by a same vendor, and the vendor is possibly developing many duplicated mini-programs to escape from mini-program auditing and management.


% \AY{EVALUATION DATA}

% Normally, the session key is generated by the back-end with login token returned by \texttt{wx.login}, and this session key is used for decryptions of user sensitive data. Therefore, since the session key cannot be leaked to the front-end, all sensitive encrypted data has to be sent back to the back-end. To investigate the potential leakage, we investigate three problems in this section. Our study shows that there is a concerning amount of mini-programs that are highly possible to either leak the session keys via sensitive network URLs, or process encrypted data with leaked session key because there is no associated network requests found after sensitive encrypted data is being acquired.




% \begin{table*}[]
% \scriptsize
% \belowrulesep=0pt
% \aboverulesep=0pt
% \setlength\tabcolsep{1.5pt}
%     \centering
%     \begin{tabular}{c|c|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
%     \toprule
%      \multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\rot{business}}&\multicolumn{1}{c|}{\rot{education}}&\multicolumn{1}{c|}{\rot{entertainment }}&\multicolumn{1}{c|}{\rot{finance}}&\multicolumn{1}{c|}{\rot{food}}&\multicolumn{1}{c|}{\rot{game}}&\multicolumn{1}{c|}{\rot{government}}&\multicolumn{1}{c|}{\rot{health}}&\multicolumn{1}{c|}{\rot{images}}&\multicolumn{1}{c|}{\rot{job}}&\multicolumn{1}{c|}{\rot{lifestyle}}&\multicolumn{1}{c|}{\rot{reading}}&\multicolumn{1}{c|}{\rot{shopping}}&\multicolumn{1}{c|}{\rot{social}}&\multicolumn{1}{c|}{\rot{sports}}&\multicolumn{1}{c|}{\rot{tool}}&\multicolumn{1}{c|}{\rot{traffic}}&\multicolumn{1}{c|}{\rot{travelling}}\\ \hline
%      \multirow{11}{*}{\rot{back-end}}&\multirow{9}{*}{\tabincell{c}{session\\key}}&\texttt{login}&14,744&48,810&3,622&1,526&34,422&21,140&11,416&9,956&454&6,164&86,823&2,426&132,115&6,486&3,849&33,303&10,124&1,166\\\cline{3-21}
%   &&\texttt{getUserInfo}&11,332&38,231&3,248&1,164&26,322&23,203&8,489&7,307&380&4,972&64,401&1,314&9,5916&5,522&3,180&29,032&7,678&955
% \\\cline{3-21}
%       &&\texttt{getUserProfile}&30&86&30&4&40&8&28&45&2&56&197&5&265&18&6&47&18&1\\\cline{3-21}
%       &&\texttt{getUserInteractiveStorage}&&&&&&\\\cline{3-21}
%      &&\texttt{getWeRunData}&161&280&42&23&120&105&102&81&5&21&226&17&609&62&1040&428&34&6\\\cline{3-21}
%      &&\texttt{getGroupEnterInfo}&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\\\cline{3-21}
%      &&\texttt{getShareInfo}&&&&&&\\\cline{3-21}
%      &&\texttt{chooseInvoice}&4&3&0&0&0&0&3&1&0&0&9&0&3&0&2&16&1&0\\\cline{3-21}
%      &&\texttt{request}&&&&&&\\\cline{2-21}
%      \bottomrule
%     \end{tabular}
%     \caption{Security-related APIs and Values\AY{Will fix that later}}
%     \label{tab:apis}
% \end{table*}

% \begin{table}[]
%     \centering
%     \scriptsize
%     \begin{tabular}{r|c|c}
%     \toprule
%     \# of mini-program a specific mini-program redirects to& \# app & \% app\\
%  >10&50&0.02\\
% 9&25&0.01\\
% 8&31&0.01\\
% 7&29&0.01\\
% 6&262&0.10\\
% 5&599&0.23\\
% 4&613&0.23\\
% 3&2920&1.11\\
% 2&34055&12.89\\
% 1&225612&85.40\\
% total&264196&100.00\\\bottomrule
%     \end{tabular}
%     \caption{Amount of mini-programs each mini-program redirects to\AY{Would like to remove}}
%     \label{tab:redirection}
% \end{table}


% \section{Case Study and Root Causes}
% \subsection{Coffee Attack}
 





==> paper/5_evaluation_backup.tex <==
\section{Evaluation}
\label{sec:evaluation}
 

\subsection{Experiment Setup}

\paragraph{Mini-program Collection} \AY{It has been reported that there are over 2 million mini-programs in \wechat market~\cite{WeChatMi59:online}. To do so, we collected mini-programs with our crawler based on the metadata collected from \wechat mini-program searching API. In total, we collected TODO mini-programs during the past year for our evaluation.} \sout{We could have downloaded all of them for the analysis, but we feel we do not have to do so, since there could be many unpopular apps, similar to the apps in the Google Play. Therefore, we decide to crawl only the popular apps. However, there is no ranking of the mini-programs, and we can only search them using keywords.
To search for popular mini-programs, we first obtain the company name from the list of Fortune 500~\cite{fortunechina}. With these company names, we first perform word segmenting with Chinese word segmentation tool \texttt{jieba}~\cite{jieba}, and then use the TF-IDF algorithm~\cite{ramos2003using} to extract the keywords from the two lists, and in total we collected 774 keywords. 
%
%The TF-IDF algorithm is widely used in search engines to evaluate the importance of a keyword. If a keyword exists frequently in a certain document but does not exist in other documents, then the keyword's TF-IDF will be higher. For example, for `Alibaba Group Holding Ltd.,', the keyword `Ltd.,' exists in most of the company names, and hence the TF-IDF value is low. However, since Alibaba does not appear in other company names, the TF-IDF value of this is relatively higher. As such, to generate keywords more relevant to company names, we ranked the keywords based on TF-IDF score, and chose the keyword with highest TF-IDF score (e.g., `Alibaba'). 
%
%Finally, we obtain 493 different keywords. 
We feed these 774 keywords into our mini-crawler, and eventually collected \totalapps mini-programs in a one week period with one \wechat account. \looseness=-1 }
% one week's downloading. 

\paragraph{Running Environment} We performed our analysis on two Linux desktops, each of which has 8 cores, Intel Core i7-8700 (3.20 GHz) CPUs and 16 GB RAM. We use a client-server mode to run our analysis, where the server machine %While we preforming our analysis, we applied a client-server mode to enable the analysis tasks to run in parallel, where the server running on one machine 
is responsible for assigning the tasks and collecting the results, and the client machine is responsible for the analysis. 



%based on all our 493 collected keywords for analysis.
 
% \paragraph{Vulnerability Detection} It is straightforward to detect the vulnerability. First, we detect whether or not a mini-program has invoked the APIs (\ie, \texttt{getPhoneNumber}) that can fetch the encrypted sensitive data from the \wechat server, as our attack works against the data encryption mechanism; If so, we then further detect whether the mini-program has the \appsecret leakage. To be more specific, we tackle (1) Sensitive API Invocation Detection and (2) Master key \appsecret Leakage Detection:      

% \begin{itemize}
% \item \paragraph{(1) Sensitive API Invocation Detection} we utilize \texttt{esprima} to generate the Abstract Syntax Tree (AST) of the mini-programs and perform a static analysis for function invocation in the JavaScript file. As shown in \cref{tab:api}, each encrypted user information (in the \textbf{E} column) is associated with a mini-program API. As such, we can detect whether a mini-program accesses an encrypted user information by detecting whether the corresponding API is being invoked. Note that there is one special case: \texttt{getPhoneNumber}. To protect user privacy, this API is can not be invoked in the code, but invoked when the user actively clicks a WXML button with \texttt{openType="getPhoneNumber"}, so as to make sure the user is aware of the requirement of his/her phone number. As such, to cover all the APIs associated with encrypted data, we also parses the WXML files to detect the usage of the user phone number.

% \item \paragraph{(2) Master key \appsecret Leakage Detection}

% For detecting the leakage of  \appsecret, as it has a fixed format (\ie, it is a 32-byte long hex string), the most intuitive way to detect \appsecret leakage is to grep the decomplied JavaScript code using regular expression (\ie, \texttt{[a-f0-9]\{32\}}). However, such a method is subject to false alerts, since many strings in a mini-program have the same format (\ie, some online databases used the 32-bytes hex string as the primary key). Fortunately, we have identified an access token query API (\ie,  \url{https://api.weixin.qq.com/cgi-bin/token?grant_type=client_credential&appid=APPID&secret=MK}) provided by \wechat server, which can assist us to verify the correctness of \appsecret. Specifically, the API is designed for the third-party developers to query an access token (Note that the access token is different from login token \token), with which the third-party developers can then initiate the network requests to the \wechat server for some of the services (\eg, binding the mini-program with the vendor's official \wechat account). The API takes two parameters: the publicly accessible mini-program ID and the mini-program \appsecret, and returns the access token when the two parameters are matched.  Therefore, in our analysis, we first collect all specious strings from the decomplied mini-programs, and then feed those strings to the access token query API to check whether the \appsecret is valid.
% \end{itemize}



 
 
 
  %\AY{In general, there are two questions to answer for coffee attack vulnerability detection. (1) is the appsecret of the mini-program leaked? (2) what kind of encrypted information does the mini-program access?}

 
%  \wechat have more than one million mini-programs available, and they did not provide 


% to generate our keyword database, which allows us to query and fetch mini-programs from \wechat. To be more specific, 



%  we use NLP techniques to generate the keyword for query. First, we used \texttt{Jieba} to perform Chinese word segmentation. Then, we used TFIDF algorithm to extract the keywords of these company names. After deduplication, we finally have a list of 493 keywords. As such, we used the 493 keywords to query the \wechat mini-program API, and collected 8,824 mini-programs for analysis

 
%  To investigate the impact of our discovered problem and attacks, we need to collect a set of mini-programs and detect the th



% We


% To collect the mini-programs, 



\begin{table*}[]
\scriptsize
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
    \centering
    \begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
\toprule
\multirow{3}{*}{Category}&\multicolumn{3}{c|}{Phone Number}&\multicolumn{3}{c|}{WeRun Data}&\multicolumn{3}{c|}{User Info}&\multicolumn{3}{c|}{Forwarded Messages}&\multicolumn{3}{c|}{Shared mini-program}&\multicolumn{3}{c|}{Group Chat Info}&\multicolumn{3}{c}{Shipping Address}\\ \cmidrule{2-22}
&\multicolumn{3}{c|}{\texttt{getPhoneNumber}}&\multicolumn{3}{c|}{\texttt{wx.getWeRunData}}&\multicolumn{3}{c|}{\texttt{wx.getUserInfo}}&\multicolumn{3}{c|}{\texttt{wx.getShareInfo}}&\multicolumn{3}{c|}{\texttt{wx.authPrivateMessage}}&\multicolumn{3}{c|}{\texttt{wx.getEnterGroupInfo}}&\multicolumn{3}{c}{\texttt{wx.chooseAddress}}\\ \cmidrule{2-22}
&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app&\# vuln&\# app&\% app\\ \midrule
Business&3&410&0.73&0&10&0.0&13&600&2.17&1&47&2.13&0&1&0.0&0&0&0.0&0&0&0.0\\
Education&10&522&1.92&2&14&14.29&22&1,108&1.99&4&169&2.37&0&0&0.0&0&0&0.0&0&0&0.0\\
Entertainment&2&121&1.65&0&2&0.0&9&277&3.25&1&52&1.92&0&1&0.0&0&0&0.0&0&0&0.0\\
Finance&3&90&3.33&0&6&0.0&6&156&3.85&1&13&7.69&0&0&0.0&0&0&0.0&0&0&0.0\\
Food&1&118&0.85&0&0&0.0&4&195&2.05&0&26&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Games&0&19&0.0&0&3&0.0&17&450&3.78&3&86&3.49&0&0&0.0&0&0&0.0&0&0&0.0\\
Government&4&192&2.08&0&16&0.0&13&353&3.68&0&17&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Health&5&186&2.69&0&10&0.0&7&239&2.93&0&24&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Images&0&11&0.0&0&2&0.0&0&100&0.0&0&13&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Job&3&92&3.26&0&0&0.0&4&142&2.82&1&13&7.69&0&0&0.0&0&0&0.0&0&0&0.0\\
Lifestyle&22&1,080&2.04&0&6&0.0&40&1,762&2.27&2&213&0.94&0&0&0.0&0&0&0.0&0&0&0.0\\
Reading&1&60&1.67&0&5&0.0&4&207&1.93&0&43&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Shopping&23&2,597&0.89&1&27&3.7&56&3,737&1.5&8&569&1.41&0&0&0.0&0&0&0.0&0&0&0.0\\
Social&0&46&0.0&0&2&0.0&0&116&0.0&0&20&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Sports&4&95&4.21&1&35&2.86&6&159&3.77&0&20&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Tool&26&695&3.74&3&35&8.57&58&2,190&2.65&4&240&1.67&0&0&0.0&0&0&0.0&0&0&0.0\\
Traffic&14&344&4.07&0&30&0.0&6&506&1.19&0&63&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Travelling&1&83&1.2&0&18&0.0&2&118&1.69&0&42&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\
Uncategorized&0&0&0.0&0&0&0.0&0&1&0.0&0&0&0.0&0&0&0.0&0&0&0.0&0&0&0.0\\ \midrule
Total&122&6,761&1.8&7&221&3.17&267&12,416&2.15&25&1,670&1.5&0&2&0.00&0&0&0.00&0&0&0.00\\ \bottomrule
    \end{tabular}
    \caption{Statistics of the identified vulnerable mini-programs.\AY{Considering the final results, may change to single column, remove the ones with 0s, and explain in the caption}}  
    \label{tab:apis}

\end{table*}


%\AY{In our paper, we are interested in two types of mini-programs: (1) the mini-programs that have been developed by IT companies that migrated their native apps into \wechat mini-program platform (e.g., mini-programs developed by Tencent and Baidu). (2) the mini-programs developed by . As such, we obtained the list of top IT companies from the report of Chinese IT companies (2020) published by Internet Society of China \cite{isc}. For the list of top commercial companies, we obtained the keyword list from Fortune China \cite{fortunechina}.}

% \AY{With the company list obtained, we use NLP techniques to generate the keyword for query. First, we used \texttt{Jieba} to perform Chinese word segmentation. Then, we used TFIDF algorithm to extract the keywords of these company names. After deduplication, we finally have a list of 493 keywords. As such, we used the 493 keywords to query the \wechat mini-program API, and collected 8,824 mini-programs for analysis.}
% \subsection{Vulnerability Detection}
% \AY{In general, there are two questions to answer for coffee attack vulnerability detection. (1) is the appsecret of the mini-program leaked? (2) what kind of encrypted information does the mini-program access?}





%\paragraph{Vulnerability}

% 
% \paragraph{Data Set} We collected our mini-programs from \wechat app via its built-in mini-program searching functionality. In \wechat app, users can either install a mini-program by clicking on a link shared by other user, or manually use keyword to search for a specific mini-program. To obtain a list of mini-programs to be downloaded, we reverse engineered \wechat, investigated the workflow of the search interface, and collected the metadata of $510,000$ mini-programs containing mini-program IDs, descriptions, and extra category info. Then, we created a crawler that runs on mobile phones to automatically download mini-programs. In average, our tool $3,000$ mini-programs a day. We used two mobile phones to work together, and eventually we obtained \totalnum mini-program packages for analysis.    

% We implemented \textsf{CoffeCAN} in JavaScript with \texttt{esprima}\cite{esprima} to generate AST of mini-program source code, and Python to support multi-process processing. We performed our analysis on two Linux computers, each of which has 8 cores, Intel Core i7-8700 (3.20 GHz) CPUs and 16 GB RAM. It took 10 days for us to finish the analysis of the \totalnum mini-programs. 


\begin{table*}[]
\centering
    \scriptsize
    \aboverulesep=0pt
    \belowrulesep=0pt
    \begin{tabular}{r|l|l|l|l|c|c|c}
    \toprule
         {\bf Company Name} & \bf The mini-program Name& \bf Accessed Data & \bf Service&AppID& refreshed&Remained&Removed \\
         \midrule
\multirow{6}{*}{Nestle (6)}&Nestle DolceGusto Member Center&info&Membership&wx0e08********cb22&\Circle&\Circle&\CIRCLE\\
&Nestle Customer Center&phone&Customer Service&wx7cff********b6fe&\CIRCLE&\Circle&\Circle\\
&Nestle Flagship Shop&info,share&Online Shopping&wx8ab4********21ec&\CIRCLE&\Circle&\Circle\\
&Nestle Ice Cream Happy Sharing&info&Online Shopping&wx856d********51bb&\Circle&\Circle&\CIRCLE\\
&Nestle Coffee Member CLub&phone,info&Membership&wx693d********d699&\Circle&\Circle&\CIRCLE\\
&We Proudly Serve&phone,info&Membership&wx1bb7********1204&\Circle&\CIRCLE&\Circle\\
\multirow{3}{*}{Tencent (3)}&Cool Run Everyday&info&Game&wxcf75********f808&\Circle&\CIRCLE&\Circle\\
&Tencent Billiards&info&Game&wx2f7f********31ee&\Circle&\Circle&\CIRCLE\\
&Tencent Everyday Battle Chess&info&Game&wx2225********fe10&\Circle&\CIRCLE&\Circle\\
\multirow{2}{*}{China Telecom (2)}&China Telecom Guangdong Job Center&info&Job Hunting&wx3879********c055&\CIRCLE&\Circle&\Circle\\
&China Telecom 5G Membership&phone&Membership&wx7712********7e10&\Circle&\Circle&\CIRCLE\\
\multirow{2}{*}{China Mobile (2)}&China Mobile 139 email&phone,info&Email service&wxbb71********41c6&\Circle&\Circle&\CIRCLE\\
&Xinjiang Mobile Network Expert&phone&Network service&wx8d02********a222&\Circle&\CIRCLE&\Circle\\
\multirow{2}{*}{China Post (2)}&China Post Car Holders&info&Car Service&wx3d12********8ac7&\Circle&\Circle&\CIRCLE\\
&China Post Library&info&Library Management&wxf174********7d1e&\Circle&\CIRCLE&\Circle\\
\multirow{2}{*}{HP (2)}&HP China Official Shop&phone,info,share&Online Shopping&wxb3bd********1a8f&\CIRCLE&\Circle&\Circle\\
&HP Shining SHop&-&Online Shopping&wx6cf0********cd25&\Circle&\CIRCLE&\Circle\\
\multirow{2}{*}{Mazda (2)}&Mazda 4S Shop&info&Car Service&wxbf35********c33e&\CIRCLE&\Circle&\Circle\\
&Mazda Ningyuan Shop&info&Online Shopping&wx9501********996b&\Circle&\CIRCLE&\Circle\\
Ford (1)&Ford Automobile Price Lookup&-&Tool&wxf17f********3dfc&\CIRCLE&\Circle&\Circle\\
Hyundai \& KIA (1)&Hyundai - KIA Car Accessories&-&Online Shopping&wx37c5********e679&\CIRCLE&\Circle&\Circle\\
Hyundai (1)&Hyundai Accessories Shop&info&Online Shopping&wxc24f********bf6d&\CIRCLE&\Circle&\Circle\\
KIA (1)&Tianjin KIA Automobile&info&Onlien Shopping&wx04a7********7052&\CIRCLE&\Circle&\Circle\\
Toyota (1)&Toyota Online Shop&phone,werun,info&Online Shopping&wx4fc9********9395&\Circle&\Circle&\CIRCLE\\
Volvo (1)&Volvo Repair&info&Car Service&wx64fd********b2f5&\CIRCLE&\Circle&\Circle\\
Cisco (1)&Cisco Collaboration&info&Product Promotion&wx165c********c840&\CIRCLE&\Circle&\Circle\\
Lenovo (1)&Lenovo Inteliggent Travelling&phone,info&Tool&wxea9c********b436&\CIRCLE&\Circle&\Circle\\
Huawei (1)&Huawei Companion Club&info&Membership&wx8ff2********f4a3&\Circle&\Circle&\CIRCLE\\
Bank of China (1)&BOC Virtual Bank&info&Virtual Bank&wx3db9********36e1&\CIRCLE&\Circle&\Circle\\
China Life (1)&Salesperson account book&phone&Tool&wx1eb6********0ab8&\CIRCLE&\Circle&\Circle\\
Ansteel Group (1)&Ansteel Milk Online Shop&info&Online Shopping&wx06ea********2f29&\Circle&\CIRCLE&\Circle\\
Pingan (1)&Pingan Free Insurance&info&Insurance Promotion&wx2880********6a98&\Circle&\Circle&\CIRCLE\\
Petro China (1)&Petro China Labor Security&-&Online Shopping&wx5e6e********7ebc&\CIRCLE&\Circle&\Circle\\
Sinopec (1)&Sinopec Gueizhou&phone,info&Car Service&wx9a95********3445&\Circle&\Circle&\CIRCLE\\
SinoPharm (1)&SinoPharm Engineering Hiring&info&Job Hunting&wxb774********d35d&\CIRCLE&\Circle&\Circle\\
Bosch China (1)&Bosch China Hiring&info&Job Hunting&wx4cfc********e1c1&\CIRCLE&\Circle&\Circle\\
Nike (1)&Nike Fitness Center&info&Sports&wx0816********41bc&\CIRCLE&\Circle&\Circle\\

\bottomrule

    \end{tabular}
    \caption{The list of the Fortune 500 companies whose mini-programs have leaked the \appsecret.\AY{Later will be reformed and moved to case study}
    }
    \label{tab:appsecret}
    
\end{table*}
 


\subsection{Evaluation Result}

Among all our \totalapps collected mini-programs, our tool successfully unpacked \totalanalyzedapps mini-programs. Among these \totalanalyzedapps mini-programs, our tool identified \leakedapps mini-programs that had leaked their {\tt MK}s. In the following, we describe how we reached these results. In particular, we first discuss the performance of our tool (\S\ref{subsubsec:tool}), followed by the statistics of all our collected mini-programs (\S\ref{subsubsec:dataset}),  the statistics of these vulnerable mini-programs (\S\ref{subsubsec:flaws}).\sout{, and finally the statistics of the vulnerable mini-programs from  the top fortune 500  Companies (\S\ref{subsubsec:top}).  }

% \begin{figure} 
% \centering
% \begin{minipage}[t]{0.495\linewidth}
% \includegraphics[width=\linewidth]{image/stat_x_time.pdf}
% \caption{Distribution of mini-program extraction time}
%  \label{fig:stat_exec}
% \end{minipage}
% % \hspace{1mm}
% \begin{minipage}[t]{0.495\linewidth}
% \includegraphics[width=\linewidth]{image/stat_analyze_time.pdf}
% \captionsetup{justification=centering}
% \caption{Distribution of mini-program analyze time}  
%  \label{fig:stat_analyze}
%  \
% \end{minipage}
% % \begin{minipage}[t]{0.495\linewidth}
% % \includegraphics[width=\linewidth]{image/stat_size.pdf}
% % \captionsetup{justification=centering}
% % \caption{Distribution of mini-program Size}  
% %  \label{fig:stat_ast}
% % \end{minipage}
% % \begin{minipage}[t]{0.495\linewidth}
% % \includegraphics[width=\linewidth]{image/stat_loc.pdf}
% % \caption{Distribution of mini-program line of codes}
% %  \label{fig:stat_loc}
% % \end{minipage}
% % \hspace{1mm}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{image/all_miniapp_cat_score.pdf}
    \caption{Heatmap of collected mini-programs, w.r.t. scores and categories} %\ZY{Black-white}
    \label{fig:heatmap_all_scores}
    \
\end{figure}





 
\subsubsection{\bf{Performance of Our Analysis Tool}} 
\label{subsubsec:tool}
%We applied our analyzer on \totalapps mini-programs collected with \keywords keywords. 

%Since the impact of our attacks can be devastating for the 3-rd party developers, and 

%We applied our tool over \totalapps mini-programs, the performance determines whether we can find the vulnerabilities 
With the crawled mini-programs, our analysis tool around 51 hours to finish, with 46 hours spent on unpacking the mini-program packages by \texttt{WXUnpacker}~\cite{decomplier}, and 4.8 hours spent on generating and analyzing the JavaScript code. \sout{In \autoref{fig:stat_exec}, we show the cumulative distribution function (CDF) of the time that is used to unpack the mini-programs. We can observe that the}\AY{The} average unpacking time of one mini-program package is \unpavg seconds, \sout{while more than \unpratio mini-programs can be unpacked within a minute.} When compared with the unpacking time, the analysis time is relatively shorter (\AY{the average analysis time is \anaavg seconds})\sout{90\% of the mini-programs are analyzed within 5 seconds), as shown in \autoref{fig:stat_analyze}.} This is because while processing the unpacked JavaScript code,  our tool only used pattern matching to search for the possible \totalanalyzedapps and API usage without involving any other sophisticated program analysis. %the  control-flow graph (CFG) extracting and praising. \looseness=-1    

%\texttt{WXUnpacker}~\cite{decomplier}

%The results of our extraction are shown as green lines in \autoref{fig:stat_exec} through \autoref{fig:stat_ast}. As shown in the figures, we observed that the extraction time elapsed to extract a mini-program package scatters from 10 seconds to 1 minutes, whereas the analysis time are relatively shorter (90\% of the mini-programs are analyzed within 5 seconds). The mini-programs we collected ranges from 12 to 20,045 lines of code, with the AST nodes ranging from 47 to 21,224. This indicates that we have collected not only tiny mini-programs with limited functions but also heavy mini-programs that provide complex functionalities. These

Among these mini-programs, we collected \sessionstrings 32-bit hex strings by string matching among the \totalanalyzedapps mini-programs. To verify the mini-program \appsecret within these hex strings, we implemented a python tool to query the results from \wechat server and executed the script with \numofthread threads. The verification process took \numofhour hours to finish. In total, our detection tool identified \leakedapps out of \totalanalyzedapps mini-programs leaked the \appsecret. 
%\ZQ{fix this paragraph}




\subsubsection{\bf{Statistics of the Collected Mini-programs}} 
\label{subsubsec:dataset}
In total, these \totalanalyzedapps mini-programs took up \totaldisk GB of disk space. %To analyze our dataset from an aggregation level, we group the mini-programs based on their sizes and then count the numbers of mini-programs in each group. \autoref{} shows the   cumulative distribution function (CDF) of the mini-programs. It can be observed that the average size of the mini-programs is [\ZY{}], and more than [\ZY{}] mini-programs are less than [\ZY{}] MB. Meanwhile, we also group the mini-programs based on their lines of code contained in the unpacked mini-program packages, as shown in \autoref{image/stat_loc.pdf}.  The  lines of code of mini-programs range from 12 to 20,045, which indicates that we have collected not only tiny mini-programs with limited functions but also mini-programs that provide complex functionalities. 
Other than analyzing the collected mini-programs from the JavaScript code, we also analyzed the these mini-programs by parsing the collected meta data.  Recall that the rating and the category  of a mini-program can be found in the meta data, and therefore, we plot the heat-map based on the categories and the ratings of our collected mini-programs, where the x-axis is the categories that the mini-program belong to and the y-axis is the ratings of these mini-programs. The more mini-programs fall into a specific category with a specific rating, the darker the color of the cell that represents the category with the rating will be. As shown in \cref{fig:heatmap_all_scores}, the mini-programs can either be rated or not rated. This is because the rating of a mini-program is displayed only when enough people rate the mini-program. In total, we found \numwithscore mini-programs that have ratings, where the mean value of these mini-programs are \meanscores, and \numwithscorefive mini-programs are rated 5.0 scores. 
% It can be observed from \autoref{fig:my_label} that aside from the mini-programs that currently do not have the ratings (only enough people rate the mini-program, most of these rated mini-programs a relatively high rating~\cite{ratings}). 
% For example, the mean value of these mini-programs are  [\ZY{}], and  [\ZY{}] with the rating of 5.0.
Interestingly, we find that the games are usually rated lower, while the mini-program in categories of life-style, shopping and tools usually have higher ratings.    
 

 

%As shown in the figures, compared with normal mini-programs, mini-programs that leaked \appsecret on average take less time to extract and to analyze, and contains less lines of codes and AST nodes. 








% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{image/company.pdf}
%     \caption{Relationships between developers and mini-programs \ZQ{This figure doesn't contribute much interesting knowledge and can be removed}}
%     \label{fig:developers}
% \end{figure}

% \begin{figure} 
% \centering
% \begin{minipage}[t]{0.463\textwidth}
% \includegraphics[width=\textwidth]{image/miniapp_cat_score.pdf}
% \caption{Heatmap of distribution in scores and categories among all mini-programs}
%  \label{fig:heatmap__all_score}
% \end{minipage}
% % \hspace{1mm}
% \begin{minipage}[t]{0.533\textwidth}
% \includegraphics[width=\textwidth]{image/miniapp_cat_prob.pdf}
% \captionsetup{justification=centering}
% \caption{Heatmap of user information access among all mini-programs}  
%  \label{fig:heatmap_all_access}
% \end{minipage}
% \end{figure*}
% \begin{figure*} 
% \centering
% \begin{minipage}[t]{0.463\textwidth}
% % \includegraphics[width=\textwidth]{image/miniapp_cat_score.pdf}
% \caption{Heatmap of distribution in scores and categories among vulnerable mini-programs}
%  \label{fig:heatmap_vuln_score}
% \end{minipage}
% \hspace{1mm}
% \begin{minipage}[t]{0.533\textwidth}
% \includegraphics[width=\linewidth]{image/vuln_miniapp_cat_prob.pdf}
% \captionsetup{justification=centering}
% \caption{Heatmap of user information access among vulnerable mini-programs}  
%  \label{fig:heatmap_vuln_access}
% \end{minipage}
% \end{figure}
% \begin{figure} 
% \centering
% \includegraphics[width=\linewidth]{image/redirection_appsecret_string.pdf}
% \caption{Relationship of confirmed miniapps that leak appsecret as String variables}
%  \label{fig:redirection_appsecret}
% \end{figure}


% \begin{table}
%     \centering
%     \scriptsize
%     \aboverulesep=0pt
%     \belowrulesep=0pt
%     \begin{tabular}{r|l|l}
%     \toprule
% {\bf \# App}&\bf Domain&\bf Servive\\ \midrule
% 34&apis.map.qq.com&Tencent Map\\ 
% 14&api.map.baidu.com&Baidu Map\\ 
% 13&pingtas.qq.com&Tencent mini-program Analytics\\ 
% 11&wx.qlogo.cn&Tencent Avatar Logo\\ 
% 10&restapi.amap.com&AutoNavi Map\\ 
% 8&webim.tim.qq.com&Tencent Web Messaging\\ 
% 7&log.aldwx.com&Third-party mini-program Analyics\\ 
% 6&api.mch.weixin.qq.com&Tencent Payment\\ 
% 5&api.aikst.cn&mini-program Template Provider\\ 
% 5&yun.tim.qq.com&mini-program Third-paty Back-end\\ 
% 4&sandcash.mixienet.com.cn&mini-program Third-paty Back-end\\ 
% 4&thirdwx.qlogo.cn&mini-program Template Provider\\ 
% 4&tcb-api.tencentcloudapi.com&Tencent Cloud Base\\ 
% 4&wxapp.yz168.cc&mini-program Third-paty Back-end\\ 
% 3&glog.aldwx.com&Third-party mini-program Analyics\\ 
% 3&api.q.qq.com&Tencent Server API\\ 
% 3&www.hhhkd.top&mini-program Third-party Back-end\\ 
% 3&tongji.dcloud.io&Third-party mini-program Analytics\\ 
% 3&aip.baidubce.com&Baidu Cloud API\\ 
% 3&iploc.ywdier.com&Third-party mini-program Back-end\\ \bottomrule

%     \end{tabular}
%     \caption{Top 20 communication domains configured by vulnerable mini-programs\AY{Not Up To Date}}
%     \label{tab:vuln_domain}
% \end{table}



% In this paper, we mainly investigate two types of vulnerabilities: the appsecret leakage, and the session key leakage. For appsecrets, the 32-bit hex string can be leaked as hard-coded strings, or as part of the parameter of network URLs. To model the potential leakage of session keys, we investigate them from two aspects: on one hand, we investigate the network URL associated with user login and login token to find whether there are sensitive third-party network APIs that are potentially leaking session key. On the other hand, we track the network request APIs associated with sensitive APIs related to encrypted data: since the decryption are only supposed to be performed at back-end, if an API associated with encrypted data does not send their data to the back-end, then the mini-program may be processing the data at the front-end and the session key is being potentially leaked.

% \paragraph{(II) Vulnerable mini-programs and information accessed} 


% As shown in \cref{fig:heatmap_score}, in general, most of the vulnerable mini-programs are not being scored yet, indicating that they are fresh-created mini-programs or mini-programs not being used by a large amount of people. During our inspection, most of these mini-programs not being scored are regional lifestyle or shopping mini-programs, such as local hair saloons and local supermarket. Aside from these mini-programs, most of the affected and scored mini-programs are over 4.0 points, which indicates that the appsecret leakage may also affect very highly rated mini-programs. As to the categories, we discover that most of the mini-programs associated with appsecret leakages are education, games, lifestyle, shopping, and sports mini-programs. Interestingly, these mini-programs are much more likely to be associated with sensitive user data, such as user phone number to register account, and user sports data. 

% From the figure, we discovered that most of the popular mini-programs are shopping mini-programs, whereas the majority of the rest of the mini-programs are associated with shopping activities as well (e.g., the first food mini-program is actually a wine shop). This means many of these mini-programs with appsecret leakage are associated with actions such as shopping, payment, and coupon, which may be dangerous since the attacker can manipulate encrypted data to make profits or steal user information.

\subsubsection{\bf{Statistics of Vulnerable Mini-programs}} 
\label{subsubsec:flaws}
%After analysis, we have collected 
With the \leakedapps vulnerable mini-programs, we further obtain more insights from them such as (I) the distribution of the categories of the vulnerable mini-programs, (II) the distribution of the sensitive information these vulnerable mini-programs accessed, and (III) the distribution of the developer information of these vulnerable mini-programs. 


%vulnerable mini-programs from top companies and finally the (IV) distribution of vulnerable mini-programs from top Companies. 
\begin{enumerate} [label=(\Roman*),leftmargin=*]
 
\item \textbf{Distribution of Categories of Vulnerable mini-programs.} \autoref{tab:apis} presents the statistics of all the identified vulnerable mini-programs. Particularly, we grouped the mini-programs based on their categories and the user information these mini-programs accessed. From \autoref{tab:apis}, we surprisingly discovered that most of \appsecret leakages occur in tool mini-programs (\toolvulnerable out of \tooltotal, \toolratio), shopping mini-programs (\shoppingvulnerable out of \shoppingtotal, \shoppingratio), and lifestyle mini-programs (\lifestylevulnerable out of \lifestyletotal, \lifestyleratio). Since many of these shopping, tool, and lifestyle apps are often involved with payment procedures, the \appsecret leakage over these mini-programs can have serious impacts (\eg, an attacker can hijack the victim's account and shop for free). 


\item \textbf{Distribution of Sensitive Information Collected by Vulnerable mini-programs.} Recall that according to different sensitive information the app accessed, the attacker can deploy different attacks against the mini-programs, and therefore, we present the statistics of different sensitive data these mini-programs accessed based on the API used. The statistics of sensitive data access are also shown in table \autoref{tab:apis} (note that a mini-program may access multiple types of sensitive data, and there are \noaccess mini-programs that did not access any sensitive data). As shown in the table, the user information (\eg, user's avatar and gender) gets used most often (\inforatio). The attacker can use the leaked \appsecret and malware to steal the sensitive information from a victim. Aside from the user information, the second most used sensitive information is phone numbers. With the leaked \appsecret, the attacker can manipulate the phone number, and deploy the account hijack attacks against these mini-programs. We currently have not found any mini-programs used the social information or shipping addresses.



\end{enumerate} 
 
\subsubsection{\bf Distribution of Vulnerable mini-programs from the Fortune 500 Companies} 
\label{subsubsec:top}
\AY{To identify problems related with high-profile companies, we first generated a dictionary containing keywords from the Fortune top 500 companies. Then, we matched the mini-program names to filter out mini-programs we are interested in, both for all mini-programs and mini-programs identified to contain \appsecret exposure. In total, \topcompanyapps mini-programs are identified, with \topcompanyappsvuln of them are vulnerable. With these data, we present the distribution of vulnerable mini-programs and the ratio of all related mini-programs in \cref{fig:company-vuln}. As shown in the figure, }\TODO{(WAITING FOR FURTHER DATA)}
\begin{figure}
    \centering
    % \includegraphics{}
    \caption{Distribution of mini-programs related to top companies}
    \label{fig:company-vuln}
\end{figure}
\sout{we manually examined all the TODO vulnerable mini-programs and identified \companyapps mini-programs exactly from the world's top commercial companies {as listed in Fortune top 500 companies}. As shown in \autoref{tab:appsecret}, we in total identified TODO mini-programs from \companies different companies. Interestingly, we have made the following discoveries: First, some high profile companies made the same mistakes across their different mini-programs (\eg, Nestle, HP, Tencent and China Telecom); Second, we found that even Tencent themselves have made the mistakes by leaking their \appsecret to the front-end. Third, most of these companies have accessed the user's phone number and user information. As discussed, these information may be subject to different attacks.  Finally, some mini-programs from the high profile companies only leaked their \appsecret, but do not access any sensitive information (\eg, Petro China Labor Security). These mini-programs cannot be attacked currently, but if they introduced some functionalities such as phone number fetching in the future, they are vulnerable to our attacks. }



%that are possibly used to register account or create orders. This is surprising since the mini-program developers involved with such important functionalities overlooked the explicit warning in the \wechat official documentations of not leaking these \appsecret, and proceed to exposing their \appsecret to the front-end. Besides, it is also interesting that although the documentation indicates that the involved mini-program will be taken off the market if \appsecret leakage is detected, there are still over 2.1\% of the mini-programs that leaked \appsecret but still appear on the market. This indicates that the mini-program vetting and \appsecret leakage checking process of mini-program framework still needs to be improved.



%in different categories may access different kinds of user information. For example, there are more shopping and lifestyle mini-programs that access phone number and user information, since the mini-programs often require user information to perform purchasing and payment. For weRunData, however, most of the mini-programs that access these information are sports and tool mini-programs. For example, we found a mini-program that require wechat sports data to monitor whether a user is sticking to the fitness plan, and a mini-program called `earn scores' to earn scores by walking and completing tasks for purchasing presents.

 


% Aside from 2 mini-programs that does not access any sensitive encrypted information, the mini-programs accessed various information including phone number, user info, share info, and weRun data. The functionalities of these mini-programs cover a wide fields, ranging from online shopping and membership to travelling and sports. As mentioned in previous texts, most of these vulnerable mini-programs are associated with online shopping and membership coupons, which can be potentially exploited by attackers to make profit if they require user information or phone number for logging in. Besides, we also found that membership mini-programs may require user share info for which \wechat group chat the user is being navigated from. These membership mini-programs may motivate existing members to share their mini-programs to attract more fresh users, and may give special discount or coupons for them. As such, these mini-programs may also be vulnerable since attackers can modify the group information in the share info. 




 
 

 






% %\subsection{Case Studies}
% \paragraph{Account Hijacking} Vulnerable mini-programs that access user phone number to register or log in user accounts are subject to account hijacking attacks, where attackers use the \appsecret to query session key for modifying login information to fake themselves as arbitrary account. In this paper, we have demonstrated this attack in \cref{sub:attack}: since the attackers can trigger user log in access either via re-entering the mini-program or by hooking and executing \texttt{wx.login} API, the attackers can immediately trigger user login to get the login token to refresh the \appsecret when \appsecret is updated. Among the \leakedapps vulnerable mini-program, one-third (51) are associated with this sensitive information, and the affected mini-programs are not limited to shopping. Aside from shopping mini-programs, we also found \appsecret leakage with phone number access among education, travelling, and public transportation mini-programs (e.g., bus e-cards). As such, the mini-program developer should be careful with the \appsecret and phone number access to avoid their mini-programs from being exploited by malicious users, which may cause loss of the company or user privacy.

% \paragraph{User Information Manipulation} Aside from phone numbers, a number of mini-programs require user information, such as the user account nickname, avatar, and region, to identify users. However, if the \appsecret is leaked, the attacker can change his or her user information, such as user nickname, gender, or user region, to perform phishing attack on other users with fake identity. We noticed that, among the vulnerable mini-programs, aside from shop mini-programs, there are games and lifestyle mini-programs. For game mini-programs that require two or more players (e.g., Tencent Battle Chess), attackers can approach other users with fake identity and avatars to scam the victim for money, although the account information in the mini-programs are believed to be verified by \wechat. 
% % For lifestyle mini-programs, we found a group mini-program that can be used to launch a lottery draw or reward point collection activity where users can receive profits or gifts. If the account information is modified, this may also

% \paragraph{User Sports Data Manipulation} The user sports data may also leak the user privacy if improperly used by mini-programs, or used to cheat in sports ranking activities. For example, we observed a mini-program developed by Behang University that integrates a daily sports ranking among other users. Some colleges or classes may require the students to perform certain sports exercises, give awards to top runners or pose punishments on last runners, the users can use the leaked appsecret to modify his/her sports data to cheat. Aside from cheating, we also observed that many mini-programs advocating `low carbon lifes' or `citizen excercises' give users score points if he/she achieves certain amount of sport activity (e.g., a certain amont of footsteps walks everyday) which can be used for getting gifts. Although we have not found \appsecret leakage in these case yet, but if the \appsecret is leaked, the mini-programs can be abused by manipulating the sports data sent to the server.

%\paragraph{(III) Vulnerable mini-programs from top companies} 

% which is surprising because the documentation of \wechat mini-program has warned the developers not to leak these \appsecret in the official documentation, but the developers still insisted on leaking these essential \appsecret. Since the \appsecret serves as a master password to verify the identity of mini-program owner, this leakage makes the mini-programs vulnerable to various Coffee attacks.


% On top of the mini-program scores, we also grouped the affected mini-programs according to accessed user information in \cref{fig:heatmap_vuln}. We found that a majority of mini-programs that leaked appsecrets are associatede with user's phone number access. This is likely because of the phone number is used by mini-programs to register and log in user account. For example, when entering Nestle member center, the mini-program will ask the user for his/her personal information access. Then, the mini-program will promt the user to log in or register to receive discounts or send promotions to the new user.


% We first captured all string values that appear in the form of 32-bit hex string, and then we send this value and the corresponding mini-program ID to \texttt{api.weixin.qq.com/cgi-bin/token} to validate whether the string value is a real appsecret. 



% \paragraph{(III) Redirected mini-programs} Interestingly, aside from the mini-program credential leakage, we also observed that these vulnerable mini-programs are redirecting to other mini-programs. If the account info can be fabricated in the vulnerable mini-program, then the victim being redirected to may suffer from the attack too if extra data is being attached and processed during the redirection. 

% \paragraph{mini-programs that are being redirected by large amount of mini-programs} As shown in \cref{fig:redirection_appsecret} and \cref{fig:redirection_key}, we observed that there are large clusters where multiple mini-program redirect to a center mini-program. For instance, in the top left of \cref{fig:redirection_appsecret}, there are 118 vunerable mini-program being redirected to by \AY{Miniapp A}, which itself does not leak appsecret. Similarly, in \cref{fig:redirection_key}, there are three massive clusters with over 200 mini-programs. This may be mini-programs that are using a same set of mini-program template or third-party cloud service that leaked the appsecret in the template or the session key in their session key network request. As such, the credential leakage may be propagated via copy-paste or mini-program template. In the next section, we will explain more details about the implication of these cases with real world cases.

% \paragraph{mini-programs that redirect to each other} As shown in \cref{fig:redirection_appsecret}, we observed that there are some small clusters where mini-programs redirects to each other. For example, in the middle of \cref{fig:redirection_appsecret}, there is a cluster where 11 vulnerable mini-program redirects to each other. As shown in \cref{tab:appsecret}, this cluster belongs to the 10 mini-programs with 11 referrers that appear very similar in the mini-program name and the Javascript code. Therefore, it is very possible that all the 11 mini-programs are developed by a same vendor, and the vendor is possibly developing many duplicated mini-programs to escape from mini-program auditing and management.


% \AY{EVALUATION DATA}

% Normally, the session key is generated by the back-end with login token returned by \texttt{wx.login}, and this session key is used for decryptions of user sensitive data. Therefore, since the session key cannot be leaked to the front-end, all sensitive encrypted data has to be sent back to the back-end. To investigate the potential leakage, we investigate three problems in this section. Our study shows that there is a concerning amount of mini-programs that are highly possible to either leak the session keys via sensitive network URLs, or process encrypted data with leaked session key because there is no associated network requests found after sensitive encrypted data is being acquired.




% \begin{table*}[]
% \scriptsize
% \belowrulesep=0pt
% \aboverulesep=0pt
% \setlength\tabcolsep{1.5pt}
%     \centering
%     \begin{tabular}{c|c|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
%     \toprule
%      \multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\rot{business}}&\multicolumn{1}{c|}{\rot{education}}&\multicolumn{1}{c|}{\rot{entertainment }}&\multicolumn{1}{c|}{\rot{finance}}&\multicolumn{1}{c|}{\rot{food}}&\multicolumn{1}{c|}{\rot{game}}&\multicolumn{1}{c|}{\rot{government}}&\multicolumn{1}{c|}{\rot{health}}&\multicolumn{1}{c|}{\rot{images}}&\multicolumn{1}{c|}{\rot{job}}&\multicolumn{1}{c|}{\rot{lifestyle}}&\multicolumn{1}{c|}{\rot{reading}}&\multicolumn{1}{c|}{\rot{shopping}}&\multicolumn{1}{c|}{\rot{social}}&\multicolumn{1}{c|}{\rot{sports}}&\multicolumn{1}{c|}{\rot{tool}}&\multicolumn{1}{c|}{\rot{traffic}}&\multicolumn{1}{c|}{\rot{travelling}}\\ \hline
%      \multirow{11}{*}{\rot{back-end}}&\multirow{9}{*}{\tabincell{c}{session\\key}}&\texttt{login}&14,744&48,810&3,622&1,526&34,422&21,140&11,416&9,956&454&6,164&86,823&2,426&132,115&6,486&3,849&33,303&10,124&1,166\\\cline{3-21}
%   &&\texttt{getUserInfo}&11,332&38,231&3,248&1,164&26,322&23,203&8,489&7,307&380&4,972&64,401&1,314&9,5916&5,522&3,180&29,032&7,678&955
% \\\cline{3-21}
%       &&\texttt{getUserProfile}&30&86&30&4&40&8&28&45&2&56&197&5&265&18&6&47&18&1\\\cline{3-21}
%       &&\texttt{getUserInteractiveStorage}&&&&&&\\\cline{3-21}
%      &&\texttt{getWeRunData}&161&280&42&23&120&105&102&81&5&21&226&17&609&62&1040&428&34&6\\\cline{3-21}
%      &&\texttt{getGroupEnterInfo}&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\\\cline{3-21}
%      &&\texttt{getShareInfo}&&&&&&\\\cline{3-21}
%      &&\texttt{chooseInvoice}&4&3&0&0&0&0&3&1&0&0&9&0&3&0&2&16&1&0\\\cline{3-21}
%      &&\texttt{request}&&&&&&\\\cline{2-21}
%      \bottomrule
%     \end{tabular}
%     \caption{Security-related APIs and Values\AY{Will fix that later}}
%     \label{tab:apis}
% \end{table*}

% \begin{table}[]
%     \centering
%     \scriptsize
%     \begin{tabular}{r|c|c}
%     \toprule
%     \# of mini-program a specific mini-program redirects to& \# app & \% app\\
%  >10&50&0.02\\
% 9&25&0.01\\
% 8&31&0.01\\
% 7&29&0.01\\
% 6&262&0.10\\
% 5&599&0.23\\
% 4&613&0.23\\
% 3&2920&1.11\\
% 2&34055&12.89\\
% 1&225612&85.40\\
% total&264196&100.00\\\bottomrule
%     \end{tabular}
%     \caption{Amount of mini-programs each mini-program redirects to\AY{Would like to remove}}
%     \label{tab:redirection}
% \end{table}


% \section{Case Study and Root Causes}
% \subsection{Coffee Attack}
 





==> paper/backup-crawler.tex <==

%\subsection{Crawler} 



%To collect a data set for our analysis, we first need to design and implement a crawler that can automatically download the mini-programs from the \wechat server. 

%Specifically, 
Similar to web crawlers, which contain a keyword-based searching component and an output parsing and indexing component, our mini-program crawler has two such components. In the following, we present how we build these two components. % (\S\ref{subsubsec:search}), and the downloading component (\S\ref{subsubsec:downlaod}). 

%corresponding to two important steps, including a meta data collector to search mini-programs (\eg, ratings and mini-program IDs) based on the fed keywords(\S\ref{subsubsec:search}), and a mini-program downloader to download the packages of mini-programs from \wechat server (\S\ref{subsubsec:downlaod}). 

\subsubsection{\bf{Mini-program Searching}}
\label{subsubsec:search}
%\AY{No such section any more. No searching, just crawling.}\ZY{We still need this. Otherwise, how could you obtain the metadata?}
%Similar to web crawler, we need to first locate the URLs that can allow us query the mini-programs. However, 
Unlike Google Play which provides a web portal (an URL) to easily search Android apps, \Tencent does not provide such a web portal and instead all the mini-programs must be queried inside the \wechat app. Therefore, we have to first locate the URLs if there is any inside the \wechat app. By manually launching the mini-program query interface and intercepts all the networking APIs invoked by \wechat, we successfully locate an \texttt{innersearch} API, as presented in \autoref{tab:inner:apis1}. This API is an in-app interface for \wechat users to query the mini-programs, which takes parameters including the searched keywords, \texttt{timestamp}, \texttt{client\_version}, \texttt{cookie}, and so on, and returns a list of the matched mini-programs with their {\tt appID}, {\tt label}, {\tt rating}, and so forth. However, we only need to take care the keywords, \texttt{timestamp}, and the \texttt{cookie} fields. 
%
%
%
%keywords  user's inputs as the keywords, and returns a list of mini-programs that contained the searched keyword in their names. We reverse engineered the traffic between \wechat server and client, and identified such the inner interface used by \wechat as shown in \autoref{tab:inner:apis1}. By default, we found that other than the user's inputs, the API accepts many inputs such as \texttt{timestamp}, \texttt{client\_version} and so forth. However, we only care about two of them, since others will not have no impacts on the query results. The two inputs are \textit{cookie} and a \texttt{query}. Specifically, \texttt{query} is the keyword that is used to retrieve mini-programs.  
%
Among them, {\tt cookie} is the most tricky field since it is distributed by \wechat servers to associate the users and gets expired every 2 hours. 
%
%Note that\textit{cookie} is the cookie distributed by \wechat server for associating the logged \wechat user, which gets updated every 2 hours. Since the \textit{cookie} can get expired, to obtain the valid results, we have to extract and update the valid \textit{cookie}  dynamically. 
Fortunately, we find that every time when we perform an in-app mini-program query with \wechat, the \wechat server will re-send a fresh \textit{cookie} to the client. Therefore, we write a script to automatically trigger the in-app query, and intercept the  \textit{cookie} sent from server, and then update it every 2 hours. In such a way, we can keep searching the mini-programs with arbitrary keywords without limitation.  \looseness=-1

\subsubsection{\bf{Mini-program Downloading}}
\label{subsubsec:downlaod}

To download the mini-programs from \wechat, a most straightforward way is that we can again reverse engineer the \wechat protocol and locate the downloading interface. However, according to analysis with \wechat app, we found the downloading interface is significantly different from the aforementioned searching interface, which we cannot identify directly through the analysis of network traffic.  Fortunately, by going through all the \wechat mini-program programming APIs, we have identified one interesting mini-program API that can allow mini-program downloading, as shown in the 2nd API in \autoref{tab:inner:apis1}.  To be more specific, this API is named \breakabletexttt{wx.navigateToMiniprogram}, which is used by  specific mini-programs for the purpose of navigating to other mini-programs. It takes a mini-program ID along with a version (release vs. debug) as parameters, and downloads the corresponding mini-program package and open it inside a mini-program.  We therefore developed a special mini-program using the \breakabletexttt{wx.navigateToMiniprogram}, and use it to continuously download the mini-programs of our interests by feeding the mini-program IDs, perfectly serving our mini-program downloading needs.  Moreover, by using the mini-program IDs, we can also collect the developer information and the update date of the mini-program, as shown in the 5th API in \autoref{tab:inner:apis1}.\looseness=-1 %different appIDs to download all the mini-programs of interest.  


%when a mini-program passes the appID to the API, and then invokes the API, \wechat will download and launch the corresponding mini-program. We therefore created a mini-program that can fetch the mini-program IDs automatically from our database,  and the invoke the \texttt{wx.navigateTomini-program} continuously to download all the corresponding mini-programs.  Eventually, we have collected \totalapps mini-programs based on all our 493 collected keywords for analysis.    


 
 


\begin{table}[]
\scriptsize
 \belowrulesep=0pt
 \aboverulesep=0pt
 \setlength\tabcolsep{3pt}
\begin{tabular}{llcc}\toprule
 {\textbf{API}} &  {\textbf{Description}}    \\
 \midrule


\textbf{{{Mp.wx.qq.com/wxa-cgi/innersearch}}}    &   mini-program Searching API      \\
   \textbf{Parameters}   &       \\  
\SFviii   \texttt{query}    &   A keyword to search the mini-programs         \\  
%\SFviii Language & \texttt{obj.lang} & \tickNo    &  \tickYes     \\
\SFviii \texttt{client\_version}       &   The \wechat client version    \\ 
\SFviii \texttt{time}       & The timestamp of this query     \\ 
\SFviii  \texttt{cookie} &  \wechat client token     \\
\SFii~ ... & Other omitted parameters\\
\textbf{Return value} &  %The  mini-program metadata  
\\
\SFviii  \texttt{appID}     & The app ID of the mini-program       \\
\SFviii   \texttt{label}     & The category of the mini-program    \\
\SFviii  \texttt{rating}   &  The user rating of the mini-program    \\
\SFii~... & Other omitted fields in the return value\\
%\SFii Profile & A\_A1\_A\_A & a\_a1\_a   &      \\
%~~~\SFii Nick name   & A\_A1\_A\_B & a\_a1\_b   &      \\
  \midrule

\textbf{Wx.nativgateTomini-program()}        &    mini-program Downloading API    \\  
   \textbf{Parameters}   &       \\  
\SFviii\texttt{appID}        &  The app ID of the mini-program          \\  
\SFii\texttt{version}    &  The version (released or debug)       \\ 
\textbf{Return value}    &  The packed file of the mini-program     \\  \midrule

 \textbf{Api.weixin.qq.com/cgi-bin/token}     & A \appsecret Validation API    \\
    \textbf{Parameters}   &       \\  
\SFviii  \texttt{appID}      &   The app ID of the mini-program     \\
\SFviii \texttt{secret}    &  A \appsecret      \\
\SFii\texttt{grant\_type}   &  The access type  \\
\textbf{Return value}    &   An access token or error message   \\

\midrule

 \textbf{Api.weixin.qq.com/sns/jscode2session}      & \appsecret Validation API (\texttt{getEK()})    \\
    \textbf{Parameters}   &       \\  
\SFviii  \texttt{appID}      &   The app ID of the mini-program     \\
\SFviii \texttt{secret}    &  The Master key (\appsecret)      \\
\SFii\texttt{jscode}   &   A login token (\token) \\
\textbf{Return value}    &  The encryption key (\sessionkey)  \\
 
\midrule

 \textbf{Mp.weixin.qq.com/mp/waverifyinfo}      & Developer Information Downloading API   \\
    \textbf{Parameters}   &       \\  
\SFviii  \texttt{appID}      &   The app ID of the mini-program     \\
\SFviii \texttt{deviceType}    &  The device type of mobile (e.g., Android)     \\
\SFii\texttt{netType}   &  Network Connection Information (e.g., WiFi) \\
\textbf{Return value}    &     \\  
\SFviii  \texttt{developerinfo}     & The developer information of the mini-program       \\
\SFii\texttt{updatedate} & The relase date of the mini-program\\
     
           
\bottomrule
\end{tabular} 
\caption{Summary of Five Important APIs Used by Our Tool.}
\label{tab:inner:apis1}
\end{table}




==> table/address.tex <==

\begin{table}[t]
\centering
\scalebox{0.73}{
\begin{tabular}{l  l  l  c }
\toprule
\multicolumn{1}{l}{\textbf{Firmware Name}}   &    \multicolumn{1}{l}{\bf Mobile App}  & \multicolumn{1}{l}{\textbf{Category}} 	& \multicolumn{1}{r}{\textbf{\# Device}} \\
\toprule
\textsf{cogobeacon}              & com.aegismobility.guardian    & Car Accessory            & 4     \\
\textsf{sd\_bl}                & fr.solem.solemwf      & Agricultural Equip.   & 2     \\
\textsf{LRFL\_nRF52}             & fr.solem.solemwf      & Agricultural Equip.   & 2    \\
\textsf{orb}                     & one.shade.app         & Smart Light              & 1      \\
\textsf{sd\_bl}                  & com.rainbird          & Agricultural Equip.   & 1     \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Firmware using private MAC address.}
\vspace{-0.3in}
\label{tab:mac}
\end{table}


\ignore{
\begin{table}
\centering
\scalebox{0.75}{
\begin{tabular}{l  l  c  l}
\toprule
\multicolumn{1}{l}{\textbf{Name}}   & \multicolumn{1}{l}{\textbf{Category}} 	& \multicolumn{1}{r}{\textbf{\# Firmware}}  & \multicolumn{1}{l}{\textbf{Addr. Type}}  \\
\toprule
cogobeacon              & Car Accessory            & 4      & Private \\
sd\_bl                  & Agricultural Equipment   & 2      & Private \\
LRFL\_nRF52             & Agricultural Equipment   & 2      & Private \\
orb                     & Smart Light              & 1      & Private \\
sd\_bl                  & Agricultural Equipment   & 1      & Private \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Firmware using private MAC address.}
\vspace{-0.2in}
\label{tab:mac}
\end{table}
}

==> table/api.tex <==
% category - policy


\begin{table}[t]
\scriptsize
\centering
\scalebox{0.93}{
\begin{tabular}{c  l  c  l}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Policy}}} 	& \multicolumn{1}{l}{\multirow{2}{*}{\textbf{SDK Function Name}}}     & \multicolumn{1}{c}{\textbf{Reg.}}  & \multirow{2}{*}{\textbf{Description}}\\
\multicolumn{1}{c}{}                                    & \multicolumn{1}{l}{}       & \multicolumn{1}{c}{\textbf{Index}}  & \multicolumn{1}{l}{}\\ 
\toprule
                            % & \texttt{SD\_BLE\_GAP\_DEVICE\_NAME\_SET}  & 1     & Set device name \\
                            & \texttt{SD\_BLE\_GAP\_ADDR\_SET}            & 0   & Configure the MAC address \\
                            % & \texttt{SD\_BLE\_PRIVACY\_SET}            & 0 \\
                            % & \texttt{SD\_BLE\_GAP\_WHITELIST\_SET}      & 1 \\
                            & \texttt{SD\_BLE\_GAP\_APPEARANCE\_SET}     & 0  & Set device description \\
                           % & \texttt{SD\_BLE\_GAP\_DEVICE\_IDENTITIES\_SET}  & 0, 1 \\
\multirow{3}{*}{\textbf{(i)}}                            & \texttt{SD\_BLE\_GATTS\_SERVICE\_ADD}      & 0, 1  & Add a BLE GATT service\\
                            & \texttt{SD\_BLE\_GATTS\_CHARACTERISTIC\_ADD}   & 2    & Add a BLE GATT characteristic \\
                            & \texttt{SD\_BLE\_UUID\_VS\_ADD}            & 0     & Specify the UUID base \\
                            & \texttt{GAP\_ConfigDeviceAddr}*                & 0     & Setup the address type \\
                            & \texttt{GATTServApp\_RegisterService}*         & 0     & Register BLE GATT service \\
\midrule
\multirow{5}{*}{\textbf{(ii)}}    & \texttt{SD\_BLE\_GAP\_SEC\_PARAMS\_REPLY}   & 2  & Reply peripheral pairing features  \\
                             & \texttt{SD\_BLE\_GAP\_AUTH}               & 1    & Reply central pairing features \\
                        %    & \texttt{SD\_BLE\_OPT\_SET}                & 1 \\
                            & \texttt{SD\_BLE\_GAP\_AUTH\_KEY\_REPLY}     & 1, 2 & Reply with an authentication key \\
                            %& \texttt{SD\_BLE\_GAP\_LESC\_OOB\_DATA\_SET}  & 2 \\
                            %& \texttt{SD\_BLE\_GAP\_KEYPRESS\_NOTIFY}    & 1 \\
                            & \texttt{SD\_BLE\_GATTS\_CHARACTERISTIC\_ADD}   & 2    & Add a BLE GATT characteristic \\
                            & \texttt{GAPBondMgr\_SetParameter}*             & 2     & Setup pairing parameters \\
                            & \texttt{GATTServApp\_RegisterService}*         & 0     & Register BLE GATT service \\
\midrule
\multirow{2}{*}{\textbf{(iii)}} & \texttt{SD\_BLE\_GAP\_LESC\_DHKEY\_REPLY}  & 0  & Reply with a DH key \\
                            & \texttt{GAPBondMgr\_SetParameter}*             & 2     & Setup pairing parameters \\
                            % & \texttt{SD\_BLE\_GAP\_ENCRYPT}            & 2 \\
                            
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Targeted SDK functions in our detection policies (Note: functions w/ * are for TI, and otherwise for Nordic).}
\vspace{-0.4in}
\label{tab:api}
\end{table}



\ignore{
\begin{table*}
\scriptsize
\centering
\scalebox{1.1}{
\begin{tabular}{c | l | l | l | l}
\toprule
\textbf{Policy} 	& \textbf{API Name}     & \textbf{SVC \#}    & \textbf{Reg. Index}  & \textbf{Description}\\
\midrule
\multirow{6}{*}{\textbf{Trackable Vulnerability Detection}}  & \texttt{SD\_BLE\_GAP\_DEVICE\_NAME\_SET}    & \texttt{0x7C}  & 1   & Setting the name of the device \\
                            & \texttt{SD\_BLE\_GAP\_ADDR\_SET}           & \texttt{0x6C}   & 0    & Configuring the broadcast MAC address \\
                            % & \texttt{SD\_BLE\_PRIVACY\_SET}            & 0 \\
                            % & \texttt{SD\_BLE\_GAP\_WHITELIST\_SET}      & 1 \\
                            & \texttt{SD\_BLE\_GAP\_APPEARANCE\_SET}     & \texttt{0x78}    & 0    & Setting device description \\
                            % & \texttt{SD\_BLE\_GAP\_DEVICE\_IDENTITIES\_SET}  & 0, 1 \\
                            & \texttt{SD\_BLE\_GATTS\_SERVICE\_ADD}      & \texttt{0xA0}    & 0, 1 & Adding a BLE GATT service \\
                            & \texttt{SD\_BLE\_GATTS\_CHARACTERISTIC\_ADD}   & \texttt{0xA2}    & 2    & Adding a BLE GATT characteristic \\
                            & \texttt{SD\_BLE\_UUID\_VS\_ADD}            & \texttt{0x63}    & 0    & Specifying the UUID base \\
\midrule
\multirow{3}{*}{\textbf{MITM Vulnerability Detection}}    & \texttt{SD\_BLE\_GAP\_SEC\_PARAMS\_REPLY}   & \texttt{0x7F}    & 2  & Exchanging pairing features as a peripheral \\
                            & \texttt{SD\_BLE\_GAP\_AUTH}               & \texttt{0x7E}    & 1     & Exchanging pairing features as a central \\
                        %    & \texttt{SD\_BLE\_OPT\_SET}                & 1 \\
                            & \texttt{SD\_BLE\_GAP\_AUTH\_KEY\_REPLY}     & \texttt{0x80}    & 1, 2 & Replying the peer device with authentication key \\
                            %& \texttt{SD\_BLE\_GAP\_LESC\_OOB\_DATA\_SET}  & 2 \\
                            %& \texttt{SD\_BLE\_GAP\_KEYPRESS\_NOTIFY}    & 1 \\
\midrule
\multirow{1}{*}{\textbf{Evasdroppable Vulnerability Detection}} & \texttt{SD\_BLE\_GAP\_LESC\_DHKEY\_REPLY}  & \texttt{0x81}     & 0 & Replying the peer device with a DH key in LESC pairing \\
                            % & \texttt{SD\_BLE\_GAP\_ENCRYPT}            & 2 \\
                            
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Target SDK functions in our implementation (Half column).}
\vspace{-0.2in}
\label{tab:api}
\end{table*}
}

==> table/attack-tbl.tex <==
\begin{table}[t]
 \setlength\tabcolsep{5pt}
\footnotesize
 {
\begin{tabular}{|lc|rr|}
\hline
\multicolumn{2}{|c|}{ \textbf{\diagbox{Keys}{Attacks}{Data}}}         %   & \multicolumn{2}{c|}{\textbf{Mini-app's Back-end}}                                         \\
%\multicolumn{2}{|c|}{}                                                     
& \textbf{\begin{tabular}[c]{@{}c@{}}Predictable  Data \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Non-Predictable   Data\end{tabular}} \\
 

\hline


{\textbf{w/ \appsecret}}             &  {\textbf{w/ {\sessionkey}}}         &  Account Hijacking  (\tickcoloredYes)      &   Data Manipulation  (\tickcoloredYes)                         \\\hline

          %        & w/ {\token}         &        {N/A}           & {N/A}  &                           \\
                                                    
  \multirow{2}{*}{\textbf{w/o \appsecret}}       &  {w/o \sessionkey} &  Replay  (\tickcoloredNo)       &  Replay  (\tickcoloredNo)                              \\ 
                        &  {w/ \sessionkey}    &   Account Hijacking  (\tickcoloredYes)   &               Data Manipulation  (\tickcoloredYes)                        \\
                                                      \hline

\end{tabular}}
\caption{Summary of possible Attacks. ``\tickcoloredYes'' means the corresponding attack works, while ``\tickcoloredNo'' means does not.  }
\label{tab:attackspossible}
\end{table}





\ignore{
\begin{table}[t]
 \setlength\tabcolsep{1pt}
\footnotesize
 {
\begin{tabular}{lc|rr|c}
\hline
\multicolumn{2}{c|}{ \textbf{\diagbox{Keys}{Attacks}{Parties}}}            & \multicolumn{2}{c|}{\textbf{Mini-app's Back-end}}                                       & \textbf{\wechat Server}                     \\
\multicolumn{2}{c|}{}                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}Predictable  \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Non-Predictable  \end{tabular}} \\
\multicolumn{2}{c|}{}                                                     & \textbf{\begin{tabular}[c]{@{}c@{}} Data\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Data\end{tabular}} \\

\hline


\multicolumn{1}{c}{\multirow{2}{*}{\textbf{w/ \appsecret}}}                                  & w/ {\token}         &    {N/A}             & {N/A}  &  Cross-user Access  (\tickcoloredNo)                              \\ 
\multicolumn{1}{c}{} & w/ {\sessionkey}         &  Account Hijack  (\tickcoloredYes)                            &   Data Manipulation  (\tickcoloredYes)                   & N/A          \\\cline{1-5} 

\multirow{3}{*}{\textbf{w/o \appsecret}}                  & w/ {\token}         &        {N/A}           & {N/A}  &  Cross-user Access (\tickcoloredNo)                              \\
                                                    
                                                      &  {w/o \sessionkey} &  Replay  (\tickcoloredNo)                              &  Replay  (\tickcoloredNo)                      & N/A            \\ 
                                                      
                                                        &  {w/ \sessionkey}    &   Account Hijack  (\tickcoloredYes)                            &  Data Manipulation  (\tickcoloredYes) & N/A                            \\
                                                      \hline

\end{tabular}}
\caption{Summary of possible Attacks. ``\tickcoloredYes'' means the attack can work against the party, while ``\tickcoloredNo'' means not.  }
\label{tab:attackspossible}
\end{table}
}

==> table/baseaddress.tex <==

\begin{table}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{l  c  c }
\toprule
\multicolumn{1}{l}{\bf Pointer Type}  & \multicolumn{1}{r}{\bf \# True Positive (\%)}    & \multicolumn{1}{r}{\bf \# False Positive (\%)}   \\
\toprule
Absolute Function Pointer    & $40$ ($95.2\%$)                      & $2$ ($4.8\%$)                       \\
Absolute String Pointer      & $14$ ($33.3\%$)                      & $28$ ($66.7\%$)                      \\
Vector Table Entry  & $40$ ($95.2\%$)                      & $2$ ($4.8\%$)                        \\
\midrule
Three Sets Combined        & $42$ ($100\%$)                      & $0$ ($0$)                      \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Base address recognition w/ one set of pointers.}
\vspace{-0.2in}
\label{tab:baseadd}
\end{table}

==> table/device.tex <==


\begin{table}
\centering
\scalebox{0.73}{
\begin{tabular}{l  l  c  c  c  c  c  c}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\bf Device Name}}  & \multicolumn{1}{l}{\multirow{2}{*}{\bf Category}}  & \multicolumn{3}{c}{\multirow{1}{*}{\bf Vulnerabilities}}   & \multicolumn{3}{c}{\multirow{1}{*}{\bf Attacks}}  \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
        &   & {\bf IT}    & {\bf AM}    & {\bf PM}   & {\bf A1}    & {\bf A2}    & {\bf A3} \\
\toprule
Nuband Activ+               & Wearable      & \checkmark    & \checkmark    & \checkmark  & \checkmark    &               & \checkmark \\
Kinsa Smart                 & Thermometer   & \checkmark    & \checkmark    & \checkmark  &               &               & \checkmark\\
Chipolo ONE                 & Tag           & \checkmark    & \checkmark    & \checkmark  & \checkmark    &               &       \\
SwitchBot Button Pusher     & Smart Home    & \checkmark    & \checkmark    & \checkmark  &               & \checkmark    &       \\
XOSS Cycling Computer       & Sensor   & \checkmark    & \checkmark    & \checkmark  & \checkmark    &               & \checkmark \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Vulnerable BLE devices and attack case studies.}
\vspace{-0.3in}
\label{tab:device}
\end{table}



==> table/ecdh.tex <==

\begin{table}
\centering
\scalebox{0.72}{
\begin{tabular}{l  l  l  c}
\toprule
\multicolumn{1}{l}{\textbf{Firmware Name}}   & {\bf Mobile App}    & \multicolumn{1}{l}{\textbf{Category}} 	& \multicolumn{1}{r}{\textbf{\# Version}} \\
\toprule
\textsf{DogBodyBoard}    & com.wowwee.chip  & Robot     & 16    \\
\textsf{BW\_Pro}         & com.ecomm.smart\_panel    & Tag       & 1     \\ 
\textsf{Smart\_Handle}   & com.exitec.smartlock     & Smart Lock    & 1 \\
\textsf{Sma05}           & com.smalife.watch    & Wearable  & 1     \\
\textsf{CPRmeter}        & com.laerdal.cprmeter2    & Medical Device    & 4 \\
\textsf{WiJumpLE}        & com.wesssrl.wijumple & Sensor    & 1  \\
\textsf{nRF Beacon}      & no.nordicsemi.android.nrfbeacon  & Beacon    & 1 \\
\textsf{Hoot Bank}       & com.qvivr.hoot   & Debit Card      & 1\\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Firmware that enforce LESC pairing.}
\vspace{-0.3in}
\label{tab:lesc}
\end{table}



\ignore{
\begin{table}
\centering
\scalebox{0.75}{
\begin{tabular}{l  l  c  l}
\toprule
\multicolumn{1}{l}{\textbf{Name}}   & \multicolumn{1}{l}{\textbf{Category}} 	& \multicolumn{1}{r}{\textbf{\# Firmware}}  & \multicolumn{1}{l}{\textbf{Pairing Method}}     \\
\toprule
\textsf{DogBodyBoard}    & Robot     & 16    & Just Works\\
\textsf{BW\_Pro}         & Tag       & 1     & Just Works \\ 
\textsf{Smart\_Handle}   & Smart Lock    & 1 & Just Works\\
\textsf{Sma05}           & Wearable  & 1     & Just Works\\
\textsf{CPRmeter}        & Medical Device    & 4 & Just Works\\
\textsf{WiJumpLE}        & Sensor    & 1 & Just Works \\
\textsf{nRF Beacon}      & Beacon    & 1 & Just Works\\
\textsf{Hoot Bank}       & Smart Debit Card      & 1 & Passkey Entry\\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Firmware that enforce LESC pairing.}
\vspace{-0.3in}
\label{tab:lesc}
\end{table}
}

==> table/highprofileapps.tex <==

\begin{table}[t]
  \centering
    \scriptsize
    \setlength\tabcolsep{2pt}
    \aboverulesep=0pt
    \belowrulesep=0pt
\begin{tabular}{@{}llllr@{}}
\toprule[1.5pt]
\textbf{Company}          & \textbf{The mini-program Name}      & \textbf{Category} & \textbf{Data}                    & \textbf{Attacks} \\ \midrule
\multirow{17}{*}{Tencent}      & AI Illustrator YUI                  & games             & \ding{192}                       & A1               \\
                              & Longzu Illusion Game                & tool              & \ding{192}                       & A1               \\
                              & Pipixia Videos                      & entertainment     & \ding{192},\ding{193}            & A1, A2           \\
                              & Hispital Copay Platform             & health            &                                  &                  \\
                              & Tencent Billiard                    & entertainment     & \ding{192}                       & A1               \\
                              & Moment Gallery                      & tool              & \ding{192}                       & A1               \\
                              & Health Data Assistant               & education         &                                  &                  \\
                              & Personality Test                    & games             & \ding{192}                       & A1               \\
                              & Everyday Cool Run                   & social            & \ding{192}                       & A1               \\
                              & Financial Regulation Platform       & tool              & \ding{192}                       & A1               \\
                              & Campus Cloud Card                   & tool              &                                  &                  \\
                              & Intelligent Welcoming Assistant     & e-learning        & \ding{194}                       & A2               \\
                              & Click to earn                       & health            & \ding{192}                       & A1               \\
                              & Video Marking                       & games             & \ding{192}                       & A1               \\
                              & Tencent Everyday Chess              & games             & \ding{192}                       & A1               \\
                              & Wepaytest                           & education         &                                  &       A3           \\
                              & Tuyan                               & games             & \ding{193}                       & A2               \\ \midrule
\multirow{6}{*}{Nestle}        & NESCAFE space                       & food              & \ding{194},\ding{192}            & A1, A2           \\
                              & Nestle Coffee Membership            & tool              & \ding{194},\ding{192}            & A1, A2           \\
                              & Yiyang Member Center                & lifestyle         & \ding{194},\ding{192}            & A1, A2           \\
                              & Nestle Customer Service             & food              & \ding{194}                       & A2               \\
                              & DolceGusto Member Center            & shopping          & \ding{194},\ding{192}            & A1, A2           \\
                              & We Proudly Serve                    & shopping          & \ding{194},\ding{192}            & A1, A2           \\ \midrule
\multirow{4}{*}{Sanofi}        & Nutrition Nursing UAT               & health            & \ding{194},\ding{192}            & A1, A2           \\
                              & Nutrition Nurses                    & business          & \ding{194},\ding{192}            & A1, A2           \\
                              & Nutrition Nursing                   & business          & \ding{194},\ding{192}            & A1, A2           \\
                              & Nutrition NursesUAT                 & business          & \ding{194},\ding{192}            & A1, A2           \\ \midrule
\multirow{4}{*}{China Unicom}  & Failure report and Complaint        & finance           & \ding{194}                       & A2               \\
                              & Unicom Club                         & finance           & \ding{194},\ding{192}            & A1, A2           \\
                              & Henan 114 Move Car                  & tool              &                                  &                  \\
                              & Fengxingdong Cloud Shop             & shopping          & \ding{194}                       & A2               \\ \midrule
\multirow{3}{*}{Bank Of China} & BOC Virtual Bank                    & shopping          & \ding{192}                       & A1               \\
                              & Data Center Meetings                & shopping          & \ding{192}                       & A1               \\
                              & BOC Technical Summit                & business          & \ding{192}                       & A1               \\\midrule
\multirow{3}{*}{Hitachi}       & Hi Design Platform                  & tool              & \ding{192}                       & A1               \\
                              & York Design                         & tool              & \ding{192}                       & A1               \\
                              & AI sense                            & business          & \ding{192}                       & A1               \\\midrule
\multirow{2}{*}{Shou Gang}     & Cloud Security Community            & tool              &                                  &        A3          \\
                              & Information Collection System & lifestyle         &                                  &                  \\
\multirow{2}{*}{China Mobile}  & Mobile Cloud Calculator             & finance           &                                  &                  \\
                              & Home Internet Assistant             & finance           &                                  &                  \\ \midrule
\multirow{2}{*}{ICBC}          & ICBC Intelligent Messaging          & lifestyle         & \ding{194}                       & A2               \\
                              & Pinyue Benefit Center               & traffic           & \ding{192},\ding{193},\ding{195} &                  \\ \midrule
\multirow{2}{*}{Volkswagen}    & Audi Sales Consultant               & shopping          & \ding{192}                       & A1               \\
                              & Audi Online 4S Shop                 & shopping          & \ding{192},\ding{193}            &                  \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The top-10 Fortune 500 companies that have the most number of mini-programs leaked the \appsecret. \ding{192} user info; \ding{193} shared info; \ding{194} phone number; \ding{195} werun data. 
%A1: Account hijack attacks; A2: promotion abuse attacks.  A3: Service theft attack.
    }
    \label{tab:appsecret}
    \vspace{-0.1in}  
\end{table}

==> table/name.tex <==
\begin{table}
\centering
\scalebox{0.8}{
\begin{tabular}{l | l | c }
\toprule
\textbf{Device Name}   & \textbf{Category} 	& \textbf{\# Firmware}  \\
\midrule
beacon              & Switch     & 6    \\
laerdal\_dfu\_target  & Medical Device    & 6 \\
S3BDX-000000        & Firearm Accessory & 5 \\
Brac                & Wearable          & 4 \\
DfuTarg             & Mouse, Headphone, Switch  & 4 \\
Nordic\_HRM         & Wearable, Robot, Medical Device   & 4 \\
Clouclip P2         & Eyeglasses, Wearable, Medical Device  & 4 \\
ShockLink           & Medical Device    & 3 \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Top 5 most popular device names in firmware and their categories.}
\vspace{-0.2in}
\label{tab:name}
\end{table}




==> table/notation.tex <==

\begin{table}
\centering
\scalebox{0.85}{
\begin{tabular}{l | l }
\toprule
\textbf{Notation}   & \textbf{Description} \\
\midrule
$X$       & The optimal base address \\
$P_A$     & Set of absolute pointers in the firmware \\
$P_F$     & Set of absolute function pointers in the firmware \\
$P_S$     & Set of absolute string pointers in the firmware \\
$P_V$     & Set of vector table entries in the firmware \\
$E$       & Set of function entries in the firmware \\
$S$       & Set of constant strings in the firmware \\
$V$       & Set of interrupt numbers in the firmware \\ 
$C$       & Set of all unique candidate base addresses \\
% $C_{1}$ & Set of candidates produced by function pointer constraint \\
% $C_{2}$ & Set of candidates produced by string pointer constraint \\
% $C_{3}$ & Set of candidates produced by vector table entry constraint \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Mathematical notations in constraint formulation.}
\vspace{-0.2in}
\label{tab:notation}
\end{table}

==> table/pair.tex <==

% Use device instead of firmware
\begin{table}
% \scriptsize
\centering
\scalebox{0.73}{
\begin{tabular}{l  l  l | r  r | r  r}
\toprule
% \multicolumn{3}{ l}{\multirow{2}{*}{\bf Item}} 	& \multicolumn{4}{c}{\multirow{1}{*}{\bf Value}} \\
\cmidrule(lr){4-7}
\multicolumn{3}{ l}{\bf Item} & \multicolumn{1}{c}{\bf N} & \multicolumn{1}{c}{\bf T} & \multicolumn{1}{c}{\bf Total} & \multicolumn{1}{c}{\bf \%} \\
\toprule
% \multicolumn{3}{ l}{ \# Apps W/ Bluetooth APIs.}				& 135,486 &  \\
\multicolumn{3}{ l}{\bf \# Total Device}		& $513$     & $25$	& \devicenum  & $100$  \\
& \multicolumn{2}{ l}{\bf Pairing Mode}	        &  &  &  &  \\
& & \multicolumn{1}{ l}{\# Peripheral only}	    & $230$     & $25$    &  $255$  & $47.4$  \\
& & \multicolumn{1}{ l}{\# Central only}	    & $6$       & $0$     &  $6$  & $1.1$  \\
& & \multicolumn{1}{ l}{\# Peripheral and central}	 & $186$     & $0$       &  $186$    & $34.5$  \\
& & \multicolumn{1}{ l}{\# No pairing}	        & $91$     & $0$   &  $91$    & $16.9$  \\
\midrule
& \multicolumn{2}{ l}{\bf \# Device w/ bonding}	       & $250$ &    $13$    &  $263$  & $48.9$  \\
\midrule 

& \multicolumn{2}{ l}{\bf \# Device w/ active MITM vulnerability}	  & $384$   & $1$      & $385$  &$71.5$  \\
& & \multicolumn{1}{ l}{ \# Device w/ \JS pairing only}	                & $317$     & $1$   &  $318$  &  $59.1$ \\
& & \multicolumn{1}{ l}{ \# Device w/ flawed \PE implementation}	        & $37$      & $0$   &  $37$  &  $6.9$  \\
& & \multicolumn{1}{ l}{ \# Device w/ flawed \OOB implementation}	        & $30$      & $0$   &  $30$  &  $5.6$  \\
\midrule

& \multicolumn{2}{ l}{\bf \# Device w/ secure pairing}	        & $6$  & $24$   &  $30$  &  $3.8$ \\
& & \multicolumn{1}{ l}{ \# Device w/ correct \PE implementation}	  & $3$     & $24$      &  $27$  &  $3.4$ \\
& & \multicolumn{1}{ l}{ \# Device w/ correct \OOB implementation}    &$3$    & $0$	  &  $3$  &  $0.4$  \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Pairing configurations of devices (N:Nordic, T:TI).}
\vspace{-0.3in}
\label{tab:pair}
\end{table}





\ignore{
\begin{table}
% \scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}{l  l  l | r  r | r  r}
\toprule
\multicolumn{3}{ l}{\multirow{2}{*}{\bf Item}} 	& \multicolumn{4}{c}{\multirow{1}{*}{\bf Value}} \\
\cmidrule(lr){4-7}
  & & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\bf N} & \multicolumn{1}{c}{\bf T} & \multicolumn{1}{c}{\bf Total} & \multicolumn{1}{c}{\bf \%} \\
\toprule
% \multicolumn{3}{ l}{ \# Apps W/ Bluetooth APIs.}				& 135,486 &  \\
\multicolumn{3}{ l}{\bf \# Total Firmware}		& $768$     & $25$	& \firmwarenum  & $100$  \\
& \multicolumn{2}{ l}{\bf Pairing Mode}	        &  &  &  &  \\
& & \multicolumn{1}{ l}{\# Peripheral only}	    & $288$     & $25$    &  $313$  & $39.5$  \\
& & \multicolumn{1}{ l}{\# Central only}	    & $8$       & $0$     &  $8$  & $1.0$  \\
& & \multicolumn{1}{ l}{\# Peripheral and central}	 & $353$     & $0$       &  $353$    & $44.5$  \\
& & \multicolumn{1}{ l}{\# No pairing}	        & $119$     & $0$   &  $119$    & $15.0$  \\
\midrule
& \multicolumn{2}{ l}{\bf \# Firmware w/ bonding}	       & $342$ &    $13$    &  $355$  & $44.8$  \\
\midrule 

& \multicolumn{2}{ l}{\bf \# Firmware vulnerable to active MITM attacks}	  & $595$   & $1$      & $596$  &$75.2$  \\
& & \multicolumn{1}{ l}{ \# Firmware w/ \JS pairing only}	                & $440$     & $1$   &  $441$  &  $55.6$ \\
& & \multicolumn{1}{ l}{ \# Firmware w/ flawed \PE implementation}	        & $86$      & $0$   &  $86$  &  $10.8$  \\
& & \multicolumn{1}{ l}{ \# Firmware w/ flawed \OOB implementation}	        & $69$      & $0$   &  $69$  &  $8.7$  \\
\midrule

& \multicolumn{2}{ l}{\bf \# Firmware w/ secure pairing}	        & $6$  & $24$   &  $30$  &  $3.8$ \\
& & \multicolumn{1}{ l}{ \# Firmware w/ correct \PE implementation}	  & $3$     & $24$      &  $27$  &  $3.4$ \\
& & \multicolumn{1}{ l}{ \# Firmware w/ correct \OOB implementation}    &$3$    & $0$	  &  $3$  &  $0.4$  \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Pairing configurations of firmware (N:Nordic, T:TI).}
\vspace{-0.3in}
\label{tab:pair}
\end{table}
}



\ignore{
% Nordic + TI
\begin{table}
% \scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}{l  l  l | r  r }
\toprule
\multicolumn{3}{ l}{\bf Item} 	& \multicolumn{1}{ r}{\bf Value} &  {\bf \%}\\
\toprule
% \multicolumn{3}{ l}{ \# Apps W/ Bluetooth APIs.}				& 135,486 &  \\
\multicolumn{3}{ l}{\bf \# Total Firmware}				            & \firmwarenum  & $100$  \\
& \multicolumn{2}{ l}{\bf Pairing Mode}	        &  &  \\
& & \multicolumn{1}{ l}{\# Peripheral only}	        &  $313$  & $39.5$  \\
& & \multicolumn{1}{ l}{\# Central only}	        &  $8$  & $1.0$  \\
& & \multicolumn{1}{ l}{\# Peripheral and central}	        &  $353$    & $44.5$  \\
& & \multicolumn{1}{ l}{\# No pairing}	        &  $119$    & $15.0$  \\
\midrule
& \multicolumn{2}{ l}{\bf \# Firmware with bonding}	        &  $355$  & $44.8$  \\
\midrule 

& \multicolumn{2}{ l}{\bf \# Firmware vulnerable to active MITM attacks}	        & $596$  &$75.2$  \\
& & \multicolumn{1}{ l}{ \# Firmware with \JS pairing only}	        &  $441$  &  $55.6$ \\
& & \multicolumn{1}{ l}{ \# Firmware with flawed \PE implementation}	        &  $86$  &  $10.8$  \\
& & \multicolumn{1}{ l}{ \# Firmware with flawed \OOB implementation}	        &  $69$  &  $8.7$  \\
\midrule

& \multicolumn{2}{ l}{\bf \# Firmware with secure pairing}	        &  $30$  &  $3.8$ \\
& & \multicolumn{1}{ l}{ \# Firmware with correct \PE implementation}	        &  $27$  &  $3.4$ \\
& & \multicolumn{1}{ l}{ \# Firmware with correct \OOB implementation}	                    &  $3$  &  $0.4$  \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Identified pairing configurations of the firmware.}
\vspace{-0.2in}
\label{tab:pair}
\end{table}
}



% Nordic only ver.
\ignore{
\begin{table}
% \scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}{l  l  l | r  r }
\toprule
\multicolumn{3}{ l}{\bf Item} 	& \multicolumn{1}{ r}{\bf Value} &  {\bf \%}\\
\toprule
% \multicolumn{3}{ l}{ \# Apps W/ Bluetooth APIs.}				& 135,486 &  \\
\multicolumn{3}{ l}{\bf \# Total Firmware}				            & \firmwarenum  & $100$  \\
& \multicolumn{2}{ l}{\bf Pairing Mode}	        &  &  \\
& & \multicolumn{1}{ l}{\# Peripheral only}	        &  $288$  & $37.5$  \\
& & \multicolumn{1}{ l}{\# Central only}	        &  $8$  & $1.0$  \\
& & \multicolumn{1}{ l}{\# Peripheral and central}	        &  $353$    & $46.0$  \\
& & \multicolumn{1}{ l}{\# No pairing}	        &  $119$    & $15.5$  \\
\midrule
& \multicolumn{2}{ l}{\bf \# Firmware with bonding}	        &  $342$  & $44.5$  \\
\midrule

& \multicolumn{2}{ l}{\bf \# Firmware vulnerable to active MITM attacks}	        & $595$  &$77.5$  \\
& & \multicolumn{1}{ l}{ \# Firmware with \JS pairing only}	        &  $440$  &  $57.3$ \\
& & \multicolumn{1}{ l}{ \# Firmware with flawed \PE implementation}	        &  $86$  &  $11.2$  \\
& & \multicolumn{1}{ l}{ \# Firmware with flawed \OOB implementation}	        &  $69$  &  $9.0$  \\
\midrule

& \multicolumn{2}{ l}{\bf \# Firmware with secure pairing}	        &  $6$  &  $0.8$ \\
& & \multicolumn{1}{ l}{ \# Firmware with correct \PE implementation}	        &  $3$  &  $0.4$ \\
& & \multicolumn{1}{ l}{ \# Firmware with correct \OOB implementation}	                    &  $3$  &  $0.4$  \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Identified pairing configurations of the firmware.}
\vspace{-0.2in}
\label{tab:pair}
\end{table}
}



\ignore{
\begin{table}
% \scriptsize
\centering
\scalebox{0.74}{
\begin{tabular}{l  r  r  | r  r  | r  r  | r  r  | r  r }
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{\textbf{Item}}} & \multicolumn{10}{c}{\bf Pairing Mode} \\
\cmidrule(lr){2-11}
&  \multicolumn{2}{c}{\bf Peripheral} &  \multicolumn{2}{c}{\bf Central} &  \multicolumn{2}{c}{\bf Peri. | Cent.} &  \multicolumn{2}{c}{\bf No Pairing} &  \multicolumn{2}{c}{\bf Total}  \\
\cmidrule(lr){2-11}
&  {\bf \#} & \multicolumn{1}{r}{\bf \%}   &  {\bf \#} & \multicolumn{1}{r}{\bf \%}  &  {\bf \#} & \multicolumn{1}{r}{\bf \%}   &  {\bf \#} & \multicolumn{1}{r}{\bf \%} &  {\bf \#} & \multicolumn{1}{r}{\bf \%}     \\
\midrule
\multicolumn{1}{ l|}{\bf Total}		& $288$ & $37.5$ & $8$ & $1.0$ & $353$ & $46.0$ & $119$ & $15.5$ & $\mathbf{768}$ & $\mathbf{100}$   \\
\midrule
\midrule

\multicolumn{1}{ l|}{\bf Bonding} & $194$ & $67.4$   & $7$ & $87.5$ & $141$  & $39.9$  & $-$ & $-$  & $\mathbf{342}$ & $\mathbf{44.5}$  \\
\midrule
\midrule

\multicolumn{1}{ l|}{\bf Just Works} & $213$ & $74.0$   & $4$ & $50.0$ & $223$  & $63.2$ & $-$ & $-$ & $\mathbf{440}$ & $\mathbf{57.3}$ \\
\multicolumn{1}{ l|}{\bf Flawed PE} & \multirow{1}{*}{$13$} & \multirow{1}{*}{$4.5$}    & \multirow{1}{*}{$0$} & \multirow{1}{*}{$0$}  & \multirow{1}{*}{$73$}  & \multirow{1}{*}{$25.3$} & \multirow{1}{*}{$-$} & \multirow{1}{*}{$-$} & \multirow{1}{*}{$\mathbf{86}$} & \multirow{1}{*}{$\mathbf{11.2}$} \\
\multicolumn{1}{ l|}{\bf Flawed OOB} & \multirow{1}{*}{$38$} & \multirow{1}{*}{$13.2$}    & \multirow{1}{*}{$3$} & \multirow{1}{*}{$37.5$}  & \multirow{1}{*}{$28$}  & \multirow{1}{*}{$7.9$} & \multirow{1}{*}{$-$} & \multirow{1}{*}{$-$} & \multirow{1}{*}{$\mathbf{69}$} & \multirow{1}{*}{$\mathbf{9.0}$} \\
\midrule
\midrule
% \multicolumn{1}{ l|}{\bf } & & &  & &  &  & & &  & \\
\multicolumn{1}{ l|}{\bf Correct PE} & $0$ & $0$     & $0$ & $0$ & $3$  & $0.8$ & $-$ & $-$ & $\mathbf{3}$ & $\mathbf{0.4}$  \\
\multicolumn{1}{ l|}{\bf Correct OOB} & $0$ & $0$   & $0$ & $0$  & $3$  & $0.8$  & $-$ & $-$  & $\mathbf{3}$ & $\mathbf{0.4}$  \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Identified pairing configurations of the firmware.}
\vspace{-0.2in}
\label{tab:pair}
\end{table}

}



\ignore{
% \begin{table*}
% \centering
% \scalebox{1}{
% \begin{tabular}{l | r | r  r | r  r | r  r | r  r | r  r }
% \toprule
% \textbf{Role}   & \textbf{\# Firmware}   & \textbf{\# Just Works}    & \textbf{\%}    & \textbf{\# Bonding}  & \textbf{\%}  & \textbf{\# Passkey}  & \textbf{\%}   & \textbf{\# OOB}  & \textbf{\%} & \textbf{\# Flawed Config.}  & \textbf{\%} \\
% \midrule
% \textbf{Peripheral}      & $288$     & $213$     & $74.0$\%      & $194$     & $67.4$\%      & $0$     & $0$      & $0$     & $0$   & $51$     & $17.7$\% \\
% \textbf{Central}         & $8$       & $4$       & $50.0$\%      & $7$       & $87.5$\%      & $0$     & $0$      & $0$     & $0$   & $3$     & $37.5$\% \\
% \textbf{Peri. \& Cent.}   & $353$     & $223$     & $63.2$\%      & $141$     & $39.9$\%     & $3$     & $0.8$\%      & $3$\%     & $0.8$\% & $101$     & $28.6$\% \\
% \textbf{No Pairing}      & $121$     &           &               &           &               &         &          &         &   &     &  \\
% \midrule
% \textbf{Total}           & $770$     & $440$     & $57.1$\%      & $342$     & $44.4$\%      & $3$     & $0.4$\%      & $3$     & $0.4$\%   & $155$     & $20.1$\% \\
% \bottomrule
% \end{tabular}
% }
% \caption{Identified pairing configurations.}
% \label{tab:pair}
% \end{table*}


\begin{table*}
% \scriptsize
\centering
\scalebox{0.85}{
\begin{tabular}{l  l  r  r  r | r  r  r | r  r  r | r  r  r | r  r  r }
\toprule
\multicolumn{2}{l}{\multirow{3}{*}{\textbf{Item}}} & \multicolumn{15}{c}{\bf Role of Firmware} \\
\cmidrule(lr){3-17}
& &  \multicolumn{3}{c}{\bf Peripheral} &  \multicolumn{3}{c}{\bf Central} &  \multicolumn{3}{c}{\bf Peri. \& Cent.} &  \multicolumn{3}{c}{\bf No Pairing} &  \multicolumn{3}{c}{\bf Total}  \\
\cmidrule(lr){3-17}
& &  {\bf \#} & {\bf \%} & {}   &  {\bf \#} & {\bf \%} & {}   &  {\bf \#} & {\bf \%} & {}   &  {\bf \#} & {\bf \%} & {} &  {\bf \#} & {\bf \%} & {}     \\

\midrule
\multicolumn{2}{ l|}{\bf Total}		& $288$ & $37.4$\% & \databar{37.4}     & $8$ & $1.0$\% & \databar{1.0}   & $353$ & $45.8$\% & \databar{45.8} & $121$ & $15.7$\% & \databar{15.7} & $\mathbf{770}$ & $\mathbf{100\%}$ & \databar{100.0}   \\
\midrule
\multicolumn{2}{ l|}{\bf Just Works} & $213$ & $74.0$\%  & \databar{74.0}    & $4$ & $50.0$\%\ & \databar{50.0} & $223$  & $63.2$\% & \databar{63.2} & $0$ & $0$ & \databar{0.0} & $\mathbf{440}$ & $\mathbf{57.1}$\% & \databar{57.1} \\
\multicolumn{2}{ l|}{\bf Passkey} & $0$ & $0$  & \databar{0}    & $0$ & $0$ & \databar{0} & $3$  & $0.8$\% & \databar{0.8} & $0$ & $0$ & \databar{0.0} & $\mathbf{3}$ & $\mathbf{0.4\%}$ & \databar{0.4} \\
\multicolumn{2}{ l|}{\bf OOB} & $0$ & $0$  & \databar{0}    & $0$ & $0$ & \databar{0} & $3$  & $0.8$\% & \databar{0.8} & $0$ & $0$ & \databar{0.0} & $\mathbf{3}$ & $\mathbf{0.4\%}$ & \databar{0.4} \\
\multicolumn{2}{ l|}{\bf Bonding} & $194$ & $67.4$\%  & \databar{67.4}    & $7$ & $87.5$\%\ & \databar{87.5} & $141$  & $39.9$\% & \databar{39.9} & $0$ & $0$ & \databar{0.0} & $\mathbf{342}$ & $\mathbf{44.4\%}$ & \databar{44.4} \\
\multicolumn{2}{ l|}{\bf Flawed Config.} & $51$ & $17.7$\%  & \databar{17.7}    & $3$ & $37.5$\% & \databar{37.5} & $101$  & $28.6$\% & \databar{28.6} & $0$ & $0$ & \databar{0.0} & $\mathbf{155}$ & $\mathbf{20.1\%}$ & \databar{20.1} \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Identified pairing configurations of the firmware in our study.}
\vspace{-0.1in}
\label{tab:pair}
\end{table*}

}

==> table/result.tex <==
% \begin{table*}
% \centering
% \scalebox{0.8}{
% \begin{tabular}{l | r  r  r | r  r  r | r  r  r | r  r  r}
% \toprule
% \multirow{3}{*}{\textbf{Category}}   & \multicolumn{12}{c}{\textbf{\# Firmware}}   \\
% \cmidrule(lr){2-13}
% & \multicolumn{3}{c|}{\textbf{Total}} & \multicolumn{3}{c|}{\textbf{Trackable}}    & \multicolumn{3}{c|}{\textbf{MITM Vulnerable}}    & \multicolumn{3}{c}{\textbf{Evasdroppable}} \\
% & \# & \% & & \# & \% & & \# & \% & & \# & \% & \\
% \midrule
% Wearable&	 $205$&	$26.6$\%&	\databar{26.6}&	 $205$&	$100$\%&	\databar{100}&	 $99$&	$48.3$\%&	\databar{48.3}&	 $204$&	$99.5$\%&	\databar{99.5} \\
% Others&	 $76$&	$9.9$\%&	\databar{9.9}&	 $76$&	$100$\%&	\databar{100}&	 $60$&	$78.9$\%&	\databar{78.9}&	 $75$&	$98.7$\%&	\databar{98.7} \\
% Sensor&	 $67$&	$8.7$\%&	\databar{8.7}&	 $67$&	$100$\%&	\databar{100}&	 $45$&	$67.2$\%&	\databar{67.2}&	 $66$&	$98.5$\%&	\databar{98.5} \\
% Tag&	 $58$&	$7.5$\%&	\databar{7.5}&	 $58$&	$100$\%&	\databar{100}&	 $43$&	$74.1$\%&	\databar{74.1}&	 $57$&	$98.3$\%&	\databar{98.3} \\
% Robot&	 $41$&	$5.3$\%&	\databar{5.3}&	 $41$&	$100$\%&	\databar{100}&	 $17$&	$41.5$\%&	\databar{41.5}&	 $25$&	$61.0$\%&	\databar{61.0} \\
% Medical Devices&	 $41$&	$5.3$\%&	\databar{5.3}&	 $41$&	$100$\%&	\databar{100}&	 $15$&	$36.6$\%&	\databar{36.6}&	 $37$&	$90.2$\%&	\databar{90.2} \\
% Bike Accessory&	 $41$&	$5.3$\%&	\databar{5.3}&	 $41$&	$100$\%&	\databar{100}&	 $24$&	$58.5$\%&	\databar{58.5}&	 $41$&	$100$\%&	\databar{100} \\
% Car Accessory&	 $26$&	$3.4$\%&	\databar{3.4}&	 $22$&	$84.6$\%&	\databar{84.6}&	 $14$&	$53.8$\%&	\databar{53.8}&	 $26$&	$100$\%&	\databar{100} \\
% Smart Light&	 $21$&	$2.7$\%&	\databar{2.7}&	 $20$&	$95.2$\%&	\databar{95.2}&	 $15$&	$71.4$\%&	\databar{71.4}&	 $21$&	$100$\%&	\databar{100} \\
% Switch&	 $20$&	$2.6$\%&	\databar{2.6}&	 $20$&	$100$\%&	\databar{100}&	 $7$&	$35.0$\%&	\databar{35.0}&	 $20$&	$100$\%&	\databar{100} \\
% Smart Home&	 $20$&	$2.6$\%&	\databar{2.6}&	 $20$&	$100$\%&	\databar{100}&	 $9$&	$45.0$\%&	\databar{45.0}&	 $20$&	$100$\%&	\databar{100} \\
% Smart Eyeglasses&	 $19$&	$2.5$\%&	\databar{2.5}&	 $19$&	$100$\%&	\databar{100}&	 $7$&	$36.8$\%&	\databar{36.8}&	 $19$&	$100$\%&	\databar{100} \\
% Thermometer&	 $16$&	$2.1$\%&	\databar{2.1}&	 $16$&	$100$\%&	\databar{100}&	 $10$&	$62.5$\%&	\databar{62.5}&	 $16$&	$100$\%&	\databar{100} \\
% Smart Lock&	 $15$&	$1.9$\%&	\databar{1.9}&	 $15$&	$100$\%&	\databar{100}&	 $7$&	$46.7$\%&	\databar{46.7}&	 $14$&	$93.3$\%&	\databar{93.3} \\
% Beacon&	 $13$&	$1.7$\%&	\databar{1.7}&	 $13$&	$100$\%&	\databar{100}&	 $7$&	$53.8$\%&	\databar{53.8}&	 $12$&	$92.3$\%&	\databar{92.3} \\
% Firearm Accessory&	 $11$&	$1.4$\%&	\databar{1.4}&	 $11$&	$100$\%&	\databar{100}&	 $7$&	$63.6$\%&	\databar{63.6}&	 $11$&	$100$\%&	\databar{100} \\
% Agricultural Equipment&	 $10$&	$1.3$\%&	\databar{1.3}&	 $5$&	$50.0$\%&	\databar{50.0}&	 $9$&	$90.0$\%&	\databar{90.0}&	 $10$&	$100$\%&	\databar{100} \\
% Battery&	 $9$&	$1.2$\%&	\databar{1.2}&	 $9$&	$100$\%&	\databar{100}&	 $7$&	$77.8$\%&	\databar{77.8}&	 $9$&	$100$\%&	\databar{100} \\
% Game Accessory&	 $9$&	$1.2$\%&	\databar{1.2}&	 $9$&	$100$\%&	\databar{100}&	 $6$&	$66.7$\%&	\databar{66.7}&	 $9$&	$100$\%&	\databar{100} \\
% Keyboard&	 $7$&	$0.9$\%&	\databar{0.9}&	 $7$&	$100$\%&	\databar{100}&	 $3$&	$42.9$\%&	\databar{42.9}&	 $7$&	$100$\%&	\databar{100} \\
% Mouse&	 $6$&	$0.8$\%&	\databar{0.8}&	 $6$&	$100$\%&	\databar{100}&	 $5$&	$83.3$\%&	\databar{83.3}&	 $6$&	$100$\%&	\databar{100} \\
% Printer&	 $6$&	$0.8$\%&	\databar{0.8}&	 $6$&	$100$\%&	\databar{100}&	 $6$&	$100$\%&	\databar{100}&	 $6$&	$100$\%&	\databar{100} \\
% Surf Board&	 $6$&	$0.8$\%&	\databar{0.8}&	 $6$&	$100$\%&	\databar{100}&	 $2$&	$33.3$\%&	\databar{33.3}&	 $6$&	$100$\%&	\databar{100} \\
% Sports Accessory&	 $4$&	$0.5$\%&	\databar{0.5}&	 $4$&	$100$\%&	\databar{100}&	 $3$&	$75.0$\%&	\databar{75.0}&	 $4$&	$100$\%&	\databar{100} \\
% Smart Toy&	 $4$&	$0.5$\%&	\databar{0.5}&	 $4$&	$100$\%&	\databar{100}&	 $3$&	$75.0$\%&	\databar{75.0}&	 $4$&	$100$\%&	\databar{100} \\
% Smart Clothes&	 $3$&	$0.4$\%&	\databar{0.4}&	 $3$&	$100$\%&	\databar{100}&	 $1$&	$33.3$\%&	\databar{33.3}&	 $3$&	$100$\%&	\databar{100} \\
% Sailing Accessory&	 $3$&	$0.4$\%&	\databar{0.4}&	 $3$&	$100$\%&	\databar{100}&	 $2$&	$66.7$\%&	\databar{66.7}&	 $3$&	$100$\%&	\databar{100} \\
% Diving Accessory&	 $3$&	$0.4$\%&	\databar{0.4}&	 $3$&	$100$\%&	\databar{100}&	 $3$&	$100$\%&	\databar{100}&	 $3$&	$100$\%&	\databar{100} \\
% Network Device&	 $3$&	$0.4$\%&	\databar{0.4}&	 $3$&	$100$\%&	\databar{100}&	 $2$&	$66.7$\%&	\databar{66.7}&	 $3$&	$100$\%&	\databar{100} \\
% Camera&	 $3$&	$0.4$\%&	\databar{0.4}&	 $3$&	$100$\%&	\databar{100}&	 $0$&	$0.0$\%&	\databar{0.0}&	 $3$&	$100$\%&	\databar{100} \\
% Alarm&	 $2$&	$0.3$\%&	\databar{0.3}&	 $2$&	$100$\%&	\databar{100}&	 $2$&	$100$\%&	\databar{100}&	 $2$&	$100$\%&	\databar{100} \\
% Headphone&	 $2$&	$0.3$\%&	\databar{0.3}&	 $2$&	$100$\%&	\databar{100}&	 $0$&	$0.0$\%&	\databar{0.0}&	 $2$&	$100$\%&	\databar{100} \\
% \midrule
% Total&	 $770$&	$100$\%&	\databar{100}&	 $760$&	$98.7$\%&	\databar{98.7}&	 $440$&	$57.1$\%&	\databar{57.1}&	 $744$&	$96.6$\%&	\databar{96.6} \\
% % Drone	        & $1$ \\
% % Buckle	        & $1$ \\
% % SIM Charger	    & $1$ \\
% % Door Bell	    & $1$ \\
% % Brainware	    & $1$ \\
% % Socks	        & $1$ \\
% % Luggage	        & $1$ \\
% % Coffee Machine	& $1$ \\
% % Scanner     	& $1$ \\

% \bottomrule
% \end{tabular}
% }
% \vspace{0.05in}
% \caption{Experiment results across different categories of firmware.}
% \label{tab:result}
% \end{table*}



%avg. size,  avg. time, #uuid, 


\ignore{
\begin{table*}
\centering
\scalebox{0.8}{
\begin{tabular}{l | r || r | r || r  r | r  r | r  r}
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{\textbf{Firmware Category}}}  & \multicolumn{1}{c}{\multirow{3}{*}{\textbf{\# Total}}}  & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Statistics}}}  & \multicolumn{6}{c}{\textbf{Vulnerabilities}}   \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-10}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg. Size}}}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg. Time}}} & \multicolumn{2}{c|}{\textbf{Trackable}}    & \multicolumn{2}{c|}{\textbf{MITM Vuln.}}    & \multicolumn{2}{c}{\textbf{Evasdroppable}} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{c}{\textbf{(KB)}}     & \multicolumn{1}{c}{\textbf{(m)}}         & \# & \multicolumn{1}{r|}{\%}    & \# & \multicolumn{1}{r|}{\%}          & \# & \% \\
\toprule
Wearable &	 $205$ &	 $98.3$ &	 $53.6$ &	 $205$&	$100.0$&	 $99$&	$48.3$&	 $204$&	$99.5$ \\
Others &	 $76$ &	 $223.5$ &	 $104.9$ &	 $76$&	$100.0$&	 $60$&	$78.9$&	 $75$&	$98.7$ \\
Sensor &	 $67$ &	 $80.9$ &	 $57.1$ &	 $67$&	$100.0$&	 $45$&	$67.2$&	 $66$&	$98.5$ \\
Tag &	 $58$ &	 $84.2$ &	 $35.2$ &	 $58$&	$100.0$&	 $43$&	$74.1$&	 $57$&	$98.3$ \\
Robot &	 $41$ &	 $117.7$ &	 $87.3$ &	 $41$&	$100.0$&	 $17$&	$41.5$&	 $25$&	$61.0$ \\
Medical Devices &	 $41$ &	 $138.6$ &	 $152.2$ &	 $41$&	$100.0$&	 $15$&	$36.6$&	 $37$&	$90.2$ \\
Bike Accessory &	 $41$ &	 $92.3$ &	 $69.9$ &	 $41$&	$100.0$&	 $24$&	$58.5$&	 $41$&	$100.0$ \\
Car Accessory &	 $26$ &	 $76.1$ &	 $89.0$ &	 $22$&	$84.6$&	 $14$&	$53.8$&	 $26$&	$100.0$ \\
Smart Light &	 $21$ &	 $81.2$ &	 $58.2$ &	 $20$&	$95.2$&	 $15$&	$71.4$&	 $21$&	$100.0$ \\
Switch &	 $20$ &	 $72.8$ &	 $61.9$ &	 $20$&	$100.0$&	 $7$&	$35.0$&	 $20$&	$100.0$ \\
Smart Home &	 $20$ &	 $63.0$ &	 $20.4$ &	 $20$&	$100.0$&	 $9$&	$45.0$&	 $20$&	$100.0$ \\
Smart Eyeglasses &	 $19$ &	 $58.1$ &	 $30.1$ &	 $19$&	$100.0$&	 $7$&	$36.8$&	 $19$&	$100.0$ \\
Thermometer &	 $16$ &	 $54.2$ &	 $15.9$ &	 $16$&	$100.0$&	 $10$&	$62.5$&	 $16$&	$100.0$ \\
Smart Lock &	 $15$ &	 $67.0$ &	 $58.7$ &	 $15$&	$100.0$&	 $7$&	$46.7$&	 $14$&	$93.3$ \\
Beacon &	 $13$ &	 $61.4$ &	 $41.9$ &	 $13$&	$100.0$&	 $7$&	$53.8$&	 $12$&	$92.3$ \\
Firearm Accessory &	 $11$ &	 $87.7$ &	 $63.2$ &	 $11$&	$100.0$&	 $7$&	$63.6$&	 $11$&	$100.0$ \\
Agricultural &	 $10$ &	 $142.8$ &	 $96.5$ &	 $5$&	$50.0$&	 $9$&	$90.0$&	 $10$&	$100.0$ \\
Battery &	 $9$ &	 $34.3$ &	 $13.3$ &	 $9$&	$100.0$&	 $7$&	$77.8$&	 $9$&	$100.0$ \\
Game Accessory &	 $9$ &	 $67.4$ &	 $22.7$ &	 $9$&	$100.0$&	 $6$&	$66.7$&	 $9$&	$100.0$ \\
Keyboard &	 $7$ &	 $63.4$ &	 $20.0$ &	 $7$&	$100.0$&	 $3$&	$42.9$&	 $7$&	$100.0$ \\
Mouse &	 $6$ &	 $58.2$ &	 $16.9$ &	 $6$&	$100.0$&	 $5$&	$83.3$&	 $6$&	$100.0$ \\
Printer &	 $6$ &	 $24.1$ &	 $3.0$ &	 $6$&	$100.0$&	 $6$&	$100.0$&	 $6$&	$100.0$ \\
Surf Board &	 $6$ &	 $71.9$ &	 $116.4$ &	 $6$&	$100.0$&	 $2$&	$33.3$&	 $6$&	$100.0$ \\
Sports Accessory &	 $4$ &	 $88.9$ &	 $86.2$ &	 $4$&	$100.0$&	 $3$&	$75.0$&	 $4$&	$100.0$ \\
Smart Toy &	 $4$ &	 $58.0$ &	 $7.2$ &	 $4$&	$100.0$&	 $3$&	$75.0$&	 $4$&	$100.0$ \\
Smart Clothes &	 $3$ &	 $57.6$ &	 $7.1$ &	 $3$&	$100.0$&	 $1$&	$33.3$&	 $3$&	$100.0$ \\
Sailing Accessory &	 $3$ &	 $73.5$ &	 $174.2$ &	 $3$&	$100.0$&	 $2$&	$66.7$&	 $3$&	$100.0$ \\
Diving Accessory &	 $3$ &	 $19.6$ &	 $2.3$ &	 $3$&	$100.0$&	 $3$&	$100.0$&	 $3$&	$100.0$ \\
Network Device &	 $3$ &	 $74.2$ &	 $88.8$ &	 $3$&	$100.0$&	 $2$&	$66.7$&	 $3$&	$100.0$ \\
Camera &	 $3$ &	 $143.0$ &	 $0.1$ &	 $3$&	$100.0$&	 $0$&	$0.0$&	 $3$&	$100.0$ \\
Alarm &	 $2$ &	 $41.7$ &	 $13.3$ &	 $2$&	$100.0$&	 $2$&	$100.0$&	 $2$&	$100.0$ \\
Headphone &	 $2$ &	 $122.7$ &	 $51.1$ &	 $2$&	$100.0$&	 $0$&	$0.0$&	 $2$&	$100.0$ \\
\midrule
Total &	 $770$ &	 $102.1$ &	 $63.9$ &	 $760$&	$98.7$&	 $440$&	$57.1$&	 $744$&	$96.6$ \\
% Drone	        & $1$ \\
% Buckle	        & $1$ \\
% SIM Charger	    & $1$ \\
% Door Bell	    & $1$ \\
% Brainware	    & $1$ \\
% Socks	        & $1$ \\
% Luggage	        & $1$ \\
% Coffee Machine	& $1$ \\
% Scanner     	& $1$ \\

\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Experiment results across different categories of firmware.}
\label{tab:result}
\end{table*}
}




% Nordic only ver.
\ignore{
\begin{table}
\centering
\scalebox{0.68}{
\begin{tabular}{l | r | r | r | r  | r  | r }
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{\textbf{Firmware Category}}}  & \multicolumn{1}{c}{\multirow{3}{*}{\textbf{\# Total}}}  & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Statistics}}}  & \multicolumn{3}{c}{\textbf{\# Vulnerabilities}}   \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-7}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg. Size}}}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Median}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Track.}}}    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Active}}}    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Passive}}} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{c}{\textbf{(KB)}}     & \multicolumn{1}{c}{\textbf{Time (m)}}   &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{MITM}}  &  \multicolumn{1}{c}{\textbf{MITM}}  \\
\midrule
Wearable &	 $204$ &	 $98.2$ &	 $42.8$ &	 $204$&	 $171$&	 $203$ \\
Others &	 $76$ &	 $223.5$ &	 $48.8$ &	 $76$&	 $63$&	 $75$ \\
Sensor &	 $67$ &	 $80.9$ &	 $9.5$ &	 $67$&	 $51$&	 $66$ \\
Tag &	 $58$ &	 $84.2$ &	 $164.3$ &	 $58$&	 $45$&	 $57$ \\
Robot &	 $41$ &	 $117.7$ &	 $37.2$ &	 $41$&	 $35$&	 $25$ \\
Medical Devices &	 $41$ &	 $138.6$ &	 $82.3$ &	 $41$&	 $22$&	 $37$ \\
Bike Accessory &	 $41$ &	 $92.3$ &	 $21.1$ &	 $41$&	 $36$&	 $41$ \\
Car Accessory &	 $25$ &	 $75.6$ &	 $250.3$ &	 $21$&	 $20$&	 $25$ \\
Smart Light &	 $21$ &	 $81.2$ &	 $179.1$ &	 $20$&	 $16$&	 $21$ \\
Switch &	 $20$ &	 $72.8$ &	 $111.8$ &	 $20$&	 $11$&	 $20$ \\
Smart Home &	 $20$ &	 $63.0$ &	 $10.3$ &	 $20$&	 $10$&	 $20$ \\
Smart Eyeglasses &	 $19$ &	 $58.1$ &	 $56.4$ &	 $19$&	 $19$&	 $19$ \\
Thermometer &	 $16$ &	 $54.2$ &	 $27.9$ &	 $16$&	 $10$&	 $16$ \\
Smart Lock &	 $15$ &	 $67.0$ &	 $1.6$ &	 $15$&	 $8$&	 $14$ \\
Beacon &	 $13$ &	 $61.4$ &	 $0.9$ &	 $13$&	 $9$&	 $12$ \\
Firearm Accessory &	 $11$ &	 $87.7$ &	 $150.1$ &	 $11$&	 $7$&	 $11$ \\
Agricultural Equipment &	 $10$ &	 $142.8$ &	 $29.6$ &	 $5$&	 $9$&	 $10$ \\
Battery &	 $9$ &	 $34.3$ &	 $1.9$ &	 $9$&	 $7$&	 $9$ \\
Game Accessory &	 $9$ &	 $67.4$ &	 $12.5$ &	 $9$&	 $8$&	 $9$ \\
Keyboard &	 $7$ &	 $63.4$ &	 $21.6$ &	 $7$&	 $7$&	 $7$ \\
Mouse &	 $6$ &	 $58.2$ &	 $20.9$ &	 $6$&	 $5$&	 $6$ \\
Printer &	 $6$ &	 $24.1$ &	 $3.5$ &	 $6$&	 $6$&	 $6$ \\
Surf Board &	 $6$ &	 $71.9$ &	 $655.9$ &	 $6$&	 $2$&	 $6$ \\
Sports Accessory &	 $4$ &	 $88.9$ &	 $136.7$ &	 $4$&	 $3$&	 $4$ \\
Smart Toy &	 $4$ &	 $58.0$ &	 $1.8$ &	 $4$&	 $3$&	 $4$ \\
Smart Clothes &	 $3$ &	 $57.6$ &	 $7.6$ &	 $3$&	 $3$&	 $3$ \\
Sailing Accessory &	 $3$ &	 $73.5$ &	 $256.1$ &	 $3$&	 $2$&	 $3$ \\
Diving Accessory &	 $3$ &	 $19.6$ &	 $2.2$ &	 $3$&	 $3$&	 $3$ \\
Network Device &	 $3$ &	 $74.2$ &	 $261.3$ &	 $3$&	 $2$&	 $3$ \\
Camera &	 $3$ &	 $143.0$ &	 $0.1$ &	 $3$&	 $0$&	 $3$ \\
Alarm &	 $2$ &	 $41.7$ &	 $23.7$ &	 $2$&	 $2$&	 $2$ \\
Headphone &	 $2$ &	 $122.7$ &	 $40.1$ &	 $2$&	 $0$&	 $2$ \\
\midrule
Total &	 $768$ &	 $102.3$ &	 $24.3$ &	 $758$&	 $595$&	 $742$ \\
% Drone	        & $1$ \\
% Buckle	        & $1$ \\
% SIM Charger	    & $1$ \\
% Door Bell	    & $1$ \\
% Brainware	    & $1$ \\
% Socks	        & $1$ \\
% Luggage	        & $1$ \\
% Coffee Machine	& $1$ \\
% Scanner     	& $1$ \\

\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Experiment results across categories of firmware.}
\vspace{-0.3in}
\label{tab:result}
\end{table}
}




% Nordic + TI, ver.1
\ignore{
\begin{table}
\centering
\scalebox{0.68}{
\begin{tabular}{l  r  r  r  r  r  r }
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{\textbf{Firmware Category}}}  & \multicolumn{1}{c}{\multirow{3}{*}{\textbf{\# Total}}}  & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Statistics}}}  & \multicolumn{3}{c}{\textbf{\# Vulnerabilities}}   \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-7}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg. Size}}}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Median}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Track.}}}    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Active}}}    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Passive}}} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{c}{\textbf{(KB)}}     & \multicolumn{1}{c}{\textbf{Time (m)}}   &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{MITM}}  &  \multicolumn{1}{c}{\textbf{MITM}}  \\
\midrule
Wearable &	 $204$ &	 $98.2$ &	 $42.8$ &	 $204$&	 $171$&	 $203$ \\
Sensor &	 $86$ &	 $92.4$ &	 $7.1$ &	 $86$&	 $51$&	 $85$ \\
Others &	 $77$ &	 $221.5$ &	 $48.8$ &	 $77$&	 $63$&	 $76$ \\
Tag &	 $58$ &	 $84.2$ &	 $164.3$ &	 $58$&	 $45$&	 $57$ \\
Medical Devices &	 $42$ &	 $136.9$ &	 $37.9$ &	 $42$&	 $22$&	 $38$ \\
Robot &	 $41$ &	 $117.7$ &	 $37.2$ &	 $41$&	 $35$&	 $25$ \\
Bike Accessory &	 $41$ &	 $92.3$ &	 $21.1$ &	 $41$&	 $36$&	 $41$ \\
Car Accessory &	 $25$ &	 $75.6$ &	 $250.3$ &	 $21$&	 $20$&	 $25$ \\
Smart Light &	 $21$ &	 $81.2$ &	 $179.1$ &	 $20$&	 $16$&	 $21$ \\
Switch &	 $20$ &	 $72.8$ &	 $111.8$ &	 $20$&	 $11$&	 $20$ \\
Smart Home &	 $20$ &	 $63.0$ &	 $10.3$ &	 $20$&	 $10$&	 $20$ \\
Smart Eyeglasses &	 $19$ &	 $58.1$ &	 $56.4$ &	 $19$&	 $19$&	 $19$ \\
Smart Lock &	 $17$ &	 $64.6$ &	 $302.6$ &	 $17$&	 $9$&	 $16$ \\
Thermometer &	 $16$ &	 $54.2$ &	 $27.9$ &	 $16$&	 $10$&	 $16$ \\
Beacon &	 $13$ &	 $61.4$ &	 $0.9$ &	 $13$&	 $9$&	 $12$ \\
Firearm Accessory &	 $11$ &	 $87.7$ &	 $150.1$ &	 $11$&	 $7$&	 $11$ \\
Agricultural Equip. &	 $10$ &	 $142.8$ &	 $29.6$ &	 $5$&	 $9$&	 $10$ \\
Battery &	 $9$ &	 $34.3$ &	 $1.9$ &	 $9$&	 $7$&	 $9$ \\
Game Accessory &	 $9$ &	 $67.4$ &	 $12.5$ &	 $9$&	 $8$&	 $9$ \\
Keyboard &	 $7$ &	 $63.4$ &	 $21.6$ &	 $7$&	 $7$&	 $7$ \\
Mouse &	 $6$ &	 $58.2$ &	 $20.9$ &	 $6$&	 $5$&	 $6$ \\
Printer &	 $6$ &	 $24.1$ &	 $3.5$ &	 $6$&	 $6$&	 $6$ \\
Smart Toy &	 $6$ &	 $54.6$ &	 $3.3$ &	 $6$&	 $3$&	 $6$ \\
Surf Board &	 $6$ &	 $71.9$ &	 $655.9$ &	 $6$&	 $2$&	 $6$ \\
Sports Accessory &	 $4$ &	 $88.9$ &	 $136.7$ &	 $4$&	 $3$&	 $4$ \\
Smart Clothes &	 $3$ &	 $57.6$ &	 $7.6$ &	 $3$&	 $3$&	 $3$ \\
Sailing Accessory &	 $3$ &	 $73.5$ &	 $256.1$ &	 $3$&	 $2$&	 $3$ \\
Diving Accessory &	 $3$ &	 $19.6$ &	 $2.2$ &	 $3$&	 $3$&	 $3$ \\
Network Device &	 $3$ &	 $74.2$ &	 $261.3$ &	 $3$&	 $2$&	 $3$ \\
Camera &	 $3$ &	 $143.0$ &	 $0.1$ &	 $3$&	 $0$&	 $3$ \\
Alarm &	 $2$ &	 $41.7$ &	 $23.7$ &	 $2$&	 $2$&	 $2$ \\
Headphone &	 $2$ &	 $122.7$ &	 $40.1$ &	 $2$&	 $0$&	 $2$ \\
\midrule
Total &	 $793$ &	 $102.7$ &	 $21.9$ &	 $783$&	 $596$&	 $767$ \\

\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Experiment results across categories of firmware. \new{Left Nordic, right ti, \# device}}
\vspace{-0.3in}
\label{tab:result}
\end{table}
}





% Nordic + TI, ver.2
\begin{table}
\centering
\scalebox{0.65}{
\begin{tabular}{l | r r | r | r | r r | r r | r r }
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{\textbf{Category}}}  & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Total}}}  & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{Statistics}}}  & \multicolumn{6}{c}{\textbf{Vulnerabilities}}   \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-11}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{\multirow{2}{*}{\bf \# F}} & \multicolumn{1}{l}{\multirow{2}{*}{\bf \# D}}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Avg. Size}}}  & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Median}}} & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{IT}}}    & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{AM}}}    & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{PM}}} \\
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\multicolumn{1}{l}{} & \multicolumn{1}{c}{\multirow{1}{*}{}} & \multicolumn{1}{c}{\multirow{1}{*}{}}   & \multicolumn{1}{c}{\textbf{(KB)}}     & \multicolumn{1}{c}{\textbf{Time (m)}}   &  \multicolumn{1}{c}{\multirow{1}{*}{\bf \# F}} & \multicolumn{1}{c}{\multirow{1}{*}{\bf \# D}} & \multicolumn{1}{c}{\multirow{1}{*}{\bf \# F}} & \multicolumn{1}{c}{\multirow{1}{*}{\bf \# D}}  &  \multicolumn{1}{c}{\multirow{1}{*}{\bf \# F}} & \multicolumn{1}{c}{\multirow{1}{*}{\bf \# D}}  \\
\toprule
\multicolumn{11}{c}{\bf Nordic-based Firmware} \\
\toprule
Wearable &	 $204$  & $138$ &	$98.2$ &	 $42.8$ &	 $204$  & $138$ &   $171$ & $112$   & $203$ & $137$ \\
Others &	 $76$   & $22$	&   $223.5$ &	 $48.8$ &	 $76$   & $22$ &    $63$    & $14$  &$75$   & $21$ \\
Sensor &	 $67$   & $51$	&   $80.9$ &	 $9.5$ &	 $67$   & $51$  & $51$  & $37$&	 $66$   & $50$ \\
Tag (Tracker)   &	 $58$   & $41$	&   $84.2$ &	 $164.3$ &	 $58$   & $41$  & $45$  & $29$&	 $57$   & $40$ \\
Robot   &	 $41$   & $21$	& $117.7$ &	 $37.2$ &	 $41$       & $21$  & $35$  & $18$&	 $25$   & $20$ \\
Medical Devices &	 $41$ & $21$   &	 $138.6$ &	 $82.3$ &	 $41$   & $21$  & $22$&  $10$   & $37$  & $20$ \\
Bike Accessory &	 $41$ &	$35$    &  $92.3$ &	 $21.1$ &	 $41$   & $35$  & $36$  & $30$  & $41$  & $35$ \\
Car Accessory &	     $25$ &	$21$    & $75.6$ &	 $250.3$ &	 $21$   & $17$  & $20$  & $17$  & $25$  & $21$ \\
Smart Light &	 $21$     &	$19$    &  $81.2$ &	 $179.1$ &	 $20$   & $18$  & $16$  & $14$  & $21$  & $19$ \\
Switch &	 $20$ & $11$  & $72.8$ &	 $111.8$ &	 $20$   & $11$  & $11$  & $8$   & $20$  & $11$ \\
Smart Home &	 $20$  &    $18$    &	 $63.0$ &	 $10.3$ & $20$  & $18$  & $10$  & $10$  & $20$  & $18$ \\
Smart Eyeglasses &	 $19$   & $7$   &	 $58.1$ &	 $56.4$ & $19$  & $7$   & $19$  & $7$   & $19$  & $7$ \\
Thermometer &	 $16$       & $13$  &	 $54.2$ &	 $27.9$ & $16$  & $13$  & $10$  & $9$   & $16$  & $13$ \\
Smart Lock &	 $15$       & $9$   &	 $67.0$ &	 $1.6$ & $15$   & $9$   & $8$   & $5$   & $14$  & $8$ \\
Beacon &	 $13$           & $12$  &	 $61.4$ &	 $0.9$ & $13$   & $12$  & $9$   & $8$   & $12$  & $11$ \\
Firearm Accessory &	 $11$   & $5$   &	 $87.7$ &	 $150.1$ &$11$  & $5$   & $7$   & $4$   & $11$  & $5$ \\
Agricultural Equip. &	 $10$ & $10$    &	 $142.8$ &	 $29.6$ &	 $5$    & $5$   & $9$   & $9$   & $10$  & $10$ \\
Battery &	 $9$ &          $9$     &	 $34.3$ &	 $1.9$ & $9$    & $9$   & $7$   & $7$   & $9$   & $9$ \\
Game Accessory &	 $9$  & $9$   &	 $67.4$ &	 $12.5$ &	 $9$    & $9$   & $8$   & $8$   & $9$   & $9$ \\
Keyboard &	 $7$     & $5$   & $63.4$ &	 $21.6$ &	 $7$    & $5$   & $7$   & $5$   & $7$   & $5$ \\
Mouse &	 $6$ &	    $6$     &$58.2$ &	 $20.9$ &	 $6$    & $6$   & $5$   & $5$   & $6$   & $6$ \\
Printer &	 $6$ &	 $2$    & $24.1$ &	 $3.5$ &	 $6$    & $2$   & $6$   & $2$   & $6$   & $2$ \\
Surf Board &	 $6$ &  $6$   &	 $71.9$ &	 $655.9$ &	 $6$    & $6$   & $2$   & $2$   & $6$   & $6$ \\
Sports Accessory &	 $4$    & $4$   &	 $88.9$ &	 $136.7$ &	 $4$    & $4$   & $3$   & $3$   & $4$   & $4$ \\
Smart Toy &	 $4$ &  $4$     &	 $58.0$ &	 $1.8$ &	 $4$    & $4$	& $3$    & $3$   & $4$   & $4$ \\
Smart Clothes &	 $3$        & $2$     &	 $57.6$ &	 $7.6$ &	 $3$    & $2$   & $3$   & $2$   & $3$   & $2$ \\
Sailing Accessory &	 $3$    & $2$   &	 $73.5$ &	 $256.1$ &	 $3$    & $2$   & $2$   & $1$   & $3$   & $2$ \\
Diving Accessory &	 $3$    & $1$   &	 $19.6$ &	 $2.2$ &	 $3$    & $1$   & $3$   & $1$   & $3$   & $1$ \\
Network Device &	 $3$    & $3$   &	 $74.2$ &	 $261.3$ &	 $3$    & $3$   & $2$   & $2$   & $3$   & $3$ \\
Camera &	 $3$            & $3$   & $143.0$ &	 $0.1$ &	 $3$    & $3$ &  $0$ & $0$   & $3$   & $3$ \\
Alarm &	 $2$    & $2$       &	 $41.7$ &	 $23.7$ &	 $2$    & $2$   & $2$   & $2$   & $2$   & $2$ \\
Headphone &	 $2$    & $1$   &	 $122.7$ &	 $40.1$ &	 $2$    & $1$   & $0$   & $0$   & $2$   & $1$ \\
\toprule
\multicolumn{11}{c}{\bf TI-based Firmware} \\
\toprule
Sensor &	    $19$    & $19$&	 $132.9$ &	 $0.2$ &	 $19$   & $19$  & $0$   & $0$   & $19$  & $19$ \\
Smart Lock &	$2$     & $2$&	 $46.3$ &	 $0.1$ &	 $2$    & $2$   & $1$   & $1$   & $2$   & $2$ \\
Smart Toy &	    $2$     & $2$ &	 $47.8$ &	 $0.1$ &	 $2$    & $2$   & $0$   & $0$   & $2$   & $2$ \\
Medical Devices&$1$     & $1$&	 $70.2$ &	 $0.1$ &	 $1$    & $1$   & $0$   & $0$   & $1$   & $1$ \\
Others &	    $1$     & $1$&	 $76.7$ &	 $0.2$ &	 $1$    & $1$   & $0$   & $0$   & $1$   & $1$ \\
\midrule
Total &	 $793$  & $538$ & $102.7$ &	 $21.9$ & $783$ & $528$ & $596$ & $385$ & $767$ & $530$ \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Experiment results across firmware categories. (F: Firmware, D: Device, IT: Identity Tracking, AM: Active MITM, PM: Passive MITM)}
\vspace{-0.2in}
\label{tab:result}
\end{table}

==> table/table_compare.tex <==
\begin{table*}[h]
\resizebox{1.6\columnwidth}{!}
{
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multicolumn{3}{c}{\multirow{2}{*}{ Available APIs}}                                   & \multicolumn{2}{c}{WeChat}        & \multicolumn{2}{c}{Alipay}     & \multicolumn{2}{c}{Baidu}       & \multicolumn{2}{c}{TickTok}                                                       \\ \cmidrule(l){4-11} 
\multicolumn{3}{c}{}                                                                  & Enabled?           & \begin{tabular}[c]{@{}c@{}}SDK Version\\ (2.14.1)\end{tabular}   & Enabled?           & \begin{tabular}[c]{@{}c@{}}SDK Version\\ (2.6.0)\end{tabular} & Enabled?            & \begin{tabular}[c]{@{}c@{}}SDK Version\\ (3.260.6)\end{tabular} & Enabled?           & \begin{tabular}[c]{@{}c@{}}SDK Version\\ (1.66.0)\end{tabular} \\ \midrule
\multirow{27}{*}{Front-end} & \multicolumn{2}{c}{Data Caching}                         & \tickYes & 1.9.6          & \tickYes & -           & \tickYes  & -           & \tickYes & 1.0.0                                                          \\ \cmidrule(l){2-11} 
                            & \multirow{6}{*}{Media}              & Map                 & \tickYes & 1.9.6          & \tickYes & 1.23.0      & \tickYes  & -           & \tickYes & 1.63.0                                                         \\ \cmidrule(l){3-11} 
                            &                                     & Image               & \tickYes & 1.2.0          & \tickYes & 1.4.0       & 3.110.3            & 3.110.3     & \tickYes & 1.0.0                                                          \\ \cmidrule(l){3-11} 
                            &                                     & Video               & \tickYes & 1.2.0          & \tickYes & 1.10.0      & \tickYes  & -           & \tickYes & 1.0.0                                                          \\ \cmidrule(l){3-11} 
                            &                                     & Audio \& Recorder   & \tickYes & 1.9.6          & \tickYes & 1.23.4      & \tickYes  & -           & \tickYes & 1.0.0                                                          \\ \cmidrule(l){3-11} 
                            &                                     & Camera              & \tickYes & 1.6.0          & \tickYes & -         & 3.15.104           & 3.15.104    & \tickYes & 1.78.0                                                         \\ \cmidrule(l){3-11} 
                            &                                     & Rich text           & \tickYes & 2.7.0          & \tickNo & N/A         & \tickNo  & N/A         & \tickNo & N/A                                                            \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Location}                             & \tickYes & 2.8.0          & \tickYes & 1.1.1       & \tickYes  & 3.150.1     & \tickYes & 1.0.0                                                          \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Data Encryption}                      & \tickYes & 2.3.1          & \tickYes & -           & \tickYes  & -           & \tickNo & N/A                                                            \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Contact \& Phone Call}                & \tickYes & 1.2.0          & \tickYes & 1.4.0       & \tickYes  & -           & \tickYes & 1.0.0                                                          \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Canvas}                               & \tickYes & 2.7.0          & \tickYes & -           & \tickYes  & -           & \tickYes & 1.0.0                                                          \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{File}                                 & \tickYes & 2.11.0         & \tickYes & 1.4.0       & \tickYes  & 3.130.1     & \tickYes & 1.15.0                                                         \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Cross-app Channel}                    & \tickYes & 1.3.0          & \tickYes & 1.13.0      & \tickYes  & 1.10.8      & \tickYes & 1.15.0                                                         \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{In-App Channel}                       & \tickYes & 1.9.6          & \tickYes & 1.4.0       & \tickYes  & 3.60.2      & \tickYes & 1.0.0                                                          \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Shareable UI}                         & \tickYes & 1.2.0          & \tickYes & 1.7.0       & \tickYes  & -           & \tickYes & 1.5.0                                                          \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Accessibility}                        & \tickYes & 2.13.0         & \tickNo & N/A         & \tickNo  & N/A         & \tickNo & N/A                                                            \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Payment}                              & \tickYes & 1.0*           & \tickYes & -           & \tickYes  & -           & \tickYes & -                                                              \\ \cmidrule(l){2-11} 
                             & \multicolumn{2}{c}{Gait \& Sports}                              & \tickYes & 1.2.0          & \tickYes &  1.17.1            & \tickNo  & N/A           & \tickNo & N/A                                                              \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{Embedding Advertisement}              & \tickYes & 2.0.4          & \tickNo & N/A         & \tickNo  & N/A         & \tickYes & 1.57.0                                                         \\ \cmidrule(l){2-11} 
                            & \multirow{3}{*}{Peripheral}         & Bluetooth           & \tickYes &   2.10.3 & \tickYes & -           & \tickNo  & N/A         & \tickNo & N/A                                                            \\ \cmidrule(l){3-11} 
                            &                                     & Wifi                & \tickYes & 1.6.0          & \tickNo & N/A         & \tickNo  & N/A         & \tickYes & 1.0.0                                                          \\ \cmidrule(l){3-11} 
                            &                                     & NFC                 & \tickYes & 1.7.0          & \tickNo & N/A         & \tickNo  & N/A         & \tickNo & N/A                                                            \\ \cmidrule(l){2-11} 
                            & \multirow{5}{*}{Sensors \& Devices} & Battery             & \tickYes & 1.2.0          & \tickYes & -         & \tickYes                  & 3.30.2      & \tickNo & N/A                                                            \\ \cmidrule(l){3-11} 
                            &                                     & Compass             & \tickYes & 1.1.0          & \tickYes & 1.9.0       & \tickYes                  & 3.30.2      & \tickYes & 1.2.0                                                          \\ \cmidrule(l){3-11} 
                            &                                     & Gyroscope           & \tickYes & 2.3.0          & \tickYes & 1.9.0       & \tickYes                  & 3.30.2      & \tickNo & N/A                                                            \\ \cmidrule(l){3-11} 
                            &                                     & Accelerometer       & \tickYes & 1.1.0          & \tickYes & 1.9.0       & \tickYes                  & 3.30.2      & \tickYes & 1.0.0                                                          \\ \cmidrule(l){3-11} 
                            &                                     & Vibration           & \tickYes & 1.2.0          & \tickYes & 1.9.0       & \tickYes                  & -           & \tickYes & 1.0.0                                                          \\ \cmidrule(l){2-11} 
                            & \multicolumn{2}{c}{AI Services}                          & \tickNo & N/A            & \tickNo & N/A         & \tickYes                  & 3.20.11     & \tickNo & N/A                                                            \\ \midrule
\multirow{4}{*}{Back-end}   & \multicolumn{2}{c}{Trust domain Policy }                  & \tickYes & 1.1.0          & \tickYes & -           & \tickYes  & -           & \tickYes & -                                                              \\ \cmidrule(l){2-11} 
                            & \multirow{3}{*}{Cloud Base}         & File Storage        & \tickYes & 1.1.0          & \tickYes & -           & \tickYes* & N/A         & \tickNo & N/A                                                            \\ \cmidrule(l){3-11} 
                            &                                     & Database Access     & \tickYes & 1.1.0          & \tickYes & -           & \tickYes* & N/A         & \tickNo & N/A                                                            \\ \cmidrule(l){3-11} 
                            &                                     & Customized Function & \tickYes & 1.1.0          & \tickYes & -           & \tickYes* & N/A         & \tickNo & N/A                                                            \\ \bottomrule
\end{tabular}}
\caption{Comparison of major mini-apps APIs and SDKs across platforms. Current SDK version is given in the brackets. ``-'' means we can not find the references available.  ``\tickYes*'' means the referred API is currently in an internal testing stage.  } 
\label{tab:compare:api}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{1.6\columnwidth}{!}
{
\begin{tabular}{@{}cccccccc@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{EFEFEF}                                    & \cellcolor[HTML]{FFFFFF}                                     & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Host}}                                                     & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{API}}    & \cellcolor[HTML]{FFFFFF}                                        & \cellcolor[HTML]{FFFFFF}                                                      \\ \cmidrule(lr){3-6}
\rowcolor[HTML]{FFFFFF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{App Name}} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{App Store}} & \textbf{App Store}                 & \textbf{\begin{tabular}[c]{@{}c@{}}No host mode\\ allowed?\end{tabular}} & \textbf{Type}                     & \textbf{Restricted}     & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Installation}} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{Network Resource Isolation}} \\ \cmidrule(r){1-2} \cmidrule(l){7-8} 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{EFEFEF}Native Apps                         & \tickYes                                      & {\color[HTML]{333333} OS}          & \tickNo                                                   & {\color[HTML]{333333} System API} & \tickNo  & \tickYes                                         & \tickNo                                                        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{EFEFEF}Google Bundle                       & \faTry                                         & {\color[HTML]{333333} App}         & \faTry                                                     & {\color[HTML]{333333} System API} & \tickYes & \faTry                                            & \tickNo                                                        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{EFEFEF}Instant App                         & \tickNo                                       & {\color[HTML]{333333} Google Play} & \tickNo                                                   & {\color[HTML]{333333} System API} & \tickYes & \tickNo                                          & \tickNo                                                        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{EFEFEF}IMessage App                        & \cellcolor[HTML]{EFEFEF}\tickYes              & \cellcolor[HTML]{EFEFEF}IMessage   & \tickYes                                                  & {\color[HTML]{333333} System API} & \tickYes & \tickYes                                         & \tickNo                                                        \\
\rowcolor[HTML]{EFEFEF} 
Chrome Extension                                            & \tickYes                                      & Chrome                             & \tickNo                                                   & In-App API                        & \tickNo  & \tickNo                                          & \cellcolor[HTML]{FFFFFF}\tickNo                                \\
\rowcolor[HTML]{EFEFEF} 
Firefox Extension                                           & \tickYes                                      & Chrome                             & \tickNo                                                   & In-App API                        & \tickNo  & \tickNo                                          & \cellcolor[HTML]{FFFFFF}\tickNo                                \\
\rowcolor[HTML]{EFEFEF} 
Mini-Apps                                                   & \tickYes                                      & App                                & \tickNo                                                   & In-App API                        & \tickNo  & \tickNo                                          & \tickYes                                                       \\ \bottomrule
\end{tabular}}
\end{table*}

  
\begin{table*}[]
\resizebox{1.6\columnwidth}{!}
{
\begin{tabular}{@{}lccccccc@{}}\toprule

                                   &                                    & \multicolumn{2}{c}{\textbf{Host}}                                                     & \multicolumn{2}{c}{\textbf{API}}    &                                       &                                                     \\ \cmidrule(r){3-6}

\multirow{-2}{*}{\textbf{App Name}} & \multirow{-2}{*}{\textbf{App Store}} & \textbf{App Store}                 & \textbf{\begin{tabular}[c]{@{}c@{}}No host mode\\ allowed?\end{tabular}} & \textbf{Type}                     & \textbf{Restricted}     & \multirow{-2}{*}{\textbf{Installation}} & \multirow{-2}{*}{\textbf{Network Resource Isolation}}  \\  \midrule

Native Apps                         & \tickYes                                      &   {OS}          & \tickNo                                                   & {System API} & \tickNo  & \tickYes                                         & \tickNo                                                        \\ 

Google Bundle                       & \faTry                                         & {App}         & \faTry                                                     & {System API} & \tickYes & \faTry                                            & \tickNo                                                        \\

Instant App                         & \tickNo                                       & {Google Play} & \tickNo                                                   & {System API} & \tickYes & \tickNo                                          & \tickNo                                                        \\

IMessage App                        & \tickYes              & IMessage   & \tickYes                                                  & {System API} & \tickYes & \tickYes                                         & \tickNo                                                        \\

Chrome Extension                                            & \tickYes                                      & Chrome                             & \tickNo                                                   & In-App API                        & \tickNo  & \tickNo                                          & \tickNo                                \\

Firefox Extension                                           & \tickYes                                      & Chrome                             & \tickNo                                                   & In-App API                        & \tickNo  & \tickNo                                          & \tickNo                                \\

Mini-Apps                                                   & \tickYes                                      & App                                & \tickNo                                                   & In-App API                        & \tickNo  & \tickNo                                          & \tickYes                                        \\\bottomrule              
\end{tabular}}
\end{table*}



  
\begin{table} 
\resizebox{0.9\columnwidth}{!}
{
 % Please add the following required packages to your document preamble:
% \usepackage{booktabs}
 
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{}                 & \textbf{Examples} & \textbf{Mini-app} & \textbf{Native app} \\ \midrule
\textbf{System resources} & Location          &            \tickYes      &             \tickYes        \\
\textbf{Host app data}    & User information  &             \tickYes     &          N/A           \\
\textbf{App data}         & Credentials       &             \tickYes     &              \tickYes       \\
 
\textbf{Back-end data}    & Remote database   &             \tickYes     &           \tickNo          \\ \bottomrule
\end{tabular}

}
\caption{Comparison between mini-apps and native apps regarding data protection. \tickYes means apps(mini-apps) have security measures against data leakage, and \tickNo\space means not. }
\label{tab:resouces}
\end{table}

==> table/tbl-term.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
 \setlength\tabcolsep{1.5pt}
\scriptsize{
\begin{tabular}{@{}clrccr@{}}
\toprule
\textbf{Symbol} & \textbf{Definition} & \textbf{Scope}  & \textbf{Length (bits)} & \textbf{Generated by} &     \textbf{Validation Period} \\ 
%\textbf{Name} & &  & \textbf{(bits)} & \textbf{by} &   \textbf{Period}   \\  
\midrule
\texttt{MK}                   & Master Key          & Miniapp-specific      & 256                    & WeChat Server                          &   $\infty$         \\
\texttt{EK}                   & Encryption Key      & User-specific         & 128                   & WeChat Server                                         &        User-specific      \\
\texttt{LT}                    & Login Token               & User-specific                  & 128                   & WeChat Server                                  &    5 mins         \\
\texttt{AT}                    & Access Token               & Miniapp-specific                  & 128                   & WeChat Server                                  &    120 mins         \\
%$\mathcal{C}$                       & Cipher              & Data encrypted using EK                          \\
%$\mathcal{P}$                  & Phone Number        & Phone numbers are used to associate users \\
\bottomrule
\end{tabular}}
%\vspace{1mm}
\caption{Summary of keys used in \wechat ecosystem.}
\label{tab:symbols}
\vspace{-0.3in}
\end{table}


==> table/uuid.tex <==

\begin{table}[t]
% \scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}{l  l  l | r  r }
\toprule
\multicolumn{3}{ l}{\bf Item} 	& \multicolumn{1}{ r}{\bf \#} &  {\bf \%} \\
\toprule
% \multicolumn{3}{ l}{ \# Apps W/ Bluetooth APIs.}				& 135,486 &  \\
\multicolumn{3}{ l}{\bf \# Service}				            & $1,807$ & $100$ \\
& \multicolumn{2}{ l}{\bf Type}	        &  &  \\    
& & \multicolumn{1}{ l}{ \# Primary service UUID}	        &  $1,779$  & $98.5$  \\
& & \multicolumn{1}{ l}{ \# Invalid service UUID}	        &  $28$    & $1.5$  \\
\midrule
\multicolumn{3}{ l}{\bf \# Characteristic}		    & $1,699$ & $100$ \\
& \multicolumn{2}{ l}{\bf Type}	        &  &  \\
& & \multicolumn{1}{ l}{ \# Standard characteristic UUID}	        &  $341$    & $20.1$  \\
& & \multicolumn{1}{ l}{ \# Customized characteristic UUID}	        &  $1,101$  & $64.8$  \\
& & \multicolumn{1}{ l}{ \# Unknown characteristic UUID}	        &  $257$    & $15.1$  \\
& \multicolumn{2}{ l}{\bf Read Permission}	        &  &  \\
& & \multicolumn{1}{ l}{ \# Characteristic w/ No Protection}	        &  $1,631$  &  $96.0$ \\
& & \multicolumn{1}{ l}{ \# Characteristic w/ Encrypted Read}	        &  $59$  &  $3.5$  \\
& & \multicolumn{1}{ l}{ \# Characteristic w/ Authenticated Read}	        &  $9$  &  $0.5$  \\

& \multicolumn{2}{ l}{\bf Write Permission}	        &  &  \\
& & \multicolumn{1}{ l}{ \# Characteristic w/ No Protection}	        &  $1,655$  &  $97.4$ \\
& & \multicolumn{1}{ l}{ \# Characteristic w/ Encrypted Write}	        &  $37$  &  $2.2$  \\
& & \multicolumn{1}{ l}{ \# Characteristic w/ Authenticated Write}	        &  $7$  &   $0.4$ \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Identified UUIDs and characteristic permissions.}
\vspace{-0.3in}
\label{tab:uuid}
\end{table}



\ignore{
\begin{table}
% \scriptsize
\centering
\scalebox{0.8}{
\begin{tabular}{l  l  l | r  r  r}
\toprule
\multicolumn{3}{ l}{} 	& \multicolumn{1}{ r}{\bf \# UUID} &  {\bf \%}\\
\midrule
% \multicolumn{3}{ l|}{ \# Apps W/ Bluetooth APIs.}				& 135,486 &  \\
\multicolumn{3}{ l|}{\bf Service UUID}				            & $1,807$ & $100$ & \databar{100.0}  \\
& \multicolumn{2}{ l|}{\bf Type}	        &  &  \\
& & \multicolumn{1}{ l|}{ Primary}	        &  $1,779$  & $98.5$  & \databar{98.5} \\
& & \multicolumn{1}{ l|}{ Invalid}	        &  $28$    & $1.5$  & \databar{1.5} \\
\midrule
\midrule
\multicolumn{3}{ l|}{\bf Characteristic UUID}		    & $1,699$ & $100$ & \databar{100.0}  \\
& \multicolumn{2}{ l|}{\bf Type}	        &  &  \\
& & \multicolumn{1}{ l|}{ Standard}	        &  $341$    & $20.1$  & \databar{20.1} \\
& & \multicolumn{1}{ l|}{ Customized}	        &  $1,101$  & $64.8$  & \databar{64.8} \\
& & \multicolumn{1}{ l|}{ Unknown}	        &  $257$    & $15.1$ & \databar{15.1}  \\

& \multicolumn{2}{ l|}{\bf Read Permission}	        &  &  \\
& & \multicolumn{1}{ l|}{ No Protection}	        &  $1,631$  &  $96.0$ & \databar{96.0} \\
& & \multicolumn{1}{ l|}{ Encrypted Read}	        &  $59$  &  $3.5$  & \databar{3.5} \\
& & \multicolumn{1}{ l|}{ Authenticated Read}	        &  $9$  &  $0.5$  & \databar{0.5} \\

& \multicolumn{2}{ l|}{\bf Write Permission}	        &  &  \\
& & \multicolumn{1}{ l|}{ No Protection}	        &  $1,655$  &  $97.4$ & \databar{97.4} \\
& & \multicolumn{1}{ l|}{ Encrypted Read}	        &  $37$  &  $2.2$  & \databar{2.2} \\
& & \multicolumn{1}{ l|}{ Authenticated Write}	        &  $7$  &   $0.4$ & \databar{0.4}  \\
\bottomrule
\end{tabular}
}
\vspace{0.05in}
\caption{Extracted UUIDs and permissions.}
\vspace{-0.2in}
\label{tab:uuid}
\end{table}
}
